TCAD Parameters for 4H-SiC: A Review

In this literature review we investigate the permittivity, density-of-state mass, band gap, impact ionization, charge carrier recombination, incomplete ionization and mobility in 4H silicon carbide. We provide a comprehensive overview over characterization methods, models and parameters to lower the entrance barrier for newcomers and allow a critical evaluation of common material property descriptions. We further highlight areas for future research by identifying gaps in the current knowledge base. For each investigated property we found a large amount of models and parameter sets based on measurements, calculations or fittings. With literal and/or graphical comparisons we reveal qualitative good agreement but also flawed data values, misinterpretations of research results and inconsistencies among multiple investigations, even those directly referencing each other. We identify parameter variations, e.g., due to temperature, with high impact that are rarely considered in 4H-SiC analyses and common values that are based on old research of deviating materials or properties. We further show the slow accommodation of recent research results within the scientific community and reveal missing characterization data but also insufficient models in state-of-the-art technology computer aided design (TCAD) tools. Overall, our review enables scientifically based decisions on 4H-SiC material parameters and unravels the demand for further investigations to validate commonly used values, confirm hypothesis and cover additional dependencies.

==> data/II_elec_plot.tex <==
\pgfplotsset{cycle list name=para}
\addplot+ [domain=1/2.50E+06:1/1.00E+07, samples=\samp] {THKON(10,29.9,120*1e-3,0*1e-3)};
\addlegendentry{\reftext{Kons97}\cite{konstantinov1997} $\parallel$}
\addplot+ [domain=1/2.00E+06:1/4.00E+06, samples=\samp] {OC(400000,15000000,1.15,0)};
\addlegendentry{\reftext{Bert00}\cite{bertilsson2000} $\parallel$}
\addplot+ [domain=1/2.50E+06:1/1.00E+07, samples=\samp] {OC(1.69e6,9.69e6,1.6,0)};
\addlegendentry{\reftext{Mori01}\cite{morisette2001} $\parallel$}
\addplot+ [domain=1/1.80E+06:1/4.00E+06, samples=\samp] {OC(1980000,9460000,1.42,0)};
\addlegendentry{\reftext{Ng03}\cite{ng2003}}
\addplot+ [domain=1/2.50E+06:1/1.00E+07, samples=\samp] {OC(7260000,23400000,1,0)};
\addlegendentry{\reftext{Zhao03}\cite{zhao2003} $\parallel$}
\addplot+ [domain=1/1.25E+06:1/3.00E+06, samples=\samp] {OC(4.08e5,1.67e7,1,0)};
\addlegendentry{\reftext{Bros04}\cite{brosselard2004} $\parallel$}
\addplot+ [domain=1/2.00E+06:1/5.00E+06, samples=\samp] {OC(176000000,33000000,1,0)};
\addlegendentry{\reftext{Hata04}\cite{hatakeyama2004} $\parallel$}
\addplot+ [domain=1/2.70E+06:1/5.00E+06, samples=\samp] {OC(16500000,25800000,1,0)};
\addlegendentry{\reftext{Choi05}\cite{choi2005} $\parallel$}
\addplot+ [domain=1/1.25E+06:1/5.00E+06, samples=\samp] {OC(2780000,10500000,1.37,0)};
\addlegendentry{\reftext{Loh08}\cite{loh2008}}
\addplot+ [domain=1/2.00E+06:1/2.70E+06, samples=\samp] {OC(460000,17800000,1,0)};
\addlegendentry{\reftext{Nguy11}\cite{nguyen2011}}
\addplot+ [domain=1/2.00E+06:1/4.00E+06, samples=\samp] {OC(3.25e5,1.71e7,1,0)};
\addlegendentry{\reftext{Bion12}\cite{biondo2012}}
\addplot+ [domain=1/1.80E+06:1/2.50E+06, samples=\samp] {OC(19330,2.888e6,4.828,0)};
\addlegendentry{\reftext{Gree12}\cite{green2012}}
\addplot+ [domain=1/1.50E+06:1/4.80E+06, samples=\samp] {OC(3360000,22600000,1,0)};
\addlegendentry{\reftext{Nguy12}\cite{nguyen2012}}
\addplot+ [domain=1/1.25E+06:1/5.00E+06, samples=\samp] {OC(3.78e6,1.05e7,1.37,0)};
\addlegendentry{\reftext{Song12}\cite{song2012}}
\addplot+ [domain=1/2.00E+06:1/5.00E+06, samples=\samp] {OC(1.803e6,1.352e7,1.2,0)};
\addlegendentry{\reftext{Sun12}\cite{sun2012}}
\addplot+ [domain=1/2.50E+06:1/1.00E+07, samples=\samp] {OC(4.075e5,1.67e7,1,0)};
\addlegendentry{\reftext{Bell14}\cite{bellone2014} $\parallel$}
\addplot+ [domain=1/2.20E+06:1/2.70E+06, samples=\samp] {OC(8190000000,39400000,1,0)};
\addlegendentry{\reftext{Niwa14}\cite{niwa2014}}
\addplot+ [domain=1/2.50E+06:1/7.00E+06, samples=\samp] {OC(990000,1.29e7,1,0)};
\addlegendentry{\reftext{Hama15}\cite{hamad2015}}
\addplot+ [domain=1/2.20E+06:1/3.30E+06, samples=\samp] {OC(143000,4930000,2.37,0)};
\addlegendentry{\reftext{Niwa15}\cite{niwa2015} $\parallel$}
\addplot+ [domain=\pgfkeysvalueof{/pgfplots/xmin}:\pgfkeysvalueof{/pgfplots/xmax}, samples=\samp] {OC(186000000,28000000,1,0)};
\addlegendentry{\reftext{Shar15}\cite{sharma2015} $\parallel$}
\addplot+ [domain=1/1.20E+06:1/5.00E+06, samples=\samp] {OC(38.6e6+-15e6,2.56e7+-0.1e6,1,0)};
\addlegendentry{\reftext{Kyur16}\cite{kyuregyan2016}}
\addplot+ [domain=\pgfkeysvalueof{/pgfplots/xmin}:\pgfkeysvalueof{/pgfplots/xmax}, samples=\samp] {OC(1310000,13000000,1,0)};
\addlegendentry{\reftext{Zhan18}\cite{zhang2018}}
\addplot+ [domain=1/2.00E+06:1/5.00E+06, samples=\samp] {OC(313000000,34500000,1,0)};
\addlegendentry{\reftext{Bali19}\cite{baliga2019} $\parallel$}
\addplot+ [domain=1/1.00E+06:1/1.00E+07, samples=\samp] {TH(10.61,27,120*1e-3,\kB * 300)};
\addlegendentry{\reftext{Nida19}\cite{nida2019} $\parallel$}
\addplot+ [domain=1/2.40E+06:1/3.20E+06, samples=\samp] {OC(339000,5150000,2.37,0)};
\addlegendentry{\reftext{Zhao19}\cite{zhao2019} $\parallel$}
\addplot+ [domain=1/9.00E+05:1/1.00E+07, samples=\samp] {THNOU(7.5,10,92.5*1e-3,14.4*1e-3)};
\addlegendentry{\reftext{Nouk20}\cite{nouketcha2020}}
\addplot+ [domain=1/2.00E+06:1/1.00E+07, samples=\samp] {OC(932000,7190000,1.95,0)};
\addlegendentry{\reftext{Chea21}\cite{cheang2021}}
\addplot+ [domain=1/1.25E+06:1/1.00E+07, samples=\samp] {OC(2800000,20700000,1,0)};
\addlegendentry{\reftext{Stef21}\cite{stefanakis2021} $\parallel$}
\addplot+ [domain=1/1.00E+06:1/1.00E+07, samples=\samp] {TH(10.6,27,95*1e-3,\kB * 300)};
\addlegendentry{\reftext{Stei23}\cite{steinmann2023} (95)}
\addplot+ [domain=1/1.00E+06:1/1.00E+07, samples=\samp] {TH(10.6,27,87*1e-3,\kB * 300)};
\addlegendentry{\reftext{Stei23}\cite{steinmann2023} (87)}
\pgfplotsset{cycle list name=perp}
\pgfplotsset{cycle list shift=\cs}\addplot+ [domain=1/2.00E+06:1/4.00E+06, samples=\samp] {OC(48000000,15000000,1.15,0)};
\addlegendentry{\reftext{Bert00}\cite{bertilsson2000} $\perp$}
\addplot+ [domain=1/2.00E+06:1/5.00E+06, samples=\samp] {OC(21000000,17000000,1,0)};
\addlegendentry{\reftext{Hata04}\cite{hatakeyama2004} $\perp$}
\addplot+ [domain=1/1.60E+06:1/2.00E+06, samples=\samp] {OC(6400000,12500000,1,0)};
\addlegendentry{\reftext{Stef20}\cite{stefanakis2020} $\perp$}
\addplot+ [domain=1/1.60E+06:1/2.10E+06, samples=\samp] {OC(6.91e6,1.44e7,1,0)};
\addlegendentry{\reftext{Kita24}\cite{kitawaki2024} $\perp$}
\addlegendimage{empty legend}
\addlegendentry{}


==> data/II_hole_plot.tex <==
\pgfplotsset{cycle list name=para}
\addplot+ [domain=1/1.50E+06:1/1.00E+07, samples=\samp] {THKON(7,32.5,120*1e-3,0*1e-3)};
\addlegendentry{\reftext{Kons97}\cite{konstantinov1997} $\parallel$}
\addplot+ [domain=1/2.50E+06:1/3.20E+06, samples=\samp] {OC(3090000,1.79e7+-0.04e7,1,0)};
\addlegendentry{\reftext{Ragh99}\cite{raghunathan1999}}
\addplot+ [domain=1/2.00E+06:1/4.00E+06, samples=\samp] {OC(1800000,15000000,1,0)};
\addlegendentry{\reftext{Bert00}\cite{bertilsson2000} $\parallel$}
\addplot+ [domain=1/1.50E+06:1/1.00E+07, samples=\samp] {OC(5180000,14000000,1,0)};
\addlegendentry{\reftext{Sher00}\cite{sheridan2000} $\parallel$}
\addplot+ [domain=1/1.50E+06:1/1.00E+07, samples=\samp] {OC(3.32e6,1.07e7,1.1,0)};
\addlegendentry{\reftext{Mori01}\cite{morisette2001} $\parallel$}
\addplot+ [domain=1/1.80E+06:1/4.00E+06, samples=\samp] {OC(4380000,11400000,1.06,0)};
\addlegendentry{\reftext{Ng03}\cite{ng2003}}
\addplot+ [domain=1/1.50E+06:1/1.00E+07, samples=\samp] {OC(6850000,14100000,1,0)};
\addlegendentry{\reftext{Zhao03}\cite{zhao2003} $\parallel$}
\addplot+ [domain=1/1.00E+06:1/3.00E+06, samples=\samp] {OC(1.63e7,1.67e7,1,0)};
\addlegendentry{\reftext{Bros04}\cite{brosselard2004} $\parallel$}
\addplot+ [domain=1/2.00E+06:1/5.00E+06, samples=\samp] {OC(341000000,25000000,1,0)};
\addlegendentry{\reftext{Hata04}\cite{hatakeyama2004} $\parallel$}
\addplot+ [domain=1/1.50E+06:1/4.00E+06, samples=\samp] {OC(5500000,13500000,1,0)};
\addlegendentry{\reftext{Choi05}\cite{choi2005} $\parallel$}
\addplot+ [domain=1/1.00E+06:1/5.00E+06, samples=\samp] {OC(3510000,10300000,1.09,0)};
\addlegendentry{\reftext{Loh08}\cite{loh2008}}
\addplot+ [domain=1/1.33E+06:1/2.00E+06, samples=\samp] {OC(3321000,10385000,1.09,0)};
\addlegendentry{\reftext{Loh09}\cite{loh2009}}
\addplot+ [domain=1/1.50E+06:1/2.70E+06, samples=\samp] {OC(15600000,17200000,1,0)};
\addlegendentry{\reftext{Nguy11}\cite{nguyen2011}}
\addplot+ [domain=1/2.00E+06:1/4.00E+06, samples=\samp] {OC(3.25e6,1.71e7,1,0)};
\addlegendentry{\reftext{Bion12}\cite{biondo2012}}
\addplot+ [domain=1/1.60E+06:1/4.00E+06, samples=\samp] {OC(6e6,1.387e7,0.96,0)};
\addlegendentry{\reftext{Gree12}\cite{green2012}}
\addplot+ [domain=1/1.50E+06:1/4.80E+06, samples=\samp] {OC(8500000,1.597e7,1,0)};
\addlegendentry{\reftext{Nguy12}\cite{nguyen2012}}
\addplot+ [domain=1/1.00E+06:1/5.00E+06, samples=\samp] {OC(4.51e6,1.05e7,1.1,0)};
\addlegendentry{\reftext{Song12}\cite{song2012}}
\addplot+ [domain=1/1.50E+06:1/4.00E+06, samples=\samp] {OC(1.861e6,9.986e6,1.11,0)};
\addlegendentry{\reftext{Sun12}\cite{sun2012}}
\addplot+ [domain=1/1.50E+06:1/1.00E+07, samples=\samp] {OC(1.63e7,1.67e7,1,0)};
\addlegendentry{\reftext{Bell14}\cite{bellone2014} $\parallel$}
\addplot+ [domain=1/1.40E+06:1/2.50E+06, samples=\samp] {OC(4513000,12820000,1,0)};
\addlegendentry{\reftext{Niwa14}\cite{niwa2014}}
\addplot+ [domain=1/2.50E+06:1/7.00E+06, samples=\samp] {OC(1610000,1.15e7,1,0)};
\addlegendentry{\reftext{Hama15}\cite{hamad2015}}
\addplot+ [domain=1/1.00E+06:1/2.35E+06, samples=\samp] {OC(3140000,11800000,1.02,0)};
\addlegendentry{\reftext{Niwa15}\cite{niwa2015} $\parallel$}
\addplot+ [domain=\pgfkeysvalueof{/pgfplots/xmin}:\pgfkeysvalueof{/pgfplots/xmax}, samples=\samp] {OC(301000000,20500000,1,0)};
\addlegendentry{\reftext{Shar15}\cite{sharma2015} $\parallel$}
\addplot+ [domain=1/1.00E+06:1/5.00E+06, samples=\samp] {OC(5.31e6+-0.3e6,13.1e6+-0.01e6,1,0)};
\addlegendentry{\reftext{Kyur16}\cite{kyuregyan2016}}
\addplot+ [domain=\pgfkeysvalueof{/pgfplots/xmin}:\pgfkeysvalueof{/pgfplots/xmax}, samples=\samp] {OC(2980000,13000000,1,0)};
\addlegendentry{\reftext{Zhan18}\cite{zhang2018}}
\addplot+ [domain=1/1.10E+06:1/4.00E+06, samples=\samp] {OC(8070000,15000000,1,0)};
\addlegendentry{\reftext{Bali19}\cite{baliga2019} $\parallel$}
\addplot+ [domain=1/1.00E+06:1/1.00E+07, samples=\samp] {THNIDA(10.87,39.49,85*1e-3,\kB * 300)};
\addlegendentry{\reftext{Nida19}\cite{nida2019} $\parallel$}
\addplot+ [domain=1/1.00E+06:1/2.50E+06, samples=\samp] {OC(3560000,11700000,1.02,0)};
\addlegendentry{\reftext{Zhao19}\cite{zhao2019} $\parallel$}
\addplot+ [domain=1/9.00E+05:1/1.00E+07, samples=\samp] {THNOU(6.62,4.8,9*1e-3,102*1e-3)};
\addlegendentry{\reftext{Nouk20}\cite{nouketcha2020}}
\addplot+ [domain=1/1.60E+06:1/1.00E+07, samples=\samp] {OC(1750000,6560000,1.45,0)};
\addlegendentry{\reftext{Chea21}\cite{cheang2021}}
\addplot+ [domain=1/1.25E+06:1/1.00E+07, samples=\samp] {OC(2500000,12100000,1,0)};
\addlegendentry{\reftext{Stef21}\cite{stefanakis2021} $\parallel$}
\addplot+ [domain=1/1.00E+06:1/1.00E+07, samples=\samp] {TH(10.9,62,95*1e-3,\kB * 300)};
\addlegendentry{\reftext{Stei23}\cite{steinmann2023} (95)}
\addplot+ [domain=1/1.00E+06:1/1.00E+07, samples=\samp] {TH(10.9,80,87*1e-3,\kB * 300)};
\addlegendentry{\reftext{Stei23}\cite{steinmann2023} (87)}
\addlegendimage{empty legend}
\addlegendentry{}
\addlegendimage{empty legend}
\addlegendentry{}
\addlegendimage{empty legend}
\addlegendentry{}
\pgfplotsset{cycle list name=perp}
\pgfplotsset{cycle list shift=\cs}\addplot+ [domain=1/2.00E+06:1/4.00E+06, samples=\samp] {OC(45000000,15000000,1,0)};
\addlegendentry{\reftext{Bert00}\cite{bertilsson2000} $\perp$}
\addplot+ [domain=1/2.00E+06:1/5.00E+06, samples=\samp] {OC(29600000,16000000,1,0)};
\addlegendentry{\reftext{Hata04}\cite{hatakeyama2004} $\perp$}
\addplot+ [domain=1/1.50E+06:1/2.00E+06, samples=\samp] {OC(6000000,13300000,1,0)};
\addlegendentry{\reftext{Stef20}\cite{stefanakis2020} $\perp$}
\addplot+ [domain=1/1.60E+06:1/2.10E+06, samples=\samp] {OC(3.46e7,1.75e7,1,0)};
\addlegendentry{\reftext{Kita24}\cite{kitawaki2024} $\perp$}
\addlegendimage{empty legend}
\addlegendentry{}
\addlegendimage{empty legend}
\addlegendentry{}


==> data/II_ref_chain.tex <==
\node[desc] at (0,0.000000*\dy) {Electron ( $\apara$ , $\aperp$ ) ( $\bpara$ , $\bperp$ ) ( c , d , m )};
\node[author] at (0,-1.500000*\dy) {\citeauthor{kyuregyan1989}};
\node[no4H, ref] (kyuregyan1989) at (0,-2.500000*\dy) {\reftext{Kyur89}\cite{kyuregyan1989} (  \num{457.0} ) ( \num{52.4} ) ( -- , -- , \num{1} )};
\coordinate (kyuregyan1989C) at ($(kyuregyan1989.west)+(\dxStart+\dy,0)$);
\node[ ref] (ioffe2023) at ($(kyuregyan1989C |- 0,-3.500000*\dy)$) {\reftext{Ioff23}\cite{ioffe2023} (  \num{457.0} ) ( \num{52.4} ) ( -- , -- , \num{1} )};
\draw (ioffe2023.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-5.500000*\dy) {\citeauthor{trew1991}};
\node[no4H, ref] (trew1991) at (0,-6.500000*\dy) {\reftext{Trew91}\cite{trew1991} (  \num{0.046} ) ( \num{12.0} ) ( -- , -- , \num{1} )};
\coordinate (trew1991C) at ($(trew1991.west)+(\dxStart+\dy,0)$);
\node[ ref] (wright1996) at ($(trew1991C |- 0,-7.500000*\dy)$) {\reftext{Wrig96}\cite{wright1996} (  \num{0.046} ) ( \num{12.0} ) ( -- , -- , \num{1} )};
\draw (wright1996.west) -| ++(-\dy,\fy*\dy);
\coordinate (wright1996C) at ($(wright1996.west)+(\dxStart+\dy,0)$);
\node[ ref] (wright1998) at ($(wright1996C |- 0,-8.500000*\dy)$) {\reftext{Wrig98}\cite{wright1998} (  \num{0.046} ) ( \num{12.0} ) ( -- , -- , \num{1} )};
\draw (wright1998.west) -| ++(-\dy,\fy*\dy);
\coordinate (wright1998C) at ($(wright1998.west)+(\dxStart+\dy,0)$);
\node[ ref] (bhatnagar2005) at ($(wright1998C |- 0,-9.500000*\dy)$) {\reftext{Bhat05}\cite{bhatnagar2005} (  \num{0.046} ) ( \num{12.0} ) ( -- , -- , \num{1} )};
\draw (bhatnagar2005.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-11.500000*\dy) {\citeauthor{ruff1994}};
\node[no4H, ref] (ruff1994) at (0,-12.500000*\dy) {\reftext{Ruff94}\cite{ruff1994} (  \num{1.66} ) ( \num{12.73} ) ( -- , -- , -- )};
\coordinate (ruff1994C) at ($(ruff1994.west)+(\dxStart+\dy,0)$);
\node[ ref] (shah1998) at ($(ruff1994C |- 0,-13.500000*\dy)$) {\reftext{Shah98}\cite{shah1998} (  \num{1.66} ) ( \num{12.73} ) ( -- , -- , \num{1} )};
\draw (shah1998.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (wang1999) at ($(shah1998.west |- 0,-14.500000*\dy)$) {\reftext{Wang99}\cite{wang1999} (  \num{1.66} ) ( \num{12.73} ) ( -- , -- , \num{1} )};
\draw (wang1999.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (choudhary2021) at ($(wang1999.west |- 0,-15.500000*\dy)$) {\reftext{Chou21}\cite{choudhary2021} (  \num{1.66} ) ( \num{12.73} ) ( -- , -- , -- )};
\draw (choudhary2021.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-17.500000*\dy) {\citeauthor{bakowski1997}};
\node[no4H, ref] (bakowski1997) at (0,-18.500000*\dy) {\reftext{Bako97}\cite{bakowski1997} (  \num{4.95} , \num{1.41} ) ( \num{2.58} ) ( -- , -- , \num{1} )};
\coordinate (bakowski1997C) at ($(bakowski1997.west)+(\dxStart+\dy,0)$);
\node[ ref] (ladesmartin2000) at ($(bakowski1997C |- 0,-19.500000*\dy)$) {\reftext{Lade00}\cite{ladesmartin2000} (  \num{3.44} ) ( \num{2.58} ) ( -- , -- , \num{1} )};
\draw (ladesmartin2000.west) -| ++(-\dy,\fy*\dy);
\coordinate (ladesmartin2000C) at ($(ladesmartin2000.west)+(\dxStart+\dy,0)$);
\node[ ref] (ayalew2004) at ($(ladesmartin2000C |- 0,-20.500000*\dy)$) {\reftext{Ayal04}\cite{ayalew2004} (  \num{3.44} ) ( \num{25.8} ) ( -- , -- , \num{1} )};
\draw (ayalew2004.west) -| ++(-\dy,\fy*\dy);
\coordinate (ayalew2004C) at ($(ayalew2004.west)+(\dxStart+\dy,0)$);
\node[guess, ref] (tripathi2019) at ($(ayalew2004C |- 0,-21.500000*\dy)$) {\reftext{Trip19}\cite{tripathi2019} (  \num{3.44} ) ( \num{25.8} ) ( -- , -- , \num{1} )};
\draw (tripathi2019.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (schroeder2006) at ($(ayalew2004.west |- 0,-22.500000*\dy)$) {\reftext{Schr06}\cite{schroeder2006} (  \num{3.44} ) ( \num{2.58} ) ( -- , -- , \num{1} )};
\draw (schroeder2006.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-24.500000*\dy) {\citeauthor{raghunathan1997}};
\node[fund, ref] (raghunathan1997) at (0,-25.500000*\dy) {\reftext{Ragh97}\cite{raghunathan1997} (  -- ) ( -- ) ( -- , -- , -- )};
\coordinate (raghunathan1997C) at ($(raghunathan1997.west)+(\dxStart+\dy,0)$);
\node[ ref] (nallet1999) at ($(raghunathan1997C |- 0,-26.500000*\dy)$) {\reftext{Nall99}\cite{nallet1999} (  \num{2.5} ) ( \num{14.8} ) ( -- , -- , \num{1} )};
\draw (nallet1999.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (akturk2008) at ($(nallet1999.west |- 0,-27.500000*\dy)$) {\reftext{Aktu08}\cite{akturk2008} (  \num{0.25} ) ( \num{18.4} ) ( -- , -- , -- )};
\draw (akturk2008.west) -| ++(-\dy,\fy*\dy);
\coordinate (akturk2008C) at ($(akturk2008.west)+(\dxStart+\dy,0)$);
\node[guess, ref] (pezzimenti2013) at ($(akturk2008C |- 0,-28.500000*\dy)$) {\reftext{Pezz13}\cite{pezzimenti2013} (  \num{0.25} ) ( \num{18.4} ) ( -- , -- , \num{1} )};
\draw (pezzimenti2013.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-30.500000*\dy) {\citeauthor{raghunathan1999}};
\node[fund, ref] (raghunathan1999) at (0,-31.500000*\dy) {\reftext{Ragh99}\cite{raghunathan1999} (  -- ) ( -- ) ( -- , -- , -- )};
\coordinate (raghunathan1999C) at ($(raghunathan1999.west)+(\dxStart+\dy,0)$);
\node[guess, ref] (nallet2000) at ($(raghunathan1999C |- 0,-32.500000*\dy)$) {\reftext{Nall00}\cite{nallet2000} (  \num{3.09} ) ( \num{18.0} ) ( -- , -- , \num{1} )};
\draw (nallet2000.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-34.500000*\dy) {\citeauthor{morisette2001}};
\node[fund, ref] (morisette2001) at (0,-35.500000*\dy) {\reftext{Mori01}\cite{morisette2001} (  \num{1.69} , -- ) ( \num{9.69} , -- ) ( -- , -- , \num{1.6} )};
\coordinate (morisette2001C) at ($(morisette2001.west)+(\dxStart+\dy,0)$);
\node[ ref] (kimoto2014a) at ($(morisette2001C |- 0,-36.500000*\dy)$) {\reftext{Kimo14a}\cite{kimoto2014a} (  \num{1.69} ) ( \num{9.69} ) ( -- , -- , \num{1.6} )};
\draw (kimoto2014a.west) -| ++(-\dy,\fy*\dy);
\coordinate (kimoto2014aC) at ($(kimoto2014a.west)+(\dxStart+\dy,0)$);
\node[ ref] (denapoli2022) at ($(kimoto2014aC |- 0,-37.500000*\dy)$) {\reftext{Dena22}\cite{denapoli2022} (  \num{1.69} ) ( \num{9.69} ) ( -- , -- , \num{1.6} )};
\draw (denapoli2022.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-39.500000*\dy) {\citeauthor{ng2003}};
\node[fund, ref] (ng2003) at (0,-40.500000*\dy) {\reftext{Ng03}\cite{ng2003} (  \num{1.98} ) ( \num{9.46} ) ( \num{-2.02e-3} , -- , \num{1.42} )};
\coordinate (ng2003C) at ($(ng2003.west)+(\dxStart+\dy,0)$);
\node[ ref] (cha2008) at ($(ng2003C |- 0,-41.500000*\dy)$) {\reftext{Cha08}\cite{cha2008} (  \num{1.98} ) ( \num{9.46} ) ( \num{-2.02e-3} , -- , \num{1.42} )};
\draw (cha2008.west) -| ++(-\dy,\fy*\dy);
\coordinate (cha2008C) at ($(cha2008.west)+(\dxStart+\dy,0)$);
\node[ ref] (chen2012) at ($(cha2008C |- 0,-42.500000*\dy)$) {\reftext{Chen12}\cite{chen2012} (  \num{1.98} ) ( \num{9.46} ) ( \num{-2.02e-3} , -- , \num{1.42} )};
\draw (chen2012.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (cha2008a) at ($(cha2008.west |- 0,-43.500000*\dy)$) {\reftext{Cha08a}\cite{cha2008a} (  \num{1.98} ) ( \num{9.46} ) ( \num{-2.02e-3} , -- , \num{1.42} )};
\draw (cha2008a.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-45.500000*\dy) {\citeauthor{brosselard2004}};
\node[fund, ref] (brosselard2004) at (0,-46.500000*\dy) {\reftext{Bros04}\cite{brosselard2004} (  \num{0.408} , -- ) ( \num{16.7} , -- ) ( -- , -- , -- )};
\coordinate (brosselard2004C) at ($(brosselard2004.west)+(\dxStart+\dy,0)$);
\node[guess, ref] (raynaud2010) at ($(brosselard2004C |- 0,-47.500000*\dy)$) {\reftext{Rayn10}\cite{raynaud2010} (  \num{0.41} ) ( \num{16.7} ) ( -- , -- , \num{1} )};
\draw (raynaud2010.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-49.500000*\dy) {\citeauthor{hatakeyama2004}};
\node[fund, ref] (hatakeyama2004) at (0,-50.500000*\dy) {\reftext{Hata04}\cite{hatakeyama2004} (  \num{176.0} , \num{21.0} ) ( \num{33.0} , \num{17.0} ) ( -- , -- , \num{1} )};
\coordinate (hatakeyama2004C) at ($(hatakeyama2004.west)+(\dxStart+\dy,0)$);
\node[ ref] (bertilsson2004) at ($(hatakeyama2004C |- 0,-51.500000*\dy)$) {\reftext{Bert04}\cite{bertilsson2004} (  \num{176.0} , \num{21.0} ) ( \num{33.0} , \num{17.0} ) ( -- , -- , \num{1} )};
\draw (bertilsson2004.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (hatakeyama2004a) at ($(bertilsson2004.west |- 0,-52.500000*\dy)$) {\reftext{Hata04a}\cite{hatakeyama2004a} (  \num{176.0} , \num{21.0} ) ( \num{33.0} , \num{17.0} ) ( -- , -- , \num{1} )};
\draw (hatakeyama2004a.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (hatakeyama2005) at ($(hatakeyama2004a.west |- 0,-53.500000*\dy)$) {\reftext{Hata05}\cite{hatakeyama2005} (  \num{176.0} , \num{21.0} ) ( \num{33.0} , \num{17.0} ) ( -- , -- , \num{1} )};
\draw (hatakeyama2005.west) -| ++(-\dy,\fy*\dy);
\coordinate (hatakeyama2005C) at ($(hatakeyama2005.west)+(\dxStart+\dy,0)$);
\node[ ref] (lophitis2018) at ($(hatakeyama2005C |- 0,-54.500000*\dy)$) {\reftext{Loph18}\cite{lophitis2018} (  \num{176.0} , \num{21.0} ) ( \num{33.0} , \num{17.0} ) ( -- , -- , \num{1} )};
\draw (lophitis2018.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (jin2024) at ($(lophitis2018.west |- 0,-55.500000*\dy)$) {\reftext{Jin24}\cite{jin2024} (  \num{176.0} , \num{21.0} ) ( \num{33.0} , \num{17.0} ) ( -- , -- , \num{1} )};
\draw (jin2024.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (hatakeyama2009) at ($(hatakeyama2005.west |- 0,-56.500000*\dy)$) {\reftext{Hata09}\cite{hatakeyama2009} (  \num{176.0} , \num{210.0} ) ( \num{33.0} , \num{17.0} ) ( -- , -- , \num{1} )};
\draw (hatakeyama2009.west) -| ++(-\dy,\fy*\dy);
\coordinate (hatakeyama2009C) at ($(hatakeyama2009.west)+(\dxStart+\dy,0)$);
\node[ ref] (hatakeyama2013) at ($(hatakeyama2009C |- 0,-57.500000*\dy)$) {\reftext{Hata13}\cite{hatakeyama2013} (  \num{176.0} , \num{21.0} ) ( \num{33.0} , \num{17.0} ) ( -- , -- , \num{1} )};
\draw (hatakeyama2013.west) -| ++(-\dy,\fy*\dy);
\coordinate (hatakeyama2013C) at ($(hatakeyama2013.west)+(\dxStart+\dy,0)$);
\node[ ref] (naugarhiya2017) at ($(hatakeyama2013C |- 0,-58.500000*\dy)$) {\reftext{Naug17}\cite{naugarhiya2017} (  \num{176.0} , \num{21.0} ) ( \num{33.0} , \num{17.0} ) ( -- , -- , \num{1} )};
\draw (naugarhiya2017.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (soler2019) at ($(hatakeyama2013.west |- 0,-59.500000*\dy)$) {\reftext{Sole19}\cite{soler2019} (  \num{176.0} , \num{210.0} ) ( \num{33.3} , \num{17.0} ) ( -- , -- , \num{1} )};
\draw (soler2019.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (buono2012) at ($(hatakeyama2009.west |- 0,-60.500000*\dy)$) {\reftext{Buon12}\cite{buono2012} (  \num{176.0} , \num{210.0} ) ( \num{33.0} , \num{17.0} ) ( -- , -- , \num{1} )};
\draw (buono2012.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (khalid2012) at ($(buono2012.west |- 0,-61.500000*\dy)$) {\reftext{Khal12}\cite{khalid2012} (  \num{21.0} ) ( \num{17.0} ) ( \num{-3.29e-2} , -- , \num{2} )};
\draw (khalid2012.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (chen2015) at ($(khalid2012.west |- 0,-62.500000*\dy)$) {\reftext{Chen15}\cite{chen2015} (  \num{176.0} , \num{21.0} ) ( \num{33.0} , \num{17.0} ) ( -- , -- , \num{1} )};
\draw (chen2015.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (megherbi2015) at ($(chen2015.west |- 0,-63.500000*\dy)$) {\reftext{Megh15}\cite{megherbi2015} (  \num{176.0} , \num{21.0} ) ( \num{33.0} , \num{17.0} ) ( -- , -- , \num{1} )};
\draw (megherbi2015.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (wang2022) at ($(megherbi2015.west |- 0,-64.500000*\dy)$) {\reftext{Wang22}\cite{wang2022} (  \num{176.0} , \num{21.0} ) ( \num{33.0} , \num{17.0} ) ( -- , -- , \num{1} )};
\draw (wang2022.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,0.000000*\dy) {\citeauthor{loh2008}};
\node[fund, ref] (loh2008) at (\xSepOne,-1.000000*\dy) {\reftext{Loh08}\cite{loh2008} (  \num{2.78} ) ( \num{10.5} ) ( -- , -- , \num{1.37} )};
\coordinate (loh2008C) at ($(loh2008.west)+(\dxStart+\dy,0)$);
\node[guess, ref] (wang2022a) at ($(loh2008C |- 0,-2.000000*\dy)$) {\reftext{Wang22a}\cite{wang2022a} (  \num{2.78} ) ( \num{10.5} ) ( -- , -- , \num{1} )};
\draw (wang2022a.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-4.000000*\dy) {\citeauthor{biondo2012}};
\node[fund, ref] (biondo2012) at (\xSepOne,-5.000000*\dy) {\reftext{Bion12}\cite{biondo2012} (  \num{0.325} ) ( \num{17.1} ) ( \num{-3.29e-2} , \num{0} , \num{1} )};
\coordinate (biondo2012C) at ($(biondo2012.west)+(\dxStart+\dy,0)$);
\node[ ref] (khalid2012) at ($(biondo2012C |- 0,-6.000000*\dy)$) {\reftext{Khal12}\cite{khalid2012} (  \num{21.0} ) ( \num{17.0} ) ( \num{-3.29e-2} , -- , \num{2} )};
\draw (khalid2012.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (das2015) at ($(khalid2012.west |- 0,-7.000000*\dy)$) {\reftext{Das15}\cite{das2015} (  \num{0.325} ) ( \num{17.1} ) ( \num{-3.29e-2} , -- , \num{1} )};
\draw (das2015.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-9.000000*\dy) {\citeauthor{sun2012}};
\node[fund, ref] (sun2012) at (\xSepOne,-10.000000*\dy) {\reftext{Sun12}\cite{sun2012} (  \num{1.803} ) ( \num{13.52} ) ( -- , -- , \num{1.2} )};
\coordinate (sun2012C) at ($(sun2012.west)+(\dxStart+\dy,0)$);
\node[ ref] (sun2012a) at ($(sun2012C |- 0,-11.000000*\dy)$) {\reftext{Sun12a}\cite{sun2012a} (  \num{1.803} ) ( \num{13.52} ) ( -- , -- , \num{1.2} )};
\draw (sun2012a.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-13.000000*\dy) {\citeauthor{niwa2014}};
\node[fund, ref] (niwa2014) at (\xSepOne,-14.000000*\dy) {\reftext{Niwa14}\cite{niwa2014} (  \num{8190.0} ) ( \num{39.4} ) ( -- , -- , \num{1} )};
\coordinate (niwa2014C) at ($(niwa2014.west)+(\dxStart+\dy,0)$);
\node[ ref] (hasegawa2017) at ($(niwa2014C |- 0,-15.000000*\dy)$) {\reftext{Hase17}\cite{hasegawa2017} (  \num{8190.0} ) ( \num{39.4} ) ( -- , -- , \num{1} )};
\draw (hasegawa2017.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-17.000000*\dy) {\citeauthor{niwa2015}};
\node[fund, ref] (niwa2015) at (\xSepOne,-18.000000*\dy) {\reftext{Niwa15}\cite{niwa2015} (  \num{0.143} , -- ) ( \num{4.93} , -- ) ( -- , -- , \num{2.37} )};
\coordinate (niwa2015C) at ($(niwa2015.west)+(\dxStart+\dy,0)$);
\node[ ref] (kimoto2018) at ($(niwa2015C |- 0,-19.000000*\dy)$) {\reftext{Kimo18}\cite{kimoto2018} (  \num{0.143} , -- ) ( \num{4.93} , -- ) ( \num{0} , \num{0} , \num{2.37} )};
\draw (kimoto2018.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (arvanitopoulos2019) at ($(kimoto2018.west |- 0,-20.000000*\dy)$) {\reftext{Arva19}\cite{arvanitopoulos2019} (  -- , \num{0.143} ) ( -- , \num{4.93} ) ( -- , -- , \num{2.37} )};
\draw (arvanitopoulos2019.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (kimoto2019) at ($(arvanitopoulos2019.west |- 0,-21.000000*\dy)$) {\reftext{Kimo19}\cite{kimoto2019} (  \num{0.143} , -- ) ( \num{4.93} , -- ) ( \num{0} , \num{0} , \num{2.37} )};
\draw (kimoto2019.west) -| ++(-\dy,\fy*\dy);
\node[desc] at (\xSepOne,-24.000000*\dy) {Hole ( $\apara$ , $\aperp$ ) ( $\bpara$ , $\bperp$ ) ( c , d , m )};
\node[author] at (\xSepOne,-25.500000*\dy) {\citeauthor{kyuregyan1989}};
\node[no4H, ref] (kyuregyan1989) at (\xSepOne,-26.500000*\dy) {\reftext{Kyur89}\cite{kyuregyan1989} (  \num{5.13} ) ( \num{15.7} ) ( -- , -- , \num{1} )};
\coordinate (kyuregyan1989C) at ($(kyuregyan1989.west)+(\dxStart+\dy,0)$);
\node[ ref] (ioffe2023) at ($(kyuregyan1989C |- 0,-27.500000*\dy)$) {\reftext{Ioff23}\cite{ioffe2023} (  \num{5.13} ) ( \num{15.7} ) ( -- , -- , \num{1} )};
\draw (ioffe2023.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-29.500000*\dy) {\citeauthor{trew1991}};
\node[no4H, ref] (trew1991) at (\xSepOne,-30.500000*\dy) {\reftext{Trew91}\cite{trew1991} (  \num{4.65} ) ( \num{12.0} ) ( -- , -- , \num{1} )};
\coordinate (trew1991C) at ($(trew1991.west)+(\dxStart+\dy,0)$);
\node[ ref] (wright1996) at ($(trew1991C |- 0,-31.500000*\dy)$) {\reftext{Wrig96}\cite{wright1996} (  \num{4.65} ) ( \num{12.0} ) ( -- , -- , \num{1} )};
\draw (wright1996.west) -| ++(-\dy,\fy*\dy);
\coordinate (wright1996C) at ($(wright1996.west)+(\dxStart+\dy,0)$);
\node[ ref] (wright1998) at ($(wright1996C |- 0,-32.500000*\dy)$) {\reftext{Wrig98}\cite{wright1998} (  \num{4.65} ) ( \num{12.0} ) ( -- , -- , \num{1} )};
\draw (wright1998.west) -| ++(-\dy,\fy*\dy);
\coordinate (wright1998C) at ($(wright1998.west)+(\dxStart+\dy,0)$);
\node[ ref] (bhatnagar2005) at ($(wright1998C |- 0,-33.500000*\dy)$) {\reftext{Bhat05}\cite{bhatnagar2005} (  \num{4.65} ) ( \num{12.0} ) ( -- , -- , \num{1} )};
\draw (bhatnagar2005.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-35.500000*\dy) {\citeauthor{ruff1994}};
\node[no4H, ref] (ruff1994) at (\xSepOne,-36.500000*\dy) {\reftext{Ruff94}\cite{ruff1994} (  \num{5.18} ) ( \num{14.0} ) ( -- , -- , -- )};
\coordinate (ruff1994C) at ($(ruff1994.west)+(\dxStart+\dy,0)$);
\node[ ref] (wang1999) at ($(ruff1994C |- 0,-37.500000*\dy)$) {\reftext{Wang99}\cite{wang1999} (  \num{5.18} ) ( \num{14.0} ) ( -- , -- , \num{1} )};
\draw (wang1999.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (choudhary2021) at ($(wang1999.west |- 0,-38.500000*\dy)$) {\reftext{Chou21}\cite{choudhary2021} (  \num{5.18} ) ( \num{14.0} ) ( -- , -- , -- )};
\draw (choudhary2021.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-40.500000*\dy) {\citeauthor{bakowski1997}};
\node[no4H, ref] (bakowski1997) at (\xSepOne,-41.500000*\dy) {\reftext{Bako97}\cite{bakowski1997} (  \num{21.6} , \num{21.6} ) ( \num{19.0} ) ( -- , -- , \num{1} )};
\coordinate (bakowski1997C) at ($(bakowski1997.west)+(\dxStart+\dy,0)$);
\node[ ref] (ladesmartin2000) at ($(bakowski1997C |- 0,-42.500000*\dy)$) {\reftext{Lade00}\cite{ladesmartin2000} (  \num{32.4} ) ( \num{19.0} ) ( -- , -- , \num{1} )};
\draw (ladesmartin2000.west) -| ++(-\dy,\fy*\dy);
\coordinate (ladesmartin2000C) at ($(ladesmartin2000.west)+(\dxStart+\dy,0)$);
\node[ ref] (schroeder2006) at ($(ladesmartin2000C |- 0,-43.500000*\dy)$) {\reftext{Schr06}\cite{schroeder2006} (  \num{32.4} ) ( \num{19.0} ) ( -- , -- , \num{1} )};
\draw (schroeder2006.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-45.500000*\dy) {\citeauthor{raghunathan1997}};
\node[fund, ref] (raghunathan1997) at (\xSepOne,-46.500000*\dy) {\reftext{Ragh97}\cite{raghunathan1997} (  \num{3.5} ) ( \num{17.0} ) ( -- , -- , \num{1} )};
\coordinate (raghunathan1997C) at ($(raghunathan1997.west)+(\dxStart+\dy,0)$);
\node[ ref] (shah1998) at ($(raghunathan1997C |- 0,-47.500000*\dy)$) {\reftext{Shah98}\cite{shah1998} (  \num{3.5} ) ( \num{17.0} ) ( -- , -- , \num{1} )};
\draw (shah1998.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (nallet1999) at ($(shah1998.west |- 0,-48.500000*\dy)$) {\reftext{Nall99}\cite{nallet1999} (  \num{2.5} ) ( \num{14.8} ) ( -- , -- , \num{1} )};
\draw (nallet1999.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (ayalew2004) at ($(nallet1999.west |- 0,-49.500000*\dy)$) {\reftext{Ayal04}\cite{ayalew2004} (  \num{3.5} ) ( \num{17.0} ) ( -- , -- , \num{1} )};
\draw (ayalew2004.west) -| ++(-\dy,\fy*\dy);
\coordinate (ayalew2004C) at ($(ayalew2004.west)+(\dxStart+\dy,0)$);
\node[guess, ref] (tripathi2019) at ($(ayalew2004C |- 0,-50.500000*\dy)$) {\reftext{Trip19}\cite{tripathi2019} (  \num{3.5} ) ( \num{17.0} ) ( -- , -- , \num{1} )};
\draw (tripathi2019.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-52.500000*\dy) {\citeauthor{raghunathan1999}};
\node[fund, ref] (raghunathan1999) at (\xSepOne,-53.500000*\dy) {\reftext{Ragh99}\cite{raghunathan1999} (  \num{3.09} ) ( \num{17.9} ) ( \num{-3.46e-3} , -- , \num{1} )};
\coordinate (raghunathan1999C) at ($(raghunathan1999.west)+(\dxStart+\dy,0)$);
\node[guess, ref] (nallet2000) at ($(raghunathan1999C |- 0,-54.500000*\dy)$) {\reftext{Nall00}\cite{nallet2000} (  \num{3.09} ) ( \num{18.0} ) ( -- , -- , \num{1} )};
\draw (nallet2000.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (adachi2005) at ($(nallet2000.west |- 0,-55.500000*\dy)$) {\reftext{Adac05}\cite{adachi2005} (  \num{3.25} ) ( \num{17.9} ) ( -- , -- , \num{1} )};
\draw (adachi2005.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (baliga2006) at ($(adachi2005.west |- 0,-56.500000*\dy)$) {\reftext{Bali06}\cite{baliga2006} (  \num{3.25} ) ( \num{17.5} ) ( -- , -- , \num{1} )};
\draw (baliga2006.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (akturk2008) at ($(baliga2006.west |- 0,-57.500000*\dy)$) {\reftext{Aktu08}\cite{akturk2008} (  \num{3.25} ) ( \num{17.1} ) ( -- , -- , -- )};
\draw (akturk2008.west) -| ++(-\dy,\fy*\dy);
\coordinate (akturk2008C) at ($(akturk2008.west)+(\dxStart+\dy,0)$);
\node[guess, ref] (pezzimenti2013) at ($(akturk2008C |- 0,-58.500000*\dy)$) {\reftext{Pezz13}\cite{pezzimenti2013} (  \num{3.25} ) ( \num{17.1} ) ( -- , -- , \num{1} )};
\draw (pezzimenti2013.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,0.000000*\dy) {\citeauthor{morisette2001}};
\node[fund, ref] (morisette2001) at (\xSepOne + \xSepTwo,-1.000000*\dy) {\reftext{Mori01}\cite{morisette2001} (  \num{3.32} , -- ) ( \num{10.7} , -- ) ( -- , -- , \num{1.1} )};
\coordinate (morisette2001C) at ($(morisette2001.west)+(\dxStart+\dy,0)$);
\node[ ref] (kimoto2014a) at ($(morisette2001C |- 0,-2.000000*\dy)$) {\reftext{Kimo14a}\cite{kimoto2014a} (  \num{3.32} ) ( \num{10.7} ) ( -- , -- , \num{1.1} )};
\draw (kimoto2014a.west) -| ++(-\dy,\fy*\dy);
\coordinate (kimoto2014aC) at ($(kimoto2014a.west)+(\dxStart+\dy,0)$);
\node[ ref] (denapoli2022) at ($(kimoto2014aC |- 0,-3.000000*\dy)$) {\reftext{Dena22}\cite{denapoli2022} (  \num{3.32} ) ( \num{10.7} ) ( -- , -- , \num{1.1} )};
\draw (denapoli2022.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-5.000000*\dy) {\citeauthor{ng2003}};
\node[fund, ref] (ng2003) at (\xSepOne + \xSepTwo,-6.000000*\dy) {\reftext{Ng03}\cite{ng2003} (  \num{4.38} ) ( \num{11.4} ) ( \num{-9.1e-4} , -- , \num{1.06} )};
\coordinate (ng2003C) at ($(ng2003.west)+(\dxStart+\dy,0)$);
\node[ ref] (loh2007) at ($(ng2003C |- 0,-7.000000*\dy)$) {\reftext{Loh07}\cite{loh2007} (  -- ) ( -- ) ( -- , -- , -- )};
\draw (loh2007.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (cha2008) at ($(loh2007.west |- 0,-8.000000*\dy)$) {\reftext{Cha08}\cite{cha2008} (  \num{4.38} ) ( \num{11.4} ) ( \num{-9.1e-4} , -- , \num{1.06} )};
\draw (cha2008.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (cha2008a) at ($(cha2008.west |- 0,-9.000000*\dy)$) {\reftext{Cha08a}\cite{cha2008a} (  \num{4.38} ) ( \num{11.4} ) ( \num{-9.1e-4} , -- , \num{1.06} )};
\draw (cha2008a.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (loh2008a) at ($(cha2008a.west |- 0,-10.000000*\dy)$) {\reftext{Loh08a}\cite{loh2008a} (  -- ) ( -- ) ( -- , -- , -- )};
\draw (loh2008a.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-12.000000*\dy) {\citeauthor{brosselard2004}};
\node[fund, ref] (brosselard2004) at (\xSepOne + \xSepTwo,-13.000000*\dy) {\reftext{Bros04}\cite{brosselard2004} (  \num{16.3} , -- ) ( \num{16.7} , -- ) ( -- , -- , -- )};
\coordinate (brosselard2004C) at ($(brosselard2004.west)+(\dxStart+\dy,0)$);
\node[guess, ref] (raynaud2010) at ($(brosselard2004C |- 0,-14.000000*\dy)$) {\reftext{Rayn10}\cite{raynaud2010} (  \num{16.3} ) ( \num{16.7} ) ( -- , -- , \num{1} )};
\draw (raynaud2010.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-16.000000*\dy) {\citeauthor{hatakeyama2004}};
\node[fund, ref] (hatakeyama2004) at (\xSepOne + \xSepTwo,-17.000000*\dy) {\reftext{Hata04}\cite{hatakeyama2004} (  \num{341.0} , \num{29.6} ) ( \num{25.0} , \num{16.0} ) ( -- , -- , \num{1} )};
\coordinate (hatakeyama2004C) at ($(hatakeyama2004.west)+(\dxStart+\dy,0)$);
\node[ ref] (bertilsson2004) at ($(hatakeyama2004C |- 0,-18.000000*\dy)$) {\reftext{Bert04}\cite{bertilsson2004} (  \num{341.0} , \num{29.6} ) ( \num{18.0} , \num{16.0} ) ( -- , -- , \num{1} )};
\draw (bertilsson2004.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (hatakeyama2004a) at ($(bertilsson2004.west |- 0,-19.000000*\dy)$) {\reftext{Hata04a}\cite{hatakeyama2004a} (  \num{341.0} , \num{29.6} ) ( \num{25.0} , \num{16.0} ) ( -- , -- , \num{1} )};
\draw (hatakeyama2004a.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (hatakeyama2005) at ($(hatakeyama2004a.west |- 0,-20.000000*\dy)$) {\reftext{Hata05}\cite{hatakeyama2005} (  \num{341.0} , \num{29.6} ) ( \num{25.0} , \num{16.0} ) ( -- , -- , \num{1} )};
\draw (hatakeyama2005.west) -| ++(-\dy,\fy*\dy);
\coordinate (hatakeyama2005C) at ($(hatakeyama2005.west)+(\dxStart+\dy,0)$);
\node[ ref] (ivanov2009) at ($(hatakeyama2005C |- 0,-21.000000*\dy)$) {\reftext{Ivan09}\cite{ivanov2009} (  -- ) ( \num{25.0} ) ( -- , -- , -- )};
\draw (ivanov2009.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (lophitis2018) at ($(ivanov2009.west |- 0,-22.000000*\dy)$) {\reftext{Loph18}\cite{lophitis2018} (  \num{341.0} , \num{29.6} ) ( \num{25.0} , \num{16.0} ) ( -- , -- , \num{1} )};
\draw (lophitis2018.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (hatakeyama2009) at ($(hatakeyama2005.west |- 0,-23.000000*\dy)$) {\reftext{Hata09}\cite{hatakeyama2009} (  \num{341.0} , \num{296.0} ) ( \num{25.0} , \num{16.0} ) ( -- , -- , \num{1} )};
\draw (hatakeyama2009.west) -| ++(-\dy,\fy*\dy);
\coordinate (hatakeyama2009C) at ($(hatakeyama2009.west)+(\dxStart+\dy,0)$);
\node[ ref] (hatakeyama2013) at ($(hatakeyama2009C |- 0,-24.000000*\dy)$) {\reftext{Hata13}\cite{hatakeyama2013} (  \num{341.0} , \num{29.6} ) ( \num{25.0} , \num{16.0} ) ( -- , -- , \num{1} )};
\draw (hatakeyama2013.west) -| ++(-\dy,\fy*\dy);
\coordinate (hatakeyama2013C) at ($(hatakeyama2013.west)+(\dxStart+\dy,0)$);
\node[ ref] (naugarhiya2017) at ($(hatakeyama2013C |- 0,-25.000000*\dy)$) {\reftext{Naug17}\cite{naugarhiya2017} (  \num{341.0} , \num{29.6} ) ( \num{25.0} , \num{16.0} ) ( -- , -- , \num{1} )};
\draw (naugarhiya2017.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (soler2019) at ($(hatakeyama2013.west |- 0,-26.000000*\dy)$) {\reftext{Sole19}\cite{soler2019} (  \num{341.0} , \num{296.0} ) ( \num{25.0} , \num{16.0} ) ( -- , -- , \num{1} )};
\draw (soler2019.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (buono2012) at ($(hatakeyama2009.west |- 0,-27.000000*\dy)$) {\reftext{Buon12}\cite{buono2012} (  \num{341.0} , \num{29.6} ) ( \num{25.0} , \num{16.0} ) ( -- , -- , \num{1} )};
\draw (buono2012.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (khalid2012) at ($(buono2012.west |- 0,-28.000000*\dy)$) {\reftext{Khal12}\cite{khalid2012} (  \num{29.0} ) ( \num{14.0} ) ( \num{-3.29e-2} , -- , \num{2} )};
\draw (khalid2012.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (chen2015) at ($(khalid2012.west |- 0,-29.000000*\dy)$) {\reftext{Chen15}\cite{chen2015} (  \num{341.0} , \num{29.6} ) ( \num{25.0} , \num{16.0} ) ( -- , -- , \num{1} )};
\draw (chen2015.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (megherbi2015) at ($(chen2015.west |- 0,-30.000000*\dy)$) {\reftext{Megh15}\cite{megherbi2015} (  \num{241.0} , \num{29.6} ) ( \num{25.0} , \num{16.0} ) ( -- , -- , \num{1} )};
\draw (megherbi2015.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (wang2022) at ($(megherbi2015.west |- 0,-31.000000*\dy)$) {\reftext{Wang22}\cite{wang2022} (  \num{341.0} , \num{29.6} ) ( \num{25.0} , \num{16.0} ) ( -- , -- , \num{1} )};
\draw (wang2022.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (yang2023) at ($(wang2022.west |- 0,-32.000000*\dy)$) {\reftext{Yang23}\cite{yang2023} (  -- ) ( -- ) ( -- , -- , -- )};
\draw (yang2023.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-34.000000*\dy) {\citeauthor{loh2008}};
\node[fund, ref] (loh2008) at (\xSepOne + \xSepTwo,-35.000000*\dy) {\reftext{Loh08}\cite{loh2008} (  \num{3.51} ) ( \num{10.3} ) ( -- , -- , \num{1.09} )};
\coordinate (loh2008C) at ($(loh2008.west)+(\dxStart+\dy,0)$);
\node[guess, ref] (wang2022a) at ($(loh2008C |- 0,-36.000000*\dy)$) {\reftext{Wang22a}\cite{wang2022a} (  \num{3.51} ) ( \num{10.3} ) ( -- , -- , \num{1} )};
\draw (wang2022a.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-38.000000*\dy) {\citeauthor{biondo2012}};
\node[fund, ref] (biondo2012) at (\xSepOne + \xSepTwo,-39.000000*\dy) {\reftext{Bion12}\cite{biondo2012} (  \num{3.25} ) ( \num{17.1} ) ( \num{-3.29e-2} , -- , \num{1} )};
\coordinate (biondo2012C) at ($(biondo2012.west)+(\dxStart+\dy,0)$);
\node[ ref] (khalid2012) at ($(biondo2012C |- 0,-40.000000*\dy)$) {\reftext{Khal12}\cite{khalid2012} (  \num{29.0} ) ( \num{14.0} ) ( \num{-3.29e-2} , -- , \num{2} )};
\draw (khalid2012.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (das2015) at ($(khalid2012.west |- 0,-41.000000*\dy)$) {\reftext{Das15}\cite{das2015} (  \num{3.25} ) ( \num{17.1} ) ( \num{-3.29e-3} , -- , \num{1} )};
\draw (das2015.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-43.000000*\dy) {\citeauthor{sun2012}};
\node[fund, ref] (sun2012) at (\xSepOne + \xSepTwo,-44.000000*\dy) {\reftext{Sun12}\cite{sun2012} (  \num{1.861} ) ( \num{9.986} ) ( -- , -- , \num{1.11} )};
\coordinate (sun2012C) at ($(sun2012.west)+(\dxStart+\dy,0)$);
\node[ ref] (sun2012a) at ($(sun2012C |- 0,-45.000000*\dy)$) {\reftext{Sun12a}\cite{sun2012a} (  \num{1.861} ) ( \num{9.986} ) ( -- , -- , \num{1.11} )};
\draw (sun2012a.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-47.000000*\dy) {\citeauthor{niwa2014}};
\node[fund, ref] (niwa2014) at (\xSepOne + \xSepTwo,-48.000000*\dy) {\reftext{Niwa14}\cite{niwa2014} (  \num{4.513} ) ( \num{12.82} ) ( -- , \num{1.38e-3} , \num{1} )};
\coordinate (niwa2014C) at ($(niwa2014.west)+(\dxStart+\dy,0)$);
\node[ ref] (mcpherson2021) at ($(niwa2014C |- 0,-49.000000*\dy)$) {\reftext{Mcph21}\cite{mcpherson2021} (  -- ) ( -- ) ( -- , -- , -- )};
\draw (mcpherson2021.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-51.000000*\dy) {\citeauthor{niwa2015}};
\node[fund, ref] (niwa2015) at (\xSepOne + \xSepTwo,-52.000000*\dy) {\reftext{Niwa15}\cite{niwa2015} (  \num{3.14} , -- ) ( \num{11.8} , -- ) ( \num{6.3e-3} , \num{1.23e-3} , \num{1.02} )};
\coordinate (niwa2015C) at ($(niwa2015.west)+(\dxStart+\dy,0)$);
\node[ ref] (kimoto2018) at ($(niwa2015C |- 0,-53.000000*\dy)$) {\reftext{Kimo18}\cite{kimoto2018} (  \num{3.14} , -- ) ( \num{11.8} , -- ) ( \num{6.3e-3} , \num{1.23e-3} , \num{1.02} )};
\draw (kimoto2018.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (arvanitopoulos2019) at ($(kimoto2018.west |- 0,-54.000000*\dy)$) {\reftext{Arva19}\cite{arvanitopoulos2019} (  -- , \num{3.14} ) ( -- , \num{11.8} ) ( -- , -- , \num{1.02} )};
\draw (arvanitopoulos2019.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (kimoto2019) at ($(arvanitopoulos2019.west |- 0,-55.000000*\dy)$) {\reftext{Kimo19}\cite{kimoto2019} (  \num{3.12} , -- ) ( \num{11.8} , -- ) ( -- , -- , \num{1.02} )};
\draw (kimoto2019.west) -| ++(-\dy,\fy*\dy);
\node[desc] at (\xSepOne + \xSepTwo,-59.500000*\dy) {Thornber ($\underbrace{\lambda / \langle \eion \rangle / \ephonon / \ekbt}_{\text{electron}}$ ) ( $\underbrace{\lambda / \langle \eion \rangle / \ephonon / \ekbt}_{\text{hole}}$)};
\node[author] at (\xSepOne + \xSepTwo,-61.000000*\dy) {\citeauthor{konstantinov1997}};
\node[fund, ref] (konstantinov1997) at (\xSepOne + \xSepTwo,-62.000000*\dy) {\reftext{Kons97}\cite{konstantinov1997} (  \num{29.9} / \num{10.0} / \num{120.0} / \num{0.0} ) ( \num{32.5} / \num{7.0} / \num{120.0} / \num{0.0}  )};
\coordinate (konstantinov1997C) at ($(konstantinov1997.west)+(\dxStart+\dy,0)$);
\node[ ref] (huang1998) at ($(konstantinov1997C |- 0,-63.000000*\dy)$) {\reftext{Huan98}\cite{huang1998} (  \num{29.9} / \num{10.0} / \num{120.0} / \num{0.0} ) ( \num{32.5} / \num{7.0} / \num{120.0} / \num{0.0}  )};
\draw (huang1998.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (konstantinov1998) at ($(huang1998.west |- 0,-64.000000*\dy)$) {\reftext{Kons98}\cite{konstantinov1998} (  \num{29.9} / \num{10.0} / \num{120.0} / \num{0.0} ) ( \num{32.5} / \num{7.0} / \num{120.0} / \num{0.0}  )};
\draw (konstantinov1998.west) -| ++(-\dy,\fy*\dy);


==> data/IncompIon_Al.tex <==
\pgfplotsset{cycle list name=meas}
\addplot+[only marks] coordinates {(4.2e15,365)};
\addlegendentry{\reftext{Mats03}\cite{matsuura2003}~\textit{d}}
\addplot+[only marks] coordinates {(1.4e15,410) (1.6e15,390) (1e16,365) (1e16,350) (7e16,340)};
\addlegendentry{\reftext{Mats04}\cite{matsuura2004}~\textit{d}}
\addplot+[only marks] coordinates {(4.1e16,305) (9e16,300) (9e16,270) (8e16,280)};
\addlegendentry{\reftext{Weis18}\cite{weisse2018}~\textit{d}}
\addlegendimage{empty legend}
\addlegendentry{}
\addlegendimage{empty legend}
\addlegendentry{}
\addlegendimage{empty legend}
\addlegendentry{}
\addlegendimage{empty legend}
\addlegendentry{}
\addplot+[only marks] coordinates {(7.71e15,266)};
\addlegendentry{\reftext{Smit98}\cite{smith1998}~\textit{c}}
\addplot+[only marks] coordinates {(1.33e17,265)};
\addlegendentry{\reftext{Saks01}\cite{saks2001}~\textit{c}}
\addplot+[only marks] coordinates {(8e16,201.3)};
\addlegendentry{\reftext{Ivan05}\cite{ivanov2005}~\textit{c}}
\addplot+[only marks] coordinates {(8e17,260) (3e18,260)};
\addlegendentry{\reftext{Pern05}\cite{pernot2005}~\textit{c}}
\addplot+[only marks] coordinates {(1e16,290) (1e16,350)};
\addlegendentry{\reftext{Hitc22}\cite{hitchcock2022}~\textit{c}}
\addplot+[only marks] coordinates {(7.71e15,212) (1.548e16,181) (6.329e15,172) (5.358e18,172)};
\addlegendentry{\reftext{Smit98}\cite{smith1998}~\textit{h}}
\addplot+[only marks] coordinates {(8e16,197.9)};
\addlegendentry{\reftext{Ivan05}\cite{ivanov2005}~\textit{h}}
\addplot+[only marks] coordinates {(1e19,191)};
\addlegendentry{\reftext{Iked80}\cite{ikeda1980}}
\addplot+[only marks] coordinates {(3.5e18,184) (2.5e18,187) (8.3e18,183) (7.2e18,182) (5.4e18,183) (4.6e18,183)};
\addlegendentry{\reftext{Scha97}\cite{schadt1997}}
\addplot+[only marks] coordinates {(4.6e18,183) (8.3e18,183)};
\addlegendentry{\reftext{Trof97}\cite{troffer1997}}
\addplot+[only marks] coordinates {(5e18,180)};
\addlegendentry{\reftext{Itoh98}\cite{itoh1998}}
\addplot+[only marks] coordinates {(1e18,230) (1e19,207)};
\addlegendentry{\reftext{Rao99}\cite{rao1999}}
\addplot+[only marks] coordinates {(2.5e16,228) (2.8e16,208) (7e18,238) (7.6e18,220)};
\addlegendentry{\reftext{Scho99}\cite{schoner1999}}
\addplot+[only marks] coordinates {(1e19,160) (1e19,165)};
\addlegendentry{\reftext{Tana00}\cite{tanaka2000}}
\addplot+[only marks] coordinates {(2e16,230) (2e17,226) (10e17,213)};
\addlegendentry{\reftext{Wagn02}\cite{wagner2002}}
\addplot+[only marks] coordinates {(4.8e17,199)};
\addlegendentry{\reftext{Ivan03}\cite{ivanov2003}}
\addplot+[only marks] coordinates {(6.2e15,203)};
\addlegendentry{\reftext{Mats03}\cite{matsuura2003}}
\addplot+[only marks] coordinates {(2.6e18,196)};
\addlegendentry{\reftext{Pens03}\cite{pensl2003}}
\addplot+[only marks] coordinates {(2.5e17,200) (4.5e18,195) (1.1e19,185)};
\addlegendentry{\reftext{Kasa04}\cite{kasamakova-kolaklieva2004}}
\addplot+[only marks] coordinates {(1.2e15,210) (1.5e15,230) (6e15,205) (6e15,220) (6e16,200) (8e18,190)};
\addlegendentry{\reftext{Mats04}\cite{matsuura2004}}
\addplot+[only marks] coordinates {(1.8e20,120) (1.8e20,140) (1.8e20,150) (1.8e20,170) (1.8e20,190)};
\addlegendentry{\reftext{Saks04}\cite{saks2004}}
\addplot+[only marks] coordinates {(2.6e18,196) (1.2e18,205) (2e18,200) (1.6e18,216) (2.7e17,221) (2.8e16,227) (1.8e15,240)};
\addlegendentry{\reftext{Schm04}\cite{schmid2004}}
\addplot+[only marks] coordinates {(8e17,180) (3e18,175) (8.5e18,162) (2.8e19,143) (1.7e20,80)};
\addlegendentry{\reftext{Pern05}\cite{pernot2005}}
\addplot+[only marks] coordinates {(2.25e19,206)};
\addlegendentry{\reftext{Ober07}\cite{obernhofer2007}}
\addplot+[only marks] coordinates {(8.7e20,0)};
\addlegendentry{\reftext{Acha08}\cite{achatz2008}}
\addplot+[only marks] coordinates {(5e19,118) (2e19,140) (1e19,154) (5e18,161) (5e19,111) (2e19,140) (1e19,153) (5e18,157)};
\addlegendentry{\reftext{Ramb08}\cite{rambach2008}}
\addplot+[only marks] coordinates {(3e15,275) (1.8e17,245) (4e17,240) (9e17,250) (8e17,200) (2.5e18,200) (2.8e19,155) (6e19,140)};
\addlegendentry{\reftext{Koiz09}\cite{koizumi2009}}
\addplot+[only marks] coordinates {(3e15,200)};
\addlegendentry{\reftext{Belj10}\cite{beljakowa2010}}
\addplot+[only marks] coordinates {(5e14,220)};
\addlegendentry{\reftext{Mand12}\cite{mandal2012}}
\addplot+[only marks] coordinates {(9.6e19,170) (1.5e20,70)};
\addlegendentry{\reftext{Ji13}\cite{ji2013}}
\addplot+[only marks] coordinates {(1e19,146)};
\addlegendentry{\reftext{Nipo13}\cite{nipoti2013}}
\addplot+[only marks] coordinates {(2.06e18,217) (2.8e17,218) (2.1e16,232) (1.6e15,250) (8.37e18,166) (4.2e19,133) (1.01e20,102)};
\addlegendentry{\reftext{Pari13}\cite{parisini2013}}
\addplot+[only marks] coordinates {(1.1e16,190) (1e17,190) (6.8e17,190) (7.5e18,190)};
\addlegendentry{\reftext{Kawa15}\cite{kawahara2015}}
\addplot+[only marks] coordinates {(5.8e14,220) (1.5e15,210) (4.6e15,200) (1.2e16,200) (2e16,200) (6.5e16,190) (3e17,190) (5.5e17,180) (7.1e18,170)};
\addlegendentry{\reftext{Asad16}\cite{asada2016}}
\addplot+[only marks] coordinates {(2e19,160) (1e19,190)};
\addlegendentry{\reftext{Cont16}\cite{contreras2016}}
\addplot+[only marks] coordinates {(1.4e17,211) (1.7e19,180) (4e18,200) (7e19,125) (1.4e17,125) (2e19,100)};
\addlegendentry{\reftext{Arvi17}\cite{arvinte2017}}
\addplot+[only marks] coordinates {(3.8e17,185) (5e17,185) (1.2e18,177) (2.5e19,120) (5e19,100)};
\addlegendentry{\reftext{Weis18}\cite{weisse2018}}
\addplot+[only marks] coordinates {(1e19,186) (1.35e19,93) (0.9e19,98) (3.9e19,72) (9.6e19,101) (8.6e19,81) (7.6e19,74)};
\addlegendentry{\reftext{Kaji21}\cite{kajikawa2021}}



\addlegendimage{empty legend}
\addlegendentry{}
\addlegendimage{empty legend}
\addlegendentry{}
\addlegendimage{empty legend}
\addlegendentry{}
\addlegendimage{empty legend}
\addlegendentry{}
\pgfplotsset{cycle list name=PB}
\pgfplotsset{cycle list shift=\cs}

\addplot+[domain=\xMinPB:\xMaxPB, no marks, samples=\samples] {PB(241.6,2.35e-5)};
\addlegendentry{\reftext{Scho94}\cite{schoner1994}}
\addplot+[domain=\xMinPB:\xMaxPB, no marks, samples=\samples] {PB(413,2.07e-4)};
\addlegendentry{\reftext{Mats04}\cite{matsuura2004}~\textit{d}}
\addplot+[domain=\xMinPB:\xMaxPB, no marks, samples=\samples] {PB(220,1.9e-5)};
\addlegendentry{\reftext{Mats04}\cite{matsuura2004}}
\addplot+[domain=\xMinPB:\xMaxPB, no marks, samples=\samples] {PB(205,1.7e-5)};
\addlegendentry{\reftext{Pern05}\cite{pernot2005}}
\addplot+[domain=\xMinPB:\xMaxPB, no marks, samples=\samples] {PB(220,2.32e-5)};
\addlegendentry{\reftext{Acha08}\cite{achatz2008}}
\addplot+[domain=\xMinPB:\xMaxPB, no marks, samples=\samples] {PB(265,3.6e-5)};
\addlegendentry{\reftext{Koiz09}\cite{koizumi2009}}
\addplot+[domain=\xMinPB:\xMaxPB, no marks, samples=\samples] {PB(210,3.1e-5)};
\addlegendentry{\reftext{Buon12}\cite{buono2012}}
\addplot+[domain=\xMinPB:\xMaxPB, no marks, samples=\samples] {PB(230,2.8e-5)};
\addlegendentry{\reftext{Arvi17}\cite{arvinte2017}}
\addplot+[domain=\xMinPB:\xMaxPB, no marks, samples=\samples] {PB(210,3e-5)};
\addlegendentry{\reftext{Weis18}\cite{weisse2018}}
\addplot+[domain=\xMinPB:\xMaxPB, no marks, samples=\samples] {logistic(214.86,8.12E+19,0.632)};
\addlegendentry{\reftext{Darm19}\cite{darmody2019} (\ref{eq:incompIon_logistic})}
\addplot+[domain=\xMinPB:\xMaxPB, no marks, samples=\samples] {PB(220,4.7e-5)};
\addlegendentry{\reftext{Kaji21}\cite{kajikawa2021}}
\addplot+[domain=\xMinPB:\xMaxPB, no marks, samples=\samples] {PB(230,1.8e-5)};
\addlegendentry{\reftext{Lech21}\cite{lechner2021}}


==> data/IncompIon_Al_stat_alpha.tex <==
\addplot+ [ boxplot prepared = { lower whisker=1.7000e-05, lower quartile=1.8750e-05, median=2.5750e-05, upper quartile=3.2250e-05, upper whisker=4.7000e-05, draw position=2},] coordinates {} node[mean,anchor=west] at (boxplot box cs: \boxplotvalue{median},0.5) {\pgfmathprintnumber{\boxplotvalue{median}}};


==> data/IncompIon_Al_stat_dE.tex <==
\addplot+ [ boxplot prepared = { lower whisker=2.0500e+02, lower quartile=2.1000e+02, median=2.2000e+02, upper quartile=2.3290e+02, upper whisker=2.6500e+02, },] coordinates {} node[mean,anchor=west] at (boxplot box cs: \boxplotvalue{median},0.5) {\pgfmathprintnumber{\boxplotvalue{median}}};


==> data/IncompIon_B.tex <==
\pgfplotsset{cycle list name=meas}
\addplot+[only marks] coordinates {(4.1e18,285) (10e18,285)};
\addlegendentry{\reftext{Trof97}\cite{troffer1997}}
\addplot+[only marks] coordinates {(5e18,285)};
\addlegendentry{\reftext{Itoh98}\cite{itoh1998}}
\addplot+[only marks] coordinates {(8.9e15,291) (3.9e15,332)};
\addlegendentry{\reftext{Srid98a}\cite{sridhara1998a}}
\addplot+[only marks] coordinates {(8e19,249) (3.8e17,287) (8.9e15,291) (2.9e17,329)};
\addlegendentry{\reftext{Trof98}\cite{troffer1998}}



\pgfplotsset{cycle list name=PB}
\pgfplotsset{cycle list shift=\cs}

\addplot+[domain=\xMinPB:\xMaxPB, no marks, samples=\samples] {PB(345,3.1e-5)};
\addlegendentry{\reftext{Lech21}\cite{lechner2021}}
\addplot+[domain=\xMinPB:\xMaxPB, no marks, samples=\samples] {PB(311,1.41E-05)};
\addlegendentry{t.w.}


==> data/IncompIon_N.tex <==
\pgfplotsset{cycle list name=meas}
\addplot+[only marks] coordinates {(5e17,130)};
\addlegendentry{\reftext{Hage73}\cite{hagen1973}~\textit{c}}
\addplot+[only marks] coordinates {(1e18,124)};
\addlegendentry{\reftext{Iked80}\cite{ikeda1980}~\textit{c}}
\addplot+[only marks] coordinates {(1e18,113)};
\addlegendentry{\reftext{Gorb87}\cite{gorban1987}~\textit{c}}
\addplot+[only marks] coordinates {(7e17,91.8) (7e17,100) (1e17,96) (5e16,105)};
\addlegendentry{\reftext{Gotz93}\cite{gotz1993}~\textit{c}}
\addplot+[only marks] coordinates {(1.5e17,100)};
\addlegendentry{\reftext{Pens93}\cite{pensl1993}~\textit{c}}
\addplot+[only marks] coordinates {(3e15,105) (2e16,125)};
\addlegendentry{\reftext{Kimo95}\cite{kimoto1995}~\textit{c}}
\addplot+[only marks] coordinates {(1.5e17,100)};
\addlegendentry{\reftext{Evwa96}\cite{evwaraye1996}~\textit{c}}
\addplot+[only marks] coordinates {(1.8e18,67) (2.1e18,61) (1.7e18,58)};
\addlegendentry{\reftext{Scha97}\cite{schadt1997}~\textit{c}}
\addplot+[only marks] coordinates {(2.8e15,119) (3e16,110) (1.3e15,132.5) (1.4e15,124.8) (8.2e15,117)};
\addlegendentry{\reftext{Ruts98}\cite{rutsch1998}~\textit{c}}
\addplot+[only marks] coordinates {(3.04e16,124)};
\addlegendentry{\reftext{Mats99}\cite{matsuura1999}~\textit{c}}
\addplot+[only marks] coordinates {(5.8e18,120) (5.6e18,75)};
\addlegendentry{\reftext{Scho99}\cite{schoner1999}~\textit{c}}
\addplot+[only marks] coordinates {(4.5e17,84)};
\addlegendentry{\reftext{Capa00}\cite{capano2000}~\textit{c}}
\addplot+[only marks] coordinates {(1.75e15,110) (2.6e16,95) (6.9e16,95) (1.1e17,95) (3.75e17,85)};
\addlegendentry{\reftext{Pern01}\cite{pernot2001}~\textit{c}}
\addplot+[only marks] coordinates {(1e15,117)};
\addlegendentry{\reftext{Ivan03}\cite{ivanov2003}~\textit{c}}
\addplot+[only marks] coordinates {(6.7e16,88)};
\addlegendentry{\reftext{Terz03}\cite{terziyska2003}~\textit{c}}
\addplot+[only marks] coordinates {(8.7e14,119) (2.2e15,114) (2.3e15,119) (3.5e16,114) (6.75e16,99) (9.5e17,78)};
\addlegendentry{\reftext{Kaga04}\cite{kagamihara2004}~\textit{c}}
\addplot+[only marks] coordinates {(3.5e18,89)};
\addlegendentry{\reftext{Laub04}\cite{laube2004}~\textit{c}}
\addplot+[only marks] coordinates {(1e14,125.5)};
\addlegendentry{\reftext{Ivan05}\cite{ivanov2005}~\textit{c}}
\addplot+[only marks] coordinates {(5.8e18,105)};
\addlegendentry{\reftext{Lich23}\cite{lichtenwalner2023}~\textit{c}}
\addlegendimage{empty legend}
\addlegendentry{}
\addlegendimage{empty legend}
\addlegendentry{}
\addplot+[only marks] coordinates {(3e17,80)};
\addlegendentry{\reftext{Hage73}\cite{hagen1973}~\textit{h}}
\addplot+[only marks] coordinates {(1e18,66)};
\addlegendentry{\reftext{Iked80}\cite{ikeda1980}~\textit{h}}
\addplot+[only marks] coordinates {(1e17,52.1) (7e17,45) (1e17,47) (5.1e16,41)};
\addlegendentry{\reftext{Gotz93}\cite{gotz1993}~\textit{h}}
\addplot+[only marks] coordinates {(1.5e17,45)};
\addlegendentry{\reftext{Pens93}\cite{pensl1993}~\textit{h}}
\addplot+[only marks] coordinates {(3e15,45) (1.2e16,65)};
\addlegendentry{\reftext{Kimo95}\cite{kimoto1995}~\textit{h}}
\addplot+[only marks] coordinates {(1.5e17,53)};
\addlegendentry{\reftext{Evwa96}\cite{evwaraye1996}~\textit{h}}
\addplot+[only marks] coordinates {(1.8e18,14) (2.1e18,13) (1.7e18,17)};
\addlegendentry{\reftext{Scha97}\cite{schadt1997}~\textit{h}}
\addplot+[only marks] coordinates {(4.2e16,67.3) (3.7e16,61.0) (1.1e15,82) (1.9e15,71.7) (8.2e15,66)};
\addlegendentry{\reftext{Ruts98}\cite{rutsch1998}~\textit{h}}
\addplot+[only marks] coordinates {(6.45e15,65.3)};
\addlegendentry{\reftext{Mats99}\cite{matsuura1999}~\textit{h}}
\addplot+[only marks] coordinates {(5.8e18,50) (5.6e18,35)};
\addlegendentry{\reftext{Scho99}\cite{schoner1999}~\textit{h}}
\addplot+[only marks] coordinates {(4.5e17,42)};
\addlegendentry{\reftext{Capa00}\cite{capano2000}~\textit{h}}
\addplot+[only marks] coordinates {(8e17,60.2)};
\addlegendentry{\reftext{Chen00}\cite{chen2000}~\textit{h}}
\addplot+[only marks] coordinates {(1.75e15,63) (2.6e16,61.5) (6.9e16,59) (1.1e17,58) (3.75e17,56)};
\addlegendentry{\reftext{Pern01}\cite{pernot2001}~\textit{h}}
\addplot+[only marks] coordinates {(6.7e16,62)};
\addlegendentry{\reftext{Terz03}\cite{terziyska2003}~\textit{h}}
\addplot+[only marks] coordinates {(8.7e14,73) (2.2e15,63) (2.3e15,69) (3.5e16,56) (6.8e16,53) (9.5e17,40)};
\addlegendentry{\reftext{Kaga04}\cite{kagamihara2004}~\textit{h}}
\addplot+[only marks] coordinates {(3.5e18,33)};
\addlegendentry{\reftext{Laub04}\cite{laube2004}~\textit{h}}
\addplot+[only marks] coordinates {(5.8e18,15)};
\addlegendentry{\reftext{Lich23}\cite{lichtenwalner2023}~\textit{h}}
\addlegendimage{empty legend}
\addlegendentry{}
\addlegendimage{empty legend}
\addlegendentry{}
\addlegendimage{empty legend}
\addlegendentry{}
\addlegendimage{empty legend}
\addlegendentry{}
\addplot+[only marks] coordinates {(6e17,29) (1e15,33)};
\addlegendentry{\reftext{Loma73}\cite{lomakina1973}}
\addplot+[only marks] coordinates {(1e17,45.5)};
\addlegendentry{\reftext{Kisi92}\cite{kisielowski1992}}
\addplot+[only marks] coordinates {(1e18,87) (2e19,87)};
\addlegendentry{\reftext{Rao99}\cite{rao1999}}
\addlegendimage{empty legend}
\addlegendentry{}
\addlegendimage{empty legend}
\addlegendentry{}
\addlegendimage{empty legend}
\addlegendentry{}
\addlegendimage{empty legend}
\addlegendentry{}



\pgfplotsset{cycle list name=PB}
\pgfplotsset{cycle list shift=\cs}

\addplot+[domain=\xMinPB:\xMaxPB, no marks, samples=\samples] {PB(99.6,1.41e-5)};
\addlegendentry{\reftext{Scho94}\cite{schoner1994}~\textit{c}}
\addplot+[domain=\xMinPB:\xMaxPB, no marks, samples=\samples] {PB(53.3, 1.65e-5)};
\addlegendentry{\reftext{Scho94}\cite{schoner1994}~\textit{h}}
\addplot+[domain=\xMinPB:\xMaxPB, no marks, samples=\samples] {PB(123.7,4.65e-5)};
\addlegendentry{\reftext{Kaga04}\cite{kagamihara2004}~\textit{c}}
\addplot+[domain=\xMinPB:\xMaxPB, no marks, samples=\samples] {PB(70.9,3.38e-5)};
\addlegendentry{\reftext{Kaga04}\cite{kagamihara2004}~\textit{h}}
\addplot+[domain=\xMinPB:\xMaxPB, no marks, samples=\samples] {PB(65,3.1e-5)};
\addlegendentry{\reftext{Buon12}\cite{buono2012}~\textit{e}}
\addplot+[domain=\xMinPB:\xMaxPB, no marks, samples=\samples] {PB(105,4.26e-5)};
\addlegendentry{\reftext{Hata13}\cite{hatakeyama2013}~\textit{e}}
\addplot+[domain=\xMinPB:\xMaxPB, no marks, samples=\samples] {PB(52.5,3.38e-5)};
\addlegendentry{\reftext{Lech21}\cite{lechner2021}}


==> data/IncompIon_P.tex <==
\pgfplotsset{cycle list name=meas}
\addplot+[only marks] coordinates {(8e16,93)};
\addlegendentry{\reftext{Capa00}\cite{capano2000}~\textit{c}}
\addplot+[only marks] coordinates {(16.5e17,90)};
\addlegendentry{\reftext{Schm02}\cite{schmid2002}~\textit{c}}
\addplot+[only marks] coordinates {(1.5e16,78) (1.7e15,80)};
\addlegendentry{\reftext{Wang02}\cite{wang2002}~\textit{c}}
\addplot+[only marks] coordinates {(2.6e18,95)};
\addlegendentry{\reftext{Laub04}\cite{laube2004}~\textit{c}}
\addplot+[only marks] coordinates {(2.4e16,120)};
\addlegendentry{\reftext{Ivan05}\cite{ivanov2005}~\textit{c}}
\addplot+[only marks] coordinates {(1.8e19,74) (5e18,101) (2.7e18,109)};
\addlegendentry{\reftext{Rao06}\cite{rao2006}~\textit{c}}
\addplot+[only marks] coordinates {(8e16,53)};
\addlegendentry{\reftext{Capa00}\cite{capano2000}~\textit{h}}
\addplot+[only marks] coordinates {(16.5e17,45)};
\addlegendentry{\reftext{Schm02}\cite{schmid2002}~\textit{h}}
\addplot+[only marks] coordinates {(1.7e16,50) (1.7e15,52)};
\addlegendentry{\reftext{Wang02}\cite{wang2002}~\textit{h}}
\addplot+[only marks] coordinates {(2.6e18,45)};
\addlegendentry{\reftext{Laub04}\cite{laube2004}~\textit{h}}
\addplot+[only marks] coordinates {(2.4e16,60.7)};
\addlegendentry{\reftext{Ivan05}\cite{ivanov2005}~\textit{h}}
\addplot+[only marks] coordinates {(1.6e19,26) (4.8e18,49) (2.3e18,53)};
\addlegendentry{\reftext{Rao06}\cite{rao2006}~\textit{h}}



\pgfplotsset{cycle list name=PB}
\pgfplotsset{cycle list shift=\cs}

\addplot+[domain=\xMinPB:\xMaxPB, no marks, samples=\samples] {PB(113,1.26E-05)};
\addlegendentry{t.w.~\textit{c}}
\addplot+[domain=\xMinPB:\xMaxPB, no marks, samples=\samples] {PB(57,9.54E-06)};
\addlegendentry{t.w.~\textit{h}}


==> data/IncompIon_TCAD.tex <==


\node[symbol] (Al) at (0,0) {Al};
\coordinate (Al0) at (Al.north);
\node[ref, lwAl] (Al1) at (Al0.north west) {\tikz \node[paper,fund] {\reftext{Hage73}\cite{hagen1973}};};
\node[value, scale=1.100000] (Alvalue1) at (Al1.west) {\num{150+-5}+$\ex$};
\node[ref, lwAl] (Al2) at (Al1.north west) {\tikz \node[paper] {\reftext{Harr95}\cite{harris1995}};};
\node[value, scale=1.100000] (Alvalue2) at (Al2.west) {\num{155}+$\ex$};
\node[ref, lwAl] (Al3) at (Al2.north west) {\tikz \node[paper] {\reftext{Harr95}\cite{harris1995}}; \tikz \node[paper,fund] {\reftext{Mats74}\cite{matsunami1974}};};
\node[value, scale=1.200000] (Alvalue3) at (Al3.west) {\num{160}+$\ex$};
\node[ref, lwAl] (Al4) at (Al3.north west) {\tikz \node[paper] {\reftext{Dali03}\cite{dalibor2003}}; \tikz \node[paper] {\reftext{Harr95}\cite{harris1995}}; \tikz \node[paper,fund] {\reftext{Suzu77}\cite{suzuki1977}};};
\node[value, scale=1.300000] (Alvalue4) at (Al4.west) {\num{168}+$\ex$};
\node[ref, lwAl] (Al5) at (Al4.north west) {\tikz \node[paper,fund] {\reftext{Suzu73}\cite{suzuki1973}};};
\node[value, scale=1.100000] (Alvalue5) at (Al5.west) {\num{170}+$\ex$};
\node[ref, lwAl] (Al6) at (Al5.north west) {\tikz \node[paper] {\reftext{Harr95}\cite{harris1995}};};
\node[value, scale=1.100000] (Alvalue6) at (Al6.west) {\num{180}};
\node[ref, lwAl] (Al7) at (Al6.north west) {\tikz \node[paper] {\reftext{Dali03}\cite{dalibor2003}};};
\node[value, scale=1.100000] (Alvalue7) at (Al7.west) {\num{183}};
\node[ref, lwAl] (Al8) at (Al7.north west) {\tikz \node[paper] {\reftext{Dali03}\cite{dalibor2003}};};
\node[value, scale=1.100000] (Alvalue8) at (Al8.west) {\num{185}};
\node[ref, lwAl] (Al9) at (Al8.north west) {\tikz \node[paper] {\reftext{Yosh18}\cite{yoshioka2018}}; \tikz \node[paper] {\reftext{Megh18}\cite{megherbi2018}}; \tikz \node[paper] {\reftext{Wije11}\cite{wijesundara2011}}; \tikz \node[paper] {\reftext{Nego04}\cite{negoro2004}}; \tikz \node[paper] {\reftext{Nego03}\cite{negoro2003}}; \tikz \node[paper] {\reftext{Levi01}\cite{levinshtein2001}}; \tikz \node[paper] {\reftext{Gao01}\cite{gao2001}};};
\node[value, scale=1.700000] (Alvalue9) at (Al9.west) {\num{190}};
\node[ref, lwAl] (Al10) at (Al9.north west) {\tikz \node[paper] {\reftext{Ioff23}\cite{ioffe2023}}; \tikz \node[paper] {\reftext{Kwas14}\cite{kwasnicki2014}}; \tikz \node[paper] {\reftext{Fan14}\cite{fan2014}}; \tikz \node[paper] {\reftext{Zhan10}\cite{zhang2010}}; \tikz \node[paper] {\reftext{Bhat05}\cite{bhatnagar2005}}; \tikz \node[paper] {\reftext{Zhao03}\cite{zhao2003}}; \tikz \node[paper] {\reftext{Dali03}\cite{dalibor2003}}; \tikz \node[paper] {\reftext{Wang99}\cite{wang1999}}; \tikz \node[paper] {\reftext{Pers98}\cite{persson1998}}; \tikz \node[paper] {\reftext{Greu97}\cite{greulich-weber1997}}; \tikz \node[paper] {\reftext{Bako97}\cite{bakowski1997}}; \tikz \node[paper] {\reftext{Harr95}\cite{harris1995}}; \tikz \node[paper] {\reftext{Frei95}\cite{freitas1995}}; \tikz \node[paper] {\reftext{Made91}\cite{madelung1991}};};
\node[value, scale=2.400000] (Alvalue10) at (Al10.west) {\num{191}};
\node[ref, lwAl] (Al11) at (Al10.north west) {\tikz \node[paper] {\reftext{Kimo14a}\cite{kimoto2014a}~\textit{h}}; \tikz \node[paper] {\reftext{Janz08}\cite{janzen2008}~\textit{h}};};
\node[value, scale=1.200000] (Alvalue11) at (Al11.west) {\num{197.9}};
\node[ref, lwAl] (Al12) at (Al11.north west) {\tikz \node[paper] {\reftext{Kimo19}\cite{kimoto2019}~\textit{h}}; \tikz \node[paper] {\reftext{Nipo18}\cite{nipoti2018}~\textit{h}}; \tikz \node[paper] {\reftext{Kimo15}\cite{kimoto2015}~\textit{h}};};
\node[value, scale=1.300000] (Alvalue12) at (Al12.west) {\num{198}};
\node[ref, lwAl] (Al13) at (Al12.north west) {\tikz \node[paper] {\reftext{Pank14}\cite{pankove2014}}; \tikz \node[paper] {\reftext{Zhu08}\cite{zhu2008}}; \tikz \node[paper] {\reftext{Neud06}\cite{neudeck2006}}; \tikz \node[paper] {\reftext{Bali06}\cite{baliga2006}}; \tikz \node[paper] {\reftext{Zett02}\cite{zetterling2002}}; \tikz \node[paper] {\reftext{Mart02}\cite{martinez2002}}; \tikz \node[paper] {\reftext{Neud01}\cite{neudeck2001}}; \tikz \node[paper] {\reftext{Habe94}\cite{haberstroh1994}}; \tikz \node[paper,fund] {\reftext{Pens93}\cite{pensl1993}};};
\node[value, scale=1.900000] (Alvalue13) at (Al13.west) {\num{200}};
\node[ref, lwAl] (Al14) at (Al13.north west) {\tikz \node[paper] {\reftext{Kimo19}\cite{kimoto2019}~\textit{c}}; \tikz \node[paper] {\reftext{Kimo15}\cite{kimoto2015}~\textit{c}};};
\node[value, scale=1.200000] (Alvalue14) at (Al14.west) {\num{201}};
\node[ref, lwAl] (Al15) at (Al14.north west) {\tikz \node[paper] {\reftext{Tian20}\cite{tian2020}}; \tikz \node[paper] {\reftext{Kimo14a}\cite{kimoto2014a}~\textit{c}}; \tikz \node[paper] {\reftext{Janz08}\cite{janzen2008}~\textit{c}};};
\node[value, scale=1.300000] (Alvalue15) at (Al15.west) {\num{201.3}};
\node[ref, lwAl] (Al16) at (Al15.north west) {\tikz \node[paper,fund] {\reftext{Alba10}\cite{albanese2010}}; \tikz \node[paper] {\reftext{Schr06}\cite{schroeder2006}}; \tikz \node[paper,fund] {\reftext{Lade00}\cite{ladesmartin2000}};};
\node[value, scale=1.300000] (Alvalue16) at (Al16.west) {\num{210+-20}};
\node[ref, lwAl] (Al17) at (Al16.north west) {\tikz \node[paper] {\reftext{Nipo18}\cite{nipoti2018}~\textit{c}}; \tikz \node[paper] {\reftext{Lutz18}\cite{lutz2018}}; \tikz \node[paper] {\reftext{Usma12}\cite{usman2012}}; \tikz \node[paper] {\reftext{Lutz11}\cite{lutz2011}}; \tikz \node[paper] {\reftext{Buon10}\cite{buono2010}};};
\node[value, scale=1.500000] (Alvalue17) at (Al17.west) {\num{210}};
\node[ref, lwAl] (Al18) at (Al17.north west) {\tikz \node[paper] {\reftext{Lu21}\cite{lu2021}}; \tikz \node[paper] {\reftext{Trew02}\cite{trew2002}};};
\node[value, scale=1.200000] (Alvalue18) at (Al18.west) {\num{220}};
\node[ref, lwAl] (Al19) at (Al18.north west) {\tikz \node[paper] {\reftext{Ayal05}\cite{ayalew2005}}; \tikz \node[paper,fund] {\reftext{Ayal04}\cite{ayalew2004}};};
\node[value, scale=1.200000] (Alvalue19) at (Al19.west) {\num{220+-20}};
\node[ref, lwAl] (Al20) at (Al19.north west) {\tikz \node[paper] {\reftext{Huan22b}\cite{huang2022b}}; \tikz \node[paper,fund] {\reftext{Huan22a}\cite{huang2022a}}; \tikz \node[paper] {\reftext{Lebe99}\cite{lebedev1999}};};
\node[value, scale=1.300000] (Alvalue20) at (Al20.west) {\num{230}};
\node[ref, lwAl] (Al21) at (Al20.north west) {\tikz \node[paper] {\reftext{Kwas14}\cite{kwasnicki2014}}; \tikz \node[paper] {\reftext{Feng04a}\cite{feng2004a}};};
\node[value, scale=1.200000] (Alvalue21) at (Al21.west) {\num{240}};
\node[ref, lwAl] (Al22) at (Al21.north west) {\tikz \node[paper] {\reftext{Tiwa19a}\cite{tiwari2019a}}; \tikz \node[paper] {\reftext{Tiwa19}\cite{tiwari2019}}; \tikz \node[paper] {\reftext{Sozz19}\cite{sozzi2019}}; \tikz \node[paper] {\reftext{Joha19}\cite{johannesson2019}}; \tikz \node[paper] {\reftext{Loph18}\cite{lophitis2018}}; \tikz \node[paper] {\reftext{Dona18}\cite{donato2018}}; \tikz \node[paper] {\reftext{Arva17}\cite{arvanitopoulos2017}};};
\node[value, scale=1.700000] (Alvalue22) at (Al22.west) {\num{265}};
\node[ref, lwAl] (Al23) at (Al22.north west) {\tikz \node[paper] {\reftext{Pank14}\cite{pankove2014}}; \tikz \node[paper, no4H] {\reftext{Heni13}\cite{henisch2013}}; \tikz \node[paper] {\reftext{Harr95}\cite{harris1995}};};
\node[value, scale=1.300000] (Alvalue23) at (Al23.west) {\num{270}};


\node[symbol] (B) at (0+ \dxAl,0) {B};
\coordinate (B0) at (B.north);
\node[ref, lwB] (B1) at (B0.north west) {\tikz \node[paper] {\reftext{Dali03}\cite{dalibor2003}};};
\node[value, scale=1.100000] (Bvalue1) at (B1.west) {\num{260}};
\node[ref, lwB] (B2) at (B1.north west) {\tikz \node[paper] {\reftext{Kimo15}\cite{kimoto2015}}; \tikz \node[paper] {\reftext{Kimo14a}\cite{kimoto2014a}};};
\node[value, scale=1.200000] (Bvalue2) at (B2.west) {\num{280}};
\node[ref, lwB] (B3) at (B2.north west) {\tikz \node[paper] {\reftext{Wije11}\cite{wijesundara2011}}; \tikz \node[paper] {\reftext{Zhu08}\cite{zhu2008}}; \tikz \node[paper] {\reftext{Nego03}\cite{negoro2003}}; \tikz \node[paper] {\reftext{Dali03}\cite{dalibor2003}}; \tikz \node[paper] {\reftext{Zett02}\cite{zetterling2002}};};
\node[value, scale=1.500000] (Bvalue3) at (B3.west) {\num{285}};
\node[ref, lwB] (B4) at (B3.north west) {\tikz \node[paper] {\reftext{Lebe99}\cite{lebedev1999}};};
\node[value, scale=1.100000] (Bvalue4) at (B4.west) {\num{290}};
\node[ref, lwB] (B5) at (B4.north west) {\tikz \node[paper] {\reftext{Loph18}\cite{lophitis2018}}; \tikz \node[paper] {\reftext{Dona18}\cite{donato2018}}; \tikz \node[paper] {\reftext{Arva17}\cite{arvanitopoulos2017}};};
\node[value, scale=1.300000] (Bvalue5) at (B5.west) {\num{293}};
\node[ref, lwB] (B6) at (B5.north west) {\tikz \node[paper] {\reftext{Rakh20}\cite{rakheja2020}}; \tikz \node[paper, no4H] {\reftext{Sull08}\cite{sullivan2008}}; \tikz \node[paper] {\reftext{Neud06}\cite{neudeck2006}}; \tikz \node[paper] {\reftext{Huh06}\cite{huh2006}}; \tikz \node[paper] {\reftext{Neud01}\cite{neudeck2001}}; \tikz \node[paper] {\reftext{Gao01}\cite{gao2001}};};
\node[value, scale=1.600000] (Bvalue6) at (B6.west) {\num{300}};
\node[ref, lwB] (B7) at (B6.north west) {\tikz \node[paper] {\reftext{Dali03}\cite{dalibor2003}};};
\node[value, scale=1.100000] (Bvalue7) at (B7.west) {\num{310}};
\node[ref, lwB] (B8) at (B7.north west) {\tikz \node[paper] {\reftext{Schr06}\cite{schroeder2006}}; \tikz \node[paper,fund] {\reftext{Lade00}\cite{ladesmartin2000}};};
\node[value, scale=1.200000] (Bvalue8) at (B8.west) {\num{320+-20}};
\node[ref, lwB] (B9) at (B8.north west) {\tikz \node[paper,fund] {\reftext{Torr22}\cite{torres2022}~\textit{h}}; \tikz \node[paper] {\reftext{Lutz18}\cite{lutz2018}}; \tikz \node[paper] {\reftext{Lutz11}\cite{lutz2011}}; \tikz \node[paper,fund] {\reftext{Saks01}\cite{saks2001}};};
\node[value, scale=1.400000] (Bvalue9) at (B9.west) {\num{320}};
\node[ref, lwB] (B10) at (B9.north west) {\tikz \node[paper,fund] {\reftext{Alba10}\cite{albanese2010}}; \tikz \node[paper] {\reftext{Ayal05}\cite{ayalew2005}}; \tikz \node[paper,fund] {\reftext{Ayal04}\cite{ayalew2004}};};
\node[value, scale=1.300000] (Bvalue10) at (B10.west) {\num{330+-30}};
\node[ref, lwB] (B11) at (B10.north west) {\tikz \node[paper,fund] {\reftext{Torr22}\cite{torres2022}~\textit{c}};};
\node[value, scale=1.100000] (Bvalue11) at (B11.west) {\num{340}};
\node[ref, lwB] (B12) at (B11.north west) {\tikz \node[paper] {\reftext{Feng04a}\cite{feng2004a}};};
\node[value, scale=1.100000] (Bvalue12) at (B12.west) {\num{350}};
\node[ref, lwB] (B13) at (B12.north west) {\tikz \node[paper] {\reftext{Rayn10}\cite{raynaud2010}};};
\node[value, scale=1.100000] (Bvalue13) at (B13.west) {\num{370}};
\node[ref, lwB] (B14) at (B13.north west) {\tikz \node[paper] {\reftext{Pank14}\cite{pankove2014}}; \tikz \node[paper, no4H] {\reftext{Heni13}\cite{henisch2013}};};
\node[value, scale=1.200000] (Bvalue14) at (B14.west) {\num{390}};
\node[ref, lwB] (B15) at (B14.north west) {\tikz \node[paper] {\reftext{Harr95}\cite{harris1995}}; \tikz \node[paper,fund] {\reftext{Suzu77}\cite{suzuki1977}};};
\node[value, scale=1.200000] (Bvalue15) at (B15.west) {\num{628}+$\ex$};
\node[ref, lwB] (B16) at (B15.north west) {\tikz \node[paper,fund] {\reftext{Deva97}\cite{devaty1997}};};
\node[value, scale=1.100000] (Bvalue16) at (B16.west) {\num{628+-1}+$\ex$};
\node[ref, lwB] (B17) at (B16.north west) {\tikz \node[paper] {\reftext{Ioff23}\cite{ioffe2023}}; \tikz \node[paper] {\reftext{Kwas14}\cite{kwasnicki2014}}; \tikz \node[paper] {\reftext{Fan14}\cite{fan2014}}; \tikz \node[paper] {\reftext{Greu97}\cite{greulich-weber1997}}; \tikz \node[paper] {\reftext{Harr95}\cite{harris1995}}; \tikz \node[paper] {\reftext{Made91}\cite{madelung1991}};};
\node[value, scale=1.600000] (Bvalue17) at (B17.west) {\num{647}};
\node[ref, lwB] (B18) at (B17.north west) {\tikz \node[paper] {\reftext{Levi01}\cite{levinshtein2001}};};
\node[value, scale=1.100000] (Bvalue18) at (B18.west) {\num{650}};
\node[ref, lwB] (B19) at (B18.north west) {\tikz \node[paper] {\reftext{Gao01}\cite{gao2001}};};
\node[value, scale=1.100000] (Bvalue19) at (B19.west) {\num{700}};


\node[symbol] (N) at (0+ \dxAl+ \dxB,0) {N};
\coordinate (N0) at (N.north);
\node[ref, lwN] (N1) at (N0.north west) {\tikz \node[paper] {\reftext{Pank14}\cite{pankove2014}}; \tikz \node[paper] {\reftext{Harr95}\cite{harris1995}~\textit{e}}; \tikz \node[paper] {\reftext{Loma74}\cite{lomakina1974}};};
\node[value, scale=1.300000] (Nvalue1) at (N1.west) {\num{33}};
\node[ref, lwN] (N2) at (N1.north west) {\tikz \node[paper] {\reftext{Harr95}\cite{harris1995}~\textit{e}};};
\node[value, scale=1.100000] (Nvalue2) at (N2.west) {\num{40}};
\node[ref, lwN] (N3) at (N2.north west) {\tikz \node[paper] {\reftext{Zhan10}\cite{zhang2010}};};
\node[value, scale=1.100000] (Nvalue3) at (N3.west) {\num{42}};
\node[ref, lwN] (N4) at (N3.north west) {\tikz \node[paper,fund] {\reftext{Son06}\cite{son2006}~\textit{h}};};
\node[value, scale=1.100000] (Nvalue4) at (N4.west) {\num{44}};
\node[ref, lwN] (N5) at (N4.north west) {\tikz \node[paper] {\reftext{Wije11}\cite{wijesundara2011}}; \tikz \node[paper] {\reftext{Neud06}\cite{neudeck2006}}; \tikz \node[paper] {\reftext{Neud01}\cite{neudeck2001}}; \tikz \node[paper] {\reftext{Mick98}\cite{mickevicius1998}~\textit{h}}; \tikz \node[paper] {\reftext{Harr95}\cite{harris1995}~\textit{h}};};
\node[value, scale=1.500000] (Nvalue5) at (N5.west) {\num{45}};
\node[ref, lwN] (N6) at (N5.north west) {\tikz \node[paper,fund] {\reftext{Alba10}\cite{albanese2010}~\textit{h}}; \tikz \node[paper] {\reftext{Schr06}\cite{schroeder2006}~\textit{h}}; \tikz \node[paper] {\reftext{Ayal05}\cite{ayalew2005}~\textit{h}}; \tikz \node[paper,fund] {\reftext{Ayal04}\cite{ayalew2004}~\textit{h}}; \tikz \node[paper,fund] {\reftext{Lade00}\cite{ladesmartin2000}~\textit{h}};};
\node[value, scale=1.500000] (Nvalue6) at (N6.west) {\num{50+-5}};
\node[ref, lwN] (N7) at (N6.north west) {\tikz \node[paper] {\reftext{Sozz19}\cite{sozzi2019}}; \tikz \node[paper] {\reftext{Zhu08}\cite{zhu2008}~\textit{h}}; \tikz \node[paper] {\reftext{Zett02}\cite{zetterling2002}~\textit{h}};};
\node[value, scale=1.300000] (Nvalue7) at (N7.west) {\num{50}};
\node[ref, lwN] (N8) at (N7.north west) {\tikz \node[paper] {\reftext{Kwas14}\cite{kwasnicki2014}}; \tikz \node[paper] {\reftext{Pers05}\cite{persson2005}~\textit{h}}; \tikz \node[paper] {\reftext{Feng04a}\cite{feng2004a}~\textit{h}}; \tikz \node[paper] {\reftext{Dali03}\cite{dalibor2003}~\textit{h}}; \tikz \node[paper] {\reftext{Lebe99}\cite{lebedev1999}~\textit{h}};};
\node[value, scale=1.500000] (Nvalue8) at (N8.west) {\num{52}};
\node[ref, lwN] (N9) at (N8.north west) {\tikz \node[paper] {\reftext{Buon12}\cite{buono2012}~\textit{h}}; \tikz \node[paper] {\reftext{Wang99}\cite{wang1999}~\textit{h}}; \tikz \node[paper] {\reftext{Pers99a}\cite{persson1999a}~\textit{h}}; \tikz \node[paper] {\reftext{Greu97}\cite{greulich-weber1997}~\textit{h}}; \tikz \node[paper] {\reftext{Bako97}\cite{bakowski1997}~\textit{h}}; \tikz \node[paper] {\reftext{Harr95}\cite{harris1995}~\textit{h}};};
\node[value, scale=1.600000] (Nvalue9) at (N9.west) {\num{52.1}};
\node[ref, lwN] (N10) at (N9.north west) {\tikz \node[paper] {\reftext{Gerh11}\cite{gerhardt2011}~\textit{h}};};
\node[value, scale=1.100000] (Nvalue10) at (N10.west) {\num{53}};
\node[ref, lwN] (N11) at (N10.north west) {\tikz \node[paper,fund] {\reftext{Suzu77}\cite{suzuki1977}};};
\node[value, scale=1.100000] (Nvalue11) at (N11.west) {\num{55+-7}};
\node[ref, lwN] (N12) at (N11.north west) {\tikz \node[paper] {\reftext{Made91}\cite{madelung1991}~\textit{h}};};
\node[value, scale=1.100000] (Nvalue12) at (N12.west) {\num{55}};
\node[ref, lwN] (N13) at (N12.north west) {\tikz \node[paper] {\reftext{Dali03}\cite{dalibor2003}~\textit{h}}; \tikz \node[paper] {\reftext{Levi01}\cite{levinshtein2001}~\textit{h}}; \tikz \node[paper] {\reftext{Iwat01}\cite{iwata2001}~\textit{h}}; \tikz \node[paper,fund] {\reftext{Choy97d}\cite{choyke1997d}~\textit{h}};};
\node[value, scale=1.400000] (Nvalue13) at (N13.west) {\num{59}};
\node[ref, lwN] (N14) at (N13.north west) {\tikz \node[paper,fund] {\reftext{Huan22}\cite{huang2022}}; \tikz \node[paper] {\reftext{Bhat05}\cite{bhatnagar2005}~\textit{h}};};
\node[value, scale=1.200000] (Nvalue14) at (N14.west) {\num{60}};
\node[ref, lwN] (N15) at (N14.north west) {\tikz \node[paper] {\reftext{Yang19}\cite{yang2019}}; \tikz \node[paper] {\reftext{Kimo19}\cite{kimoto2019}~\textit{h}}; \tikz \node[paper] {\reftext{Kimo15}\cite{kimoto2015}~\textit{h}}; \tikz \node[paper] {\reftext{Kwas14}\cite{kwasnicki2014}};};
\node[value, scale=1.400000] (Nvalue15) at (N15.west) {\num{61}};
\node[ref, lwN] (N16) at (N15.north west) {\tikz \node[paper,fund] {\reftext{Ivan03a}\cite{ivanov2003a}~\textit{h}};};
\node[value, scale=1.100000] (Nvalue16) at (N16.west) {\num{61.4+-0.5}};
\node[ref, lwN] (N17) at (N16.north west) {\tikz \node[paper] {\reftext{Tian20}\cite{tian2020}}; \tikz \node[paper] {\reftext{Kimo14a}\cite{kimoto2014a}~\textit{h}}; \tikz \node[paper] {\reftext{Janz08}\cite{janzen2008}~\textit{h}}; \tikz \node[paper,fund] {\reftext{Ivan05}\cite{ivanov2005}~\textit{h}};};
\node[value, scale=1.400000] (Nvalue17) at (N17.west) {\num{61.4}};
\node[ref, lwN] (N18) at (N17.north west) {\tikz \node[paper,fund] {\reftext{Pern00}\cite{pernot2000}~\textit{h}};};
\node[value, scale=1.100000] (Nvalue18) at (N18.west) {\num{62}};
\node[ref, lwN] (N19) at (N18.north west) {\tikz \node[paper] {\reftext{Rakh20}\cite{rakheja2020}}; \tikz \node[paper] {\reftext{Joha19}\cite{johannesson2019}}; \tikz \node[paper] {\reftext{Usma12}\cite{usman2012}}; \tikz \node[paper] {\reftext{Buon10}\cite{buono2010}}; \tikz \node[paper] {\reftext{Wang99}\cite{wang1999}~\textit{e}}; \tikz \node[paper] {\reftext{Bako97}\cite{bakowski1997}~\textit{e}};};
\node[value, scale=1.600000] (Nvalue19) at (N19.west) {\num{65}};
\node[ref, lwN] (N20) at (N19.north west) {\tikz \node[paper] {\reftext{Ioff23}\cite{ioffe2023}~\textit{h}}; \tikz \node[paper] {\reftext{Fan14}\cite{fan2014}~\textit{h}}; \tikz \node[paper] {\reftext{Izzo08}\cite{izzo2008}~\textit{h}}; \tikz \node[paper] {\reftext{Harr95}\cite{harris1995}~\textit{h}}; \tikz \node[paper] {\reftext{Made91}\cite{madelung1991}~\textit{h}};};
\node[value, scale=1.500000] (Nvalue20) at (N20.west) {\num{66}};
\node[ref, lwN] (N21) at (N20.north west) {\tikz \node[paper] {\reftext{Megh18}\cite{megherbi2018}}; \tikz \node[paper] {\reftext{Dona18}\cite{donato2018}~\textit{h}}; \tikz \node[paper] {\reftext{Ayal05}\cite{ayalew2005}~\textit{e}}; \tikz \node[paper,fund] {\reftext{Ayal04}\cite{ayalew2004}~\textit{e}};};
\node[value, scale=1.400000] (Nvalue21) at (N21.west) {\num{70}};
\node[ref, lwN] (N22) at (N21.north west) {\tikz \node[paper] {\reftext{Tiwa19a}\cite{tiwari2019a}}; \tikz \node[paper] {\reftext{Tiwa19}\cite{tiwari2019}};};
\node[value, scale=1.200000] (Nvalue22) at (N22.west) {\num{70.9}};
\node[ref, lwN] (N23) at (N22.north west) {\tikz \node[paper] {\reftext{Loph18}\cite{lophitis2018}}; \tikz \node[paper] {\reftext{Arva17}\cite{arvanitopoulos2017}};};
\node[value, scale=1.200000] (Nvalue23) at (N23.west) {\num{71}};
\node[ref, lwN] (N24) at (N23.north west) {\tikz \node[paper] {\reftext{Lutz18}\cite{lutz2018}}; \tikz \node[paper] {\reftext{Lutz11}\cite{lutz2011}};};
\node[value, scale=1.200000] (Nvalue24) at (N24.west) {\num{77}};
\node[ref, lwN] (N25) at (N24.north west) {\tikz \node[paper, no4H] {\reftext{Sull08}\cite{sullivan2008}}; \tikz \node[paper] {\reftext{Harr95}\cite{harris1995}~\textit{h}};};
\node[value, scale=1.200000] (Nvalue25) at (N25.west) {\num{80}};
\node[ref, lwN] (N26) at (N25.north west) {\tikz \node[paper] {\reftext{Bhat05}\cite{bhatnagar2005}~\textit{e}}; \tikz \node[paper] {\reftext{Mick98}\cite{mickevicius1998}~\textit{c}};};
\node[value, scale=1.200000] (Nvalue26) at (N26.west) {\num{81}};
\node[ref, lwN] (N27) at (N26.north west) {\tikz \node[paper] {\reftext{Pank14}\cite{pankove2014}}; \tikz \node[paper] {\reftext{Harr95}\cite{harris1995}~\textit{e}};};
\node[value, scale=1.200000] (Nvalue27) at (N27.west) {\num{90}};
\node[ref, lwN] (N28) at (N27.north west) {\tikz \node[paper] {\reftext{Schr06}\cite{schroeder2006}~\textit{c}}; \tikz \node[paper,fund] {\reftext{Lade00}\cite{ladesmartin2000}~\textit{c}};};
\node[value, scale=1.200000] (Nvalue28) at (N28.west) {\num{90+-10}};
\node[ref, lwN] (N29) at (N28.north west) {\tikz \node[paper,fund] {\reftext{Alba10}\cite{albanese2010}~\textit{c}}; \tikz \node[paper] {\reftext{Ayal05}\cite{ayalew2005}~\textit{c}}; \tikz \node[paper,fund] {\reftext{Ayal04}\cite{ayalew2004}~\textit{c}};};
\node[value, scale=1.300000] (Nvalue29) at (N29.west) {\num{90+-5}};
\node[ref, lwN] (N30) at (N29.north west) {\tikz \node[paper] {\reftext{Bhat05}\cite{bhatnagar2005}~\textit{c}};};
\node[value, scale=1.100000] (Nvalue30) at (N30.west) {\num{91}};
\node[ref, lwN] (N31) at (N30.north west) {\tikz \node[paper] {\reftext{Buon12}\cite{buono2012}~\textit{c}}; \tikz \node[paper] {\reftext{Wang99}\cite{wang1999}~\textit{c}}; \tikz \node[paper] {\reftext{Pers99a}\cite{persson1999a}~\textit{c}}; \tikz \node[paper] {\reftext{Greu97}\cite{greulich-weber1997}~\textit{c}}; \tikz \node[paper] {\reftext{Bako97}\cite{bakowski1997}~\textit{c}}; \tikz \node[paper] {\reftext{Harr95}\cite{harris1995}~\textit{c}};};
\node[value, scale=1.600000] (Nvalue31) at (N31.west) {\num{91.8}};
\node[ref, lwN] (N32) at (N31.north west) {\tikz \node[paper] {\reftext{Kwas14}\cite{kwasnicki2014}}; \tikz \node[paper] {\reftext{Zhu08}\cite{zhu2008}~\textit{c}}; \tikz \node[paper] {\reftext{Pers05}\cite{persson2005}~\textit{c}}; \tikz \node[paper] {\reftext{Feng04a}\cite{feng2004a}~\textit{c}}; \tikz \node[paper] {\reftext{Dali03}\cite{dalibor2003}~\textit{c}}; \tikz \node[paper] {\reftext{Zett02}\cite{zetterling2002}~\textit{c}}; \tikz \node[paper] {\reftext{Lebe99}\cite{lebedev1999}~\textit{c}};};
\node[value, scale=1.700000] (Nvalue32) at (N32.west) {\num{92}};
\node[ref, lwN] (N33) at (N32.north west) {\tikz \node[paper, no4H] {\reftext{Heni13}\cite{henisch2013}}; \tikz \node[paper] {\reftext{Gerh11}\cite{gerhardt2011}~\textit{c}}; \tikz \node[paper] {\reftext{Bali06}\cite{baliga2006}}; \tikz \node[paper] {\reftext{Gao01}\cite{gao2001}}; \tikz \node[paper] {\reftext{Harr95}\cite{harris1995}~\textit{c}};};
\node[value, scale=1.500000] (Nvalue33) at (N33.west) {\num{100}};
\node[ref, lwN] (N34) at (N33.north west) {\tikz \node[paper] {\reftext{Dali03}\cite{dalibor2003}~\textit{c}}; \tikz \node[paper] {\reftext{Levi01}\cite{levinshtein2001}~\textit{c}}; \tikz \node[paper] {\reftext{Iwat01}\cite{iwata2001}~\textit{c}}; \tikz \node[paper,fund] {\reftext{Choy97d}\cite{choyke1997d}~\textit{c}};};
\node[value, scale=1.400000] (Nvalue34) at (N34.west) {\num{102}};
\node[ref, lwN] (N35) at (N34.north west) {\tikz \node[paper,fund] {\reftext{Pern00}\cite{pernot2000}~\textit{c}};};
\node[value, scale=1.100000] (Nvalue35) at (N35.west) {\num{110}};
\node[ref, lwN] (N36) at (N35.north west) {\tikz \node[paper] {\reftext{Dona18}\cite{donato2018}~\textit{c}};};
\node[value, scale=1.100000] (Nvalue36) at (N36.west) {\num{120}};
\node[ref, lwN] (N37) at (N36.north west) {\tikz \node[paper] {\reftext{Ioff23}\cite{ioffe2023}~\textit{c}}; \tikz \node[paper] {\reftext{Fan14}\cite{fan2014}~\textit{c}}; \tikz \node[paper] {\reftext{Izzo08}\cite{izzo2008}~\textit{c}}; \tikz \node[paper] {\reftext{Harr95}\cite{harris1995}~\textit{c}}; \tikz \node[paper] {\reftext{Made91}\cite{madelung1991}~\textit{c}};};
\node[value, scale=1.500000] (Nvalue37) at (N37.west) {\num{124}};
\node[ref, lwN] (N38) at (N37.north west) {\tikz \node[paper] {\reftext{Janz08}\cite{janzen2008}~\textit{c}};};
\node[value, scale=1.100000] (Nvalue38) at (N38.west) {\num{125.5}};
\node[ref, lwN] (N39) at (N38.north west) {\tikz \node[paper] {\reftext{Kimo19}\cite{kimoto2019}~\textit{c}}; \tikz \node[paper] {\reftext{Kimo15}\cite{kimoto2015}~\textit{c}}; \tikz \node[paper] {\reftext{Kimo14a}\cite{kimoto2014a}~\textit{c}};};
\node[value, scale=1.300000] (Nvalue39) at (N39.west) {\num{126}};
\node[ref, lwN] (N40) at (N39.north west) {\tikz \node[paper] {\reftext{Harr95}\cite{harris1995}~\textit{c}};};
\node[value, scale=1.100000] (Nvalue40) at (N40.west) {\num{130}};
\node[ref, lwN] (N41) at (N40.north west) {\tikz \node[paper,fund] {\reftext{Son06}\cite{son2006}~\textit{c}};};
\node[value, scale=1.100000] (Nvalue41) at (N41.west) {\num{142}};


\node[symbol] (P) at (0+ \dxAl+ \dxB+ \dxN,0) {P};
\coordinate (P0) at (P.north);
\node[ref, lwP] (P1) at (P0.north west) {\tikz \node[paper] {\reftext{Nego04a}\cite{negoro2004a}};};
\node[value, scale=1.100000] (Pvalue1) at (P1.west) {\num{45}};
\node[ref, lwP] (P2) at (P1.north west) {\tikz \node[paper,fund] {\reftext{Alba10}\cite{albanese2010}~\textit{h}};};
\node[value, scale=1.100000] (Pvalue2) at (P2.west) {\num{50+-5}};
\node[ref, lwP] (P3) at (P2.north west) {\tikz \node[paper] {\reftext{Dhan10}\cite{dhanaraj2010}~\textit{h}}; \tikz \node[paper] {\reftext{Zett02}\cite{zetterling2002}~\textit{h}}; \tikz \node[paper] {\reftext{Hand00}\cite{handy2000}~\textit{h}};};
\node[value, scale=1.300000] (Pvalue3) at (P3.west) {\num{53}};
\node[ref, lwP] (P4) at (P3.north west) {\tikz \node[paper] {\reftext{Zhu08}\cite{zhu2008}~\textit{h}};};
\node[value, scale=1.100000] (Pvalue4) at (P4.west) {\num{54}};
\node[ref, lwP] (P5) at (P4.north west) {\tikz \node[paper] {\reftext{Dona18}\cite{donato2018}~\textit{h}};};
\node[value, scale=1.100000] (Pvalue5) at (P5.west) {\num{55}};
\node[ref, lwP] (P6) at (P5.north west) {\tikz \node[paper,fund] {\reftext{Son06}\cite{son2006}~\textit{h}};};
\node[value, scale=1.100000] (Pvalue6) at (P6.west) {\num{56}};
\node[ref, lwP] (P7) at (P6.north west) {\tikz \node[paper] {\reftext{Kimo19}\cite{kimoto2019}~\textit{h}}; \tikz \node[paper] {\reftext{Nipo18}\cite{nipoti2018}~\textit{h}}; \tikz \node[paper] {\reftext{Kimo15}\cite{kimoto2015}~\textit{h}}; \tikz \node[paper] {\reftext{Kwas14}\cite{kwasnicki2014}};};
\node[value, scale=1.400000] (Pvalue7) at (P7.west) {\num{60}};
\node[ref, lwP] (P8) at (P7.north west) {\tikz \node[paper] {\reftext{Kimo14a}\cite{kimoto2014a}~\textit{h}}; \tikz \node[paper] {\reftext{Scab11a}\cite{scaburri2011a}~\textit{h}}; \tikz \node[paper] {\reftext{Scab11}\cite{scaburri2011}~\textit{h}};};
\node[value, scale=1.300000] (Pvalue8) at (P8.west) {\num{60.7}};
\node[ref, lwP] (P9) at (P8.north west) {\tikz \node[paper,fund] {\reftext{Son06}\cite{son2006}~\textit{c}};};
\node[value, scale=1.100000] (Pvalue9) at (P9.west) {\num{76}};
\node[ref, lwP] (P10) at (P9.north west) {\tikz \node[paper] {\reftext{Wije11}\cite{wijesundara2011}}; \tikz \node[paper] {\reftext{Neud06}\cite{neudeck2006}}; \tikz \node[paper] {\reftext{Neud01}\cite{neudeck2001}};};
\node[value, scale=1.300000] (Pvalue10) at (P10.west) {\num{80}};
\node[ref, lwP] (P11) at (P10.north west) {\tikz \node[paper,fund] {\reftext{Alba10}\cite{albanese2010}~\textit{c}};};
\node[value, scale=1.100000] (Pvalue11) at (P11.west) {\num{90+-5}};
\node[ref, lwP] (P12) at (P11.north west) {\tikz \node[paper] {\reftext{Dhan10}\cite{dhanaraj2010}~\textit{c}}; \tikz \node[paper] {\reftext{Zhu08}\cite{zhu2008}~\textit{c}}; \tikz \node[paper] {\reftext{Zett02}\cite{zetterling2002}~\textit{c}}; \tikz \node[paper] {\reftext{Hand00}\cite{handy2000}~\textit{c}};};
\node[value, scale=1.400000] (Pvalue12) at (P12.west) {\num{93}};
\node[ref, lwP] (P13) at (P12.north west) {\tikz \node[paper] {\reftext{Dona18}\cite{donato2018}~\textit{c}};};
\node[value, scale=1.100000] (Pvalue13) at (P13.west) {\num{102}};
\node[ref, lwP] (P14) at (P13.north west) {\tikz \node[paper] {\reftext{Kimo19}\cite{kimoto2019}~\textit{c}}; \tikz \node[paper] {\reftext{Nipo18}\cite{nipoti2018}~\textit{c}}; \tikz \node[paper] {\reftext{Kimo15}\cite{kimoto2015}~\textit{c}}; \tikz \node[paper] {\reftext{Kimo14a}\cite{kimoto2014a}~\textit{c}}; \tikz \node[paper] {\reftext{Scab11a}\cite{scaburri2011a}~\textit{c}}; \tikz \node[paper] {\reftext{Scab11}\cite{scaburri2011}~\textit{c}};};
\node[value, scale=1.600000] (Pvalue14) at (P14.west) {\num{120}};


==> data/IncompIon_ref_chainN.tex <==
\node[desc] at (0,0.000000*\dy) {n-type ( Don ) ( N, \nih, \nik ) ( P, \phh, \phk )};
\node[author] at (0,-1.500000*\dy) {\citeauthor{lomakina1973}};
\node[fund, ref] (lomakina1973) at (0,-2.500000*\dy) {\reftext{Loma73}\cite{lomakina1973} (  -- ) ( M , -- , -- ) ( -- , -- , --  )};
\coordinate (lomakina1973C) at ($(lomakina1973.west)+(\dxStart+\dy,0)$);
\node[ ref] (lomakina1974) at ($(lomakina1973C |- 0,-3.500000*\dy)$) {\reftext{Loma74}\cite{lomakina1974} (  -- ) ( $\num{33}$ , -- , -- ) ( -- , -- , --  )};
\draw (lomakina1974.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-5.500000*\dy) {\citeauthor{suzuki1977}};
\node[fund, ref] (suzuki1977) at (0,-6.500000*\dy) {\reftext{Suzu77}\cite{suzuki1977} (  -- ) ( $\num{55+-7}$ , -- , -- ) ( -- , -- , --  )};
\coordinate (suzuki1977C) at ($(suzuki1977.west)+(\dxStart+\dy,0)$);
\node[ ref] (madelung1991) at ($(suzuki1977C |- 0,-7.500000*\dy)$) {\reftext{Made91}\cite{madelung1991} (  -- ) ( -- , M , $\num{124}$ ) ( -- , -- , --  )};
\draw (madelung1991.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-9.500000*\dy) {\citeauthor{ikeda1980}};
\node[fund, ref] (ikeda1980) at (0,-10.500000*\dy) {\reftext{Iked80}\cite{ikeda1980} (  -- ) ( -- , $\num{66}$ , $\num{124}$ ) ( -- , -- , --  )};
\coordinate (ikeda1980C) at ($(ikeda1980.west)+(\dxStart+\dy,0)$);
\node[ ref] (madelung1991) at ($(ikeda1980C |- 0,-11.500000*\dy)$) {\reftext{Made91}\cite{madelung1991} (  -- ) ( -- , M , $\num{124}$ ) ( -- , -- , --  )};
\draw (madelung1991.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (izzo2008) at ($(madelung1991.west |- 0,-12.500000*\dy)$) {\reftext{Izzo08}\cite{izzo2008} (  -- ) ( -- , $\num{66}$ , $\num{124}$ ) ( -- , -- , --  )};
\draw (izzo2008.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (fan2014) at ($(izzo2008.west |- 0,-13.500000*\dy)$) {\reftext{Fan14}\cite{fan2014} (  -- ) ( -- , $\num{66}$ , $\num{124}$ ) ( -- , -- , --  )};
\draw (fan2014.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (donato2018) at ($(fan2014.west |- 0,-14.500000*\dy)$) {\reftext{Dona18}\cite{donato2018} (  -- ) ( -- , $\num{70}$ , $\num{120}$ ) ( -- , $\num{55}$ , $\num{102}$  )};
\draw (donato2018.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (ioffe2023) at ($(donato2018.west |- 0,-15.500000*\dy)$) {\reftext{Ioff23}\cite{ioffe2023} (  -- ) ( -- , $\num{66}$ , $\num{124}$ ) ( -- , -- , --  )};
\draw (ioffe2023.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-17.500000*\dy) {\citeauthor{gotz1993}};
\node[fund, ref] (gotz1993) at (0,-18.500000*\dy) {\reftext{Gotz93}\cite{gotz1993} (  -- ) ( -- , M , M ) ( -- , -- , --  )};
\coordinate (gotz1993C) at ($(gotz1993.west)+(\dxStart+\dy,0)$);
\node[ ref] (pensl1993) at ($(gotz1993C |- 0,-19.500000*\dy)$) {\reftext{Pens93}\cite{pensl1993} (  -- ) ( -- , $\num{45}$ , $\num{100}$ ) ( -- , -- , --  )};
\draw (pensl1993.west) -| ++(-\dy,\fy*\dy);
\coordinate (pensl1993C) at ($(pensl1993.west)+(\dxStart+\dy,0)$);
\node[guess, ref] (gao2001) at ($(pensl1993C |- 0,-20.500000*\dy)$) {\reftext{Gao01}\cite{gao2001} (  -- ) ( $\num{100}$ , -- , -- ) ( -- , -- , --  )};
\draw (gao2001.west) -| ++(-\dy,\fy*\dy);
\node[no4H, ref] (henisch2013) at ($(gao2001.west |- 0,-21.500000*\dy)$) {\reftext{Heni13}\cite{henisch2013} (  -- ) ( $\num{100}$ , -- , -- ) ( -- , -- , --  )};
\draw (henisch2013.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (bakowski1997) at ($(pensl1993.west |- 0,-22.500000*\dy)$) {\reftext{Bako97}\cite{bakowski1997} (  -- ) ( $\num{65}$ , $\num{52.1}$ , $\num{91.8}$ ) ( -- , -- , --  )};
\draw (bakowski1997.west) -| ++(-\dy,\fy*\dy);
\coordinate (bakowski1997C) at ($(bakowski1997.west)+(\dxStart+\dy,0)$);
\node[ ref] (wang1999) at ($(bakowski1997C |- 0,-23.500000*\dy)$) {\reftext{Wang99}\cite{wang1999} (  -- ) ( $\num{65}$ , $\num{52.1}$ , $\num{91.8}$ ) ( -- , -- , --  )};
\draw (wang1999.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (zhao2003) at ($(wang1999.west |- 0,-24.500000*\dy)$) {\reftext{Zhao03}\cite{zhao2003} (  $\num{65}$ ) ( -- , -- , -- ) ( -- , -- , --  )};
\draw (zhao2003.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (buono2010) at ($(zhao2003.west |- 0,-25.500000*\dy)$) {\reftext{Buon10}\cite{buono2010} (  -- ) ( $\num{65}$ , -- , -- ) ( -- , -- , --  )};
\draw (buono2010.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (usman2012) at ($(buono2010.west |- 0,-26.500000*\dy)$) {\reftext{Usma12}\cite{usman2012} (  -- ) ( $\num{65}$ , -- , -- ) ( -- , -- , --  )};
\draw (usman2012.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (greulich-weber1997) at ($(bakowski1997.west |- 0,-27.500000*\dy)$) {\reftext{Greu97}\cite{greulich-weber1997} (  -- ) ( -- , $\num{52.1}$ , $\num{91.8}$ ) ( -- , -- , --  )};
\draw (greulich-weber1997.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (lebedev1999) at ($(greulich-weber1997.west |- 0,-28.500000*\dy)$) {\reftext{Lebe99}\cite{lebedev1999} (  -- ) ( -- , $\num{52}$ , $\num{92}$ ) ( -- , -- , --  )};
\draw (lebedev1999.west) -| ++(-\dy,\fy*\dy);
\coordinate (lebedev1999C) at ($(lebedev1999.west)+(\dxStart+\dy,0)$);
\node[ ref] (arvanitopoulos2017) at ($(lebedev1999C |- 0,-29.500000*\dy)$) {\reftext{Arva17}\cite{arvanitopoulos2017} (  -- ) ( $\num{71}$ , -- , -- ) ( -- , -- , --  )};
\draw (arvanitopoulos2017.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (persson1999a) at ($(lebedev1999.west |- 0,-30.500000*\dy)$) {\reftext{Pers99a}\cite{persson1999a} (  -- ) ( -- , $\num{52.1}$ , $\num{91.8}$ ) ( -- , -- , --  )};
\draw (persson1999a.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (zetterling2002) at ($(persson1999a.west |- 0,-31.500000*\dy)$) {\reftext{Zett02}\cite{zetterling2002} (  -- ) ( -- , $\num{50}$ , $\num{92}$ ) ( -- , $\num{53}$ , $\num{93}$  )};
\draw (zetterling2002.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (bertilsson2004) at ($(zetterling2002.west |- 0,-32.500000*\dy)$) {\reftext{Bert04}\cite{bertilsson2004} (  $\num{52}$ ) ( -- , -- , -- ) ( -- , -- , --  )};
\draw (bertilsson2004.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (bertilsson2004a) at ($(bertilsson2004.west |- 0,-33.500000*\dy)$) {\reftext{Bert04a}\cite{bertilsson2004a} (  $\num{52.1}$ ) ( -- , -- , -- ) ( -- , -- , --  )};
\draw (bertilsson2004a.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (feng2004a) at ($(bertilsson2004a.west |- 0,-34.500000*\dy)$) {\reftext{Feng04a}\cite{feng2004a} (  -- ) ( -- , $\num{52}$ , $\num{92}$ ) ( -- , -- , --  )};
\draw (feng2004a.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (persson2005) at ($(feng2004a.west |- 0,-35.500000*\dy)$) {\reftext{Pers05}\cite{persson2005} (  -- ) ( -- , $\num{52}$ , $\num{92}$ ) ( -- , -- , --  )};
\draw (persson2005.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (zhu2008) at ($(persson2005.west |- 0,-36.500000*\dy)$) {\reftext{Zhu08}\cite{zhu2008} (  -- ) ( -- , $\num{50}$ , $\num{92}$ ) ( -- , $\num{54}$ , $\num{93}$  )};
\draw (zhu2008.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-38.500000*\dy) {\citeauthor{harris1995}};
\node[ ref] (harris1995) at (0,-39.500000*\dy) {\reftext{Harr95}\cite{harris1995} (  -- ) ( M , M , M ) ( -- , -- , --  )};
\coordinate (harris1995C) at ($(harris1995.west)+(\dxStart+\dy,0)$);
\node[ ref] (baliga2006) at ($(harris1995C |- 0,-40.500000*\dy)$) {\reftext{Bali06}\cite{baliga2006} (  -- ) ( $\num{100}$ , -- , -- ) ( -- , -- , --  )};
\draw (baliga2006.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,0.000000*\dy) {\citeauthor{kimoto1995}};
\node[fund, ref] (kimoto1995) at (\xSepOne,-1.000000*\dy) {\reftext{Kimo95}\cite{kimoto1995} (  -- ) ( -- , M , M ) ( -- , -- , --  )};
\coordinate (kimoto1995C) at ($(kimoto1995.west)+(\dxStart+\dy,0)$);
\node[ ref] (sozzi2019) at ($(kimoto1995C |- 0,-2.000000*\dy)$) {\reftext{Sozz19}\cite{sozzi2019} (  -- ) ( $\num{50}$ , -- , -- ) ( -- , -- , --  )};
\draw (sozzi2019.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-4.000000*\dy) {\citeauthor{evwaraye1996}};
\node[fund, ref] (evwaraye1996) at (\xSepOne,-5.000000*\dy) {\reftext{Evwa96}\cite{evwaraye1996} (  -- ) ( -- , $\num{53}$ , $\num{100}$ ) ( -- , -- , --  )};
\coordinate (evwaraye1996C) at ($(evwaraye1996.west)+(\dxStart+\dy,0)$);
\node[ ref] (gerhardt2011) at ($(evwaraye1996C |- 0,-6.000000*\dy)$) {\reftext{Gerh11}\cite{gerhardt2011} (  -- ) ( -- , $\num{53}$ , $\num{100}$ ) ( -- , -- , --  )};
\draw (gerhardt2011.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-8.000000*\dy) {\citeauthor{choyke1997d}};
\node[fund, ref] (choyke1997d) at (\xSepOne,-9.000000*\dy) {\reftext{Choy97d}\cite{choyke1997d} (  -- ) ( -- , $\num{59}$ , $\num{102}$ ) ( -- , -- , --  )};
\coordinate (choyke1997dC) at ($(choyke1997d.west)+(\dxStart+\dy,0)$);
\node[ ref] (iwata2001) at ($(choyke1997dC |- 0,-10.000000*\dy)$) {\reftext{Iwat01}\cite{iwata2001} (  -- ) ( -- , $\num{59}$ , $\num{102}$ ) ( -- , -- , --  )};
\draw (iwata2001.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (levinshtein2001) at ($(iwata2001.west |- 0,-11.000000*\dy)$) {\reftext{Levi01}\cite{levinshtein2001} (  -- ) ( -- , $\num{59}$ , $\num{102}$ ) ( -- , -- , --  )};
\draw (levinshtein2001.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (donato2018) at ($(levinshtein2001.west |- 0,-12.000000*\dy)$) {\reftext{Dona18}\cite{donato2018} (  -- ) ( -- , $\num{70}$ , $\num{120}$ ) ( -- , $\num{55}$ , $\num{102}$  )};
\draw (donato2018.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-14.000000*\dy) {\citeauthor{pensl1998}};
\node[ ref] (pensl1998) at (\xSepOne,-15.000000*\dy) {\reftext{Pens98}\cite{pensl1998} (  -- ) ( -- , -- , -- ) ( -- , -- , --  )};
\coordinate (pensl1998C) at ($(pensl1998.west)+(\dxStart+\dy,0)$);
\node[ ref] (neudeck2001) at ($(pensl1998C |- 0,-16.000000*\dy)$) {\reftext{Neud01}\cite{neudeck2001} (  -- ) ( $\num{45}$ , -- , -- ) ( $\num{80}$ , -- , --  )};
\draw (neudeck2001.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (neudeck2006) at ($(neudeck2001.west |- 0,-17.000000*\dy)$) {\reftext{Neud06}\cite{neudeck2006} (  -- ) ( $\num{45}$ , -- , -- ) ( $\num{80}$ , -- , --  )};
\draw (neudeck2006.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-19.000000*\dy) {\citeauthor{capano2000}};
\node[fund, ref] (capano2000) at (\xSepOne,-20.000000*\dy) {\reftext{Capa00}\cite{capano2000} (  -- ) ( -- , $\num{42}$ , $\num{84}$ ) ( -- , $\num{53}$ , $\num{93}$  )};
\coordinate (capano2000C) at ($(capano2000.west)+(\dxStart+\dy,0)$);
\node[ ref] (handy2000) at ($(capano2000C |- 0,-21.000000*\dy)$) {\reftext{Hand00}\cite{handy2000} (  -- ) ( -- , -- , -- ) ( -- , $\num{53}$ , $\num{93}$  )};
\draw (handy2000.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (zetterling2002) at ($(handy2000.west |- 0,-22.000000*\dy)$) {\reftext{Zett02}\cite{zetterling2002} (  -- ) ( -- , $\num{50}$ , $\num{92}$ ) ( -- , $\num{53}$ , $\num{93}$  )};
\draw (zetterling2002.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (zhu2008) at ($(zetterling2002.west |- 0,-23.000000*\dy)$) {\reftext{Zhu08}\cite{zhu2008} (  -- ) ( -- , $\num{50}$ , $\num{92}$ ) ( -- , $\num{54}$ , $\num{93}$  )};
\draw (zhu2008.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (dhanaraj2010) at ($(zhu2008.west |- 0,-24.000000*\dy)$) {\reftext{Dhan10}\cite{dhanaraj2010} (  -- ) ( -- , -- , -- ) ( -- , $\num{53}$ , $\num{93}$  )};
\draw (dhanaraj2010.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (zhang2010) at ($(dhanaraj2010.west |- 0,-25.000000*\dy)$) {\reftext{Zhan10}\cite{zhang2010} (  -- ) ( $\num{42}$ , -- , -- ) ( -- , -- , --  )};
\draw (zhang2010.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-27.000000*\dy) {\citeauthor{ladesmartin2000}};
\node[fund, ref] (ladesmartin2000) at (\xSepOne,-28.000000*\dy) {\reftext{Lade00}\cite{ladesmartin2000} (  -- ) ( -- , $\num{50+-5}$ , $\num{90+-10}$ ) ( -- , -- , --  )};
\coordinate (ladesmartin2000C) at ($(ladesmartin2000.west)+(\dxStart+\dy,0)$);
\node[ ref] (schroeder2006) at ($(ladesmartin2000C |- 0,-29.000000*\dy)$) {\reftext{Schr06}\cite{schroeder2006} (  -- ) ( -- , $\num{50+-5}$ , $\num{90+-10}$ ) ( -- , -- , --  )};
\draw (schroeder2006.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-31.000000*\dy) {\citeauthor{laube2002}};
\node[ ref] (laube2002) at (\xSepOne,-32.000000*\dy) {\reftext{Laub02}\cite{laube2002} (  -- ) ( -- , $\num{33+-5}$ , $\num{89+-5}$ ) ( -- , $\num{45+-5}$ , $\num{95+-5}$  )};
\coordinate (laube2002C) at ($(laube2002.west)+(\dxStart+\dy,0)$);
\node[ ref] (negoro2004a) at ($(laube2002C |- 0,-33.000000*\dy)$) {\reftext{Nego04a}\cite{negoro2004a} (  -- ) ( -- , -- , -- ) ( $\num{45}$ , -- , --  )};
\draw (negoro2004a.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-35.000000*\dy) {\citeauthor{adachi2003}};
\node[ ref] (adachi2003) at (\xSepOne,-36.000000*\dy) {\reftext{Adac03}\cite{adachi2003} (  -- ) ( -- , -- , -- ) ( -- , -- , --  )};
\coordinate (adachi2003C) at ($(adachi2003.west)+(\dxStart+\dy,0)$);
\node[ ref] (bhatnagar2005) at ($(adachi2003C |- 0,-37.000000*\dy)$) {\reftext{Bhat05}\cite{bhatnagar2005} (  -- ) ( $\num{81}$ , $\num{60}$ , $\num{91}$ ) ( -- , -- , --  )};
\draw (bhatnagar2005.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-39.000000*\dy) {\citeauthor{ivanov2003a}};
\node[fund, ref] (ivanov2003a) at (\xSepOne,-40.000000*\dy) {\reftext{Ivan03a}\cite{ivanov2003a} (  -- ) ( -- , $\num{61.4+-0.5}$ , -- ) ( -- , -- , --  )};
\coordinate (ivanov2003aC) at ($(ivanov2003a.west)+(\dxStart+\dy,0)$);
\node[ ref] (yang2019) at ($(ivanov2003aC |- 0,-41.000000*\dy)$) {\reftext{Yang19}\cite{yang2019} (  -- ) ( $\num{61}$ , -- , -- ) ( -- , -- , --  )};
\draw (yang2019.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (tian2020) at ($(yang2019.west |- 0,-42.000000*\dy)$) {\reftext{Tian20}\cite{tian2020} (  -- ) ( $\num{61.4}$ , -- , -- ) ( -- , -- , --  )};
\draw (tian2020.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,0.000000*\dy) {\citeauthor{ayalew2004}};
\node[fund, ref] (ayalew2004) at (\xSepOne + \xSepTwo,-1.000000*\dy) {\reftext{Ayal04}\cite{ayalew2004} (  -- ) ( $\num{70}$ , $\num{50+-5}$ , $\num{90+-5}$ ) ( -- , -- , --  )};
\coordinate (ayalew2004C) at ($(ayalew2004.west)+(\dxStart+\dy,0)$);
\node[ ref] (ayalew2005) at ($(ayalew2004C |- 0,-2.000000*\dy)$) {\reftext{Ayal05}\cite{ayalew2005} (  -- ) ( $\num{70}$ , $\num{50+-5}$ , $\num{90+-5}$ ) ( -- , -- , --  )};
\draw (ayalew2005.west) -| ++(-\dy,\fy*\dy);
\coordinate (ayalew2005C) at ($(ayalew2005.west)+(\dxStart+\dy,0)$);
\node[ ref] (pezzimenti2013) at ($(ayalew2005C |- 0,-3.000000*\dy)$) {\reftext{Pezz13}\cite{pezzimenti2013} (  $\num{70}$ ) ( -- , -- , -- ) ( -- , -- , --  )};
\draw (pezzimenti2013.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (megherbi2018) at ($(pezzimenti2013.west |- 0,-4.000000*\dy)$) {\reftext{Megh18}\cite{megherbi2018} (  -- ) ( $\num{70}$ , -- , -- ) ( -- , -- , --  )};
\draw (megherbi2018.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (megherbi2018a) at ($(megherbi2018.west |- 0,-5.000000*\dy)$) {\reftext{Megh18a}\cite{megherbi2018a} (  $\num{70}$ ) ( -- , -- , -- ) ( -- , -- , --  )};
\draw (megherbi2018a.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-7.000000*\dy) {\citeauthor{kagamihara2004}};
\node[ ref] (kagamihara2004) at (\xSepOne + \xSepTwo,-8.000000*\dy) {\reftext{Kaga04}\cite{kagamihara2004} (  -- ) ( -- , 70.9 , 123.7 ) ( -- , -- , --  )};
\coordinate (kagamihara2004C) at ($(kagamihara2004.west)+(\dxStart+\dy,0)$);
\node[guess, ref] (tiwari2019) at ($(kagamihara2004C |- 0,-9.000000*\dy)$) {\reftext{Tiwa19}\cite{tiwari2019} (  -- ) ( $\num{70.9}$ , -- , -- ) ( -- , -- , --  )};
\draw (tiwari2019.west) -| ++(-\dy,\fy*\dy);
\coordinate (tiwari2019C) at ($(tiwari2019.west)+(\dxStart+\dy,0)$);
\node[ ref] (tiwari2019a) at ($(tiwari2019C |- 0,-10.000000*\dy)$) {\reftext{Tiwa19a}\cite{tiwari2019a} (  -- ) ( $\num{70.9}$ , -- , -- ) ( -- , -- , --  )};
\draw (tiwari2019a.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-12.000000*\dy) {\citeauthor{ivanov2005}};
\node[fund, ref] (ivanov2005) at (\xSepOne + \xSepTwo,-13.000000*\dy) {\reftext{Ivan05}\cite{ivanov2005} (  -- ) ( -- , $\num{61.4}$ , $\num{125.5}$ ) ( -- , $\num{60.7}$ , $\num{120+-20}$  )};
\coordinate (ivanov2005C) at ($(ivanov2005.west)+(\dxStart+\dy,0)$);
\node[ ref] (janzen2008) at ($(ivanov2005C |- 0,-14.000000*\dy)$) {\reftext{Janz08}\cite{janzen2008} (  -- ) ( -- , $\num{61.4}$ , $\num{125.5}$ ) ( -- , -- , --  )};
\draw (janzen2008.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (scaburri2011) at ($(janzen2008.west |- 0,-15.000000*\dy)$) {\reftext{Scab11}\cite{scaburri2011} (  -- ) ( -- , -- , -- ) ( -- , $\num{60.7}$ , $\num{120}$  )};
\draw (scaburri2011.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (scaburri2011a) at ($(scaburri2011.west |- 0,-16.000000*\dy)$) {\reftext{Scab11a}\cite{scaburri2011a} (  -- ) ( -- , -- , -- ) ( -- , $\num{60.7}$ , $\num{120}$  )};
\draw (scaburri2011a.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (kimoto2014a) at ($(scaburri2011a.west |- 0,-17.000000*\dy)$) {\reftext{Kimo14a}\cite{kimoto2014a} (  66 ) ( -- , $\num{61.4}$ , $\num{126}$ ) ( -- , $\num{60.7}$ , $\num{120}$  )};
\draw (kimoto2014a.west) -| ++(-\dy,\fy*\dy);
\coordinate (kimoto2014aC) at ($(kimoto2014a.west)+(\dxStart+\dy,0)$);
\node[ ref] (kimoto2019) at ($(kimoto2014aC |- 0,-18.000000*\dy)$) {\reftext{Kimo19}\cite{kimoto2019} (  -- ) ( -- , $\num{61}$ , $\num{126}$ ) ( -- , $\num{60}$ , $\num{120}$  )};
\draw (kimoto2019.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (kimoto2015) at ($(kimoto2014a.west |- 0,-19.000000*\dy)$) {\reftext{Kimo15}\cite{kimoto2015} (  -- ) ( -- , $\num{61}$ , $\num{126}$ ) ( -- , $\num{60}$ , $\num{120}$  )};
\draw (kimoto2015.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (nipoti2018) at ($(kimoto2015.west |- 0,-20.000000*\dy)$) {\reftext{Nipo18}\cite{nipoti2018} (  -- ) ( -- , -- , -- ) ( -- , $\num{60}$ , $\num{120}$  )};
\draw (nipoti2018.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-22.000000*\dy) {\citeauthor{sullivan2008}};
\node[no4H, ref] (sullivan2008) at (\xSepOne + \xSepTwo,-23.000000*\dy) {\reftext{Sull08}\cite{sullivan2008} (  -- ) ( $\num{80}$ , -- , -- ) ( -- , -- , --  )};
\coordinate (sullivan2008C) at ($(sullivan2008.west)+(\dxStart+\dy,0)$);
\node[ ref] (rakheja2020) at ($(sullivan2008C |- 0,-24.000000*\dy)$) {\reftext{Rakh20}\cite{rakheja2020} (  -- ) ( $\num{65}$ , -- , -- ) ( -- , -- , --  )};
\draw (rakheja2020.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-26.000000*\dy) {\citeauthor{tamaki2008a}};
\node[ ref] (tamaki2008a) at (\xSepOne + \xSepTwo,-27.000000*\dy) {\reftext{Tama08a}\cite{tamaki2008a} (  66 ) ( -- , -- , -- ) ( -- , -- , --  )};
\coordinate (tamaki2008aC) at ($(tamaki2008a.west)+(\dxStart+\dy,0)$);
\node[ ref] (menon2011) at ($(tamaki2008aC |- 0,-28.000000*\dy)$) {\reftext{Meno11}\cite{menon2011} (  -- ) ( -- , -- , -- ) ( -- , -- , --  )};
\draw (menon2011.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-30.000000*\dy) {\citeauthor{habib2011}};
\node[ ref] (habib2011) at (\xSepOne + \xSepTwo,-31.000000*\dy) {\reftext{Habi11}\cite{habib2011} (  $\num{60}$ ) ( -- , -- , -- ) ( -- , -- , --  )};
\coordinate (habib2011C) at ($(habib2011.west)+(\dxStart+\dy,0)$);
\node[ ref] (chen2020a) at ($(habib2011C |- 0,-32.000000*\dy)$) {\reftext{Chen20a}\cite{chen2020a} (  $\num{60}$ ) ( -- , -- , -- ) ( -- , -- , --  )};
\draw (chen2020a.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-34.000000*\dy) {\citeauthor{buono2012}};
\node[ ref] (buono2012) at (\xSepOne + \xSepTwo,-35.000000*\dy) {\reftext{Buon12}\cite{buono2012} (  -- ) ( 65 , $\num{52.1}$ , $\num{91.8}$ ) ( -- , -- , --  )};
\coordinate (buono2012C) at ($(buono2012.west)+(\dxStart+\dy,0)$);
\node[ ref] (johannesson2019) at ($(buono2012C |- 0,-36.000000*\dy)$) {\reftext{Joha19}\cite{johannesson2019} (  -- ) ( $\num{65}$ , -- , -- ) ( -- , -- , --  )};
\draw (johannesson2019.west) -| ++(-\dy,\fy*\dy);


==> data/IncompIon_ref_chainP.tex <==
\node[desc] at (0,0.000000*\dy) {p-type ( Acc ) ( Al, \alh, \alk ) ( B, \boh, \bok )};
\node[author] at (0,-1.500000*\dy) {\citeauthor{ikeda1980}};
\node[fund, ref] (ikeda1980) at (0,-2.500000*\dy) {\reftext{Iked80}\cite{ikeda1980} (  -- ) ( $\num{191}$ , -- , -- ) ( $\num{647}$ , -- , --  )};
\coordinate (ikeda1980C) at ($(ikeda1980.west)+(\dxStart+\dy,0)$);
\node[ ref] (madelung1991) at ($(ikeda1980C |- 0,-3.500000*\dy)$) {\reftext{Made91}\cite{madelung1991} (  -- ) ( $\num{191}$ , -- , -- ) ( $\num{647}$ , -- , --  )};
\draw (madelung1991.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (freitas1995) at ($(madelung1991.west |- 0,-4.500000*\dy)$) {\reftext{Frei95}\cite{freitas1995} (  -- ) ( $\num{191}$ , -- , -- ) ( -- , -- , --  )};
\draw (freitas1995.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (bakowski1997) at ($(freitas1995.west |- 0,-5.500000*\dy)$) {\reftext{Bako97}\cite{bakowski1997} (  -- ) ( $\num{191}$ , -- , -- ) ( -- , -- , --  )};
\draw (bakowski1997.west) -| ++(-\dy,\fy*\dy);
\coordinate (bakowski1997C) at ($(bakowski1997.west)+(\dxStart+\dy,0)$);
\node[ ref] (wang1999) at ($(bakowski1997C |- 0,-6.500000*\dy)$) {\reftext{Wang99}\cite{wang1999} (  -- ) ( $\num{191}$ , -- , -- ) ( -- , -- , --  )};
\draw (wang1999.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (zhao2003) at ($(wang1999.west |- 0,-7.500000*\dy)$) {\reftext{Zhao03}\cite{zhao2003} (  -- ) ( $\num{191}$ , -- , -- ) ( -- , -- , --  )};
\draw (zhao2003.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (greulich-weber1997) at ($(bakowski1997.west |- 0,-8.500000*\dy)$) {\reftext{Greu97}\cite{greulich-weber1997} (  -- ) ( $\num{191}$ , -- , -- ) ( $\num{647}$ , -- , --  )};
\draw (greulich-weber1997.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (persson1998) at ($(greulich-weber1997.west |- 0,-9.500000*\dy)$) {\reftext{Pers98}\cite{persson1998} (  -- ) ( $\num{191}$ , -- , -- ) ( -- , -- , --  )};
\draw (persson1998.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (levinshtein2001) at ($(persson1998.west |- 0,-10.500000*\dy)$) {\reftext{Levi01}\cite{levinshtein2001} (  -- ) ( $\num{190}$ , -- , -- ) ( $\num{650}$ , -- , --  )};
\draw (levinshtein2001.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (li2003) at ($(levinshtein2001.west |- 0,-11.500000*\dy)$) {\reftext{Li03}\cite{li2003} (  $\num{191}$ ) ( -- , -- , -- ) ( -- , -- , --  )};
\draw (li2003.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (negoro2003) at ($(li2003.west |- 0,-12.500000*\dy)$) {\reftext{Nego03}\cite{negoro2003} (  -- ) ( $\num{190}$ , -- , -- ) ( $\num{285}$ , -- , --  )};
\draw (negoro2003.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (negoro2004) at ($(negoro2003.west |- 0,-13.500000*\dy)$) {\reftext{Nego04}\cite{negoro2004} (  -- ) ( $\num{190}$ , -- , -- ) ( -- , -- , --  )};
\draw (negoro2004.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (zhang2010) at ($(negoro2004.west |- 0,-14.500000*\dy)$) {\reftext{Zhan10}\cite{zhang2010} (  -- ) ( $\num{191}$ , -- , -- ) ( -- , -- , --  )};
\draw (zhang2010.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (habib2011) at ($(zhang2010.west |- 0,-15.500000*\dy)$) {\reftext{Habi11}\cite{habib2011} (  $\num{191}$ ) ( -- , -- , -- ) ( -- , -- , --  )};
\draw (habib2011.west) -| ++(-\dy,\fy*\dy);
\coordinate (habib2011C) at ($(habib2011.west)+(\dxStart+\dy,0)$);
\node[ ref] (chen2020a) at ($(habib2011C |- 0,-16.500000*\dy)$) {\reftext{Chen20a}\cite{chen2020a} (  $\num{191}$ ) ( -- , -- , -- ) ( -- , -- , --  )};
\draw (chen2020a.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (wijesundara2011) at ($(habib2011.west |- 0,-17.500000*\dy)$) {\reftext{Wije11}\cite{wijesundara2011} (  -- ) ( $\num{190}$ , -- , -- ) ( $\num{285}$ , -- , --  )};
\draw (wijesundara2011.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (fan2014) at ($(wijesundara2011.west |- 0,-18.500000*\dy)$) {\reftext{Fan14}\cite{fan2014} (  -- ) ( $\num{191}$ , -- , -- ) ( $\num{647}$ , -- , --  )};
\draw (fan2014.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (megherbi2015) at ($(fan2014.west |- 0,-19.500000*\dy)$) {\reftext{Megh15}\cite{megherbi2015} (  $\num{191}$ ) ( -- , -- , -- ) ( -- , -- , --  )};
\draw (megherbi2015.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (megherbi2018) at ($(megherbi2015.west |- 0,-20.500000*\dy)$) {\reftext{Megh18}\cite{megherbi2018} (  -- ) ( $\num{190}$ , -- , -- ) ( -- , -- , --  )};
\draw (megherbi2018.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (yoshioka2018) at ($(megherbi2018.west |- 0,-21.500000*\dy)$) {\reftext{Yosh18}\cite{yoshioka2018} (  -- ) ( $\num{190}$ , -- , -- ) ( -- , -- , --  )};
\draw (yoshioka2018.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (liu2021) at ($(yoshioka2018.west |- 0,-22.500000*\dy)$) {\reftext{Liu21}\cite{liu2021} (  $\num{191}$ ) ( -- , -- , -- ) ( -- , -- , --  )};
\draw (liu2021.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (ioffe2023) at ($(liu2021.west |- 0,-23.500000*\dy)$) {\reftext{Ioff23}\cite{ioffe2023} (  -- ) ( $\num{191}$ , -- , -- ) ( $\num{647}$ , -- , --  )};
\draw (ioffe2023.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-25.500000*\dy) {\citeauthor{pensl1993}};
\node[fund, ref] (pensl1993) at (0,-26.500000*\dy) {\reftext{Pens93}\cite{pensl1993} (  -- ) ( $\num{200}$ , -- , -- ) ( -- , -- , --  )};
\coordinate (pensl1993C) at ($(pensl1993.west)+(\dxStart+\dy,0)$);
\node[ ref] (haberstroh1994) at ($(pensl1993C |- 0,-27.500000*\dy)$) {\reftext{Habe94}\cite{haberstroh1994} (  -- ) ( $\num{200}$ , -- , -- ) ( -- , -- , --  )};
\draw (haberstroh1994.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (zetterling2002) at ($(haberstroh1994.west |- 0,-28.500000*\dy)$) {\reftext{Zett02}\cite{zetterling2002} (  -- ) ( $\num{200}$ , -- , -- ) ( $\num{285}$ , -- , --  )};
\draw (zetterling2002.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (zhu2008) at ($(zetterling2002.west |- 0,-29.500000*\dy)$) {\reftext{Zhu08}\cite{zhu2008} (  -- ) ( $\num{200}$ , -- , -- ) ( $\num{285}$ , -- , --  )};
\draw (zhu2008.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-31.500000*\dy) {\citeauthor{harris1995}};
\node[ ref] (harris1995) at (0,-32.500000*\dy) {\reftext{Harr95}\cite{harris1995} (  -- ) ( M , -- , -- ) ( M , -- , --  )};
\coordinate (harris1995C) at ($(harris1995.west)+(\dxStart+\dy,0)$);
\node[ ref] (baliga2006) at ($(harris1995C |- 0,-33.500000*\dy)$) {\reftext{Bali06}\cite{baliga2006} (  -- ) ( $\num{200}$ , -- , -- ) ( -- , -- , --  )};
\draw (baliga2006.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-35.500000*\dy) {\citeauthor{troffer1997}};
\node[fund, ref] (troffer1997) at (0,-36.500000*\dy) {\reftext{Trof97}\cite{troffer1997} (  -- ) ( M , -- , -- ) ( M , -- , --  )};
\coordinate (troffer1997C) at ($(troffer1997.west)+(\dxStart+\dy,0)$);
\node[guess, ref] (zetterling2002) at ($(troffer1997C |- 0,-37.500000*\dy)$) {\reftext{Zett02}\cite{zetterling2002} (  -- ) ( $\num{200}$ , -- , -- ) ( $\num{285}$ , -- , --  )};
\draw (zetterling2002.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (zhu2008) at ($(zetterling2002.west |- 0,-38.500000*\dy)$) {\reftext{Zhu08}\cite{zhu2008} (  -- ) ( $\num{200}$ , -- , -- ) ( $\num{285}$ , -- , --  )};
\draw (zhu2008.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (pezzimenti2009) at ($(zhu2008.west |- 0,-39.500000*\dy)$) {\reftext{Pezz09}\cite{pezzimenti2009} (  $\num{190}$ ) ( -- , -- , -- ) ( -- , -- , --  )};
\draw (pezzimenti2009.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (wijesundara2011) at ($(pezzimenti2009.west |- 0,-40.500000*\dy)$) {\reftext{Wije11}\cite{wijesundara2011} (  -- ) ( $\num{190}$ , -- , -- ) ( $\num{285}$ , -- , --  )};
\draw (wijesundara2011.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (pezzimenti2013) at ($(wijesundara2011.west |- 0,-41.500000*\dy)$) {\reftext{Pezz13}\cite{pezzimenti2013} (  $\num{190}$ ) ( -- , -- , -- ) ( -- , -- , --  )};
\draw (pezzimenti2013.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,0.000000*\dy) {\citeauthor{itoh1998}};
\node[fund, ref] (itoh1998) at (\xSepOne,-1.000000*\dy) {\reftext{Itoh98}\cite{itoh1998} (  -- ) ( $\num{180}$ , -- , -- ) ( $\num{285}$ , -- , --  )};
\coordinate (itoh1998C) at ($(itoh1998.west)+(\dxStart+\dy,0)$);
\node[ ref] (negoro2003) at ($(itoh1998C |- 0,-2.000000*\dy)$) {\reftext{Nego03}\cite{negoro2003} (  -- ) ( $\num{190}$ , -- , -- ) ( $\num{285}$ , -- , --  )};
\draw (negoro2003.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-4.000000*\dy) {\citeauthor{pensl1998}};
\node[ ref] (pensl1998) at (\xSepOne,-5.000000*\dy) {\reftext{Pens98}\cite{pensl1998} (  -- ) ( -- , -- , -- ) ( -- , -- , --  )};
\coordinate (pensl1998C) at ($(pensl1998.west)+(\dxStart+\dy,0)$);
\node[ ref] (neudeck2001) at ($(pensl1998C |- 0,-6.000000*\dy)$) {\reftext{Neud01}\cite{neudeck2001} (  -- ) ( $\num{200}$ , -- , -- ) ( $\num{300}$ , -- , --  )};
\draw (neudeck2001.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (neudeck2006) at ($(neudeck2001.west |- 0,-7.000000*\dy)$) {\reftext{Neud06}\cite{neudeck2006} (  -- ) ( $\num{200}$ , -- , -- ) ( $\num{300}$ , -- , --  )};
\draw (neudeck2006.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-9.000000*\dy) {\citeauthor{smith1998}};
\node[fund, ref] (smith1998) at (\xSepOne,-10.000000*\dy) {\reftext{Smit98}\cite{smith1998} (  -- ) ( -- , M , $\num{266}$ ) ( -- , -- , --  )};
\coordinate (smith1998C) at ($(smith1998.west)+(\dxStart+\dy,0)$);
\node[ ref] (smith1999) at ($(smith1998C |- 0,-11.000000*\dy)$) {\reftext{Smit99}\cite{smith1999} (  -- ) ( -- , $\num{212}$ , $\num{266}$ ) ( -- , -- , --  )};
\draw (smith1999.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-13.000000*\dy) {\citeauthor{lebedev1999}};
\node[ ref] (lebedev1999) at (\xSepOne,-14.000000*\dy) {\reftext{Lebe99}\cite{lebedev1999} (  -- ) ( $\num{230}$ , -- , -- ) ( $\num{290}$ , -- , --  )};
\coordinate (lebedev1999C) at ($(lebedev1999.west)+(\dxStart+\dy,0)$);
\node[ ref] (lu2021) at ($(lebedev1999C |- 0,-15.000000*\dy)$) {\reftext{Lu21}\cite{lu2021} (  -- ) ( $\num{220}$ , -- , -- ) ( -- , -- , --  )};
\draw (lu2021.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-17.000000*\dy) {\citeauthor{ladesmartin2000}};
\node[fund, ref] (ladesmartin2000) at (\xSepOne,-18.000000*\dy) {\reftext{Lade00}\cite{ladesmartin2000} (  -- ) ( $\num{210+-20}$ , -- , -- ) ( $\num{320+-20}$ , -- , --  )};
\coordinate (ladesmartin2000C) at ($(ladesmartin2000.west)+(\dxStart+\dy,0)$);
\node[ ref] (schroeder2006) at ($(ladesmartin2000C |- 0,-19.000000*\dy)$) {\reftext{Schr06}\cite{schroeder2006} (  -- ) ( $\num{210+-20}$ , -- , -- ) ( $\num{320+-20}$ , -- , --  )};
\draw (schroeder2006.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (buono2010) at ($(schroeder2006.west |- 0,-20.000000*\dy)$) {\reftext{Buon10}\cite{buono2010} (  -- ) ( $\num{210}$ , -- , -- ) ( -- , -- , --  )};
\draw (buono2010.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (lutz2011) at ($(buono2010.west |- 0,-21.000000*\dy)$) {\reftext{Lutz11}\cite{lutz2011} (  -- ) ( $\num{210}$ , -- , -- ) ( $\num{320}$ , -- , --  )};
\draw (lutz2011.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (usman2012) at ($(lutz2011.west |- 0,-22.000000*\dy)$) {\reftext{Usma12}\cite{usman2012} (  -- ) ( $\num{210}$ , -- , -- ) ( -- , -- , --  )};
\draw (usman2012.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (lutz2018) at ($(usman2012.west |- 0,-23.000000*\dy)$) {\reftext{Lutz18}\cite{lutz2018} (  -- ) ( $\num{210}$ , -- , -- ) ( $\num{320}$ , -- , --  )};
\draw (lutz2018.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-25.000000*\dy) {\citeauthor{tanaka2000}};
\node[fund, ref] (tanaka2000) at (\xSepOne,-26.000000*\dy) {\reftext{Tana00}\cite{tanaka2000} (  -- ) ( M , -- , -- ) ( -- , -- , --  )};
\coordinate (tanaka2000C) at ($(tanaka2000.west)+(\dxStart+\dy,0)$);
\node[ ref] (bhatnagar2005) at ($(tanaka2000C |- 0,-27.000000*\dy)$) {\reftext{Bhat05}\cite{bhatnagar2005} (  -- ) ( $\num{191}$ , -- , -- ) ( -- , -- , --  )};
\draw (bhatnagar2005.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-29.000000*\dy) {\citeauthor{storasta2002}};
\node[no4H, ref] (storasta2002) at (\xSepOne,-30.000000*\dy) {\reftext{Stor02}\cite{storasta2002} (  -- ) ( -- , -- , -- ) ( M , -- , --  )};
\coordinate (storasta2002C) at ($(storasta2002.west)+(\dxStart+\dy,0)$);
\node[ ref] (huh2006) at ($(storasta2002C |- 0,-31.000000*\dy)$) {\reftext{Huh06}\cite{huh2006} (  -- ) ( -- , -- , -- ) ( $\num{300}$ , -- , --  )};
\draw (huh2006.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-33.000000*\dy) {\citeauthor{zhang2003}};
\node[fund, ref] (zhang2003) at (\xSepOne,-34.000000*\dy) {\reftext{Zhan03}\cite{zhang2003} (  -- ) ( -- , -- , -- ) ( \numrange{230}{280} , -- , --  )};
\coordinate (zhang2003C) at ($(zhang2003.west)+(\dxStart+\dy,0)$);
\node[ ref] (muzykov2012) at ($(zhang2003C |- 0,-35.000000*\dy)$) {\reftext{Muzy12}\cite{muzykov2012} (  -- ) ( -- , -- , -- ) ( \numrange{230}{280} , -- , --  )};
\draw (muzykov2012.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-37.000000*\dy) {\citeauthor{ayalew2004}};
\node[fund, ref] (ayalew2004) at (\xSepOne,-38.000000*\dy) {\reftext{Ayal04}\cite{ayalew2004} (  -- ) ( $\num{220+-20}$ , -- , -- ) ( $\num{330+-30}$ , -- , --  )};
\coordinate (ayalew2004C) at ($(ayalew2004.west)+(\dxStart+\dy,0)$);
\node[ ref] (ayalew2005) at ($(ayalew2004C |- 0,-39.000000*\dy)$) {\reftext{Ayal05}\cite{ayalew2005} (  -- ) ( $\num{220+-20}$ , -- , -- ) ( $\num{330+-30}$ , -- , --  )};
\draw (ayalew2005.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,0.000000*\dy) {\citeauthor{ivanov2005}};
\node[fund, ref] (ivanov2005) at (\xSepOne + \xSepTwo,-1.000000*\dy) {\reftext{Ivan05}\cite{ivanov2005} (  -- ) ( -- , $\num{197.9}$ , $\num{201.3}$ ) ( -- , -- , --  )};
\coordinate (ivanov2005C) at ($(ivanov2005.west)+(\dxStart+\dy,0)$);
\node[ ref] (janzen2008) at ($(ivanov2005C |- 0,-2.000000*\dy)$) {\reftext{Janz08}\cite{janzen2008} (  -- ) ( -- , $\num{197.9}$ , $\num{201.3}$ ) ( -- , -- , --  )};
\draw (janzen2008.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (kimoto2014a) at ($(janzen2008.west |- 0,-3.000000*\dy)$) {\reftext{Kimo14a}\cite{kimoto2014a} (  191 ) ( -- , $\num{197.9}$ , $\num{201.3}$ ) ( $\num{280}$ , -- , --  )};
\draw (kimoto2014a.west) -| ++(-\dy,\fy*\dy);
\coordinate (kimoto2014aC) at ($(kimoto2014a.west)+(\dxStart+\dy,0)$);
\node[ ref] (kimoto2019) at ($(kimoto2014aC |- 0,-4.000000*\dy)$) {\reftext{Kimo19}\cite{kimoto2019} (  -- ) ( -- , $\num{198}$ , $\num{201}$ ) ( -- , -- , --  )};
\draw (kimoto2019.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (kimoto2015) at ($(kimoto2014a.west |- 0,-5.000000*\dy)$) {\reftext{Kimo15}\cite{kimoto2015} (  -- ) ( -- , $\num{198}$ , $\num{201}$ ) ( $\num{280}$ , -- , --  )};
\draw (kimoto2015.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (nipoti2018) at ($(kimoto2015.west |- 0,-6.000000*\dy)$) {\reftext{Nipo18}\cite{nipoti2018} (  -- ) ( -- , $\num{198}$ , $\num{210}$ ) ( -- , -- , --  )};
\draw (nipoti2018.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (tian2020) at ($(nipoti2018.west |- 0,-7.000000*\dy)$) {\reftext{Tian20}\cite{tian2020} (  -- ) ( $\num{201.3}$ , -- , -- ) ( -- , -- , --  )};
\draw (tian2020.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-9.000000*\dy) {\citeauthor{pensl2005}};
\node[ ref] (pensl2005) at (\xSepOne + \xSepTwo,-10.000000*\dy) {\reftext{Pens05}\cite{pensl2005} (  -- , -- , -- ) ( -- , -- , -- ) ( -- , -- , --  )};
\coordinate (pensl2005C) at ($(pensl2005.west)+(\dxStart+\dy,0)$);
\node[no4H, ref] (sullivan2008) at ($(pensl2005C |- 0,-11.000000*\dy)$) {\reftext{Sull08}\cite{sullivan2008} (  -- ) ( -- , -- , -- ) ( $\num{300}$ , -- , --  )};
\draw (sullivan2008.west) -| ++(-\dy,\fy*\dy);
\coordinate (sullivan2008C) at ($(sullivan2008.west)+(\dxStart+\dy,0)$);
\node[ ref] (rakheja2020) at ($(sullivan2008C |- 0,-12.000000*\dy)$) {\reftext{Rakh20}\cite{rakheja2020} (  -- ) ( -- , -- , -- ) ( $\num{300}$ , -- , --  )};
\draw (rakheja2020.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-14.000000*\dy) {\citeauthor{tamaki2008a}};
\node[ ref] (tamaki2008a) at (\xSepOne + \xSepTwo,-15.000000*\dy) {\reftext{Tama08a}\cite{tamaki2008a} (  191 ) ( -- , -- , -- ) ( -- , -- , --  )};
\coordinate (tamaki2008aC) at ($(tamaki2008a.west)+(\dxStart+\dy,0)$);
\node[ ref] (menon2011) at ($(tamaki2008aC |- 0,-16.000000*\dy)$) {\reftext{Meno11}\cite{menon2011} (  -- ) ( -- , -- , -- ) ( -- , -- , --  )};
\draw (menon2011.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-18.000000*\dy) {\citeauthor{koizumi2009}};
\node[fund, ref] (koizumi2009) at (\xSepOne + \xSepTwo,-19.000000*\dy) {\reftext{Koiz09}\cite{koizumi2009} (  -- ) ( 265 , -- , -- ) ( -- , -- , --  )};
\coordinate (koizumi2009C) at ($(koizumi2009.west)+(\dxStart+\dy,0)$);
\node[guess, ref] (arvanitopoulos2017) at ($(koizumi2009C |- 0,-20.000000*\dy)$) {\reftext{Arva17}\cite{arvanitopoulos2017} (  -- ) ( $\num{265}$ , -- , -- ) ( $\num{293}$ , -- , --  )};
\draw (arvanitopoulos2017.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (donato2018) at ($(arvanitopoulos2017.west |- 0,-21.000000*\dy)$) {\reftext{Dona18}\cite{donato2018} (  -- ) ( $\num{265}$ , -- , -- ) ( $\num{293}$ , -- , --  )};
\draw (donato2018.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (lophitis2018) at ($(donato2018.west |- 0,-22.000000*\dy)$) {\reftext{Loph18}\cite{lophitis2018} (  -- ) ( $\num{265}$ , -- , -- ) ( $\num{293}$ , -- , --  )};
\draw (lophitis2018.west) -| ++(-\dy,\fy*\dy);
\coordinate (lophitis2018C) at ($(lophitis2018.west)+(\dxStart+\dy,0)$);
\node[ ref] (tiwari2019) at ($(lophitis2018C |- 0,-23.000000*\dy)$) {\reftext{Tiwa19}\cite{tiwari2019} (  -- ) ( $\num{265}$ , -- , -- ) ( -- , -- , --  )};
\draw (tiwari2019.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (tiwari2019a) at ($(tiwari2019.west |- 0,-24.000000*\dy)$) {\reftext{Tiwa19a}\cite{tiwari2019a} (  -- ) ( $\num{265}$ , -- , -- ) ( -- , -- , --  )};
\draw (tiwari2019a.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (johannesson2019) at ($(lophitis2018.west |- 0,-25.000000*\dy)$) {\reftext{Joha19}\cite{johannesson2019} (  -- ) ( $\num{265}$ , -- , -- ) ( -- , -- , --  )};
\draw (johannesson2019.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (sozzi2019) at ($(johannesson2019.west |- 0,-26.000000*\dy)$) {\reftext{Sozz19}\cite{sozzi2019} (  -- ) ( $\num{265}$ , -- , -- ) ( -- , -- , --  )};
\draw (sozzi2019.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-28.000000*\dy) {\citeauthor{arvinte2017}};
\node[fund, ref] (arvinte2017) at (\xSepOne + \xSepTwo,-29.000000*\dy) {\reftext{Arvi17}\cite{arvinte2017} (  -- ) ( 230+-10 , -- , -- ) ( -- , -- , --  )};
\coordinate (arvinte2017C) at ($(arvinte2017.west)+(\dxStart+\dy,0)$);
\node[ ref] (bader2020) at ($(arvinte2017C |- 0,-30.000000*\dy)$) {\reftext{Bade20}\cite{bader2020} (  $\num{200}$ ) ( -- , -- , -- ) ( -- , -- , --  )};
\draw (bader2020.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-32.000000*\dy) {\citeauthor{huang2022a}};
\node[fund, ref] (huang2022a) at (\xSepOne + \xSepTwo,-33.000000*\dy) {\reftext{Huan22a}\cite{huang2022a} (  -- ) ( $\num{230}$ , -- , -- ) ( -- , -- , --  )};
\coordinate (huang2022aC) at ($(huang2022a.west)+(\dxStart+\dy,0)$);
\node[ ref] (huang2022b) at ($(huang2022aC |- 0,-34.000000*\dy)$) {\reftext{Huan22b}\cite{huang2022b} (  -- ) ( $\num{230}$ , -- , -- ) ( -- , -- , --  )};
\draw (huang2022b.west) -| ++(-\dy,\fy*\dy);


==> data/IncompIon_ref_chain_alpha.tex <==
\node[desc] at (0,0.000000*\dy) {n-type ( Don, $\alpha$ ) ( N, $\alpha$ ) ( P, $\alpha$ )};
\node[author] at (0,-1.500000*\dy) {\citeauthor{tamaki2008a}};
\node[fund, ref] (tamaki2008a) at (0,-2.500000*\dy) {\reftext{Tama08a}\cite{tamaki2008a} (  \num{66}, \num{1.9e-5} ) ( -- ) ( --  )};
\coordinate (tamaki2008aC) at ($(tamaki2008a.west)+(\dxStart+\dy,0)$);
\node[ ref] (song2012) at ($(tamaki2008aC |- 0,-3.500000*\dy)$) {\reftext{Song12}\cite{song2012} (  \num{67}, \num{1.9e-5} ) ( -- ) ( --  )};
\draw (song2012.west) -| ++(-\dy,\fy*\dy);
\coordinate (song2012C) at ($(song2012.west)+(\dxStart+\dy,0)$);
\node[ ref] (khalid2012) at ($(song2012C |- 0,-4.500000*\dy)$) {\reftext{Khal12}\cite{khalid2012} (  \num{650}, \num{1.9e-5} ) ( -- ) ( --  )};
\draw (khalid2012.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (kimoto2014a) at ($(song2012.west |- 0,-5.500000*\dy)$) {\reftext{Kimo14a}\cite{kimoto2014a} (  \num{66}, \num{1.9e-5} ) ( -- ) ( --  )};
\draw (kimoto2014a.west) -| ++(-\dy,\fy*\dy);
\coordinate (kimoto2014aC) at ($(kimoto2014a.west)+(\dxStart+\dy,0)$);
\node[ ref] (dibenedetto2024) at ($(kimoto2014aC |- 0,-6.500000*\dy)$) {\reftext{Dibe24}\cite{dibenedetto2024} (  -- ) ( \num{60}, \num{3.1e-5} ) ( --  )};
\draw (dibenedetto2024.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-8.500000*\dy) {\citeauthor{hatakeyama2013}};
\node[fund, ref] (hatakeyama2013) at (0,-9.500000*\dy) {\reftext{Hata13}\cite{hatakeyama2013} (  -- ) ( \num{105}, \num{4.26e-5} ) ( --  )};
\coordinate (hatakeyama2013C) at ($(hatakeyama2013.west)+(\dxStart+\dy,0)$);
\node[ ref] (uhnevionak2015) at ($(hatakeyama2013C |- 0,-10.500000*\dy)$) {\reftext{Uhne15}\cite{uhnevionak2015} (  -- ) ( \num{105}, \num{4.26e-5} ) ( --  )};
\draw (uhnevionak2015.west) -| ++(-\dy,\fy*\dy);
\coordinate (uhnevionak2015C) at ($(uhnevionak2015.west)+(\dxStart+\dy,0)$);
\node[guess, ref] (maximenko2023) at ($(uhnevionak2015C |- 0,-11.500000*\dy)$) {\reftext{Maxi23}\cite{maximenko2023} (  -- ) ( \num{105}, \num{4.26e-5} ) ( --  )};
\draw (maximenko2023.west) -| ++(-\dy,\fy*\dy);
\node[desc] at (\xSepOne,0.000000*\dy) {p-type ( Acc, $\alpha$ ) ( Al, $\alpha$ ) ( B, $\alpha$ )};
\node[author] at (\xSepOne,-1.500000*\dy) {\citeauthor{pernot2005}};
\node[fund, ref] (pernot2005) at (\xSepOne,-2.500000*\dy) {\reftext{Pern05}\cite{pernot2005} (  -- ) ( \num{205}, \num{1.7e-5} ) ( --  )};
\coordinate (pernot2005C) at ($(pernot2005.west)+(\dxStart+\dy,0)$);
\node[ ref] (uhnevionak2015) at ($(pernot2005C |- 0,-3.500000*\dy)$) {\reftext{Uhne15}\cite{uhnevionak2015} (  -- ) ( \num{205}, \num{1.7e-5} ) ( --  )};
\draw (uhnevionak2015.west) -| ++(-\dy,\fy*\dy);
\coordinate (uhnevionak2015C) at ($(uhnevionak2015.west)+(\dxStart+\dy,0)$);
\node[guess, ref] (maximenko2023) at ($(uhnevionak2015C |- 0,-4.500000*\dy)$) {\reftext{Maxi23}\cite{maximenko2023} (  -- ) ( \num{205}, \num{1.7e-5} ) ( --  )};
\draw (maximenko2023.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-6.500000*\dy) {\citeauthor{tamaki2008a}};
\node[fund, ref] (tamaki2008a) at (\xSepOne,-7.500000*\dy) {\reftext{Tama08a}\cite{tamaki2008a} (  \num{191}, \num{3e-5} ) ( -- ) ( --  )};
\coordinate (tamaki2008aC) at ($(tamaki2008a.west)+(\dxStart+\dy,0)$);
\node[ ref] (song2012) at ($(tamaki2008aC |- 0,-8.500000*\dy)$) {\reftext{Song12}\cite{song2012} (  \num{19}, \num{3e-5} ) ( -- ) ( --  )};
\draw (song2012.west) -| ++(-\dy,\fy*\dy);
\coordinate (song2012C) at ($(song2012.west)+(\dxStart+\dy,0)$);
\node[ ref] (khalid2012) at ($(song2012C |- 0,-9.500000*\dy)$) {\reftext{Khal12}\cite{khalid2012} (  \num{19}, \num{3e-5} ) ( -- ) ( --  )};
\draw (khalid2012.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (kimoto2014a) at ($(song2012.west |- 0,-10.500000*\dy)$) {\reftext{Kimo14a}\cite{kimoto2014a} (  \num{191}, \num{3e-5} ) ( -- ) ( --  )};
\draw (kimoto2014a.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-12.500000*\dy) {\citeauthor{koizumi2009}};
\node[fund, ref] (koizumi2009) at (\xSepOne,-13.500000*\dy) {\reftext{Koiz09}\cite{koizumi2009} (  -- ) ( \num{265}, \num{3.6e-5} ) ( --  )};
\coordinate (koizumi2009C) at ($(koizumi2009.west)+(\dxStart+\dy,0)$);
\node[ ref] (hatakeyama2013) at ($(koizumi2009C |- 0,-14.500000*\dy)$) {\reftext{Hata13}\cite{hatakeyama2013} (  -- ) ( \num{265}, \num{3.6e-5} ) ( --  )};
\draw (hatakeyama2013.west) -| ++(-\dy,\fy*\dy);
\coordinate (hatakeyama2013C) at ($(hatakeyama2013.west)+(\dxStart+\dy,0)$);
\node[ ref] (dibenedetto2014) at ($(hatakeyama2013C |- 0,-15.500000*\dy)$) {\reftext{Dibe14}\cite{dibenedetto2014} (  -- ) ( \num{265}, \num{3.6e-5} ) ( --  )};
\draw (dibenedetto2014.west) -| ++(-\dy,\fy*\dy);
\coordinate (dibenedetto2014C) at ($(dibenedetto2014.west)+(\dxStart+\dy,0)$);
\node[ ref] (dibenedetto2024) at ($(dibenedetto2014C |- 0,-16.500000*\dy)$) {\reftext{Dibe24}\cite{dibenedetto2024} (  -- ) ( \num{265}, \num{3.6e-5} ) ( --  )};
\draw (dibenedetto2024.west) -| ++(-\dy,\fy*\dy);


==> data/IncompIon_undef.tex <==


\node[symbol] (NA) at (0,0) {$\ea$};
\coordinate (NA0) at (NA.north);
\node[ref, lwNA] (NA1) at (NA0.north west) {\tikz \node[paper] {\reftext{Megh18a}\cite{megherbi2018a}}; \tikz \node[paper] {\reftext{Bell14}\cite{bellone2014}}; \tikz \node[paper] {\reftext{Pezz13}\cite{pezzimenti2013}}; \tikz \node[paper] {\reftext{Bell11}\cite{bellone2011}}; \tikz \node[paper] {\reftext{Pezz09}\cite{pezzimenti2009}}; \tikz \node[paper] {\reftext{Pezz08}\cite{pezzimenti2008}};};
\node[value, scale=1.600000] (NAvalue1) at (NA1.west) {\num{190}};
\node[ref, lwNA] (NA2) at (NA1.north west) {\tikz \node[paper] {\reftext{Liu21}\cite{liu2021}}; \tikz \node[paper] {\reftext{Chen20a}\cite{chen2020a}}; \tikz \node[paper] {\reftext{Megh15}\cite{megherbi2015}}; \tikz \node[paper] {\reftext{Habi11}\cite{habib2011}}; \tikz \node[paper] {\reftext{Li03}\cite{li2003}};};
\node[value, scale=1.500000] (NAvalue2) at (NA2.west) {\num{191}};
\node[ref, lwNA] (NA3) at (NA2.north west) {\tikz \node[paper] {\reftext{Rao22}\cite{rao2022}}; \tikz \node[paper] {\reftext{Bade20}\cite{bader2020}}; \tikz \node[paper] {\reftext{Nawa10}\cite{nawaz2010}}; \tikz \node[paper] {\reftext{Bala05}\cite{balachandran2005}};};
\node[value, scale=1.400000] (NAvalue3) at (NA3.west) {\num{200}};
\node[ref, lwNA] (NA4) at (NA3.north west) {\tikz \node[paper] {\reftext{Pear23}\cite{pearton2023}};};
\node[value, scale=1.100000] (NAvalue4) at (NA4.west) {\num{250}};


\node[symbol] (ND) at (0+ \dxNA,0) {$\ed$};
\coordinate (ND0) at (ND.north);
\node[ref, lwND] (ND1) at (ND0.north west) {\tikz \node[paper] {\reftext{Bade20}\cite{bader2020}}; \tikz \node[paper] {\reftext{Pezz09}\cite{pezzimenti2009}}; \tikz \node[paper] {\reftext{Pezz08}\cite{pezzimenti2008}};};
\node[value, scale=1.300000] (NDvalue1) at (ND1.west) {\num{50}};
\node[ref, lwND] (ND2) at (ND1.north west) {\tikz \node[paper] {\reftext{Bert04}\cite{bertilsson2004}};};
\node[value, scale=1.100000] (NDvalue2) at (ND2.west) {\num{52}};
\node[ref, lwND] (ND3) at (ND2.north west) {\tikz \node[paper] {\reftext{Bert04a}\cite{bertilsson2004a}};};
\node[value, scale=1.100000] (NDvalue3) at (ND3.west) {\num{52.1}};
\node[ref, lwND] (ND4) at (ND3.north west) {\tikz \node[paper] {\reftext{Pear23}\cite{pearton2023}}; \tikz \node[paper] {\reftext{Chen20a}\cite{chen2020a}}; \tikz \node[paper] {\reftext{Habi11}\cite{habib2011}};};
\node[value, scale=1.300000] (NDvalue4) at (ND4.west) {\num{60}};
\node[ref, lwND] (ND5) at (ND4.north west) {\tikz \node[paper] {\reftext{Liu21}\cite{liu2021}}; \tikz \node[paper] {\reftext{Megh15}\cite{megherbi2015}}; \tikz \node[paper] {\reftext{Zhao03}\cite{zhao2003}}; \tikz \node[paper] {\reftext{Li03}\cite{li2003}};};
\node[value, scale=1.400000] (NDvalue5) at (ND5.west) {\num{65}};
\node[ref, lwND] (ND6) at (ND5.north west) {\tikz \node[paper] {\reftext{Megh18a}\cite{megherbi2018a}}; \tikz \node[paper] {\reftext{Bell14}\cite{bellone2014}}; \tikz \node[paper] {\reftext{Pezz13}\cite{pezzimenti2013}}; \tikz \node[paper] {\reftext{Bell11}\cite{bellone2011}};};
\node[value, scale=1.400000] (NDvalue6) at (ND6.west) {\num{70}};
\node[ref, lwND] (ND7) at (ND6.north west) {\tikz \node[paper] {\reftext{Rosc98}\cite{roschke1998}};};
\node[value, scale=1.100000] (NDvalue7) at (ND7.west) {\num{80}};
\node[ref, lwND] (ND8) at (ND7.north west) {\tikz \node[paper] {\reftext{Rao22}\cite{rao2022}}; \tikz \node[paper] {\reftext{Nawa10}\cite{nawaz2010}}; \tikz \node[paper] {\reftext{Bala05}\cite{balachandran2005}};};
\node[value, scale=1.300000] (NDvalue8) at (ND8.west) {\num{100}};


==> data/bandgap_figure_models.tex <==
\pgfplotsset{cycle list name=meas}
\addplot+[only marks, error bars/.cd, y dir=both, y explicit]coordinates {(4,3.263) +- (0,0.003)};
\addlegendentry{\reftext{Choy64}\cite{choyke1964} $\egx$}
\addplot+[only marks] coordinates {(4.7,3.265) (77,3.264) (121.8,3.2615) (181,3.256) (195.7,3.2534)};
\addlegendentry{\reftext{Choy64a}\cite{choyke1964a} $\egx$}
\addplot+[only marks] coordinates {(300,3.23)};
\addlegendentry{\reftext{Zanm64}\cite{zanmarchi1964} $\egx$}
\addplot+[only marks] coordinates {(77,3.2639)};
\addlegendentry{\reftext{Iked80b}\cite{ikeda1980b} $\egx$}
\addplot+[only marks] coordinates {(4.2,3.265)};
\addlegendentry{\reftext{Kord95}\cite{kordina1995} $\egx$}
\addplot+[only marks, error bars/.cd, y dir=both, y explicit]coordinates {(40,3.41) +- (0,0.03)};
\addlegendentry{\reftext{Evwa96}\cite{evwaraye1996} $\eg$}
\addplot+[only marks] coordinates {(4.25,3.2653) (11.05,3.26469) (22.14,3.264828) (26.125,3.2647) (34.1945,3.2648) (33.286,3.2645) (43.219,3.26448) (46.236,3.26457) (48.185,3.2644) (53.067,3.26435) (58.1127,3.2643) (62.181,3.26417) (66.086,3.26409) (76.012,3.26386) (81.060,3.26385) (83.989,3.26379) (90,3.26351) (94.946,3.2629) (102.127,3.26326) (109.185,3.2626)};
\addlegendentry{\reftext{Itoh96}\cite{itoh1996} $\egx$}
\addplot+[only marks] coordinates {(2,3.266)};
\addlegendentry{\reftext{Ivan98}\cite{ivanov1998} $\egx$}
\addplot+[only marks] table [x expr=\thisrowno{0}, y expr=\thisrowno{1}, col sep=comma] {data/bandgap_miller2000.csv};\addlegendentry{\reftext{Mill00}\cite{miller2000} $\eg$}\addplot+[only marks] coordinates {(2,3.267)};
\addlegendentry{\reftext{Srid00}\cite{sridhara2000} $\egx$}
\addplot+[only marks, error bars/.cd, y dir=both, y explicit]coordinates {(300,3.26) +- (0,0.098)};
\addlegendentry{\reftext{Ahuj02}\cite{ahuja2002} $\eg$}
\addplot+[only marks] coordinates {(2,3.285)};
\addlegendentry{\reftext{Ivan02}\cite{ivanov2002} $\eg$}
\addplot+[only marks] coordinates {(300,3.18)};
\addlegendentry{\reftext{Shal02}\cite{shalish2002} $\eg$}
\addplot+[only marks] coordinates {(75.1,3.2658) (189.27,3.2552) (295.7,3.2329) (370.386,3.215) (450.215,3.193)};
\addlegendentry{\reftext{Griv07}\cite{grivickas2007} $\egx$}
\addplot+[only marks] coordinates {(0,3.28)};
\addlegendentry{\reftext{Ng10}\cite{ng2010} $\eg$}
\addplot+[only marks] coordinates {(0,3.285)};
\addlegendentry{\reftext{Khal12}\cite{khalid2012} $\eg$}
\addplot+[only marks] coordinates {(0,3.285)};
\addlegendentry{\reftext{Stef14}\cite{stefanakis2014} $\eg$}
\addplot+[only marks] coordinates {(300,3.22)};
\addlegendentry{\reftext{Fang18}\cite{fang2018} $\eg$}
\addplot+[only marks] coordinates {(1.4,3.2659)};
\addlegendentry{\reftext{Klah20}\cite{klahold2020} $\egx$}
\addplot+[only marks, error bars/.cd, y dir=both, y explicit]coordinates {(300,3.3) +- (0,0.02)};
\addlegendentry{\reftext{Main24}\cite{mainali2024} $\eg$}
\pgfplotsset{cycle list name=VA}
\pgfplotsset{cycle list shift=\cs}

\addplot+[domain=4:200, no marks, samples=\samp] {VA(3.265,0,3.3e-4,1050)};
\addlegendentry{\reftext{Lade00}\cite{ladesmartin2000} $\egx$ (\ref{eq:bandgap_varshni})}
\addplot+[domain=4:600, no marks, samples=\samp] {VA(3.265,0,3.3e-2,1e5)};
\addlegendentry{\reftext{Lade00}\cite{ladesmartin2000} $\egx$ (\ref{eq:bandgap_varshni})}
\addplot+[domain=300:700, no marks, samples=\samp] {VA(3.342,0,3.3e-4,0)};
\addlegendentry{\reftext{Lade00}\cite{ladesmartin2000} $\egx$ (\ref{eq:bandgap_varshni})}
\addplot+[domain=0:800, no marks, samples=\samp] {VA(3.23,300,6.5e-4,1300)};
\addlegendentry{\reftext{Levi01}\cite{levinshtein2001} $\eg$ (\ref{eq:bandgap_varshni})}
\addplot+[domain=0:650, no marks, samples=\samp] {VA(3.285,0,3.5e-4,1100)};
\addlegendentry{\reftext{Gale02}\cite{galeckas2002} $\eg$ (\ref{eq:bandgap_varshni})}
\addplot+[domain=300:650, no marks, samples=\samp] {VA(3.2625,300,2.4e-4,0)};
\addlegendentry{\reftext{Gale02}\cite{galeckas2002} $\eg$ (\ref{eq:bandgap_varshni})}
\addplot+[domain=\pgfkeysvalueof{/pgfplots/xmin}:\pgfkeysvalueof{/pgfplots/xmax}, no marks, samples=\samp] {VA(3.26,300,4.15e-4,-131)};
\addlegendentry{\reftext{Bala05}\cite{balachandran2005} $\eg$ (\ref{eq:bandgap_varshni})}
\addplot+[domain=\pgfkeysvalueof{/pgfplots/xmin}:\pgfkeysvalueof{/pgfplots/xmax}, no marks, samples=\samp] {VA(3.23,300,7.036e-4,1509)};
\addlegendentry{\reftext{Tama08a}\cite{tamaki2008a} $\eg$ (\ref{eq:bandgap_varshni})}
\addplot+[domain=\pgfkeysvalueof{/pgfplots/xmin}:\pgfkeysvalueof{/pgfplots/xmax}, no marks, samples=\samp] {VA(3.285,0,2.206e-2,1e5)};
\addlegendentry{\reftext{Khal12}\cite{khalid2012} $\eg$ (\ref{eq:bandgap_varshni})}
\addplot+[domain=0:800, no marks, samples=\samp] {VA(3.265,0,9.06e-4,2030)};
\addlegendentry{\reftext{Hata13}\cite{hatakeyama2013} $\egx$ (\ref{eq:bandgap_varshni})}
\addplot+[domain=\pgfkeysvalueof{/pgfplots/xmin}:\pgfkeysvalueof{/pgfplots/xmax}, no marks, samples=\samp] {VA(3.285,0,3.3e-4,240)};
\addlegendentry{\reftext{Stef14}\cite{stefanakis2014} $\eg$ (\ref{eq:bandgap_varshni})}
\addplot+[domain=300:620, no marks, samples=\samp] {VA(3.28,300,5.27e-4,0)};
\addlegendentry{\reftext{Chen22}\cite{cheng2022} $\eg$ (\ref{eq:bandgap_varshni})}
\pgfplotsset{cycle list name=PA}
\pgfplotsset{cycle list shift=\csPA}

\addplot+[domain=0:500, no marks, samples=\samp] {PA(3.267,3e-4,450,2.9)};
\addlegendentry{\reftext{Griv07}\cite{grivickas2007} $\egx$ (\ref{eq:bandgap_passler})}


==> data/bandgap_fund_stat.tex <==
\addplot+ [ boxplot prepared = { lower whisker=3.1800, lower quartile=3.2100, median=3.2612, upper quartile=3.2850, upper whisker=3.3000, },] coordinates {} node[mean,anchor=west] at (boxplot box cs: \boxplotvalue{median},0.5) {\pgfmathprintnumber{\boxplotvalue{median}}};
\addplot+ [ boxplot prepared = { lower whisker=3.2630, lower quartile=3.2650, median=3.2654, upper quartile=3.2668, upper whisker=3.2670, },] coordinates {} node[mean,anchor=west] at (boxplot box cs: \boxplotvalue{upper whisker},0.5) {\pgfmathprintnumber{\boxplotvalue{median}}};


==> data/bandgap_lindefelt.tex <==
\addplot+ [domain=\pgfkeysvalueof{/pgfplots/xmin}:\pgfkeysvalueof{/pgfplots/xmax}, samples=\samp] { Lindefeltn(-0.015,-0.00293,0.019,0.00874)};
\addlegendentry{\reftext{Lind98}\cite{lindefelt1998} $\Delta \egn$}
\addplot+ [domain=\pgfkeysvalueof{/pgfplots/xmin}:\pgfkeysvalueof{/pgfplots/xmax}, samples=\samp] { Lindefeltp(-0.0157,-0.000387,0.013,0.00115,0)};
\addlegendentry{\reftext{Lind98}\cite{lindefelt1998} $\Delta \egp$}
\addplot+ [domain=\pgfkeysvalueof{/pgfplots/xmin}:\pgfkeysvalueof{/pgfplots/xmax}, samples=\samp] { Lindefeltn(-0.01791,-0.0022,0.02823,0.00624)};
\addlegendentry{\reftext{Pers99}\cite{persson1999} $\Delta \egn$}
\addplot+ [domain=\pgfkeysvalueof{/pgfplots/xmin}:\pgfkeysvalueof{/pgfplots/xmax}, samples=\samp] { Lindefeltp(-0.01615,-0.00107,-0.03507,0.00674,0.05696)};
\addlegendentry{\reftext{Pers99}\cite{persson1999} $\Delta \egp$}


==> data/bandgap_lindefelt_cv.tex <==
\addplot+ [domain=\pgfkeysvalueof{/pgfplots/xmin}:\pgfkeysvalueof{/pgfplots/xmax}, samples=\samp] { Lindefeltc(-0.015,-0.00293,-0.0157,-0.000387)};
\addlegendentry{\reftext{Lind98}\cite{lindefelt1998} $\mid \Delta \ecb \mid$}
\addplot+ [domain=\pgfkeysvalueof{/pgfplots/xmin}:\pgfkeysvalueof{/pgfplots/xmax}, samples=\samp] { Lindefeltc(-0.01791,-0.0022,-0.01615,-0.00107)};
\addlegendentry{\reftext{Pers99}\cite{persson1999} $\mid \Delta \ecb \mid$}
\addplot+ [domain=\pgfkeysvalueof{/pgfplots/xmin}:\pgfkeysvalueof{/pgfplots/xmax}, samples=\samp] { Lindefeltv(0.019,0.00874,0.013,0.00115,0)};
\addlegendentry{\reftext{Lind98}\cite{lindefelt1998} $\Delta \evb$}
\addplot+ [domain=\pgfkeysvalueof{/pgfplots/xmin}:\pgfkeysvalueof{/pgfplots/xmax}, samples=\samp] { Lindefeltv(0.02823,0.00624,-0.03507,0.00674,0.05696)};
\addlegendentry{\reftext{Pers99}\cite{persson1999} $\Delta \evb$}


==> data/bandgap_lindefelt_cv_ratio.tex <==
\addplot+ [domain=\pgfkeysvalueof{/pgfplots/xmin}:\pgfkeysvalueof{/pgfplots/xmax}, samples=\samp] { Lindefeltshare(-0.015,-0.00293,-0.0157,-0.000387,0.019,0.00874,0.013,0.00115,0)};
\addplot+ [domain=\pgfkeysvalueof{/pgfplots/xmin}:\pgfkeysvalueof{/pgfplots/xmax}, samples=\samp] { Lindefeltshare(-0.01791,-0.0022,-0.01615,-0.00107,0.02823,0.00624,-0.03507,0.00674,0.05696)};


==> data/bandgap_ref_chain_Ex.tex <==
\node[desc] at (0,0.000000*\dy) {Exciton ($\ex$)};
\node[author] at (0,-1.500000*\dy) {\citeauthor{nedzvetskii1969}};
\node[no4H, ref] (nedzvetskii1969) at (0,-2.500000*\dy) {\reftext{Nedz69}\cite{nedzvetskii1969} (  --  )};
\coordinate (nedzvetskii1969C) at ($(nedzvetskii1969.west)+(\dxStart+\dy,0)$);
\node[ ref] (matsunami1974) at ($(nedzvetskii1969C |- 0,-3.500000*\dy)$) {\reftext{Mats74}\cite{matsunami1974} (  10  )};
\draw (matsunami1974.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (suzuki1977) at ($(matsunami1974.west |- 0,-4.500000*\dy)$) {\reftext{Suzu77}\cite{suzuki1977} (  10  )};
\draw (suzuki1977.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-6.500000*\dy) {\citeauthor{dubrovskii1975}};
\node[fund, ref] (dubrovskii1975) at (0,-7.500000*\dy) {\reftext{Dubr75}\cite{dubrovskii1975} (  20  )};
\coordinate (dubrovskii1975C) at ($(dubrovskii1975.west)+(\dxStart+\dy,0)$);
\node[ ref] (ikeda1980) at ($(dubrovskii1975C |- 0,-8.500000*\dy)$) {\reftext{Iked80}\cite{ikeda1980} (  20  )};
\draw (ikeda1980.west) -| ++(-\dy,\fy*\dy);
\coordinate (ikeda1980C) at ($(ikeda1980.west)+(\dxStart+\dy,0)$);
\node[ ref] (fan2014) at ($(ikeda1980C |- 0,-9.500000*\dy)$) {\reftext{Fan14}\cite{fan2014} (  20  )};
\draw (fan2014.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (freitas1995) at ($(ikeda1980.west |- 0,-10.500000*\dy)$) {\reftext{Frei95}\cite{freitas1995} (  20  )};
\draw (freitas1995.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (devaty1997) at ($(freitas1995.west |- 0,-11.500000*\dy)$) {\reftext{Deva97}\cite{devaty1997} (  20  )};
\draw (devaty1997.west) -| ++(-\dy,\fy*\dy);
\coordinate (devaty1997C) at ($(devaty1997.west)+(\dxStart+\dy,0)$);
\node[ ref] (ladesmartin2000) at ($(devaty1997C |- 0,-12.500000*\dy)$) {\reftext{Lade00}\cite{ladesmartin2000} (  40  )};
\draw (ladesmartin2000.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (ayalew2004) at ($(ladesmartin2000.west |- 0,-13.500000*\dy)$) {\reftext{Ayal04}\cite{ayalew2004} (  20  )};
\draw (ayalew2004.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (egilsson1999) at ($(devaty1997.west |- 0,-14.500000*\dy)$) {\reftext{Egil99}\cite{egilsson1999} (  20  )};
\draw (egilsson1999.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (masri2002) at ($(egilsson1999.west |- 0,-15.500000*\dy)$) {\reftext{Masr02}\cite{masri2002} (  20  )};
\draw (masri2002.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (hatakeyama2013) at ($(masri2002.west |- 0,-16.500000*\dy)$) {\reftext{Hata13}\cite{hatakeyama2013} (  20  )};
\draw (hatakeyama2013.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,0.000000*\dy) {\citeauthor{sankin1975}};
\node[no4H, ref] (sankin1975) at (\xSepOne,-1.000000*\dy) {\reftext{Sank75}\cite{sankin1975} (  78  )};
\coordinate (sankin1975C) at ($(sankin1975.west)+(\dxStart+\dy,0)$);
\node[ ref] (pankove2014) at ($(sankin1975C |- 0,-2.000000*\dy)$) {\reftext{Pank14}\cite{pankove2014} (  20  )};
\draw (pankove2014.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-4.000000*\dy) {\citeauthor{ivanov2002}};
\node[fund, ref] (ivanov2002) at (\xSepOne,-5.000000*\dy) {\reftext{Ivan02}\cite{ivanov2002} (  20.5  )};
\coordinate (ivanov2002C) at ($(ivanov2002.west)+(\dxStart+\dy,0)$);
\node[ ref] (janzen2008) at ($(ivanov2002C |- 0,-6.000000*\dy)$) {\reftext{Janz08}\cite{janzen2008} (  21  )};
\draw (janzen2008.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (kimoto2014a) at ($(janzen2008.west |- 0,-7.000000*\dy)$) {\reftext{Kimo14a}\cite{kimoto2014a} (  20  )};
\draw (kimoto2014a.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-9.000000*\dy) {\citeauthor{grivickas2007}};
\node[fund, ref] (grivickas2007) at (\xSepOne,-10.000000*\dy) {\reftext{Griv07}\cite{grivickas2007} (  30  )};
\coordinate (grivickas2007C) at ($(grivickas2007.west)+(\dxStart+\dy,0)$);
\node[ ref] (scajev2010) at ($(grivickas2007C |- 0,-11.000000*\dy)$) {\reftext{Scaj10}\cite{scajev2010} (  30  )};
\draw (scajev2010.west) -| ++(-\dy,\fy*\dy);


==> data/bandgap_ref_chain_bandgap.tex <==
\node[desc] at (0,0.000000*\dy) {Band Gap ($\eg$, $\egx$, $T$)};
\node[author] at (0,-1.500000*\dy) {\citeauthor{choyke1964}};
\node[fund, ref] (choyke1964) at (0,-2.500000*\dy) {\reftext{Choy64}\cite{choyke1964} (  -- , 3.263 , 4  )};
\coordinate (choyke1964C) at ($(choyke1964.west)+(\dxStart+\dy,0)$);
\node[calc, ref] (junginger1970) at ($(choyke1964C |- 0,-3.500000*\dy)$) {\reftext{Jung70}\cite{junginger1970} (3.26 , -- , -- )};
\draw (junginger1970.west) -| ++(-\dy,\fy*\dy);
\coordinate (junginger1970C) at ($(junginger1970.west)+(\dxStart+\dy,0)$);
\node[guess, ref] (afanasev1996) at ($(junginger1970C |- 0,-4.500000*\dy)$) {\reftext{Afan96}\cite{afanasev1996} (  3.26 , -- , 300  )};
\draw (afanasev1996.west) -| ++(-\dy,\fy*\dy);
\coordinate (afanasev1996C) at ($(afanasev1996.west)+(\dxStart+\dy,0)$);
\node[ ref] (tilak2007) at ($(afanasev1996C |- 0,-5.500000*\dy)$) {\reftext{Tila07}\cite{tilak2007} (  3.26 , -- , --  )};
\draw (tilak2007.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (scaburri2011a) at ($(tilak2007.west |- 0,-6.500000*\dy)$) {\reftext{Scab11a}\cite{scaburri2011a} (  3.26 , -- , --  )};
\draw (scaburri2011a.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (yoder1996) at ($(afanasev1996.west |- 0,-7.500000*\dy)$) {\reftext{Yode96}\cite{yoder1996} (  3.26 , -- , --  )};
\draw (yoder1996.west) -| ++(-\dy,\fy*\dy);
\coordinate (yoder1996C) at ($(yoder1996.west)+(\dxStart+\dy,0)$);
\node[ ref] (su2010) at ($(yoder1996C |- 0,-8.500000*\dy)$) {\reftext{Su10}\cite{su2010} (  3.26 , -- , --  )};
\draw (su2010.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (neilainglesias2012) at ($(su2010.west |- 0,-9.500000*\dy)$) {\reftext{Neil12}\cite{neilainglesias2012} (  3.26 , -- , --  )};
\draw (neilainglesias2012.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (matsunami1997) at ($(yoder1996.west |- 0,-10.500000*\dy)$) {\reftext{Mats97}\cite{matsunami1997} (  3.26 , -- , --  )};
\draw (matsunami1997.west) -| ++(-\dy,\fy*\dy);
\coordinate (matsunami1997C) at ($(matsunami1997.west)+(\dxStart+\dy,0)$);
\node[ ref] (lebedev1999) at ($(matsunami1997C |- 0,-11.500000*\dy)$) {\reftext{Lebe99}\cite{lebedev1999} (  3.2 , -- , --  )};
\draw (lebedev1999.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (wright1998) at ($(matsunami1997.west |- 0,-12.500000*\dy)$) {\reftext{Wrig98}\cite{wright1998} (  3.26 , -- , 300  )};
\draw (wright1998.west) -| ++(-\dy,\fy*\dy);
\coordinate (wright1998C) at ($(wright1998.west)+(\dxStart+\dy,0)$);
\node[ ref] (hefner2001) at ($(wright1998C |- 0,-13.500000*\dy)$) {\reftext{Hefn01}\cite{hefner2001} (  3.26 , -- , --  )};
\draw (hefner2001.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (mcnutt2004) at ($(hefner2001.west |- 0,-14.500000*\dy)$) {\reftext{Mcnu04}\cite{mcnutt2004} (  3.26 , -- , 300  )};
\draw (mcnutt2004.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (baliga2006) at ($(mcnutt2004.west |- 0,-15.500000*\dy)$) {\reftext{Bali06}\cite{baliga2006} (  3.26 , -- , --  )};
\draw (baliga2006.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (baliga2019) at ($(baliga2006.west |- 0,-16.500000*\dy)$) {\reftext{Bali19}\cite{baliga2019} (  3.26 , -- , --  )};
\draw (baliga2019.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (chow2000) at ($(wright1998.west |- 0,-17.500000*\dy)$) {\reftext{Chow00}\cite{chow2000} (  3.26 , -- , --  )};
\draw (chow2000.west) -| ++(-\dy,\fy*\dy);
\coordinate (chow2000C) at ($(chow2000.west)+(\dxStart+\dy,0)$);
\node[ ref] (dhanaraj2010) at ($(chow2000C |- 0,-18.500000*\dy)$) {\reftext{Dhan10}\cite{dhanaraj2010} (  3.3 , -- , --  )};
\draw (dhanaraj2010.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (elasser2000) at ($(chow2000.west |- 0,-19.500000*\dy)$) {\reftext{Elas00}\cite{elasser2000} (  3.26 , -- , 300  )};
\draw (elasser2000.west) -| ++(-\dy,\fy*\dy);
\coordinate (elasser2000C) at ($(elasser2000.west)+(\dxStart+\dy,0)$);
\node[ ref] (li2003) at ($(elasser2000C |- 0,-20.500000*\dy)$) {\reftext{Li03}\cite{li2003} (  3.359 , -- , 0  )};
\draw (li2003.west) -| ++(-\dy,\fy*\dy);
\coordinate (li2003C) at ($(li2003.west)+(\dxStart+\dy,0)$);
\node[ ref] (megherbi2018a) at ($(li2003C |- 0,-21.500000*\dy)$) {\reftext{Megh18a}\cite{megherbi2018a} (  3.2 , -- , 300  )};
\draw (megherbi2018a.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (zeghdar2019) at ($(megherbi2018a.west |- 0,-22.500000*\dy)$) {\reftext{Zegh19}\cite{zeghdar2019} (  3.26 , -- , 300  )};
\draw (zeghdar2019.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (zeghdar2020) at ($(zeghdar2019.west |- 0,-23.500000*\dy)$) {\reftext{Zegh20}\cite{zeghdar2020} (  3.26 , -- , 300  )};
\draw (zeghdar2020.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (zhao2003) at ($(li2003.west |- 0,-24.500000*\dy)$) {\reftext{Zhao03}\cite{zhao2003} (  3.359 , -- , 0  )};
\draw (zhao2003.west) -| ++(-\dy,\fy*\dy);
\coordinate (zhao2003C) at ($(zhao2003.west)+(\dxStart+\dy,0)$);
\node[ ref] (das2015) at ($(zhao2003C |- 0,-25.500000*\dy)$) {\reftext{Das15}\cite{das2015} (  3.359 , -- , 0  )};
\draw (das2015.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (werner2001) at ($(elasser2000.west |- 0,-26.500000*\dy)$) {\reftext{Wern01}\cite{werner2001} (  3.26 , -- , --  )};
\draw (werner2001.west) -| ++(-\dy,\fy*\dy);
\coordinate (werner2001C) at ($(werner2001.west)+(\dxStart+\dy,0)$);
\node[ ref] (manikam2011) at ($(werner2001C |- 0,-27.500000*\dy)$) {\reftext{Mani11}\cite{manikam2011} (  3.26 , -- , --  )};
\draw (manikam2011.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (elasser2002) at ($(werner2001.west |- 0,-28.500000*\dy)$) {\reftext{Elas02}\cite{elasser2002} (  3.26 , -- , 300  )};
\draw (elasser2002.west) -| ++(-\dy,\fy*\dy);
\coordinate (elasser2002C) at ($(elasser2002.west)+(\dxStart+\dy,0)$);
\node[ ref] (philip2006) at ($(elasser2002C |- 0,-29.500000*\dy)$) {\reftext{Phil06}\cite{philip2006} (  3.26 , -- , --  )};
\draw (philip2006.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (lee2002) at ($(elasser2002.west |- 0,-30.500000*\dy)$) {\reftext{Lee02}\cite{lee2002} (  3.26 , -- , 300  )};
\draw (lee2002.west) -| ++(-\dy,\fy*\dy);
\coordinate (lee2002C) at ($(lee2002.west)+(\dxStart+\dy,0)$);
\node[ ref] (chen2015) at ($(lee2002C |- 0,-31.500000*\dy)$) {\reftext{Chen15}\cite{chen2015} (  3.26 , -- , 300  )};
\draw (chen2015.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (han2003) at ($(lee2002.west |- 0,-32.500000*\dy)$) {\reftext{Han03}\cite{han2003} (  3.26 , -- , --  )};
\draw (han2003.west) -| ++(-\dy,\fy*\dy);
\coordinate (han2003C) at ($(han2003.west)+(\dxStart+\dy,0)$);
\node[ ref] (gerhardt2011) at ($(han2003C |- 0,-33.500000*\dy)$) {\reftext{Gerh11}\cite{gerhardt2011} (  3.26 , -- , --  )};
\draw (gerhardt2011.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (balachandran2005) at ($(han2003.west |- 0,-34.500000*\dy)$) {\reftext{Bala05}\cite{balachandran2005} (  3.26 , -- , 300  )};
\draw (balachandran2005.west) -| ++(-\dy,\fy*\dy);
\coordinate (balachandran2005C) at ($(balachandran2005.west)+(\dxStart+\dy,0)$);
\node[ ref] (nawaz2010) at ($(balachandran2005C |- 0,-35.500000*\dy)$) {\reftext{Nawa10}\cite{nawaz2010} (  3.26 , -- , 300  )};
\draw (nawaz2010.west) -| ++(-\dy,\fy*\dy);
\coordinate (nawaz2010C) at ($(nawaz2010.west)+(\dxStart+\dy,0)$);
\node[ ref] (usman2014) at ($(nawaz2010C |- 0,-36.500000*\dy)$) {\reftext{Usma14}\cite{usman2014} (  3.24 , -- , 300  )};
\draw (usman2014.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (zhu2008) at ($(balachandran2005.west |- 0,-37.500000*\dy)$) {\reftext{Zhu08}\cite{zhu2008} (  3.26 , -- , --  )};
\draw (zhu2008.west) -| ++(-\dy,\fy*\dy);
\coordinate (zhu2008C) at ($(zhu2008.west)+(\dxStart+\dy,0)$);
\node[ ref] (liu2015) at ($(zhu2008C |- 0,-38.500000*\dy)$) {\reftext{Liu15}\cite{liu2015} (  3.26 , -- , --  )};
\draw (liu2015.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (kaminski2009) at ($(zhu2008.west |- 0,-39.500000*\dy)$) {\reftext{Kami09}\cite{kaminski2009} (  3.26 , -- , --  )};
\draw (kaminski2009.west) -| ++(-\dy,\fy*\dy);
\coordinate (kaminski2009C) at ($(kaminski2009.west)+(\dxStart+\dy,0)$);
\node[ ref] (kaminski2014) at ($(kaminski2009C |- 0,-40.500000*\dy)$) {\reftext{Kami14}\cite{kaminski2014} (  3.26 , -- , --  )};
\draw (kaminski2014.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (kimoto2015) at ($(kaminski2009.west |- 0,-41.500000*\dy)$) {\reftext{Kimo15}\cite{kimoto2015} (  3.26 , -- , --  )};
\draw (kimoto2015.west) -| ++(-\dy,\fy*\dy);
\coordinate (kimoto2015C) at ($(kimoto2015.west)+(\dxStart+\dy,0)$);
\node[ ref] (baierhofer2019) at ($(kimoto2015C |- 0,-42.500000*\dy)$) {\reftext{Baie19}\cite{baierhofer2019} (  3.268 , -- , --  )};
\draw (baierhofer2019.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (ostling2024) at ($(baierhofer2019.west |- 0,-43.500000*\dy)$) {\reftext{Ostl24}\cite{ostling2024} (  3.26 , -- , --  )};
\draw (ostling2024.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (chow2017) at ($(kimoto2015.west |- 0,-44.500000*\dy)$) {\reftext{Chow17}\cite{chow2017} (  3.26 , -- , --  )};
\draw (chow2017.west) -| ++(-\dy,\fy*\dy);
\coordinate (chow2017C) at ($(chow2017.west)+(\dxStart+\dy,0)$);
\node[ ref] (bader2020) at ($(chow2017C |- 0,-45.500000*\dy)$) {\reftext{Bade20}\cite{bader2020} (  3.3 , -- , 300  )};
\draw (bader2020.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (yoshida1995) at ($(junginger1970.west |- 0,-46.500000*\dy)$) {\reftext{Yosh95}\cite{yoshida1995} (  -- , 3.263 , --  )};
\draw (yoshida1995.west) -| ++(-\dy,\fy*\dy);
\coordinate (yoshida1995C) at ($(yoshida1995.west)+(\dxStart+\dy,0)$);
\node[ ref] (bellotti1999) at ($(yoshida1995C |- 0,-47.500000*\dy)$) {\reftext{Bell99}\cite{bellotti1999} (  3.26 , -- , --  )};
\draw (bellotti1999.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (kohlscheen2003) at ($(bellotti1999.west |- 0,-48.500000*\dy)$) {\reftext{Kohl03}\cite{kohlscheen2003} (  3.26 , -- , --  )};
\draw (kohlscheen2003.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (choi2005) at ($(kohlscheen2003.west |- 0,-49.500000*\dy)$) {\reftext{Choi05}\cite{choi2005} (  3.26 , -- , --  )};
\draw (choi2005.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (tanner2007) at ($(choi2005.west |- 0,-50.500000*\dy)$) {\reftext{Tann07}\cite{tanner2007} (  3.26 , -- , --  )};
\draw (tanner2007.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (raynaud2010) at ($(tanner2007.west |- 0,-51.500000*\dy)$) {\reftext{Rayn10}\cite{raynaud2010} (  3.263 , -- , 0  )};
\draw (raynaud2010.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (zippelius2011) at ($(raynaud2010.west |- 0,-52.500000*\dy)$) {\reftext{Zipp11}\cite{zippelius2011} (  3.26 , -- , --  )};
\draw (zippelius2011.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (biondo2012) at ($(zippelius2011.west |- 0,-53.500000*\dy)$) {\reftext{Bion12}\cite{biondo2012} (  3.26 , -- , 0  )};
\draw (biondo2012.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (uhnevionak2015) at ($(biondo2012.west |- 0,-54.500000*\dy)$) {\reftext{Uhne15}\cite{uhnevionak2015} (  3.26 , -- , 0  )};
\draw (uhnevionak2015.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (pearton2023) at ($(uhnevionak2015.west |- 0,-55.500000*\dy)$) {\reftext{Pear23}\cite{pearton2023} (  3.25 , -- , --  )};
\draw (pearton2023.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (camassel2008) at ($(yoshida1995.west |- 0,-56.500000*\dy)$) {\reftext{Cama08}\cite{camassel2008} (  3.263 , -- , --  )};
\draw (camassel2008.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (lutz2011) at ($(camassel2008.west |- 0,-57.500000*\dy)$) {\reftext{Lutz11}\cite{lutz2011} (  3.263 , -- , 0  )};
\draw (lutz2011.west) -| ++(-\dy,\fy*\dy);
\coordinate (lutz2011C) at ($(lutz2011.west)+(\dxStart+\dy,0)$);
\node[ ref] (johannesson2016) at ($(lutz2011C |- 0,-58.500000*\dy)$) {\reftext{Joha16}\cite{johannesson2016} (  3.263 , -- , 0  )};
\draw (johannesson2016.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (fan2014) at ($(lutz2011.west |- 0,-59.500000*\dy)$) {\reftext{Fan14}\cite{fan2014} (  -- , 3.263 , --  )};
\draw (fan2014.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,0.000000*\dy) {\citeauthor{choyke1964a}};
\node[fund, ref] (choyke1964a) at (\xSepOne,-1.000000*\dy) {\reftext{Choy64a}\cite{choyke1964a} (  -- , M , M  )};
\coordinate (choyke1964aC) at ($(choyke1964a.west)+(\dxStart+\dy,0)$);
\node[guess, ref] (patrick1965) at ($(choyke1964aC |- 0,-2.000000*\dy)$) {\reftext{Patr65}\cite{patrick1965} (  -- , 3.265 , --  )};
\draw (patrick1965.west) -| ++(-\dy,\fy*\dy);
\coordinate (patrick1965C) at ($(patrick1965.west)+(\dxStart+\dy,0)$);
\node[ ref] (ladesmartin2000) at ($(patrick1965C |- 0,-3.000000*\dy)$) {\reftext{Lade00}\cite{ladesmartin2000} (  -- , M , M  )};
\draw (ladesmartin2000.west) -| ++(-\dy,\fy*\dy);
\coordinate (ladesmartin2000C) at ($(ladesmartin2000.west)+(\dxStart+\dy,0)$);
\node[ ref] (johannesson2019) at ($(ladesmartin2000C |- 0,-4.000000*\dy)$) {\reftext{Joha19}\cite{johannesson2019} (  3.26 , -- , --  )};
\draw (johannesson2019.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (rakheja2020) at ($(johannesson2019.west |- 0,-5.000000*\dy)$) {\reftext{Rakh20}\cite{rakheja2020} (  3.23 , -- , 300  )};
\draw (rakheja2020.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (lechner2021) at ($(rakheja2020.west |- 0,-6.000000*\dy)$) {\reftext{Lech21}\cite{lechner2021} (  3.265 , -- , 0  )};
\draw (lechner2021.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (ayalew2004) at ($(ladesmartin2000.west |- 0,-7.000000*\dy)$) {\reftext{Ayal04}\cite{ayalew2004} (  -- , 3.265 , 0  )};
\draw (ayalew2004.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (yoshioka2018) at ($(ayalew2004.west |- 0,-8.000000*\dy)$) {\reftext{Yosh18}\cite{yoshioka2018} (  3.26 , -- , --  )};
\draw (yoshioka2018.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (choyke1969) at ($(patrick1965.west |- 0,-9.000000*\dy)$) {\reftext{Choy69}\cite{choyke1969} (  -- , 3.265 , 4  )};
\draw (choyke1969.west) -| ++(-\dy,\fy*\dy);
\coordinate (choyke1969C) at ($(choyke1969.west)+(\dxStart+\dy,0)$);
\node[ ref] (suzuki1977) at ($(choyke1969C |- 0,-10.000000*\dy)$) {\reftext{Suzu77}\cite{suzuki1977} (  -- , 3.265 , --  )};
\draw (suzuki1977.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (freitas1995) at ($(suzuki1977.west |- 0,-11.000000*\dy)$) {\reftext{Frei95}\cite{freitas1995} (  3.285 , 3.265 , 4  )};
\draw (freitas1995.west) -| ++(-\dy,\fy*\dy);
\coordinate (freitas1995C) at ($(freitas1995.west)+(\dxStart+\dy,0)$);
\node[ ref] (persson1999) at ($(freitas1995C |- 0,-12.000000*\dy)$) {\reftext{Pers99}\cite{persson1999} (  3.29 , -- , --  )};
\draw (persson1999.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (berger1996) at ($(freitas1995.west |- 0,-13.000000*\dy)$) {\reftext{Berg96}\cite{berger1996} (  -- , 3.265 , --  )};
\draw (berger1996.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (troffer1998) at ($(berger1996.west |- 0,-14.000000*\dy)$) {\reftext{Trof98}\cite{troffer1998} (  3.265 , -- , --  )};
\draw (troffer1998.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (egilsson2004) at ($(troffer1998.west |- 0,-15.000000*\dy)$) {\reftext{Egil04}\cite{egilsson2004} (  -- , 3.265 , 2  )};
\draw (egilsson2004.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (feng2004a) at ($(egilsson2004.west |- 0,-16.000000*\dy)$) {\reftext{Feng04a}\cite{feng2004a} (  -- , 3.26 , --  )};
\draw (feng2004a.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (hatakeyama2013) at ($(feng2004a.west |- 0,-17.000000*\dy)$) {\reftext{Hata13}\cite{hatakeyama2013} (  3.285 , 3.265 , 0  )};
\draw (hatakeyama2013.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (kimoto2014a) at ($(hatakeyama2013.west |- 0,-18.000000*\dy)$) {\reftext{Kimo14a}\cite{kimoto2014a} (  -- , 3.265 , 2  )};
\draw (kimoto2014a.west) -| ++(-\dy,\fy*\dy);
\coordinate (kimoto2014aC) at ($(kimoto2014a.west)+(\dxStart+\dy,0)$);
\node[ ref] (elahipanah2017) at ($(kimoto2014aC |- 0,-19.000000*\dy)$) {\reftext{Elah17}\cite{elahipanah2017} (  3.2 , -- , --  )};
\draw (elahipanah2017.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (rescher2018) at ($(elahipanah2017.west |- 0,-20.000000*\dy)$) {\reftext{Resc18}\cite{rescher2018} (  3.26 , -- , --  )};
\draw (rescher2018.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (kimoto2019) at ($(rescher2018.west |- 0,-21.000000*\dy)$) {\reftext{Kimo19}\cite{kimoto2019} (  3.292 , -- , 0  )};
\draw (kimoto2019.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (berens2021) at ($(kimoto2019.west |- 0,-22.000000*\dy)$) {\reftext{Bere21}\cite{berens2021} (  3.26 , -- , --  )};
\draw (berens2021.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (capan2022) at ($(berens2021.west |- 0,-23.000000*\dy)$) {\reftext{Capa22}\cite{capan2022} (  3.26 , -- , --  )};
\draw (capan2022.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (denapoli2022) at ($(capan2022.west |- 0,-24.000000*\dy)$) {\reftext{Dena22}\cite{denapoli2022} (  3.26 , -- , 0  )};
\draw (denapoli2022.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (tanaka2024) at ($(denapoli2022.west |- 0,-25.000000*\dy)$) {\reftext{Tana24}\cite{tanaka2024} (  3.26 , -- , 300  )};
\draw (tanaka2024.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (pankove2014) at ($(kimoto2014a.west |- 0,-26.000000*\dy)$) {\reftext{Pank14}\cite{pankove2014} (  3.28 , 3.265 , --  )};
\draw (pankove2014.west) -| ++(-\dy,\fy*\dy);
\coordinate (pankove2014C) at ($(pankove2014.west)+(\dxStart+\dy,0)$);
\node[ ref] (schadt1997) at ($(pankove2014C |- 0,-27.000000*\dy)$) {\reftext{Scha97}\cite{schadt1997} (  3.28 , -- , 0  )};
\draw (schadt1997.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (marshall1974) at ($(choyke1969.west |- 0,-28.000000*\dy)$) {\reftext{Mars74}\cite{marshall1974} (  -- , 3.265 , 4.2  )};
\draw (marshall1974.west) -| ++(-\dy,\fy*\dy);
\coordinate (marshall1974C) at ($(marshall1974.west)+(\dxStart+\dy,0)$);
\node[ ref] (hudgins2003) at ($(marshall1974C |- 0,-29.000000*\dy)$) {\reftext{Hudg03}\cite{hudgins2003} (  3.25 , -- , 300  )};
\draw (hudgins2003.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (haberstroh1994) at ($(marshall1974.west |- 0,-30.000000*\dy)$) {\reftext{Habe94}\cite{haberstroh1994} (  -- , 3.265 , --  )};
\draw (haberstroh1994.west) -| ++(-\dy,\fy*\dy);
\coordinate (haberstroh1994C) at ($(haberstroh1994.west)+(\dxStart+\dy,0)$);
\node[ ref] (casady1996) at ($(haberstroh1994C |- 0,-31.000000*\dy)$) {\reftext{Casa96}\cite{casady1996} (  3.26 , -- , --  )};
\draw (casady1996.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (huang1998) at ($(casady1996.west |- 0,-32.000000*\dy)$) {\reftext{Huan98}\cite{huang1998} (  3.26 , -- , --  )};
\draw (huang1998.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (bechstedt2004) at ($(huang1998.west |- 0,-33.000000*\dy)$) {\reftext{Bech04}\cite{bechstedt2004} (  3.27 , -- , --  )};
\draw (bechstedt2004.west) -| ++(-\dy,\fy*\dy);
\coordinate (bechstedt2004C) at ($(bechstedt2004.west)+(\dxStart+\dy,0)$);
\node[ ref] (nava2008) at ($(bechstedt2004C |- 0,-34.000000*\dy)$) {\reftext{Nava08}\cite{nava2008} (  3.27 , -- , 0  )};
\draw (nava2008.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (garcia2013) at ($(haberstroh1994.west |- 0,-35.000000*\dy)$) {\reftext{Garc13}\cite{garcia2013} (  3.265 , -- , 0  )};
\draw (garcia2013.west) -| ++(-\dy,\fy*\dy);
\coordinate (garcia2013C) at ($(garcia2013.west)+(\dxStart+\dy,0)$);
\node[ ref] (jimenez-ramos2024) at ($(garcia2013C |- 0,-36.000000*\dy)$) {\reftext{Jime24}\cite{jimenez-ramos2024} (  3.265 , -- , 0  )};
\draw (jimenez-ramos2024.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-38.000000*\dy) {\citeauthor{zanmarchi1964}};
\node[fund, ref] (zanmarchi1964) at (\xSepOne,-39.000000*\dy) {\reftext{Zanm64}\cite{zanmarchi1964} (  -- , 3.23 , 300  )};
\coordinate (zanmarchi1964C) at ($(zanmarchi1964.west)+(\dxStart+\dy,0)$);
\node[guess, ref] (ivanov2000) at ($(zanmarchi1964C |- 0,-40.000000*\dy)$) {\reftext{Ivan00}\cite{ivanov2000} (  3.23 , -- , 297  )};
\draw (ivanov2000.west) -| ++(-\dy,\fy*\dy);
\coordinate (ivanov2000C) at ($(ivanov2000.west)+(\dxStart+\dy,0)$);
\node[ ref] (arpatzanis2006) at ($(ivanov2000C |- 0,-41.000000*\dy)$) {\reftext{Arpa06}\cite{arpatzanis2006} (  3.23 , -- , --  )};
\draw (arpatzanis2006.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (levinshtein2001) at ($(ivanov2000.west |- 0,-42.000000*\dy)$) {\reftext{Levi01}\cite{levinshtein2001} (  3.23 , -- , 300  )};
\draw (levinshtein2001.west) -| ++(-\dy,\fy*\dy);
\coordinate (levinshtein2001C) at ($(levinshtein2001.west)+(\dxStart+\dy,0)$);
\node[ ref] (bhatnagar2005) at ($(levinshtein2001C |- 0,-43.000000*\dy)$) {\reftext{Bhat05}\cite{bhatnagar2005} (  3.23 , -- , 300  )};
\draw (bhatnagar2005.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (habib2011) at ($(bhatnagar2005.west |- 0,-44.000000*\dy)$) {\reftext{Habi11}\cite{habib2011} (  3.26 , -- , 0  )};
\draw (habib2011.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (zatko2021) at ($(habib2011.west |- 0,-45.000000*\dy)$) {\reftext{Zatk21}\cite{zatko2021} (  3.23 , -- , 300  )};
\draw (zatko2021.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (ioffe2023) at ($(zatko2021.west |- 0,-46.000000*\dy)$) {\reftext{Ioff23}\cite{ioffe2023} (  3.23 , 3.2 , 300  )};
\draw (ioffe2023.west) -| ++(-\dy,\fy*\dy);
\coordinate (ioffe2023C) at ($(ioffe2023.west)+(\dxStart+\dy,0)$);
\node[ ref] (banerjee2021) at ($(ioffe2023C |- 0,-47.000000*\dy)$) {\reftext{Bane21}\cite{banerjee2021} (  3.1934 , -- , 300  )};
\draw (banerjee2021.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (tamaki2008a) at ($(levinshtein2001.west |- 0,-48.000000*\dy)$) {\reftext{Tama08a}\cite{tamaki2008a} (  3.23 , -- , 300  )};
\draw (tamaki2008a.west) -| ++(-\dy,\fy*\dy);
\coordinate (tamaki2008aC) at ($(tamaki2008a.west)+(\dxStart+\dy,0)$);
\node[ ref] (menon2011) at ($(tamaki2008aC |- 0,-49.000000*\dy)$) {\reftext{Meno11}\cite{menon2011} (  -- , -- , --  )};
\draw (menon2011.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (song2012) at ($(menon2011.west |- 0,-50.000000*\dy)$) {\reftext{Song12}\cite{song2012} (  3.23 , -- , 300  )};
\draw (song2012.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-52.000000*\dy) {\citeauthor{dubrovskii1977}};
\node[calc, ref] (dubrovskii1977) at (\xSepOne,-53.000000*\dy) {\reftext{Dubr77}\cite{dubrovskii1977} (  3.2 , -- , 0  )};
\coordinate (dubrovskii1977C) at ($(dubrovskii1977.west)+(\dxStart+\dy,0)$);
\node[ ref] (madelung1991) at ($(dubrovskii1977C |- 0,-54.000000*\dy)$) {\reftext{Made91}\cite{madelung1991} (  -- , 3.2 , 300  )};
\draw (madelung1991.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (madelung1996) at ($(madelung1991.west |- 0,-55.000000*\dy)$) {\reftext{Made96}\cite{madelung1996} (  -- , 3.2 , 300  )};
\draw (madelung1996.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (trew2002) at ($(madelung1996.west |- 0,-56.000000*\dy)$) {\reftext{Trew02}\cite{trew2002} (  3.2 , -- , --  )};
\draw (trew2002.west) -| ++(-\dy,\fy*\dy);
\coordinate (trew2002C) at ($(trew2002.west)+(\dxStart+\dy,0)$);
\node[ ref] (neudeck2006) at ($(trew2002C |- 0,-57.000000*\dy)$) {\reftext{Neud06}\cite{neudeck2006} (  3.2 , -- , 300  )};
\draw (neudeck2006.west) -| ++(-\dy,\fy*\dy);
\coordinate (neudeck2006C) at ($(neudeck2006.west)+(\dxStart+\dy,0)$);
\node[ ref] (wijesundara2011a) at ($(neudeck2006C |- 0,-58.000000*\dy)$) {\reftext{Wije11a}\cite{wijesundara2011a} (  3.2 , -- , --  )};
\draw (wijesundara2011a.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (wijesundara2011b) at ($(wijesundara2011a.west |- 0,-59.000000*\dy)$) {\reftext{Wije11b}\cite{wijesundara2011b} (  3.26 , -- , --  )};
\draw (wijesundara2011b.west) -| ++(-\dy,\fy*\dy);
\coordinate (wijesundara2011bC) at ($(wijesundara2011b.west)+(\dxStart+\dy,0)$);
\node[ ref] (langpoklakpam2022) at ($(wijesundara2011bC |- 0,-60.000000*\dy)$) {\reftext{Lang22}\cite{langpoklakpam2022} (  3.26 , -- , --  )};
\draw (langpoklakpam2022.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (arvinte2017) at ($(wijesundara2011b.west |- 0,-61.000000*\dy)$) {\reftext{Arvi17}\cite{arvinte2017} (  3.2 , -- , 300  )};
\draw (arvinte2017.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (zetterling2002) at ($(trew2002.west |- 0,-62.000000*\dy)$) {\reftext{Zett02}\cite{zetterling2002} (  3.2 , -- , --  )};
\draw (zetterling2002.west) -| ++(-\dy,\fy*\dy);
\coordinate (zetterling2002C) at ($(zetterling2002.west)+(\dxStart+\dy,0)$);
\node[ ref] (ostling2011) at ($(zetterling2002C |- 0,-63.000000*\dy)$) {\reftext{Ostl11}\cite{ostling2011} (  3.2 , -- , --  )};
\draw (ostling2011.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (buttay2011) at ($(zetterling2002.west |- 0,-64.000000*\dy)$) {\reftext{Butt11}\cite{buttay2011} (  3.2 , -- , --  )};
\draw (buttay2011.west) -| ++(-\dy,\fy*\dy);
\coordinate (buttay2011C) at ($(buttay2011.west)+(\dxStart+\dy,0)$);
\node[ ref] (fujita2015) at ($(buttay2011C |- 0,-65.000000*\dy)$) {\reftext{Fuji15}\cite{fujita2015} (  3.2 , -- , --  )};
\draw (fujita2015.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (cressler2013) at ($(buttay2011.west |- 0,-66.000000*\dy)$) {\reftext{Cres13}\cite{cressler2013} (  3.2 , -- , --  )};
\draw (cressler2013.west) -| ++(-\dy,\fy*\dy);
\coordinate (cressler2013C) at ($(cressler2013.west)+(\dxStart+\dy,0)$);
\node[ ref] (hassan2018) at ($(cressler2013C |- 0,-67.000000*\dy)$) {\reftext{Hass18}\cite{hassan2018} (  3.2 , -- , --  )};
\draw (hassan2018.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (ioffe2023) at ($(cressler2013.west |- 0,-68.000000*\dy)$) {\reftext{Ioff23}\cite{ioffe2023} (  3.23 , 3.2 , 300  )};
\draw (ioffe2023.west) -| ++(-\dy,\fy*\dy);
\coordinate (ioffe2023C) at ($(ioffe2023.west)+(\dxStart+\dy,0)$);
\node[ ref] (banerjee2021) at ($(ioffe2023C |- 0,-69.000000*\dy)$) {\reftext{Bane21}\cite{banerjee2021} (  3.1934 , -- , 300  )};
\draw (banerjee2021.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,0.000000*\dy) {\citeauthor{backes1994}};
\node[calc, ref] (backes1994) at (\xSepOne + \xSepTwo,-1.000000*\dy) {\reftext{Back94}\cite{backes1994} (  3.28 , -- , 0  )};
\coordinate (backes1994C) at ($(backes1994.west)+(\dxStart+\dy,0)$);
\node[ ref] (vanhaeringen1997) at ($(backes1994C |- 0,-2.000000*\dy)$) {\reftext{Vanh97}\cite{vanhaeringen1997} (  3.28 , -- , 0  )};
\draw (vanhaeringen1997.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-4.000000*\dy) {\citeauthor{itoh1994}};
\node[ ref] (itoh1994) at (\xSepOne + \xSepTwo,-5.000000*\dy) {\reftext{Itoh94}\cite{itoh1994} (  3.26 , -- , --  )};
\coordinate (itoh1994C) at ($(itoh1994.west)+(\dxStart+\dy,0)$);
\node[ ref] (wang1999) at ($(itoh1994C |- 0,-6.000000*\dy)$) {\reftext{Wang99}\cite{wang1999} (  3.26 , -- , 300  )};
\draw (wang1999.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-8.000000*\dy) {\citeauthor{harris1995}};
\node[ ref] (harris1995) at (\xSepOne + \xSepTwo,-9.000000*\dy) {\reftext{Harr95}\cite{harris1995} (  -- , M , --  )};
\coordinate (harris1995C) at ($(harris1995.west)+(\dxStart+\dy,0)$);
\node[ ref] (reshanov2005) at ($(harris1995C |- 0,-10.000000*\dy)$) {\reftext{Resh05}\cite{reshanov2005} (  3.26 , -- , 300  )};
\draw (reshanov2005.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-12.000000*\dy) {\citeauthor{kordina1995}};
\node[fund, ref] (kordina1995) at (\xSepOne + \xSepTwo,-13.000000*\dy) {\reftext{Kord95}\cite{kordina1995} (  -- , 3.265 , 4.2  )};
\coordinate (kordina1995C) at ($(kordina1995.west)+(\dxStart+\dy,0)$);
\node[ ref] (egilsson1999) at ($(kordina1995C |- 0,-14.000000*\dy)$) {\reftext{Egil99}\cite{egilsson1999} (  -- , 3.266 , 4.2  )};
\draw (egilsson1999.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-16.000000*\dy) {\citeauthor{itoh1996}};
\node[fund, ref] (itoh1996) at (\xSepOne + \xSepTwo,-17.000000*\dy) {\reftext{Itoh96}\cite{itoh1996} (  -- , M , M  )};
\coordinate (itoh1996C) at ($(itoh1996.west)+(\dxStart+\dy,0)$);
\node[ ref] (galeckas1997) at ($(itoh1996C |- 0,-18.000000*\dy)$) {\reftext{Gale97}\cite{galeckas1997} (  3.275 , -- , --  )};
\draw (galeckas1997.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-20.000000*\dy) {\citeauthor{miller2000}};
\node[fund, ref] (miller2000) at (\xSepOne + \xSepTwo,-21.000000*\dy) {\reftext{Mill00}\cite{miller2000} (  3.378 , -- , 15  )};
\coordinate (miller2000C) at ($(miller2000.west)+(\dxStart+\dy,0)$);
\node[ ref] (scajev2009) at ($(miller2000C |- 0,-22.000000*\dy)$) {\reftext{Scaj09}\cite{scajev2009} (  3.3762 , -- , 0  )};
\draw (scajev2009.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-24.000000*\dy) {\citeauthor{galeckas2002}};
\node[ ref] (galeckas2002) at (\xSepOne + \xSepTwo,-25.000000*\dy) {\reftext{Gale02}\cite{galeckas2002} (  M , -- , M  )};
\coordinate (galeckas2002C) at ($(galeckas2002.west)+(\dxStart+\dy,0)$);
\node[ ref] (wolfowicz2017) at ($(galeckas2002C |- 0,-26.000000*\dy)$) {\reftext{Wolf17}\cite{wolfowicz2017} (  3.28 , -- , 5  )};
\draw (wolfowicz2017.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-28.000000*\dy) {\citeauthor{ivanov2002}};
\node[fund, ref] (ivanov2002) at (\xSepOne + \xSepTwo,-29.000000*\dy) {\reftext{Ivan02}\cite{ivanov2002} (  3.285 , -- , 2  )};
\coordinate (ivanov2002C) at ($(ivanov2002.west)+(\dxStart+\dy,0)$);
\node[ ref] (ivanov2003) at ($(ivanov2002C |- 0,-30.000000*\dy)$) {\reftext{Ivan03}\cite{ivanov2003} (  3.287 , 3.266 , 2  )};
\draw (ivanov2003.west) -| ++(-\dy,\fy*\dy);
\coordinate (ivanov2003C) at ($(ivanov2003.west)+(\dxStart+\dy,0)$);
\node[ ref] (ivanov2005) at ($(ivanov2003C |- 0,-31.000000*\dy)$) {\reftext{Ivan05}\cite{ivanov2005} (  3.287 , -- , --  )};
\draw (ivanov2005.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (janzen2008) at ($(ivanov2003.west |- 0,-32.000000*\dy)$) {\reftext{Janz08}\cite{janzen2008} (  3.287 , -- , 2  )};
\draw (janzen2008.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-34.000000*\dy) {\citeauthor{grivickas2007}};
\node[fund, ref] (grivickas2007) at (\xSepOne + \xSepTwo,-35.000000*\dy) {\reftext{Griv07}\cite{grivickas2007} (  -- , M , M  )};
\coordinate (grivickas2007C) at ($(grivickas2007.west)+(\dxStart+\dy,0)$);
\node[ ref] (levcenco2011) at ($(grivickas2007C |- 0,-36.000000*\dy)$) {\reftext{Levc11}\cite{levcenco2011} (  3.267 , -- , 0  )};
\draw (levcenco2011.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-38.000000*\dy) {\citeauthor{higashiwaki2014}};
\node[ ref] (higashiwaki2014) at (\xSepOne + \xSepTwo,-39.000000*\dy) {\reftext{Higa14}\cite{higashiwaki2014} (  3.3 , -- , --  )};
\coordinate (higashiwaki2014C) at ($(higashiwaki2014.west)+(\dxStart+\dy,0)$);
\node[ ref] (zheng2020) at ($(higashiwaki2014C |- 0,-40.000000*\dy)$) {\reftext{Zhen20}\cite{zheng2020} (  3.3 , -- , --  )};
\draw (zheng2020.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-42.000000*\dy) {\citeauthor{stefanakis2014}};
\node[fund, ref] (stefanakis2014) at (\xSepOne + \xSepTwo,-43.000000*\dy) {\reftext{Stef14}\cite{stefanakis2014} (  3.285 , -- , 0  )};
\coordinate (stefanakis2014C) at ($(stefanakis2014.west)+(\dxStart+\dy,0)$);
\node[ ref] (tripathi2019) at ($(stefanakis2014C |- 0,-44.000000*\dy)$) {\reftext{Trip19}\cite{tripathi2019} (  3.23 , -- , --  )};
\draw (tripathi2019.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (khanna2023) at ($(tripathi2019.west |- 0,-45.000000*\dy)$) {\reftext{Khan23}\cite{khanna2023} (  3.285 , -- , 0  )};
\draw (khanna2023.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-47.000000*\dy) {\citeauthor{choi2016}};
\node[ ref] (choi2016) at (\xSepOne + \xSepTwo,-48.000000*\dy) {\reftext{Choi16}\cite{choi2016} (  3.28 , -- , --  )};
\coordinate (choi2016C) at ($(choi2016.west)+(\dxStart+\dy,0)$);
\node[ ref] (naugarhiya2017) at ($(choi2016C |- 0,-49.000000*\dy)$) {\reftext{Naug17}\cite{naugarhiya2017} (  3.28 , -- , --  )};
\draw (naugarhiya2017.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-51.000000*\dy) {\citeauthor{arvanitopoulos2017}};
\node[ ref] (arvanitopoulos2017) at (\xSepOne + \xSepTwo,-52.000000*\dy) {\reftext{Arva17}\cite{arvanitopoulos2017} (  3.29 , -- , 0  )};
\coordinate (arvanitopoulos2017C) at ($(arvanitopoulos2017.west)+(\dxStart+\dy,0)$);
\node[ ref] (choudhary2021) at ($(arvanitopoulos2017C |- 0,-53.000000*\dy)$) {\reftext{Chou21}\cite{choudhary2021} (  3.26 , -- , 300  )};
\draw (choudhary2021.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-55.000000*\dy) {unknown};
\node[ ref] (unknown2325) at (\xSepOne + \xSepTwo,-56.000000*\dy) {unknown (  3.25 , -- , --  )};
\coordinate (unknown2325C) at ($(unknown2325.west)+(\dxStart+\dy,0)$);
\node[ ref] (agarwal1999) at ($(unknown2325C |- 0,-57.000000*\dy)$) {\reftext{Agar99}\cite{agarwal1999} (  3.25 , -- , --  )};
\draw (agarwal1999.west) -| ++(-\dy,\fy*\dy);
\coordinate (agarwal1999C) at ($(agarwal1999.west)+(\dxStart+\dy,0)$);
\node[ ref] (ozpineci2004) at ($(agarwal1999C |- 0,-58.000000*\dy)$) {\reftext{Ozpi04}\cite{ozpineci2004} (  3.26 , -- , --  )};
\draw (ozpineci2004.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (nallet1999) at ($(agarwal1999.west |- 0,-59.000000*\dy)$) {\reftext{Nall99}\cite{nallet1999} (  3.25 , -- , 0  )};
\draw (nallet1999.west) -| ++(-\dy,\fy*\dy);
\coordinate (nallet1999C) at ($(nallet1999.west)+(\dxStart+\dy,0)$);
\node[ ref] (cha2008) at ($(nallet1999C |- 0,-60.000000*\dy)$) {\reftext{Cha08}\cite{cha2008} (  3.25 , -- , 300  )};
\draw (cha2008.west) -| ++(-\dy,\fy*\dy);
\coordinate (cha2008C) at ($(cha2008.west)+(\dxStart+\dy,0)$);
\node[ ref] (chen2012) at ($(cha2008C |- 0,-61.000000*\dy)$) {\reftext{Chen12}\cite{chen2012} (  3.25 , -- , 300  )};
\draw (chen2012.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (pearton2018) at ($(nallet1999.west |- 0,-62.000000*\dy)$) {\reftext{Pear18}\cite{pearton2018} (  3.25 , -- , --  )};
\draw (pearton2018.west) -| ++(-\dy,\fy*\dy);
\coordinate (pearton2018C) at ($(pearton2018.west)+(\dxStart+\dy,0)$);
\node[ ref] (soler2019) at ($(pearton2018C |- 0,-63.000000*\dy)$) {\reftext{Sole19}\cite{soler2019} (  3.2 , -- , --  )};
\draw (soler2019.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (kim2024) at ($(soler2019.west |- 0,-64.000000*\dy)$) {\reftext{Kim24}\cite{kim2024} (  3.25 , -- , --  )};
\draw (kim2024.west) -| ++(-\dy,\fy*\dy);


==> data/bandgap_ref_chain_doping.tex <==
\node[desc] at (0,0.000000*\dy) {Lindefelt ( $\anc$ / $\anv$ ) [ $\bnc$ / $\bnv$ ] \{ $\apc$ / $\apv$ \} $\mid$ $\bpc$ / $\bpv$ $\mid$ ( $\cpv$ )};
\node[author] at (0,-1.500000*\dy) {\citeauthor{lindefelt1998}};
\node[fund, ref] (lindefelt1998) at (0,-2.500000*\dy) {\reftext{Lind98}\cite{lindefelt1998} (  \num{-0.015} / \num{0.019} )  [ \num{-0.00293} / \num{0.00874} ] \{ \num{-0.0157} / \num{0.013} \} $\mid$ \num{-0.000387} / \num{0.00115} $\mid$ ( -- )};
\coordinate (lindefelt1998C) at ($(lindefelt1998.west)+(\dxStart+\dy,0)$);
\node[ ref] (levinshtein2001) at ($(lindefelt1998C |- 0,-3.500000*\dy)$) {\reftext{Levi01}\cite{levinshtein2001} (  \num{-0.015} / \num{1.9e-2} )  [ \num{-2.93e-3} / \num{8.74e-3} ] \{ \num{-1.57e-2} / \num{1.3e-2} \} $\mid$ \num{-3.87e-4} / \num{1.15e-3} $\mid$ ( -- )};
\draw (levinshtein2001.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (wellmann2001) at ($(levinshtein2001.west |- 0,-4.500000*\dy)$) {\reftext{Well01}\cite{wellmann2001} (  -- / -- )  [ -- / -- ] \{ -- / -- \} $\mid$ -- / -- $\mid$ ( -- )};
\draw (wellmann2001.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (cha2008) at ($(wellmann2001.west |- 0,-5.500000*\dy)$) {\reftext{Cha08}\cite{cha2008} (  \num{-15e-3} / \num{19e-3} )  [ \num{-2.93e-3} / \num{8.74e-3} ] \{ -- / -- \} $\mid$ -- / -- $\mid$ ( -- )};
\draw (cha2008.west) -| ++(-\dy,\fy*\dy);
\coordinate (cha2008C) at ($(cha2008.west)+(\dxStart+\dy,0)$);
\node[ ref] (chen2012) at ($(cha2008C |- 0,-6.500000*\dy)$) {\reftext{Chen12}\cite{chen2012} (  \num{-15e-3} / \num{19e-3} )  [ \num{-2.93e-3} / \num{8.74e-3} ] \{ -- / -- \} $\mid$ -- / -- $\mid$ ( -- )};
\draw (chen2012.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (albanese2010) at ($(cha2008.west |- 0,-7.500000*\dy)$) {\reftext{Alba10}\cite{albanese2010} (  \num{-0.015} / \num{0.019} )  [ \num{0.017} ] \{ \num{-0.0157} / \num{0.013} \} $\mid$ \num{0.0154} $\mid$ ( -- )};
\draw (albanese2010.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (zhang2010) at ($(albanese2010.west |- 0,-8.500000*\dy)$) {\reftext{Zhan10}\cite{zhang2010} (  \num{-0.015} / \num{0.019} )  [ \num{-0.00293} / \num{0.00874} ] \{ -- / -- \} $\mid$ -- / -- $\mid$ ( -- )};
\draw (zhang2010.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (bellone2011) at ($(zhang2010.west |- 0,-9.500000*\dy)$) {\reftext{Bell11}\cite{bellone2011} (  \num{-0.015} / \num{0.019} )  [ \num{0.0117} ] \{ \num{-0.0157} / \num{0.013} \} $\mid$ \num{0.00154} $\mid$ ( -- )};
\draw (bellone2011.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (habib2011) at ($(bellone2011.west |- 0,-10.500000*\dy)$) {\reftext{Habi11}\cite{habib2011} (  \num{-1.5e-2} / \num{1.9e-2} )  [ \num{-2.93e-3} / \num{8.74e-3} ] \{ \num{-1.57e-2} / \num{1.3e-2} \} $\mid$ \num{-3.87e-4} / \num{1.15e-3} $\mid$ ( -- )};
\draw (habib2011.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (buono2012) at ($(habib2011.west |- 0,-11.500000*\dy)$) {\reftext{Buon12}\cite{buono2012} (  \num{-0.015} / \num{-0.019} )  [ \num{-0.00293} / \num{-0.00874} ] \{ -- / -- \} $\mid$ -- / -- $\mid$ ( -- )};
\draw (buono2012.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (pezzimenti2013) at ($(buono2012.west |- 0,-12.500000*\dy)$) {\reftext{Pezz13}\cite{pezzimenti2013} (  \num{-0.015} / \num{0.019} )  [ \num{0.0117} ] \{ \num{-0.0157} / \num{0.013} \} $\mid$ \num{1.54e-3} $\mid$ ( -- )};
\draw (pezzimenti2013.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (stefanakis2014) at ($(pezzimenti2013.west |- 0,-13.500000*\dy)$) {\reftext{Stef14}\cite{stefanakis2014} (  \num{-0.015} / \num{0.019} )  [ \num{-0.00293} / \num{0.00874} ] \{ \num{-0.0157} / \num{0.013} \} $\mid$ \num{-0.000387} / \num{0.00115} $\mid$ ( -- )};
\draw (stefanakis2014.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (megherbi2018a) at ($(stefanakis2014.west |- 0,-14.500000*\dy)$) {\reftext{Megh18a}\cite{megherbi2018a} (  \num{-1.5e-2} / \num{1.9e-2} )  [ \num{1.17e2} ] \{ \num{-1.57e-2} / \num{1.3e-2} \} $\mid$ \num{1.54e-3} $\mid$ ( -- )};
\draw (megherbi2018a.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (zeghdar2019) at ($(megherbi2018a.west |- 0,-15.500000*\dy)$) {\reftext{Zegh19}\cite{zeghdar2019} (  \num{-1.5e-2} / \num{1.9e-2} )  [ \num{1.17e-2} ] \{ \num{-1.57e-2} / \num{1.3e-2} \} $\mid$ \num{1.54e-3} $\mid$ ( -- )};
\draw (zeghdar2019.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (zeghdar2020) at ($(zeghdar2019.west |- 0,-16.500000*\dy)$) {\reftext{Zegh20}\cite{zeghdar2020} (  \num{-1.5e-2} / \num{1.9e-2} )  [ \num{1.17e-2} ] \{ \num{-1.57e-2} / \num{1.3e-2} \} $\mid$ \num{1.54e-3} $\mid$ ( -- )};
\draw (zeghdar2020.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (ioffe2023) at ($(zeghdar2020.west |- 0,-17.500000*\dy)$) {\reftext{Ioff23}\cite{ioffe2023} (  \num{-0.015} / \num{-0.019} )  [ \num{-0.00293} / \num{-0.00874} ] \{ \num{-0.0157} / \num{-0.013} \} $\mid$ \num{-0.000387} / \num{-0.00115} $\mid$ ( -- )};
\draw (ioffe2023.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (maximenko2023) at ($(ioffe2023.west |- 0,-18.500000*\dy)$) {\reftext{Maxi23}\cite{maximenko2023} (  \num{-1.5e-2} / \num{1.9e-2} )  [ \num{-2.93e-3} / \num{8.74e-3} ] \{ \num{-1.57e-2} / \num{1.3e-2} \} $\mid$ \num{-3.87e-4} / \num{1.15e-3} $\mid$ ( -- )};
\draw (maximenko2023.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-20.500000*\dy) {\citeauthor{persson1999}};
\node[fund, ref] (persson1999) at (0,-21.500000*\dy) {\reftext{Pers99}\cite{persson1999} (  \num{-0.01791} / \num{0.02823} )  [ \num{-0.0022} / \num{0.00624} ] \{ \num{-0.01615} / \num{-0.03507} \} $\mid$ \num{-0.00107} / \num{0.00674} $\mid$ ( \num{0.05696} )};
\coordinate (persson1999C) at ($(persson1999.west)+(\dxStart+\dy,0)$);
\node[ ref] (nipoti2016) at ($(persson1999C |- 0,-22.500000*\dy)$) {\reftext{Nipo16}\cite{nipoti2016} (  -- / -- )  [ -- / -- ] \{ -- / -- \} $\mid$ -- / -- $\mid$ ( -- )};
\draw (nipoti2016.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (lophitis2018) at ($(nipoti2016.west |- 0,-23.500000*\dy)$) {\reftext{Loph18}\cite{lophitis2018} (  \num{-0.01791} / \num{0.02823} )  [ \num{-0.0022} / \num{0.00624} ] \{ \num{-0.07311} / \num{0.03507} \} $\mid$ \num{-0.00107} / \num{0.00674} $\mid$ ( -- )};
\draw (lophitis2018.west) -| ++(-\dy,\fy*\dy);
\node[desc] at (0,-26.500000*\dy) {Slotboom ( $C_\mathrm{n}$ / $N_\mathrm{n}$ ) ( $C_\mathrm{p}$ / $N_\mathrm{p}$ ) ( $G$ )};
\node[author] at (0,-28.000000*\dy) {\citeauthor{ladesmartin2000}};
\node[fund, ref] (ladesmartin2000) at (0,-29.000000*\dy) {\reftext{Lade00}\cite{ladesmartin2000} (  \num{0.02} / \num{1.00000000000000E+17} ) ( \num{0.009} / \num{1.00000000000000E+17} ) ( \num{0.5} )};
\coordinate (ladesmartin2000C) at ($(ladesmartin2000.west)+(\dxStart+\dy,0)$);
\node[ ref] (ayalew2004) at ($(ladesmartin2000C |- 0,-30.000000*\dy)$) {\reftext{Ayal04}\cite{ayalew2004} (  \num{0.02} / \num{1.00000000000000E+17} ) ( \num{0.009} / \num{1.00000000000000E+17} ) ( \num{0.5} )};
\draw (ayalew2004.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (lechner2021) at ($(ayalew2004.west |- 0,-31.000000*\dy)$) {\reftext{Lech21}\cite{lechner2021} (  \num{0.02} / \num{1.00000000000000E+17} ) ( -- / -- ) ( \num{0.5} )};
\draw (lechner2021.west) -| ++(-\dy,\fy*\dy);


==> data/bandgap_ref_chain_temp.tex <==
\node[desc] at (0,0.000000*\dy) {Varshni ($\eg$, $\egx$, $\alpha$, $\tg$, $\beta$)};
\node[author] at (0,-1.500000*\dy) {\citeauthor{choyke1957}};
\node[no4H, ref] (choyke1957) at (0,-2.500000*\dy) {\reftext{Choy57}\cite{choyke1957} (  -- , -- , \num{3.3e-4} , -- , --  )};
\coordinate (choyke1957C) at ($(choyke1957.west)+(\dxStart+\dy,0)$);
\node[no4H, ref] (ruff1994) at ($(choyke1957C |- 0,-3.500000*\dy)$) {\reftext{Ruff94}\cite{ruff1994} (  \num{3} , -- , \num{3.3e-4} , \num{300} , \num{0}  )};
\draw (ruff1994.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (wright1998) at ($(ruff1994.west |- 0,-4.500000*\dy)$) {\reftext{Wrig98}\cite{wright1998} (  \num{3.26} , -- , \num{3.3e-4} , \num{300} , \num{0}  )};
\draw (wright1998.west) -| ++(-\dy,\fy*\dy);
\coordinate (wright1998C) at ($(wright1998.west)+(\dxStart+\dy,0)$);
\node[ ref] (mcnutt2004) at ($(wright1998C |- 0,-5.500000*\dy)$) {\reftext{Mcnu04}\cite{mcnutt2004} (  \num{3.26} , -- , \num{3.3e-3} , \num{300} , \num{0}  )};
\draw (mcnutt2004.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (nallet1999) at ($(wright1998.west |- 0,-6.500000*\dy)$) {\reftext{Nall99}\cite{nallet1999} (  \num{3.25} , -- , \num{3.3e-4} , \num{0} , \num{0}  )};
\draw (nallet1999.west) -| ++(-\dy,\fy*\dy);
\coordinate (nallet1999C) at ($(nallet1999.west)+(\dxStart+\dy,0)$);
\node[ ref] (cha2008) at ($(nallet1999C |- 0,-7.500000*\dy)$) {\reftext{Cha08}\cite{cha2008} (  \num{3.25} , -- , \num{3.3e-4} , \num{300} , \num{0}  )};
\draw (cha2008.west) -| ++(-\dy,\fy*\dy);
\coordinate (cha2008C) at ($(cha2008.west)+(\dxStart+\dy,0)$);
\node[ ref] (chen2012) at ($(cha2008C |- 0,-8.500000*\dy)$) {\reftext{Chen12}\cite{chen2012} (  \num{3.25} , -- , \num{3.3e-4} , \num{300} , \num{0}  )};
\draw (chen2012.west) -| ++(-\dy,\fy*\dy);
\coordinate (chen2012C) at ($(chen2012.west)+(\dxStart+\dy,0)$);
\node[ ref] (megherbi2015) at ($(chen2012C |- 0,-9.500000*\dy)$) {\reftext{Megh15}\cite{megherbi2015} (  -- , -- , \num{3.3e-4} , \num{0} , \num{0}  )};
\draw (megherbi2015.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (wang1999) at ($(nallet1999.west |- 0,-10.500000*\dy)$) {\reftext{Wang99}\cite{wang1999} (  \num{3.26} , -- , \num{3.3e-4} , \num{300} , \num{0}  )};
\draw (wang1999.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (lee2002) at ($(wang1999.west |- 0,-11.500000*\dy)$) {\reftext{Lee02}\cite{lee2002} (  \num{3.26} , -- , \num{3.3e-4} , \num{300} , \num{0}  )};
\draw (lee2002.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (li2003) at ($(lee2002.west |- 0,-12.500000*\dy)$) {\reftext{Li03}\cite{li2003} (  \num{3.359} , -- , \num{3.3e-4} , \num{0} , \num{0}  )};
\draw (li2003.west) -| ++(-\dy,\fy*\dy);
\coordinate (li2003C) at ($(li2003.west)+(\dxStart+\dy,0)$);
\node[ ref] (pezzimenti2013) at ($(li2003C |- 0,-13.500000*\dy)$) {\reftext{Pezz13}\cite{pezzimenti2013} (  \num{3.2} , -- , \num{3.3e-4} , \num{300} , \num{0}  )};
\draw (pezzimenti2013.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (megherbi2018a) at ($(pezzimenti2013.west |- 0,-14.500000*\dy)$) {\reftext{Megh18a}\cite{megherbi2018a} (  \num{3.2} , -- , \num{3.3e-4} , \num{300} , \num{0}  )};
\draw (megherbi2018a.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (zeghdar2019) at ($(megherbi2018a.west |- 0,-15.500000*\dy)$) {\reftext{Zegh19}\cite{zeghdar2019} (  \num{3.26} , -- , \num{3.3e-4} , \num{300} , \num{0}  )};
\draw (zeghdar2019.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (zeghdar2020) at ($(zeghdar2019.west |- 0,-16.500000*\dy)$) {\reftext{Zegh20}\cite{zeghdar2020} (  \num{3.26} , -- , \num{3.3e-4} , \num{300} , \num{0}  )};
\draw (zeghdar2020.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (zhao2003) at ($(li2003.west |- 0,-17.500000*\dy)$) {\reftext{Zhao03}\cite{zhao2003} (  \num{3.359} , -- , \num{3.3e-4} , \num{0} , \num{0}  )};
\draw (zhao2003.west) -| ++(-\dy,\fy*\dy);
\coordinate (zhao2003C) at ($(zhao2003.west)+(\dxStart+\dy,0)$);
\node[ ref] (das2015) at ($(zhao2003C |- 0,-18.500000*\dy)$) {\reftext{Das15}\cite{das2015} (  \num{3.359} , -- , \num{3.3e-4} , \num{0} , \num{0}  )};
\draw (das2015.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (albanese2010) at ($(zhao2003.west |- 0,-19.500000*\dy)$) {\reftext{Alba10}\cite{albanese2010} (  \num{3.2} , -- , \num{3.3e-4} , \num{300} , \num{0}  )};
\draw (albanese2010.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (raynaud2010) at ($(albanese2010.west |- 0,-20.500000*\dy)$) {\reftext{Rayn10}\cite{raynaud2010} (  \num{3.263} , -- , \num{3.3e-4} , \num{0} , \num{0}  )};
\draw (raynaud2010.west) -| ++(-\dy,\fy*\dy);
\coordinate (raynaud2010C) at ($(raynaud2010.west)+(\dxStart+\dy,0)$);
\node[ ref] (maximenko2023) at ($(raynaud2010C |- 0,-21.500000*\dy)$) {\reftext{Maxi23}\cite{maximenko2023} (  \num{3.23} , -- , \num{3.3e-4} , \num{300} , \num{0}  )};
\draw (maximenko2023.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (bellone2011) at ($(raynaud2010.west |- 0,-22.500000*\dy)$) {\reftext{Bell11}\cite{bellone2011} (  \num{3.2} , -- , \num{3.3e-4} , \num{300} , \num{0}  )};
\draw (bellone2011.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (rao2022) at ($(bellone2011.west |- 0,-23.500000*\dy)$) {\reftext{Rao22}\cite{rao2022} (  \num{3.26} , -- , \num{3.3e-4} , \num{0} , \num{0}  )};
\draw (rao2022.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (dibenedetto2024) at ($(rao2022.west |- 0,-24.500000*\dy)$) {\reftext{Dibe24}\cite{dibenedetto2024} (  \num{3.26} , -- , \num{3.3e-4} , \num{300} , --  )};
\draw (dibenedetto2024.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-26.500000*\dy) {\citeauthor{yoshida1995}};
\node[ ref] (yoshida1995) at (0,-27.500000*\dy) {\reftext{Yosh95}\cite{yoshida1995} (  -- , \num{3.263} , -- , -- , --  )};
\coordinate (yoshida1995C) at ($(yoshida1995.west)+(\dxStart+\dy,0)$);
\node[ ref] (casady1996) at ($(yoshida1995C |- 0,-28.500000*\dy)$) {\reftext{Casa96}\cite{casady1996} (  \num{3.26} , -- , -- , -- , --  )};
\draw (casady1996.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (biondo2012) at ($(casady1996.west |- 0,-29.500000*\dy)$) {\reftext{Bion12}\cite{biondo2012} (  \num{3.26} , -- , \num{3.3e-4} , \num{0} , --  )};
\draw (biondo2012.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-31.500000*\dy) {\citeauthor{ladesmartin2000}};
\node[fund, ref] (ladesmartin2000) at (0,-32.500000*\dy) {\reftext{Lade00}\cite{ladesmartin2000} (  -- , M , M , M , M  )};
\coordinate (ladesmartin2000C) at ($(ladesmartin2000.west)+(\dxStart+\dy,0)$);
\node[guess, ref] (ayalew2004) at ($(ladesmartin2000C |- 0,-33.500000*\dy)$) {\reftext{Ayal04}\cite{ayalew2004} (  -- , \num{3.265} , \num{3.3e-2} , \num{0} , \num{100000}  )};
\draw (ayalew2004.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (arvanitopoulos2017) at ($(ayalew2004.west |- 0,-34.500000*\dy)$) {\reftext{Arva17}\cite{arvanitopoulos2017} (  \num{3.29} , -- , \num{3.3e-2} , \num{0} , \num{100000}  )};
\draw (arvanitopoulos2017.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (lophitis2018) at ($(arvanitopoulos2017.west |- 0,-35.500000*\dy)$) {\reftext{Loph18}\cite{lophitis2018} (  \num{3.265} , -- , \num{3.3e-2} , \num{0} , \num{100000}  )};
\draw (lophitis2018.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,0.000000*\dy) {\citeauthor{levinshtein2001}};
\node[fund, ref] (levinshtein2001) at (\xSepOne,-1.000000*\dy) {\reftext{Levi01}\cite{levinshtein2001} (  \num{3.23} , -- , \num{6.5e-4} , \num{300} , \num{1300}  )};
\coordinate (levinshtein2001C) at ($(levinshtein2001.west)+(\dxStart+\dy,0)$);
\node[ ref] (bhatnagar2005) at ($(levinshtein2001C |- 0,-2.000000*\dy)$) {\reftext{Bhat05}\cite{bhatnagar2005} (  \num{3.23} , -- , \num{6.5e-4} , \num{300} , \num{1300}  )};
\draw (bhatnagar2005.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (habib2011) at ($(bhatnagar2005.west |- 0,-3.000000*\dy)$) {\reftext{Habi11}\cite{habib2011} (  \num{3.26} , -- , \num{6.5e-4} , \num{0} , \num{1300}  )};
\draw (habib2011.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (lutz2011) at ($(habib2011.west |- 0,-4.000000*\dy)$) {\reftext{Lutz11}\cite{lutz2011} (  \num{3.263} , -- , \num{6.5e4} , \num{0} , \num{1300}  )};
\draw (lutz2011.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (garcia2013) at ($(lutz2011.west |- 0,-5.000000*\dy)$) {\reftext{Garc13}\cite{garcia2013} (  \num{3.265} , -- , \num{6.5e-4} , \num{0} , \num{1300}  )};
\draw (garcia2013.west) -| ++(-\dy,\fy*\dy);
\coordinate (garcia2013C) at ($(garcia2013.west)+(\dxStart+\dy,0)$);
\node[ ref] (jimenez-ramos2024) at ($(garcia2013C |- 0,-6.000000*\dy)$) {\reftext{Jime24}\cite{jimenez-ramos2024} (  \num{3.265} , -- , \num{6.5e-4} , \num{0} , \num{1300}  )};
\draw (jimenez-ramos2024.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (johannesson2016) at ($(garcia2013.west |- 0,-7.000000*\dy)$) {\reftext{Joha16}\cite{johannesson2016} (  \num{3.263} , -- , \num{6.5e-4} , \num{0} , \num{1300}  )};
\draw (johannesson2016.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (lutz2018) at ($(johannesson2016.west |- 0,-8.000000*\dy)$) {\reftext{Lutz18}\cite{lutz2018} (  \num{3.263} , -- , \num{6.5e4} , \num{0} , \num{1300}  )};
\draw (lutz2018.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (liu2021) at ($(lutz2018.west |- 0,-9.000000*\dy)$) {\reftext{Liu21}\cite{liu2021} (  \num{3.25} , -- , \num{6.5e-4} , \num{0} , \num{1300}  )};
\draw (liu2021.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (ioffe2023) at ($(liu2021.west |- 0,-10.000000*\dy)$) {\reftext{Ioff23}\cite{ioffe2023} (  \num{3.23} , \num{3.2} , \num{6.5e-4} , \num{300} , \num{1300}  )};
\draw (ioffe2023.west) -| ++(-\dy,\fy*\dy);
\coordinate (ioffe2023C) at ($(ioffe2023.west)+(\dxStart+\dy,0)$);
\node[ ref] (uhnevionak2015) at ($(ioffe2023C |- 0,-11.000000*\dy)$) {\reftext{Uhne15}\cite{uhnevionak2015} (  \num{3.26} , -- , \num{6.5e-4} , \num{0} , \num{1300}  )};
\draw (uhnevionak2015.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-13.000000*\dy) {\citeauthor{balachandran2005}};
\node[fund, ref] (balachandran2005) at (\xSepOne,-14.000000*\dy) {\reftext{Bala05}\cite{balachandran2005} (  \num{3.26} , -- , \num{4.15e-4} , \num{300} , \num{-131}  )};
\coordinate (balachandran2005C) at ($(balachandran2005.west)+(\dxStart+\dy,0)$);
\node[ ref] (nawaz2010) at ($(balachandran2005C |- 0,-15.000000*\dy)$) {\reftext{Nawa10}\cite{nawaz2010} (  \num{3.26} , -- , \num{4.15e-4} , \num{300} , \num{-131}  )};
\draw (nawaz2010.west) -| ++(-\dy,\fy*\dy);
\coordinate (nawaz2010C) at ($(nawaz2010.west)+(\dxStart+\dy,0)$);
\node[ ref] (usman2014) at ($(nawaz2010C |- 0,-16.000000*\dy)$) {\reftext{Usma14}\cite{usman2014} (  \num{3.24} , -- , \num{4.15e-4} , \num{300} , \num{-131}  )};
\draw (usman2014.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-18.000000*\dy) {\citeauthor{grivickas2007}};
\node[ ref] (grivickas2007) at (\xSepOne,-19.000000*\dy) {\reftext{Griv07}\cite{grivickas2007} (  -- , M , -- , -- , --  )};
\coordinate (grivickas2007C) at ($(grivickas2007.west)+(\dxStart+\dy,0)$);
\node[ ref] (levcenco2011) at ($(grivickas2007C |- 0,-20.000000*\dy)$) {\reftext{Levc11}\cite{levcenco2011} (  \num{3.267} , -- , \num{3.2e-4} , \num{0} , \num{565}  )};
\draw (levcenco2011.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-22.000000*\dy) {\citeauthor{tamaki2008a}};
\node[fund, ref] (tamaki2008a) at (\xSepOne,-23.000000*\dy) {\reftext{Tama08a}\cite{tamaki2008a} (  \num{3.23} , -- , \num{7.036e-4} , \num{300} , \num{1509}  )};
\coordinate (tamaki2008aC) at ($(tamaki2008a.west)+(\dxStart+\dy,0)$);
\node[guess, ref] (song2012) at ($(tamaki2008aC |- 0,-24.000000*\dy)$) {\reftext{Song12}\cite{song2012} (  \num{3.23} , -- , \num{7.036e-4} , \num{300} , \num{1509}  )};
\draw (song2012.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-26.000000*\dy) {\citeauthor{kimoto2014a}};
\node[fund, ref] (kimoto2014a) at (\xSepOne,-27.000000*\dy) {\reftext{Kimo14a}\cite{kimoto2014a} (  -- , \num{3.265} , \num{8.2e-4} , \num{0} , \num{1800}  )};
\coordinate (kimoto2014aC) at ($(kimoto2014a.west)+(\dxStart+\dy,0)$);
\node[ ref] (kimoto2019) at ($(kimoto2014aC |- 0,-28.000000*\dy)$) {\reftext{Kimo19}\cite{kimoto2019} (  \num{3.292} , -- , \num{8.2e-4} , \num{0} , \num{1800}  )};
\draw (kimoto2019.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (denapoli2022) at ($(kimoto2019.west |- 0,-29.000000*\dy)$) {\reftext{Dena22}\cite{denapoli2022} (  \num{3.26} , -- , \num{8.2e-4} , \num{0} , \num{1300}  )};
\draw (denapoli2022.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (tanaka2024) at ($(denapoli2022.west |- 0,-30.000000*\dy)$) {\reftext{Tana24}\cite{tanaka2024} (  \num{3.26} , -- , \num{8.2e-4} , \num{300} , \num{1800}  )};
\draw (tanaka2024.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-32.000000*\dy) {\citeauthor{stefanakis2014}};
\node[fund, ref] (stefanakis2014) at (\xSepOne,-33.000000*\dy) {\reftext{Stef14}\cite{stefanakis2014} (  \num{3.285} , -- , \num{3.3e-4} , \num{0} , \num{240}  )};
\coordinate (stefanakis2014C) at ($(stefanakis2014.west)+(\dxStart+\dy,0)$);
\node[ ref] (khanna2023) at ($(stefanakis2014C |- 0,-34.000000*\dy)$) {\reftext{Khan23}\cite{khanna2023} (  \num{3.285} , -- , \num{3.3e-4} , \num{0} , \num{240}  )};
\draw (khanna2023.west) -| ++(-\dy,\fy*\dy);
\node[desc] at (\xSepOne,-37.000000*\dy) {Passler ($\egx$, $\varepsilon$, $\Theta_\mathrm{p}$, $p$)};
\node[author] at (\xSepOne,-38.500000*\dy) {\citeauthor{grivickas2007}};
\node[fund, ref] (grivickas2007) at (\xSepOne,-39.500000*\dy) {\reftext{Griv07}\cite{grivickas2007} (  3.267 , 3e-4 , 450 , 2.9  )};
\coordinate (grivickas2007C) at ($(grivickas2007.west)+(\dxStart+\dy,0)$);
\node[ ref] (stefanakis2014) at ($(grivickas2007C |- 0,-40.500000*\dy)$) {\reftext{Stef14}\cite{stefanakis2014} (  3.27 , 3e-4 , 450 , 2.9  )};
\draw (stefanakis2014.west) -| ++(-\dy,\fy*\dy);


==> data/bandgap_values.tex <==


\node[symbol] (subEg) at (0,0) {$\eg$};
\coordinate (subEg0) at (subEg.north);
\node[ref, lwsubEg] (subEg1) at (subEg0.north west) {\tikz \node[paper, calc] {\reftext{Park94}\cite{park1994}};};
\node[value, scale=1.100000] (subEgvalue1) at (subEg1.west) {\num{2.14}};
\node[ref, lwsubEg] (subEg2) at (subEg1.north west) {\tikz \node[paper, calc] {\reftext{Kaec96}\cite{kaeckell1996}};};
\node[value, scale=1.100000] (subEgvalue2) at (subEg2.west) {\num{2.18}};
\node[ref, lwsubEg] (subEg3) at (subEg2.north west) {\tikz \node[paper, calc] {\reftext{Dong04}\cite{dong2004}};};
\node[value, scale=1.100000] (subEgvalue3) at (subEg3.west) {\num{2.194}};
\node[ref, lwsubEg] (subEg4) at (subEg3.north west) {\tikz \node[paper, calc] {\reftext{Chin06}\cite{ching2006}};};
\node[value, scale=1.100000] (subEgvalue4) at (subEg4.west) {\num{2.433}};
\node[ref, lwsubEg] (subEg5) at (subEg4.north west) {\tikz \node[paper, calc] {\reftext{Nuru15}\cite{nuruzzaman2015}};};
\node[value, scale=1.100000] (subEgvalue5) at (subEg5.west) {\num{2.45}};
\node[ref, lwsubEg] (subEg6) at (subEg5.north west) {\tikz \node[paper, calc] {\reftext{Jung70}\cite{junginger1970}};};
\node[value, scale=1.100000] (subEgvalue6) at (subEg6.west) {\num{2.8}};
\node[ref, lwsubEg] (subEg7) at (subEg6.north west) {\tikz \node[paper, calc] {\reftext{Gavr90}\cite{gavrilenko1990}};};
\node[value, scale=1.100000] (subEgvalue7) at (subEg7.west) {\num{2.89}};
\node[ref, lwsubEg] (subEg8) at (subEg7.north west) {\tikz \node[paper, calc] {\reftext{Pers97}\cite{persson1997}};};
\node[value, scale=1.100000] (subEgvalue8) at (subEg8.west) {\num{2.9}};
\node[ref, lwsubEg] (subEg9) at (subEg8.north west) {\tikz \node[paper, calc] {\reftext{Bell00}\cite{bellotti2000}};};
\node[value, scale=1.100000] (subEgvalue9) at (subEg9.west) {\num{3.05}};
\node[ref, lwsubEg] (subEg10) at (subEg9.north west) {\tikz \node[paper, varshni] {\reftext{Ruff94}\cite{ruff1994}};};
\node[value, scale=1.100000] (subEgvalue10) at (subEg10.west) {\num{3.099}};
\node[ref, lwsubEg] (subEg11) at (subEg10.north west) {\tikz \node[paper, calc] {\reftext{Zhao00a}\cite{zhao2000a}};};
\node[value, scale=1.100000] (subEgvalue11) at (subEg11.west) {\num{3.11}};
\node[ref, lwsubEg] (subEg12) at (subEg11.north west) {\tikz \node[paper, calc] {\reftext{Yama18}\cite{yamaguchi2018}};};
\node[value, scale=1.100000] (subEgvalue12) at (subEg12.west) {\num{3.12}};
\node[ref, lwsubEg] (subEg13) at (subEg12.north west) {\tikz \node[paper, calc] {\reftext{Kuro19}\cite{kuroiwa2019}};};
\node[value, scale=1.100000] (subEgvalue13) at (subEg13.west) {\num{3.15}};
\node[ref, lwsubEg] (subEg14) at (subEg13.north west) {\tikz \node[paper, calc] {\reftext{Torr22}\cite{torres2022}}; \tikz \node[paper, calc] {\reftext{Lu21}\cite{lu2021}};};
\node[value, scale=1.200000] (subEgvalue14) at (subEg14.west) {\num{3.17}};
\node[ref, lwsubEg] (subEg15) at (subEg14.north west) {\tikz \node[paper, calc] {\reftext{Huan22b}\cite{huang2022b}};};
\node[value, scale=1.100000] (subEgvalue15) at (subEg15.west) {\num{3.18}};
\node[ref, lwsubEg] (subEg16) at (subEg15.north west) {\tikz \node[paper, calc] {\reftext{Yan20}\cite{yan2020}};};
\node[value, scale=1.100000] (subEgvalue16) at (subEg16.west) {\num{3.19}};
\node[ref, lwsubEg] (subEg17) at (subEg16.north west) {\tikz \node[paper, calc] {\reftext{Dubr77}\cite{dubrovskii1977}};};
\node[value, scale=1.100000] (subEgvalue17) at (subEg17.west) {\num{3.2}};
\node[ref, lwsubEg] (subEg18) at (subEg17.north west) {\tikz \node[paper, varshni] {\reftext{Liu21}\cite{liu2021}}; \tikz \node[paper, varshni] {\reftext{Nall99}\cite{nallet1999}};};
\node[value, scale=1.200000] (subEgvalue18) at (subEg18.west) {\num{3.25}};
\node[ref, lwsubEg] (subEg19) at (subEg18.north west) {\tikz \node[paper, varshni] {\reftext{Rao22}\cite{rao2022}}; \tikz \node[paper, varshni] {\reftext{Dena22}\cite{denapoli2022}}; \tikz \node[paper, calc] {\reftext{Sine21}\cite{sinelnik2021}}; \tikz \node[paper, varshni] {\reftext{Uhne15}\cite{uhnevionak2015}}; \tikz \node[paper] {\reftext{Dibe14}\cite{dibenedetto2014}}; \tikz \node[paper] {\reftext{Bion12}\cite{biondo2012}}; \tikz \node[paper, varshni] {\reftext{Habi11}\cite{habib2011}};};
\node[value, scale=1.700000] (subEgvalue19) at (subEg19.west) {\num{3.26}};
\node[ref, lwsubEg] (subEg20) at (subEg19.north west) {\tikz \node[paper, varshni] {\reftext{Lutz18}\cite{lutz2018}}; \tikz \node[paper, varshni] {\reftext{Joha16}\cite{johannesson2016}}; \tikz \node[paper, varshni] {\reftext{Lutz11}\cite{lutz2011}}; \tikz \node[paper, varshni] {\reftext{Rayn10}\cite{raynaud2010}};};
\node[value, scale=1.400000] (subEgvalue20) at (subEg20.west) {\num{3.263}};
\node[ref, lwsubEg] (subEg21) at (subEg20.north west) {\tikz \node[paper, varshni] {\reftext{Jime24}\cite{jimenez-ramos2024}}; \tikz \node[paper, varshni] {\reftext{Lech21}\cite{lechner2021}}; \tikz \node[paper, varshni] {\reftext{Loph18}\cite{lophitis2018}}; \tikz \node[paper] {\reftext{Nipo16}\cite{nipoti2016}}; \tikz \node[paper, varshni] {\reftext{Garc13}\cite{garcia2013}}; \tikz \node[paper, varshni] {\reftext{Song12}\cite{song2012}}; \tikz \node[paper, varshni] {\reftext{Tama08a}\cite{tamaki2008a}};};
\node[value, scale=1.700000] (subEgvalue21) at (subEg21.west) {\num{3.265}};
\node[ref, lwsubEg] (subEg22) at (subEg21.north west) {\tikz \node[paper, varshni] {\reftext{Levc11}\cite{levcenco2011}}; \tikz \node[paper, varshni] {\reftext{Bhat05}\cite{bhatnagar2005}}; \tikz \node[paper, varshni] {\reftext{Levi01}\cite{levinshtein2001}};};
\node[value, scale=1.300000] (subEgvalue22) at (subEg22.west) {\num{3.267}};
\node[ref, lwsubEg] (subEg23) at (subEg22.north west) {\tikz \node[paper] {\reftext{Nava08}\cite{nava2008}}; \tikz \node[paper, calc] {\reftext{Chen97}\cite{chen1997}};};
\node[value, scale=1.200000] (subEgvalue23) at (subEg23.west) {\num{3.27}};
\node[ref, lwsubEg] (subEg24) at (subEg23.north west) {\tikz \node[paper, fund] {\reftext{Ng10}\cite{ng2010}}; \tikz \node[paper] {\reftext{Vanh97}\cite{vanhaeringen1997}}; \tikz \node[paper] {\reftext{Scha97}\cite{schadt1997}}; \tikz \node[paper, calc] {\reftext{Back94}\cite{backes1994}};};
\node[value, scale=1.400000] (subEgvalue24) at (subEg24.west) {\num{3.28}};
\node[ref, lwsubEg] (subEg25) at (subEg24.north west) {\tikz \node[paper, varshni] {\reftext{Khan23}\cite{khanna2023}}; \tikz \node[paper, varshni] {\reftext{Stef14}\cite{stefanakis2014}}; \tikz \node[paper, varshni] {\reftext{Khal12}\cite{khalid2012}}; \tikz \node[paper] {\reftext{Masr02}\cite{masri2002}}; \tikz \node[paper, fund] {\reftext{Ivan02}\cite{ivanov2002}}; \tikz \node[paper, varshni] {\reftext{Gale02}\cite{galeckas2002}}; \tikz \node[paper] {\reftext{Frei95}\cite{freitas1995}};};
\node[value, scale=1.700000] (subEgvalue25) at (subEg25.west) {\num{3.285}};
\node[ref, lwsubEg] (subEg26) at (subEg25.north west) {\tikz \node[paper] {\reftext{Janz08}\cite{janzen2008}}; \tikz \node[paper] {\reftext{Ivan03}\cite{ivanov2003}};};
\node[value, scale=1.200000] (subEgvalue26) at (subEg26.west) {\num{3.287}};
\node[ref, lwsubEg] (subEg27) at (subEg26.north west) {\tikz \node[paper, varshni] {\reftext{Arva17}\cite{arvanitopoulos2017}};};
\node[value, scale=1.100000] (subEgvalue27) at (subEg27.west) {\num{3.29}};
\node[ref, lwsubEg] (subEg28) at (subEg27.north west) {\tikz \node[paper, varshni] {\reftext{Kimo19}\cite{kimoto2019}};};
\node[value, scale=1.100000] (subEgvalue28) at (subEg28.west) {\num{3.292}};
\node[ref, lwsubEg] (subEg29) at (subEg28.north west) {\tikz \node[paper, varshni] {\reftext{Tana24}\cite{tanaka2024}};};
\node[value, scale=1.100000] (subEgvalue29) at (subEg29.west) {\num{3.295}};
\node[ref, lwsubEg] (subEg30) at (subEg29.north west) {\tikz \node[paper, varshni] {\reftext{Megh18a}\cite{megherbi2018a}}; \tikz \node[paper, varshni] {\reftext{Pezz13}\cite{pezzimenti2013}}; \tikz \node[paper, varshni] {\reftext{Bell11}\cite{bellone2011}}; \tikz \node[paper, varshni] {\reftext{Alba10}\cite{albanese2010}};};
\node[value, scale=1.400000] (subEgvalue30) at (subEg30.west) {\num{3.299}};
\node[ref, lwsubEg] (subEg31) at (subEg30.north west) {\tikz \node[paper, varshni] {\reftext{Maxi23}\cite{maximenko2023}};};
\node[value, scale=1.100000] (subEgvalue31) at (subEg31.west) {\num{3.329}};
\node[ref, lwsubEg] (subEg32) at (subEg31.north west) {\tikz \node[paper, varshni] {\reftext{Chen12}\cite{chen2012}}; \tikz \node[paper, varshni] {\reftext{Cha08}\cite{cha2008}};};
\node[value, scale=1.200000] (subEgvalue32) at (subEg32.west) {\num{3.349}};
\node[ref, lwsubEg] (subEg33) at (subEg32.north west) {\tikz \node[paper, calc] {\reftext{Son04}\cite{son2004}}; \tikz \node[paper, calc] {\reftext{Umme98}\cite{ummels1998}};};
\node[value, scale=1.200000] (subEgvalue33) at (subEg33.west) {\num{3.35}};
\node[ref, lwsubEg] (subEg34) at (subEg33.north west) {\tikz \node[paper, varshni] {\reftext{Zegh20}\cite{zeghdar2020}}; \tikz \node[paper, varshni] {\reftext{Zegh19}\cite{zeghdar2019}}; \tikz \node[paper, varshni] {\reftext{Das15}\cite{das2015}}; \tikz \node[paper, varshni] {\reftext{Zhao03}\cite{zhao2003}}; \tikz \node[paper, varshni] {\reftext{Li03}\cite{li2003}}; \tikz \node[paper, varshni] {\reftext{Lee02}\cite{lee2002}}; \tikz \node[paper, varshni] {\reftext{Wang99}\cite{wang1999}}; \tikz \node[paper, varshni] {\reftext{Wrig98}\cite{wright1998}};};
\node[value, scale=1.800000] (subEgvalue34) at (subEg34.west) {\num{3.359}};
\node[ref, lwsubEg] (subEg35) at (subEg34.north west) {\tikz \node[paper] {\reftext{Scaj09}\cite{scajev2009}};};
\node[value, scale=1.100000] (subEgvalue35) at (subEg35.west) {\num{3.3762}};
\node[ref, lwsubEg] (subEg36) at (subEg35.north west) {\tikz \node[paper, varshni] {\reftext{Usma14}\cite{usman2014}};};
\node[value, scale=1.100000] (subEgvalue36) at (subEg36.west) {\num{3.461}};
\node[ref, lwsubEg] (subEg37) at (subEg36.north west) {\tikz \node[paper, varshni] {\reftext{Nawa10}\cite{nawaz2010}}; \tikz \node[paper, varshni] {\reftext{Bala05}\cite{balachandran2005}};};
\node[value, scale=1.200000] (subEgvalue37) at (subEg37.west) {\num{3.481}};
\node[ref, lwsubEg] (subEg38) at (subEg37.north west) {\tikz \node[paper, calc] {\reftext{Wenz95}\cite{wenzien1995}};};
\node[value, scale=1.100000] (subEgvalue38) at (subEg38.west) {\num{3.56}};
\node[ref, lwsubEg] (subEg39) at (subEg38.north west) {\tikz \node[paper, varshni] {\reftext{Mcnu04}\cite{mcnutt2004}};};
\node[value, scale=1.100000] (subEgvalue39) at (subEg39.west) {\num{4.25}};


\node[symbol] (subEgx) at (0+ \dxsubEg,0) {$\egx$};
\coordinate (subEgx0) at (subEgx.north);
\node[ref, lwsubEgx] (subEgx1) at (subEgx0.north west) {\tikz \node[paper, varshni] {\reftext{Ioff23}\cite{ioffe2023}};};
\node[value, scale=1.100000] (subEgxvalue1) at (subEgx1.west) {\num{3.237}};
\node[ref, lwsubEgx] (subEgx2) at (subEgx1.north west) {\tikz \node[paper, fund] {\reftext{Choy64}\cite{choyke1964}};};
\node[value, scale=1.100000] (subEgxvalue2) at (subEgx2.west) {\num{3.263+-0.003}};
\node[ref, lwsubEgx] (subEgx3) at (subEgx2.north west) {\tikz \node[paper, varshni] {\reftext{Kimo14a}\cite{kimoto2014a}}; \tikz \node[paper, varshni] {\reftext{Hata13}\cite{hatakeyama2013}}; \tikz \node[paper] {\reftext{Egil04}\cite{egilsson2004}}; \tikz \node[paper, varshni] {\reftext{Ayal04}\cite{ayalew2004}}; \tikz \node[paper] {\reftext{Masr02}\cite{masri2002}}; \tikz \node[paper, varshni] {\reftext{Lade00}\cite{ladesmartin2000}}; \tikz \node[paper] {\reftext{Choy97d}\cite{choyke1997d}}; \tikz \node[paper, fund] {\reftext{Kord95}\cite{kordina1995}}; \tikz \node[paper] {\reftext{Frei95}\cite{freitas1995}}; \tikz \node[paper] {\reftext{Mars74}\cite{marshall1974}}; \tikz \node[paper] {\reftext{Hage73}\cite{hagen1973}}; \tikz \node[paper] {\reftext{Choy69}\cite{choyke1969}}; \tikz \node[paper, fund] {\reftext{Choy64a}\cite{choyke1964a}};};
\node[value, scale=2.300000] (subEgxvalue3) at (subEgx3.west) {\num{3.265}};
\node[ref, lwsubEgx] (subEgx4) at (subEgx3.north west) {\tikz \node[paper, fund] {\reftext{Itoh96}\cite{itoh1996}};};
\node[value, scale=1.100000] (subEgxvalue4) at (subEgx4.west) {\num{3.2653}};
\node[ref, lwsubEgx] (subEgx5) at (subEgx4.north west) {\tikz \node[paper, fund] {\reftext{Klah20}\cite{klahold2020}};};
\node[value, scale=1.100000] (subEgxvalue5) at (subEgx5.west) {\num{3.2659}};
\node[ref, lwsubEgx] (subEgx6) at (subEgx5.north west) {\tikz \node[paper] {\reftext{Ivan03}\cite{ivanov2003}}; \tikz \node[paper] {\reftext{Egil99}\cite{egilsson1999}}; \tikz \node[paper, fund] {\reftext{Ivan98}\cite{ivanov1998}};};
\node[value, scale=1.300000] (subEgxvalue6) at (subEgx6.west) {\num{3.266}};
\node[ref, lwsubEgx] (subEgx7) at (subEgx6.north west) {\tikz \node[paper, fund] {\reftext{Srid00}\cite{sridhara2000}};};
\node[value, scale=1.100000] (subEgxvalue7) at (subEgx7.west) {\num{3.267}};
\node[ref, lwsubEgx] (subEgx8) at (subEgx7.north west) {\tikz \node[paper, passler] {\reftext{Stef14}\cite{stefanakis2014}}; \tikz \node[paper, passler] {\reftext{Griv07}\cite{grivickas2007}};};
\node[value, scale=1.200000] (subEgxvalue8) at (subEgx8.west) {\num{3.27}};


\node[symbol] (rtEg) at (0+ \dxsubEg+ \dxsubEgx,0) {$\eg$};
\coordinate (rtEg0) at (rtEg.north);
\node[ref, lwrtEg] (rtEg1) at (rtEg0.north west) {\tikz \node[paper, varshni] {\reftext{Ruff94}\cite{ruff1994}};};
\node[value, scale=1.100000] (rtEgvalue1) at (rtEg1.west) {\num{3}};
\node[ref, lwrtEg] (rtEg2) at (rtEg1.north west) {\tikz \node[paper] {\reftext{Sand11}\cite{sandeep2011}};};
\node[value, scale=1.100000] (rtEgvalue2) at (rtEg2.west) {\num{3.03}};
\node[ref, lwrtEg] (rtEg3) at (rtEg2.north west) {\tikz \node[paper, varshni] {\reftext{Nall99}\cite{nallet1999}};};
\node[value, scale=1.100000] (rtEgvalue3) at (rtEg3.west) {\num{3.151}};
\node[ref, lwrtEg] (rtEg4) at (rtEg3.north west) {\tikz \node[paper, varshni] {\reftext{Rao22}\cite{rao2022}};};
\node[value, scale=1.100000] (rtEgvalue4) at (rtEg4.west) {\num{3.161}};
\node[ref, lwrtEg] (rtEg5) at (rtEg4.north west) {\tikz \node[paper, varshni] {\reftext{Rayn10}\cite{raynaud2010}};};
\node[value, scale=1.100000] (rtEgvalue5) at (rtEg5.west) {\num{3.164}};
\node[ref, lwrtEg] (rtEg6) at (rtEg5.north west) {\tikz \node[paper, fund] {\reftext{Shal02}\cite{shalish2002}};};
\node[value, scale=1.100000] (rtEgvalue6) at (rtEg6.west) {\num{3.18}};
\node[ref, lwrtEg] (rtEg7) at (rtEg6.north west) {\tikz \node[paper] {\reftext{Bane21}\cite{banerjee2021}};};
\node[value, scale=1.100000] (rtEgvalue7) at (rtEg7.west) {\num{3.1934}};
\node[ref, lwrtEg] (rtEg8) at (rtEg7.north west) {\tikz \node[paper] {\reftext{Sozz19}\cite{sozzi2019}}; \tikz \node[paper, varshni] {\reftext{Megh18a}\cite{megherbi2018a}}; \tikz \node[paper] {\reftext{Cabe18}\cite{cabello2018}}; \tikz \node[paper] {\reftext{Arvi17}\cite{arvinte2017}}; \tikz \node[paper, varshni] {\reftext{Pezz13}\cite{pezzimenti2013}}; \tikz \node[paper, varshni] {\reftext{Bell11}\cite{bellone2011}}; \tikz \node[paper, varshni] {\reftext{Alba10}\cite{albanese2010}}; \tikz \node[paper] {\reftext{Pezz08}\cite{pezzimenti2008}}; \tikz \node[paper] {\reftext{Neud06}\cite{neudeck2006}}; \tikz \node[paper] {\reftext{Neud01}\cite{neudeck2001}};};
\node[value, scale=2.000000] (rtEgvalue8) at (rtEg8.west) {\num{3.2}};
\node[ref, lwrtEg] (rtEg9) at (rtEg8.north west) {\tikz \node[paper, varshni] {\reftext{Liu21}\cite{liu2021}};};
\node[value, scale=1.100000] (rtEgvalue9) at (rtEg9.west) {\num{3.213}};
\node[ref, lwrtEg] (rtEg10) at (rtEg9.north west) {\tikz \node[paper, varshni] {\reftext{Dena22}\cite{denapoli2022}};};
\node[value, scale=1.100000] (rtEgvalue10) at (rtEg10.west) {\num{3.214}};
\node[ref, lwrtEg] (rtEg11) at (rtEg10.north west) {\tikz \node[paper, fund] {\reftext{Fang18}\cite{fang2018}};};
\node[value, scale=1.100000] (rtEgvalue11) at (rtEg11.west) {\num{3.22}};
\node[ref, lwrtEg] (rtEg12) at (rtEg11.north west) {\tikz \node[paper, varshni] {\reftext{Uhne15}\cite{uhnevionak2015}}; \tikz \node[paper, varshni] {\reftext{Habi11}\cite{habib2011}};};
\node[value, scale=1.200000] (rtEgvalue12) at (rtEg12.west) {\num{3.223}};
\node[ref, lwrtEg] (rtEg13) at (rtEg12.north west) {\tikz \node[paper, varshni] {\reftext{Lutz18}\cite{lutz2018}}; \tikz \node[paper, varshni] {\reftext{Joha16}\cite{johannesson2016}}; \tikz \node[paper, varshni] {\reftext{Lutz11}\cite{lutz2011}};};
\node[value, scale=1.300000] (rtEgvalue13) at (rtEg13.west) {\num{3.226}};
\node[ref, lwrtEg] (rtEg14) at (rtEg13.north west) {\tikz \node[paper, varshni] {\reftext{Jime24}\cite{jimenez-ramos2024}}; \tikz \node[paper, varshni] {\reftext{Garc13}\cite{garcia2013}};};
\node[value, scale=1.200000] (rtEgvalue14) at (rtEg14.west) {\num{3.228}};
\node[ref, lwrtEg] (rtEg15) at (rtEg14.north west) {\tikz \node[paper, varshni] {\reftext{Maxi23}\cite{maximenko2023}}; \tikz \node[paper, varshni] {\reftext{Khan23}\cite{khanna2023}}; \tikz \node[paper] {\reftext{Zatk21}\cite{zatko2021}}; \tikz \node[paper] {\reftext{Rakh20}\cite{rakheja2020}}; \tikz \node[paper] {\reftext{Resc18a}\cite{rescher2018a}}; \tikz \node[paper, varshni] {\reftext{Stef14}\cite{stefanakis2014}}; \tikz \node[paper, varshni] {\reftext{Song12}\cite{song2012}}; \tikz \node[paper] {\reftext{Donn12}\cite{donnarumma2012}}; \tikz \node[paper, varshni] {\reftext{Tama08a}\cite{tamaki2008a}}; \tikz \node[paper, varshni] {\reftext{Bhat05}\cite{bhatnagar2005}}; \tikz \node[paper] {\reftext{Mori01}\cite{morisette2001}}; \tikz \node[paper, varshni] {\reftext{Levi01}\cite{levinshtein2001}};};
\node[value, scale=2.200000] (rtEgvalue15) at (rtEg15.west) {\num{3.23}};
\node[ref, lwrtEg] (rtEg16) at (rtEg15.north west) {\tikz \node[paper, varshni] {\reftext{Levc11}\cite{levcenco2011}};};
\node[value, scale=1.100000] (rtEgvalue16) at (rtEg16.west) {\num{3.234}};
\node[ref, lwrtEg] (rtEg17) at (rtEg16.north west) {\tikz \node[paper, varshni] {\reftext{Lech21}\cite{lechner2021}}; \tikz \node[paper, varshni] {\reftext{Loph18}\cite{lophitis2018}};};
\node[value, scale=1.200000] (rtEgvalue17) at (rtEg17.west) {\num{3.235}};
\node[ref, lwrtEg] (rtEg18) at (rtEg17.north west) {\tikz \node[paper, varshni] {\reftext{Usma14}\cite{usman2014}};};
\node[value, scale=1.100000] (rtEgvalue18) at (rtEg18.west) {\num{3.24}};
\node[ref, lwrtEg] (rtEg19) at (rtEg18.north west) {\tikz \node[paper, varshni] {\reftext{Chen12}\cite{chen2012}}; \tikz \node[paper, varshni] {\reftext{Cha08}\cite{cha2008}}; \tikz \node[paper] {\reftext{Hudg03}\cite{hudgins2003}};};
\node[value, scale=1.300000] (rtEgvalue19) at (rtEg19.west) {\num{3.25}};
\node[ref, lwrtEg] (rtEg20) at (rtEg19.north west) {\tikz \node[paper, varshni] {\reftext{Kimo19}\cite{kimoto2019}};};
\node[value, scale=1.100000] (rtEgvalue20) at (rtEg20.west) {\num{3.257}};
\node[ref, lwrtEg] (rtEg21) at (rtEg20.north west) {\tikz \node[paper, varshni] {\reftext{Tana24}\cite{tanaka2024}}; \tikz \node[paper] {\reftext{Dibe24}\cite{dibenedetto2024}}; \tikz \node[paper] {\reftext{Chou21}\cite{choudhary2021}}; \tikz \node[paper, varshni] {\reftext{Zegh20}\cite{zeghdar2020}}; \tikz \node[paper, varshni] {\reftext{Zegh19}\cite{zeghdar2019}}; \tikz \node[paper] {\reftext{Megh18}\cite{megherbi2018}}; \tikz \node[paper, varshni] {\reftext{Arva17}\cite{arvanitopoulos2017}}; \tikz \node[paper, varshni] {\reftext{Das15}\cite{das2015}}; \tikz \node[paper] {\reftext{Chen15}\cite{chen2015}}; \tikz \node[paper] {\reftext{Mand12}\cite{mandal2012}}; \tikz \node[paper, varshni] {\reftext{Nawa10}\cite{nawaz2010}}; \tikz \node[paper] {\reftext{Resh05}\cite{reshanov2005}}; \tikz \node[paper, varshni] {\reftext{Bala05}\cite{balachandran2005}}; \tikz \node[paper, varshni] {\reftext{Mcnu04}\cite{mcnutt2004}}; \tikz \node[paper, varshni] {\reftext{Zhao03}\cite{zhao2003}}; \tikz \node[paper, varshni] {\reftext{Li03}\cite{li2003}}; \tikz \node[paper] {\reftext{Elas03}\cite{elasser2003}}; \tikz \node[paper, varshni] {\reftext{Lee02}\cite{lee2002}}; \tikz \node[paper] {\reftext{Elas02}\cite{elasser2002}}; \tikz \node[paper] {\reftext{Elas00}\cite{elasser2000}}; \tikz \node[paper, varshni] {\reftext{Wang99}\cite{wang1999}}; \tikz \node[paper, varshni] {\reftext{Wrig98}\cite{wright1998}}; \tikz \node[paper] {\reftext{Afan96}\cite{afanasev1996}};};
\node[value, scale=3.300000] (rtEgvalue21) at (rtEg21.west) {\num{3.26}};
\node[ref, lwrtEg] (rtEg22) at (rtEg21.north west) {\tikz \node[paper, fund] {\reftext{Ahuj02}\cite{ahuja2002}};};
\node[value, scale=1.100000] (rtEgvalue22) at (rtEg22.west) {\num{3.26+-0.098}};
\node[ref, lwrtEg] (rtEg23) at (rtEg22.north west) {\tikz \node[paper, varshni] {\reftext{Gale02}\cite{galeckas2002}}; \tikz \node[paper, varshni] {\reftext{Gale02}\cite{galeckas2002}};};
\node[value, scale=1.200000] (rtEgvalue23) at (rtEg23.west) {\num{3.263}};
\node[ref, lwrtEg] (rtEg24) at (rtEg23.north west) {\tikz \node[paper, varshni] {\reftext{Khal12}\cite{khalid2012}};};
\node[value, scale=1.100000] (rtEgvalue24) at (rtEg24.west) {\num{3.265}};
\node[ref, lwrtEg] (rtEg25) at (rtEg24.north west) {\tikz \node[paper, varshni] {\reftext{Chen22}\cite{cheng2022}}; \tikz \node[paper] {\reftext{Shur06}\cite{shur2006}};};
\node[value, scale=1.200000] (rtEgvalue25) at (rtEg25.west) {\num{3.28}};
\node[ref, lwrtEg] (rtEg26) at (rtEg25.north west) {\tikz \node[paper] {\reftext{Bade20}\cite{bader2020}};};
\node[value, scale=1.100000] (rtEgvalue26) at (rtEg26.west) {\num{3.3}};
\node[ref, lwrtEg] (rtEg27) at (rtEg26.north west) {\tikz \node[paper, fund] {\reftext{Main24}\cite{mainali2024}};};
\node[value, scale=1.100000] (rtEgvalue27) at (rtEg27.west) {\num{3.3+-0.02}};


\node[symbol] (rtEgx) at (0+ \dxsubEg+ \dxsubEgx+ \dxrtEg,0) {$\egx$};
\coordinate (rtEgx0) at (rtEgx.north);
\node[ref, lwrtEgx] (rtEgx1) at (rtEgx0.north west) {\tikz \node[paper, varshni] {\reftext{Ioff23}\cite{ioffe2023}}; \tikz \node[paper] {\reftext{Made96}\cite{madelung1996}}; \tikz \node[paper] {\reftext{Made91}\cite{madelung1991}};};
\node[value, scale=1.300000] (rtEgxvalue1) at (rtEgx1.west) {\num{3.2}};
\node[ref, lwrtEgx] (rtEgx2) at (rtEgx1.north west) {\tikz \node[paper, varshni] {\reftext{Kimo14a}\cite{kimoto2014a}}; \tikz \node[paper, varshni] {\reftext{Hata13}\cite{hatakeyama2013}}; \tikz \node[paper, passler] {\reftext{Griv07}\cite{grivickas2007}}; \tikz \node[paper, fund] {\reftext{Zanm64}\cite{zanmarchi1964}};};
\node[value, scale=1.400000] (rtEgxvalue2) at (rtEgx2.west) {\num{3.23}};
\node[ref, lwrtEgx] (rtEgx3) at (rtEgx2.north west) {\tikz \node[paper, varshni] {\reftext{Ayal04}\cite{ayalew2004}};};
\node[value, scale=1.100000] (rtEgxvalue3) at (rtEgx3.west) {\num{3.235}};
\node[ref, lwrtEgx] (rtEgx4) at (rtEgx3.north west) {\tikz \node[paper, passler] {\reftext{Stef14}\cite{stefanakis2014}};};
\node[value, scale=1.100000] (rtEgxvalue4) at (rtEgx4.west) {\num{3.24}};
\node[ref, lwrtEgx] (rtEgx5) at (rtEgx4.north west) {\tikz \node[paper, varshni] {\reftext{Lade00}\cite{ladesmartin2000}};};
\node[value, scale=1.100000] (rtEgxvalue5) at (rtEgx5.west) {\num{3.243}};


\node[symbol] (NAEg) at (0+ \dxsubEg+ \dxsubEgx+ \dxrtEg+ \dxrtEgx,0) {$\eg$};
\coordinate (NAEg0) at (NAEg.north);
\node[ref, lwNAEg] (NAEg1) at (NAEg0.north west) {\tikz \node[paper] {\reftext{Sze07}\cite{sze2007}};};
\node[value, scale=1.100000] (NAEgvalue1) at (NAEg1.west) {\num{3}};
\node[ref, lwNAEg] (NAEg2) at (NAEg1.north west) {\tikz \node[paper] {\reftext{Shah98}\cite{shah1998}};};
\node[value, scale=1.100000] (NAEgvalue2) at (NAEg2.west) {\num{3.19}};
\node[ref, lwNAEg] (NAEg3) at (NAEg2.north west) {\tikz \node[paper] {\reftext{Mukh23}\cite{mukherjee2023}}; \tikz \node[paper] {\reftext{Mukh20a}\cite{mukherjee2020a}}; \tikz \node[paper] {\reftext{Sole19}\cite{soler2019}}; \tikz \node[paper] {\reftext{Guo19}\cite{guo2019}}; \tikz \node[paper] {\reftext{Hass18}\cite{hassan2018}}; \tikz \node[paper] {\reftext{Elah17}\cite{elahipanah2017}}; \tikz \node[paper] {\reftext{Mant15}\cite{mantooth2015}}; \tikz \node[paper] {\reftext{Fuji15}\cite{fujita2015}}; \tikz \node[paper] {\reftext{Mant13}\cite{mantooth2013}}; \tikz \node[paper] {\reftext{Cres13}\cite{cressler2013}}; \tikz \node[paper] {\reftext{Buon12}\cite{buono2012}}; \tikz \node[paper] {\reftext{Wije11a}\cite{wijesundara2011a}}; \tikz \node[paper] {\reftext{Ostl11}\cite{ostling2011}}; \tikz \node[paper] {\reftext{Butt11}\cite{buttay2011}}; \tikz \node[paper] {\reftext{Mill07}\cite{millan2007}}; \tikz \node[paper] {\reftext{Cima07}\cite{cimalla2007}}; \tikz \node[paper] {\reftext{Kuma05}\cite{kumar2005}}; \tikz \node[paper] {\reftext{Bert04}\cite{bertilsson2004}}; \tikz \node[paper] {\reftext{Zett02}\cite{zetterling2002}}; \tikz \node[paper] {\reftext{Trew02}\cite{trew2002}}; \tikz \node[paper] {\reftext{Powe02}\cite{powell2002}}; \tikz \node[paper] {\reftext{Gao01}\cite{gao2001}}; \tikz \node[paper] {\reftext{Lebe99}\cite{lebedev1999}}; \tikz \node[paper] {\reftext{Zett98}\cite{zetterling1998}}; \tikz \node[paper] {\reftext{Weit98}\cite{weitzel1998}}; \tikz \node[paper] {\reftext{Rosc98}\cite{roschke1998}}; \tikz \node[paper] {\reftext{Mick98}\cite{mickevicius1998}}; \tikz \node[paper] {\reftext{Trew97}\cite{trew1997}}; \tikz \node[paper] {\reftext{Chel97}\cite{chelnokov1997}}; \tikz \node[paper] {\reftext{Weit96}\cite{weitzel1996}}; \tikz \node[paper] {\reftext{Neud95}\cite{neudeck1995}};};
\node[value, scale=4.100000] (NAEgvalue3) at (NAEg3.west) {\num{3.2}};
\node[ref, lwNAEg] (NAEg4) at (NAEg3.north west) {\tikz \node[paper] {\reftext{Kars20}\cite{karsthof2020}}; \tikz \node[paper] {\reftext{Trip19}\cite{tripathi2019}}; \tikz \node[paper] {\reftext{Ryba17}\cite{rybalka2017}}; \tikz \node[paper] {\reftext{Liol15}\cite{lioliou2015}}; \tikz \node[paper] {\reftext{Klei09}\cite{klein2009}}; \tikz \node[paper] {\reftext{Donn09}\cite{donnarumma2009}}; \tikz \node[paper] {\reftext{Arpa06}\cite{arpatzanis2006}};};
\node[value, scale=1.700000] (NAEgvalue4) at (NAEg4.west) {\num{3.23}};
\node[ref, lwNAEg] (NAEg5) at (NAEg4.north west) {\tikz \node[paper] {\reftext{Werb07}\cite{werber2007}};};
\node[value, scale=1.100000] (NAEgvalue5) at (NAEg5.west) {\num{3.24}};
\node[ref, lwNAEg] (NAEg6) at (NAEg5.north west) {\tikz \node[paper] {\reftext{Kim24}\cite{kim2024}}; \tikz \node[paper] {\reftext{Pear23}\cite{pearton2023}}; \tikz \node[paper] {\reftext{Pear18}\cite{pearton2018}}; \tikz \node[paper] {\reftext{Scaj10}\cite{scajev2010}}; \tikz \node[paper] {\reftext{Ng04}\cite{ng2004}}; \tikz \node[paper] {\reftext{Agar99}\cite{agarwal1999}}; \tikz \node[paper] {\reftext{Srir97}\cite{sriram1997}}; \tikz \node[paper] {\reftext{Shen97}\cite{shenoy1997}}; \tikz \node[paper] {\reftext{Agar96}\cite{agarwal1996}};};
\node[value, scale=1.900000] (NAEgvalue6) at (NAEg6.west) {\num{3.25}};
\node[ref, lwNAEg] (NAEg7) at (NAEg6.north west) {\tikz \node[paper] {\reftext{Ostl24}\cite{ostling2024}}; \tikz \node[paper] {\reftext{Wolf23}\cite{wolfspeed2023}}; \tikz \node[paper] {\reftext{Xi22}\cite{xi2022}}; \tikz \node[paper] {\reftext{Lang22}\cite{langpoklakpam2022}}; \tikz \node[paper] {\reftext{Gao22a}\cite{gao2022a}}; \tikz \node[paper] {\reftext{Capa22}\cite{capan2022}}; \tikz \node[paper] {\reftext{Bere21}\cite{berens2021}}; \tikz \node[paper] {\reftext{Nouk20}\cite{nouketcha2020}}; \tikz \node[paper] {\reftext{Mats20}\cite{matsunami2020}}; \tikz \node[paper] {\reftext{Jiya20}\cite{jiya2020}}; \tikz \node[paper] {\reftext{Joha19}\cite{johannesson2019}}; \tikz \node[paper] {\reftext{Bali19}\cite{baliga2019}}; \tikz \node[paper] {\reftext{Yosh18}\cite{yoshioka2018}}; \tikz \node[paper] {\reftext{Resc18}\cite{rescher2018}}; \tikz \node[paper] {\reftext{Lebe17}\cite{lebedev2017}}; \tikz \node[paper] {\reftext{Chow17}\cite{chow2017}}; \tikz \node[paper] {\reftext{Liu15}\cite{liu2015}}; \tikz \node[paper] {\reftext{Kimo15}\cite{kimoto2015}}; \tikz \node[paper] {\reftext{Chow15}\cite{chowdhury2015}}; \tikz \node[paper] {\reftext{Kami14}\cite{kaminski2014}}; \tikz \node[paper] {\reftext{Neil12}\cite{neilainglesias2012}}; \tikz \node[paper] {\reftext{Zipp11}\cite{zippelius2011}}; \tikz \node[paper] {\reftext{Wije11b}\cite{wijesundara2011b}}; \tikz \node[paper] {\reftext{Scab11a}\cite{scaburri2011a}}; \tikz \node[paper] {\reftext{Mani11}\cite{manikam2011}}; \tikz \node[paper] {\reftext{Jone11}\cite{jones2011}}; \tikz \node[paper] {\reftext{Gerh11}\cite{gerhardt2011}}; \tikz \node[paper] {\reftext{Su10}\cite{su2010}}; \tikz \node[paper] {\reftext{Kami09}\cite{kaminski2009}}; \tikz \node[paper] {\reftext{Zhu08}\cite{zhu2008}}; \tikz \node[paper] {\reftext{Tila07}\cite{tilak2007}}; \tikz \node[paper] {\reftext{Tann07}\cite{tanner2007}}; \tikz \node[paper] {\reftext{Will06}\cite{willander2006}}; \tikz \node[paper] {\reftext{Schr06}\cite{schroeder2006}}; \tikz \node[paper] {\reftext{Phil06}\cite{philip2006}}; \tikz \node[paper] {\reftext{Chow06}\cite{chow2006}}; \tikz \node[paper] {\reftext{Bali06}\cite{baliga2006}}; \tikz \node[paper] {\reftext{Choi05}\cite{choi2005}}; \tikz \node[paper] {\reftext{Ozpi04}\cite{ozpineci2004}}; \tikz \node[paper] {\reftext{Dhar04}\cite{dhar2004}}; \tikz \node[paper] {\reftext{Cole04}\cite{cole2004}}; \tikz \node[paper] {\reftext{Chow04}\cite{chow2004}}; \tikz \node[paper] {\reftext{Kohl03}\cite{kohlscheen2003}}; \tikz \node[paper] {\reftext{Han03}\cite{han2003}}; \tikz \node[paper] {\reftext{Zhan02}\cite{zhang2002}}; \tikz \node[paper] {\reftext{Wein02}\cite{weingartner2002}}; \tikz \node[paper] {\reftext{Keme02}\cite{kemerley2002}}; \tikz \node[paper] {\reftext{Wern01}\cite{werner2001}}; \tikz \node[paper] {\reftext{Hefn01}\cite{hefner2001}}; \tikz \node[paper] {\reftext{Zhao00}\cite{zhao2000}}; \tikz \node[paper] {\reftext{Dmit00}\cite{dmitriev2000}}; \tikz \node[paper] {\reftext{Chow00a}\cite{chow2000a}}; \tikz \node[paper] {\reftext{Chow00}\cite{chow2000}}; \tikz \node[paper] {\reftext{Bell99}\cite{bellotti1999}}; \tikz \node[paper] {\reftext{Huan98}\cite{huang1998}}; \tikz \node[paper] {\reftext{Mats97}\cite{matsunami1997}}; \tikz \node[paper] {\reftext{Chow97}\cite{chow1997}}; \tikz \node[paper] {\reftext{Yode96}\cite{yoder1996}}; \tikz \node[paper] {\reftext{Wrig96}\cite{wright1996}}; \tikz \node[paper] {\reftext{Chow96}\cite{chow1996}}; \tikz \node[paper] {\reftext{Casa96}\cite{casady1996}}; \tikz \node[paper] {\reftext{Itoh94}\cite{itoh1994}};};
\node[value, scale=7.000000] (NAEgvalue7) at (NAEg7.west) {\num{3.26}};
\node[ref, lwNAEg] (NAEg8) at (NAEg7.north west) {\tikz \node[paper] {\reftext{Cama08}\cite{camassel2008}};};
\node[value, scale=1.100000] (NAEgvalue8) at (NAEg8.west) {\num{3.263}};
\node[ref, lwNAEg] (NAEg9) at (NAEg8.north west) {\tikz \node[paper] {\reftext{Kwas14}\cite{kwasnicki2014}}; \tikz \node[paper] {\reftext{Rao99}\cite{rao1999}}; \tikz \node[paper] {\reftext{Trof98}\cite{troffer1998}}; \tikz \node[paper] {\reftext{Scho94}\cite{schoner1994}}; \tikz \node[paper] {\reftext{Free90}\cite{freer1990}};};
\node[value, scale=1.500000] (NAEgvalue9) at (NAEg9.west) {\num{3.265}};
\node[ref, lwNAEg] (NAEg10) at (NAEg9.north west) {\tikz \node[paper] {\reftext{Baie19}\cite{baierhofer2019}};};
\node[value, scale=1.100000] (NAEgvalue10) at (NAEg10.west) {\num{3.268}};
\node[ref, lwNAEg] (NAEg11) at (NAEg10.north west) {\tikz \node[paper] {\reftext{Klep21}\cite{kleppinger2021}}; \tikz \node[paper] {\reftext{Chen08}\cite{chen2008}}; \tikz \node[paper] {\reftext{Bech04}\cite{bechstedt2004}};};
\node[value, scale=1.300000] (NAEgvalue11) at (NAEg11.west) {\num{3.27}};
\node[ref, lwNAEg] (NAEg12) at (NAEg11.north west) {\tikz \node[paper] {\reftext{Gale97}\cite{galeckas1997}};};
\node[value, scale=1.100000] (NAEgvalue12) at (NAEg12.west) {\num{3.275}};
\node[ref, lwNAEg] (NAEg13) at (NAEg12.north west) {\tikz \node[paper] {\reftext{Naug17}\cite{naugarhiya2017}}; \tikz \node[paper] {\reftext{Choi16}\cite{choi2016}}; \tikz \node[paper] {\reftext{Pank14}\cite{pankove2014}}; \tikz \node[paper] {\reftext{Pens05}\cite{pensl2005}};};
\node[value, scale=1.400000] (NAEgvalue13) at (NAEg13.west) {\num{3.28}};
\node[ref, lwNAEg] (NAEg14) at (NAEg13.north west) {\tikz \node[paper] {\reftext{Ivan05}\cite{ivanov2005}};};
\node[value, scale=1.100000] (NAEgvalue14) at (NAEg14.west) {\num{3.287}};
\node[ref, lwNAEg] (NAEg15) at (NAEg14.north west) {\tikz \node[paper] {\reftext{Pers99}\cite{persson1999}}; \tikz \node[paper] {\reftext{Pers98}\cite{persson1998}};};
\node[value, scale=1.200000] (NAEgvalue15) at (NAEg15.west) {\num{3.29}};
\node[ref, lwNAEg] (NAEg16) at (NAEg15.north west) {\tikz \node[paper] {\reftext{Zhen20}\cite{zheng2020}}; \tikz \node[paper] {\reftext{Bisw20}\cite{biswas2020}}; \tikz \node[paper] {\reftext{Adit15}\cite{aditya2015}}; \tikz \node[paper] {\reftext{Higa14}\cite{higashiwaki2014}}; \tikz \node[paper] {\reftext{Dhan10}\cite{dhanaraj2010}}; \tikz \node[paper] {\reftext{Codr00}\cite{codreanu2000}};};
\node[value, scale=1.600000] (NAEgvalue16) at (NAEg16.west) {\num{3.3}};
\node[ref, lwNAEg] (NAEg17) at (NAEg16.north west) {\tikz \node[paper] {\reftext{Chow93}\cite{chow1993}};};
\node[value, scale=1.100000] (NAEgvalue17) at (NAEg17.west) {\num{3.33}};
\node[ref, lwNAEg] (NAEg18) at (NAEg17.north west) {\tikz \node[paper] {\reftext{Zoll99}\cite{zollner1999}};};
\node[value, scale=1.100000] (NAEgvalue18) at (NAEg18.west) {\num{3.4}};


\node[symbol] (NAEgx) at (0+ \dxsubEg+ \dxsubEgx+ \dxrtEg+ \dxrtEgx+ \dxNAEg,0) {$\egx$};
\coordinate (NAEgx0) at (NAEgx.north);
\node[ref, lwNAEgx] (NAEgx1) at (NAEgx0.north west) {\tikz \node[paper] {\reftext{Feng04a}\cite{feng2004a}};};
\node[value, scale=1.100000] (NAEgxvalue1) at (NAEgx1.west) {\num{3.26}};
\node[ref, lwNAEgx] (NAEgx2) at (NAEgx1.north west) {\tikz \node[paper] {\reftext{Fan14}\cite{fan2014}}; \tikz \node[paper] {\reftext{Yosh95}\cite{yoshida1995}};};
\node[value, scale=1.200000] (NAEgxvalue2) at (NAEgx2.west) {\num{3.263}};
\node[ref, lwNAEgx] (NAEgx3) at (NAEgx2.north west) {\tikz \node[paper] {\reftext{Pank14}\cite{pankove2014}}; \tikz \node[paper] {\reftext{Berg96}\cite{berger1996}}; \tikz \node[paper] {\reftext{Habe94}\cite{haberstroh1994}}; \tikz \node[paper] {\reftext{Suzu77}\cite{suzuki1977}}; \tikz \node[paper] {\reftext{Patr66}\cite{patrick1966}}; \tikz \node[paper] {\reftext{Patr65}\cite{patrick1965}};};
\node[value, scale=1.600000] (NAEgxvalue3) at (NAEgx3.west) {\num{3.265}};


\node[symbol] (Ex) at (0+ \dxsubEg+ \dxsubEgx+ \dxrtEg+ \dxrtEgx+ \dxNAEg+ \dxNAEgx,0) {$\ex$};
\coordinate (Ex0) at (Ex.north);
\node[ref, lwEx] (Ex1) at (Ex0.north west) {\tikz \node[paper, fund] {\reftext{Iked80b}\cite{ikeda1980b}}; \tikz \node[paper] {\reftext{Suzu77}\cite{suzuki1977}}; \tikz \node[paper] {\reftext{Mats74}\cite{matsunami1974}};};
\node[value, scale=1.300000] (Exvalue1) at (Ex1.west) {\num{10}};
\node[ref, lwEx] (Ex2) at (Ex1.north west) {\tikz \node[paper, fund] {\reftext{Dubr75}\cite{dubrovskii1975}};};
\node[value, scale=1.100000] (Exvalue2) at (Ex2.west) {\num{20+-1.5}};
\node[ref, lwEx] (Ex3) at (Ex2.north west) {\tikz \node[paper] {\reftext{Pank14}\cite{pankove2014}}; \tikz \node[paper] {\reftext{Kimo14a}\cite{kimoto2014a}}; \tikz \node[paper] {\reftext{Fan14}\cite{fan2014}}; \tikz \node[paper] {\reftext{Hata13}\cite{hatakeyama2013}}; \tikz \node[paper] {\reftext{Ayal04}\cite{ayalew2004}}; \tikz \node[paper] {\reftext{Masr02}\cite{masri2002}}; \tikz \node[paper] {\reftext{Egil99}\cite{egilsson1999}}; \tikz \node[paper] {\reftext{Deva97}\cite{devaty1997}}; \tikz \node[paper] {\reftext{Frei95}\cite{freitas1995}}; \tikz \node[paper] {\reftext{Iked80}\cite{ikeda1980}};};
\node[value, scale=2.000000] (Exvalue3) at (Ex3.west) {\num{20}};
\node[ref, lwEx] (Ex4) at (Ex3.north west) {\tikz \node[paper, fund] {\reftext{Ivan02}\cite{ivanov2002}};};
\node[value, scale=1.100000] (Exvalue4) at (Ex4.west) {\num{20.5+-1}};
\node[ref, lwEx] (Ex5) at (Ex4.north west) {\tikz \node[paper] {\reftext{Janz08}\cite{janzen2008}};};
\node[value, scale=1.100000] (Exvalue5) at (Ex5.west) {\num{21}};
\node[ref, lwEx] (Ex6) at (Ex5.north west) {\tikz \node[paper, fund] {\reftext{Griv07}\cite{grivickas2007}};};
\node[value, scale=1.100000] (Exvalue6) at (Ex6.west) {\num{30+-10}};
\node[ref, lwEx] (Ex7) at (Ex6.north west) {\tikz \node[paper] {\reftext{Scaj10}\cite{scajev2010}};};
\node[value, scale=1.100000] (Exvalue7) at (Ex7.west) {\num{30}};
\node[ref, lwEx] (Ex8) at (Ex7.north west) {\tikz \node[paper, fund] {\reftext{Klah20}\cite{klahold2020}}; \tikz \node[paper] {\reftext{Lade00}\cite{ladesmartin2000}};};
\node[value, scale=1.200000] (Exvalue8) at (Ex8.west) {\num{40}};


==> data/dos_TCAD.tex <==


\node[symbol] (e) at (0,0) {$\mde$};
\coordinate (e0) at (e.north);
\node[ref, lwe] (e1) at (e0.north west) {\tikz \node[paper, calculated] {\reftext{Rodr21}\cite{rodrigues2021}}; \tikz \node[paper] {\reftext{Kuzn95}\cite{kuznetsov1995}}; \tikz \node[paper] {\reftext{Scho94}\cite{schoner1994}}; \tikz \node[paper] {\reftext{Scha94a}\cite{schadt1994a}}; \tikz \node[paper] {\reftext{Pens93}\cite{pensl1993}}; \tikz \node[paper] {\reftext{Gotz93}\cite{gotz1993}};};
\node[value, scale=1.600000] (evalue1) at (e1.west) {\num{0.19}};
\node[ref, lwe] (e2) at (e1.north west) {\tikz \node[paper] {\reftext{Kim24}\cite{kim2024}}; \tikz \node[paper] {\reftext{Arpa06}\cite{arpatzanis2006}}; \tikz \node[paper] {\reftext{Itoh95}\cite{itoh1995}}; \tikz \node[paper, calculated] {\reftext{Loma74}\cite{lomakina1974}}; \tikz \node[paper, calculated] {\reftext{Loma73}\cite{lomakina1973}};};
\node[value, scale=1.500000] (evalue2) at (e2.west) {\num{0.20}};
\node[ref, lwe] (e3) at (e2.north west) {\tikz \node[paper, calculated] {\reftext{Wenz95}\cite{wenzien1995}}; \tikz \node[paper, calculated] {\reftext{Kack94}\cite{kackell1994}};};
\node[value, scale=1.200000] (evalue3) at (e3.west) {\num{0.32}};
\node[ref, lwe] (e4) at (e3.north west) {\tikz \node[paper, calculated] {\reftext{Bell00}\cite{bellotti2000}};};
\node[value, scale=1.100000] (evalue4) at (e4.west) {\num{0.33}};
\node[ref, lwe] (e5) at (e4.north west) {\tikz \node[paper, calculated] {\reftext{Penn01}\cite{pennington2001}};};
\node[value, scale=1.100000] (evalue5) at (e5.west) {\num{0.34}};
\node[ref, lwe] (e6) at (e5.north west) {\tikz \node[paper, calculated] {\reftext{Dong04}\cite{dong2004}}; \tikz \node[paper, calculated] {\reftext{Naka97}\cite{nakashima1997}}; \tikz \node[paper, calculated] {\reftext{Lamb95}\cite{lambrecht1995}}; \tikz \node[paper, calculated] {\reftext{Hari95}\cite{harima1995}};};
\node[value, scale=1.400000] (evalue6) at (e6.west) {\num{0.35}};
\node[ref, lwe] (e7) at (e6.north west) {\tikz \node[paper] {\reftext{Yang19}\cite{yang2019}}; \tikz \node[paper, calculated] {\reftext{Kuro19}\cite{kuroiwa2019}}; \tikz \node[paper, calculated] {\reftext{Tiwa99}\cite{tiwald1999}};};
\node[value, scale=1.300000] (evalue7) at (e7.west) {\num{0.36}};
\node[ref, lwe] (e8) at (e7.north west) {\tikz \node[paper] {\reftext{Ioff23}\cite{ioffe2023}}; \tikz \node[paper] {\reftext{Scaj13a}\cite{scajev2013a}}; \tikz \node[paper] {\reftext{Song12}\cite{song2012}}; \tikz \node[paper] {\reftext{Rayn10}\cite{raynaud2010}}; \tikz \node[paper] {\reftext{Alba10}\cite{albanese2010}}; \tikz \node[paper, calculated] {\reftext{Donn09}\cite{donnarumma2009}}; \tikz \node[paper] {\reftext{Tama08a}\cite{tamaki2008a}}; \tikz \node[paper] {\reftext{Resh05}\cite{reshanov2005}}; \tikz \node[paper, calculated] {\reftext{Pers05}\cite{persson2005}}; \tikz \node[paper, calculated] {\reftext{Son04}\cite{son2004}}; \tikz \node[paper] {\reftext{Lee02}\cite{lee2002}}; \tikz \node[paper] {\reftext{Levi01}\cite{levinshtein2001}}; \tikz \node[paper, calculated] {\reftext{Iwat01}\cite{iwata2001}}; \tikz \node[paper, calculated] {\reftext{Zhao00a}\cite{zhao2000a}}; \tikz \node[paper, calculated] {\reftext{Zhao00}\cite{zhao2000}}; \tikz \node[paper, calculated] {\reftext{Iwat00a}\cite{iwata2000a}}; \tikz \node[paper, calculated] {\reftext{Iwat00}\cite{iwata2000}}; \tikz \node[paper] {\reftext{Ivan00}\cite{ivanov2000}}; \tikz \node[paper, calculated] {\reftext{Pers99b}\cite{persson1999b}}; \tikz \node[paper, calculated] {\reftext{Pers99a}\cite{persson1999a}}; \tikz \node[paper] {\reftext{Egil99}\cite{egilsson1999}}; \tikz \node[paper] {\reftext{Shah98}\cite{shah1998}}; \tikz \node[paper] {\reftext{Pers98a}\cite{persson1998a}}; \tikz \node[paper, calculated] {\reftext{Mick98a}\cite{mickevicius1998a}}; \tikz \node[paper, calculated] {\reftext{Mick98}\cite{mickevicius1998}}; \tikz \node[paper, calculated] {\reftext{Lind98}\cite{lindefelt1998}}; \tikz \node[paper, calculated] {\reftext{Kino98}\cite{kinoshita1998}}; \tikz \node[paper] {\reftext{Huan98}\cite{huang1998}}; \tikz \node[paper, calculated] {\reftext{Pers97}\cite{persson1997}}; \tikz \node[paper, calculated] {\reftext{Lamb97}\cite{lambrecht1997}}; \tikz \node[paper] {\reftext{Hemm97}\cite{hemmingsson1997}}; \tikz \node[paper] {\reftext{Bako97}\cite{bakowski1997}}; \tikz \node[paper, calculated] {\reftext{Pers96}\cite{persson1996}}; \tikz \node[paper, calculated] {\reftext{Nils96}\cite{nilsson1996}}; \tikz \node[paper, calculated] {\reftext{Son95}\cite{son1995}}; \tikz \node[paper, calculated] {\reftext{Josh95}\cite{joshi1995}}; \tikz \node[paper] {\reftext{Iked80}\cite{ikeda1980}};};
\node[value, scale=4.700000] (evalue8) at (e8.west) {\num{0.37}};
\node[ref, lwe] (e9) at (e8.north west) {\tikz \node[paper] {\reftext{Pere06}\cite{perez-tomas2006}};};
\node[value, scale=1.100000] (evalue9) at (e9.west) {\num{0.38}};
\node[ref, lwe] (e10) at (e9.north west) {\tikz \node[paper] {\reftext{Pear23}\cite{pearton2023}}; \tikz \node[paper] {\reftext{Maxi23}\cite{maximenko2023}}; \tikz \node[paper] {\reftext{Khan23}\cite{khanna2023}}; \tikz \node[paper, calculated] {\reftext{Ishi21}\cite{ishikawa2021}}; \tikz \node[paper, calculated] {\reftext{Rakh20}\cite{rakheja2020}}; \tikz \node[paper] {\reftext{Nouk20}\cite{nouketcha2020}}; \tikz \node[paper, calculated] {\reftext{Klah20}\cite{klahold2020}}; \tikz \node[paper, calculated] {\reftext{Kimo14a}\cite{kimoto2014a}}; \tikz \node[paper] {\reftext{Hata13}\cite{hatakeyama2013}}; \tikz \node[paper] {\reftext{Scab11a}\cite{scaburri2011a}}; \tikz \node[paper, calculated] {\reftext{Janz08}\cite{janzen2008}}; \tikz \node[paper] {\reftext{Nego04a}\cite{negoro2004a}}; \tikz \node[paper, calculated] {\reftext{Feng04a}\cite{feng2004a}}; \tikz \node[paper] {\reftext{Ayal04}\cite{ayalew2004}}; \tikz \node[paper, calculated] {\reftext{Kohl03}\cite{kohlscheen2003}}; \tikz \node[paper, calculated] {\reftext{Ivan03a}\cite{ivanov2003a}}; \tikz \node[paper, calculated] {\reftext{Son00}\cite{son2000}}; \tikz \node[paper, calculated] {\reftext{Pern00}\cite{pernot2000}}; \tikz \node[paper] {\reftext{Lade00}\cite{ladesmartin2000}}; \tikz \node[paper, calculated] {\reftext{Chen00}\cite{chen2000}}; \tikz \node[paper] {\reftext{Well97}\cite{wellenhofer1997}}; \tikz \node[paper, calculated] {\reftext{Pers97}\cite{persson1997}}; \tikz \node[paper, calculated] {\reftext{Deva97}\cite{devaty1997}}; \tikz \node[paper, calculated] {\reftext{Volm96}\cite{volm1996}}; \tikz \node[paper, calculated] {\reftext{Kaec96}\cite{kaeckell1996}}; \tikz \node[paper, calculated] {\reftext{Karc95}\cite{karch1995}};};
\node[value, scale=3.600000] (evalue10) at (e10.west) {\num{0.39}};
\node[ref, lwe] (e11) at (e10.north west) {\tikz \node[paper] {\reftext{Luo20}\cite{luo2020}}; \tikz \node[paper] {\reftext{Sozz19}\cite{sozzi2019}}; \tikz \node[paper] {\reftext{Aktu09}\cite{akturk2009}}; \tikz \node[paper] {\reftext{Fang05}\cite{fang2005}}; \tikz \node[paper, calculated] {\reftext{Pers97}\cite{persson1997}};};
\node[value, scale=1.500000] (evalue11) at (e11.west) {\num{0.40}};
\node[ref, lwe] (e12) at (e11.north west) {\tikz \node[paper, calculated] {\reftext{Ng11}\cite{ng2011}}; \tikz \node[paper, calculated] {\reftext{Ng10}\cite{ng2010}}; \tikz \node[paper] {\reftext{Tila07}\cite{tilak2007}}; \tikz \node[paper] {\reftext{Penn04}\cite{pennington2004}};};
\node[value, scale=1.400000] (evalue12) at (e12.west) {\num{0.41}};
\node[ref, lwe] (e13) at (e12.north west) {\tikz \node[paper] {\reftext{Nipo16}\cite{nipoti2016}}; \tikz \node[paper] {\reftext{Neim06}\cite{neimontas2006}}; \tikz \node[paper, calculated] {\reftext{Chen97}\cite{chen1997}};};
\node[value, scale=1.300000] (evalue13) at (e13.west) {\num{0.42}};
\node[ref, lwe] (e14) at (e13.north west) {\tikz \node[paper] {\reftext{Bion12}\cite{biondo2012}};};
\node[value, scale=1.100000] (evalue14) at (e14.west) {\num{0.80}};


\node[symbol] (h) at (0+ \dxe,0) {$\mdh$};
\coordinate (h0) at (h.north);
\node[ref, lwh] (h1) at (h0.north west) {\tikz \node[paper] {\reftext{Koiz09}\cite{koizumi2009}};};
\node[value, scale=1.100000] (hvalue1) at (h1.west) {\num{0.50}};
\node[ref, lwh] (h2) at (h1.north west) {\tikz \node[paper, calculated] {\reftext{Kuro19}\cite{kuroiwa2019}};};
\node[value, scale=1.100000] (hvalue2) at (h2.west) {\num{0.76}};
\node[ref, lwh] (h3) at (h2.north west) {\tikz \node[paper] {\reftext{Pear23}\cite{pearton2023}}; \tikz \node[paper] {\reftext{Maxi23}\cite{maximenko2023}}; \tikz \node[paper] {\reftext{Khan23}\cite{khanna2023}}; \tikz \node[paper] {\reftext{Nouk20}\cite{nouketcha2020}}; \tikz \node[paper, calculated] {\reftext{Vasc19}\cite{vasconcelos2019}}; \tikz \node[paper, calculated] {\reftext{Janz08}\cite{janzen2008}}; \tikz \node[paper] {\reftext{Ayal04}\cite{ayalew2004}}; \tikz \node[paper, calculated] {\reftext{Flor03}\cite{flores2003}}; \tikz \node[paper, calculated] {\reftext{Zhao00}\cite{zhao2000}}; \tikz \node[paper] {\reftext{Lade00}\cite{ladesmartin2000}};};
\node[value, scale=2.000000] (hvalue3) at (h3.west) {\num{0.82}};
\node[ref, lwh] (h4) at (h3.north west) {\tikz \node[paper, calculated] {\reftext{Ishi24}\cite{ishikawa2024}}; \tikz \node[paper, calculated] {\reftext{Rakh20}\cite{rakheja2020}}; \tikz \node[paper, calculated] {\reftext{Klah20}\cite{klahold2020}}; \tikz \node[paper, calculated] {\reftext{Kimo14a}\cite{kimoto2014a}}; \tikz \node[paper, calculated] {\reftext{Feng04a}\cite{feng2004a}}; \tikz \node[paper, calculated] {\reftext{Kohl03}\cite{kohlscheen2003}}; \tikz \node[paper, calculated] {\reftext{Son00}\cite{son2000}};};
\node[value, scale=1.700000] (hvalue4) at (h4.west) {\num{0.91}};
\node[ref, lwh] (h5) at (h4.north west) {\tikz \node[paper] {\reftext{Scaj13a}\cite{scajev2013a}};};
\node[value, scale=1.100000] (hvalue5) at (h5.west) {\num{0.94}};
\node[ref, lwh] (h6) at (h5.north west) {\tikz \node[paper] {\reftext{Ioff23}\cite{ioffe2023}}; \tikz \node[paper] {\reftext{Song12}\cite{song2012}}; \tikz \node[paper] {\reftext{Tama08a}\cite{tamaki2008a}}; \tikz \node[paper] {\reftext{Neim06}\cite{neimontas2006}}; \tikz \node[paper] {\reftext{Fang05}\cite{fang2005}}; \tikz \node[paper] {\reftext{Levi01}\cite{levinshtein2001}}; \tikz \node[paper] {\reftext{Ivan00}\cite{ivanov2000}}; \tikz \node[paper] {\reftext{Hemm97}\cite{hemmingsson1997}}; \tikz \node[paper] {\reftext{Kuzn95}\cite{kuznetsov1995}}; \tikz \node[paper] {\reftext{Scho94}\cite{schoner1994}}; \tikz \node[paper] {\reftext{Pens93}\cite{pensl1993}};};
\node[value, scale=2.100000] (hvalue6) at (h6.west) {\num{1.00}};
\node[ref, lwh] (h7) at (h6.north west) {\tikz \node[paper] {\reftext{Yang19}\cite{yang2019}}; \tikz \node[paper] {\reftext{Bion12}\cite{biondo2012}}; \tikz \node[paper] {\reftext{Rayn10}\cite{raynaud2010}}; \tikz \node[paper] {\reftext{Alba10}\cite{albanese2010}}; \tikz \node[paper] {\reftext{Pere06}\cite{perez-tomas2006}}; \tikz \node[paper] {\reftext{Lee02}\cite{lee2002}}; \tikz \node[paper] {\reftext{Shah98}\cite{shah1998}}; \tikz \node[paper] {\reftext{Huan98}\cite{huang1998}};};
\node[value, scale=1.800000] (hvalue7) at (h7.west) {\num{1.20}};
\node[ref, lwh] (h8) at (h7.north west) {\tikz \node[paper] {\reftext{Resh05}\cite{reshanov2005}};};
\node[value, scale=1.100000] (hvalue8) at (h8.west) {\num{1.26}};
\node[ref, lwh] (h9) at (h8.north west) {\tikz \node[paper, calculated] {\reftext{Pers05}\cite{persson2005}}; \tikz \node[paper, calculated] {\reftext{Son04}\cite{son2004}}; \tikz \node[paper, calculated] {\reftext{Pers99b}\cite{persson1999b}}; \tikz \node[paper, calculated] {\reftext{Bako97}\cite{bakowski1997}};};
\node[value, scale=1.400000] (hvalue9) at (h9.west) {\num{1.29}};
\node[ref, lwh] (h10) at (h9.north west) {\tikz \node[paper, calculated] {\reftext{Pers99b}\cite{persson1999b}}; \tikz \node[paper, calculated] {\reftext{Pers97}\cite{persson1997}};};
\node[value, scale=1.200000] (hvalue10) at (h10.west) {\num{1.30}};
\node[ref, lwh] (h11) at (h10.north west) {\tikz \node[paper, calculated] {\reftext{Pers97}\cite{persson1997}};};
\node[value, scale=1.100000] (hvalue11) at (h11.west) {\num{1.31}};
\node[ref, lwh] (h12) at (h11.north west) {\tikz \node[paper, calculated] {\reftext{Lamb97}\cite{lambrecht1997}};};
\node[value, scale=1.100000] (hvalue12) at (h12.west) {\num{1.34}};
\node[ref, lwh] (h13) at (h12.north west) {\tikz \node[paper, calculated] {\reftext{Pers98a}\cite{persson1998a}};};
\node[value, scale=1.100000] (hvalue13) at (h13.west) {\num{1.41}};
\node[ref, lwh] (h14) at (h13.north west) {\tikz \node[paper, calculated] {\reftext{Dong04}\cite{dong2004}};};
\node[value, scale=1.100000] (hvalue14) at (h14.west) {\num{1.45}};
\node[ref, lwh] (h15) at (h14.north west) {\tikz \node[paper, calculated] {\reftext{Lind98}\cite{lindefelt1998}};};
\node[value, scale=1.100000] (hvalue15) at (h15.west) {\num{1.87}};
\node[ref, lwh] (h16) at (h15.north west) {\tikz \node[paper, calculated] {\reftext{Lu21}\cite{lu2021}};};
\node[value, scale=1.100000] (hvalue16) at (h16.west) {\num{1.97}};
\node[ref, lwh] (h17) at (h16.north west) {\tikz \node[paper] {\reftext{Sozz19}\cite{sozzi2019}}; \tikz \node[paper] {\reftext{Nipo16}\cite{nipoti2016}};};
\node[value, scale=1.200000] (hvalue17) at (h17.west) {\num{2.60}};
\node[ref, lwh] (h18) at (h17.north west) {\tikz \node[paper] {\reftext{Luo20}\cite{luo2020}}; \tikz \node[paper] {\reftext{Hata13}\cite{hatakeyama2013}};};
\node[value, scale=1.200000] (hvalue18) at (h18.west) {\num{2.64}};
\node[ref, lwh] (h19) at (h18.north west) {\tikz \node[paper, calculated] {\reftext{Pern05}\cite{pernot2005}};};
\node[value, scale=1.100000] (hvalue19) at (h19.west) {\num{2.65}};
\node[ref, lwh] (h20) at (h19.north west) {\tikz \node[paper, calculated] {\reftext{Kack94}\cite{kackell1994}};};
\node[value, scale=1.100000] (hvalue20) at (h20.west) {\num{2.91}};
\node[ref, lwh] (h21) at (h20.north west) {\tikz \node[paper, calculated] {\reftext{Kaec96}\cite{kaeckell1996}};};
\node[value, scale=1.100000] (hvalue21) at (h21.west) {\num{5.22}};


==> data/dos_dosmass_stat.tex <==
\addplot+ [ boxplot prepared = { lower whisker=0.1900, lower quartile=0.3450, median=0.3700, upper quartile=0.3900, upper whisker=0.4200, },] coordinates {} node[mean,anchor=west] at (boxplot box cs: \boxplotvalue{upper whisker},0.5) {\pgfmathprintnumber{\boxplotvalue{median}}};
\addplot+ [ boxplot prepared = { lower whisker=0.1760, lower quartile=0.3600, median=0.4100, upper quartile=0.4225, upper whisker=0.4800, },] coordinates {} node[mean,anchor=west] at (boxplot box cs: \boxplotvalue{upper whisker},0.5) {\pgfmathprintnumber{\boxplotvalue{median}}};
\addplot+ [ boxplot prepared = { lower whisker=0.1900, lower quartile=0.2800, median=0.3100, upper quartile=0.3300, upper whisker=0.4800, },] coordinates {} node[mean,anchor=west] at (boxplot box cs: \boxplotvalue{upper whisker},0.5) {\pgfmathprintnumber{\boxplotvalue{median}}};
\addplot+ [ boxplot prepared = { lower whisker=0.5000, lower quartile=0.8200, median=0.8500, upper quartile=1.0900, upper whisker=2.6000, },] coordinates {} node[mean,anchor=west] at (boxplot box cs: \boxplotvalue{median},0.5) {\pgfmathprintnumber{\boxplotvalue{median}}};
\addplot+ [ boxplot prepared = { lower whisker=0.4800, lower quartile=0.7650, median=0.8050, upper quartile=0.8400, upper whisker=0.8400, },] coordinates {} node[mean,anchor=west] at (boxplot box cs: \boxplotvalue{upper whisker},0.5) {\pgfmathprintnumber{\boxplotvalue{median}}};
\addplot+ [ boxplot prepared = { lower whisker=0.4300, lower quartile=0.7150, median=0.7800, upper quartile=0.8000, upper whisker=0.8800, },] coordinates {} node[mean,anchor=west] at (boxplot box cs: \boxplotvalue{upper whisker},0.5) {\pgfmathprintnumber{\boxplotvalue{median}}};
\addplot+ [ boxplot prepared = { lower whisker=0.5400, lower quartile=0.5900, median=0.6200, upper quartile=1.4600, upper whisker=3.1900, },] coordinates {} node[mean,anchor=west] at (boxplot box cs: \boxplotvalue{median},0.5) {\pgfmathprintnumber{\boxplotvalue{median}}};
\addplot+ [ boxplot prepared = { lower whisker=0.4500, lower quartile=0.5375, median=0.5850, upper quartile=0.5900, upper whisker=0.6200, },] coordinates {} node[mean,anchor=west] at (boxplot box cs: \boxplotvalue{upper whisker},0.5) {\pgfmathprintnumber{\boxplotvalue{median}}};
\addplot+ [ boxplot prepared = { lower whisker=0.6100, lower quartile=1.2100, median=1.4900, upper quartile=1.5000, upper whisker=1.5800, },] coordinates {} node[mean,anchor=east] at (boxplot box cs: \boxplotvalue{median},0.5) {\pgfmathprintnumber{\boxplotvalue{median}}};
\addplot+ [ boxplot prepared = { lower whisker=1.4800, lower quartile=1.5600, median=1.6000, upper quartile=1.6400, upper whisker=1.7500, },] coordinates {} node[mean,anchor=west] at (boxplot box cs: \boxplotvalue{upper whisker},0.5) {\pgfmathprintnumber{\boxplotvalue{median}}};
\addplot+ [ boxplot prepared = { lower whisker=1.3200, lower quartile=1.4450, median=1.5550, upper quartile=1.6300, upper whisker=1.7300, },] coordinates {} node[mean,anchor=west] at (boxplot box cs: \boxplotvalue{upper whisker},0.5) {\pgfmathprintnumber{\boxplotvalue{median}}};
\addplot+ [ boxplot prepared = { lower whisker=0.2100, lower quartile=0.2100, median=0.2100, upper quartile=0.2100, upper whisker=0.2200, },] coordinates {} node[mean,anchor=west] at (boxplot box cs: \boxplotvalue{upper whisker},0.5) {\pgfmathprintnumber{\boxplotvalue{median}}};


==> data/dos_mass_stat.tex <==
\addplot+ [ boxplot prepared = { lower whisker=0.4300, lower quartile=0.5625, median=0.5800, upper quartile=0.6125, upper whisker=1.2000, },] coordinates {} node[mean,anchor=east] at (boxplot box cs: \boxplotvalue{lower whisker},0.5) {\pgfmathprintnumber{\boxplotvalue{median}}};
\addplot+ [ boxplot prepared = { lower whisker=0.1300, lower quartile=0.2700, median=0.2800, upper quartile=0.3100, upper whisker=0.4300, },] coordinates {} node[mean,anchor=west] at (boxplot box cs: \boxplotvalue{upper whisker},0.5) {\pgfmathprintnumber{\boxplotvalue{median}}};
\addplot+ [ boxplot prepared = { lower whisker=0.1900, lower quartile=0.3000, median=0.3100, upper quartile=0.3400, upper whisker=0.3900, },] coordinates {} node[mean,anchor=west] at (boxplot box cs: \boxplotvalue{upper whisker},0.5) {\pgfmathprintnumber{\boxplotvalue{median}}};
\addplot+ [ boxplot prepared = { lower whisker=0.5400, lower quartile=0.6200, median=0.8600, upper quartile=3.5000, upper whisker=4.2300, },] coordinates {} node[mean,anchor=west] at (boxplot box cs: \boxplotvalue{median},0.5) {\pgfmathprintnumber{\boxplotvalue{median}}};
\addplot+ [ boxplot prepared = { lower whisker=0.5400, lower quartile=0.7450, median=1.8200, upper quartile=2.7250, upper whisker=3.0400, },] coordinates {} node[mean,anchor=west] at (boxplot box cs: \boxplotvalue{median},0.5) {\pgfmathprintnumber{\boxplotvalue{median}}};
\addplot+ [ boxplot prepared = { lower whisker=1.4800, lower quartile=1.5000, median=1.5800, upper quartile=1.6850, upper whisker=1.7300, },] coordinates {} node[mean,anchor=east] at (boxplot box cs: \boxplotvalue{lower whisker},0.5) {\pgfmathprintnumber{\boxplotvalue{median}}};


==> data/dos_ref_chain_e.tex <==
\node[desc] at (0,0.000000*\dy) {Electron ($\mde$ $\mid$ $\mdeperp$, $\memg$, $\memk$ $\mid$ $\mdepara$, $\meml$)};
\node[author] at (0,-1.500000*\dy) {\citeauthor{lomakina1973}};
\node[fund, ref] (lomakina1973) at (0,-2.500000*\dy) {\reftext{Loma73}\cite{lomakina1973} (  -- $\mid$ 0.21 , -- , -- $\mid$ 0.19 , --  )};
\coordinate (lomakina1973C) at ($(lomakina1973.west)+(\dxStart+\dy,0)$);
\node[ ref] (harris1995) at ($(lomakina1973C |- 0,-3.500000*\dy)$) {\reftext{Harr95}\cite{harris1995} (  -- $\mid$ M , -- , -- $\mid$ M , --  )};
\draw (harris1995.west) -| ++(-\dy,\fy*\dy);
\coordinate (harris1995C) at ($(harris1995.west)+(\dxStart+\dy,0)$);
\node[ ref] (perez-tomas2006) at ($(harris1995C |- 0,-4.500000*\dy)$) {\reftext{Pere06}\cite{perez-tomas2006} (  0.38 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (perez-tomas2006.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-6.500000*\dy) {\citeauthor{tairov1977}};
\node[ ref] (tairov1977) at (0,-7.500000*\dy) {\reftext{Tair77}\cite{tairov1977} (  M $\mid$ M , -- , -- $\mid$ M , --  )};
\coordinate (tairov1977C) at ($(tairov1977.west)+(\dxStart+\dy,0)$);
\node[ ref] (ikeda1980) at ($(tairov1977C |- 0,-8.500000*\dy)$) {\reftext{Iked80}\cite{ikeda1980} (  0.37 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (ikeda1980.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-10.500000*\dy) {\citeauthor{look1983}};
\node[no4H, ref] (look1983) at (0,-11.500000*\dy) {\reftext{Look83}\cite{look1983} (  -- $\mid$ -- , -- , -- $\mid$ -- , --  )};
\coordinate (look1983C) at ($(look1983.west)+(\dxStart+\dy,0)$);
\node[ ref] (fang2005) at ($(look1983C |- 0,-12.500000*\dy)$) {\reftext{Fang05}\cite{fang2005} (  0.4 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (fang2005.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-14.500000*\dy) {\citeauthor{gotz1993}};
\node[fund, ref] (gotz1993) at (0,-15.500000*\dy) {\reftext{Gotz93}\cite{gotz1993} (  0.19 $\mid$ 0.176 , -- , -- $\mid$ 0.224 , --  )};
\coordinate (gotz1993C) at ($(gotz1993.west)+(\dxStart+\dy,0)$);
\node[ ref] (pensl1993) at ($(gotz1993C |- 0,-16.500000*\dy)$) {\reftext{Pens93}\cite{pensl1993} (  0.19 $\mid$ 0.17 , -- , -- $\mid$ 0.22 , --  )};
\draw (pensl1993.west) -| ++(-\dy,\fy*\dy);
\coordinate (pensl1993C) at ($(pensl1993.west)+(\dxStart+\dy,0)$);
\node[ ref] (kuznetsov1995) at ($(pensl1993C |- 0,-17.500000*\dy)$) {\reftext{Kuzn95}\cite{kuznetsov1995} (  0.19 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (kuznetsov1995.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (schadt1994a) at ($(pensl1993.west |- 0,-18.500000*\dy)$) {\reftext{Scha94a}\cite{schadt1994a} (  0.19 $\mid$ 0.17 , -- , -- $\mid$ 0.22 , --  )};
\draw (schadt1994a.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (schoner1994) at ($(schadt1994a.west |- 0,-19.500000*\dy)$) {\reftext{Scho94}\cite{schoner1994} (  0.19 $\mid$ 0.18 , -- , -- $\mid$ 0.22 , --  )};
\draw (schoner1994.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (harris1995) at ($(schoner1994.west |- 0,-20.500000*\dy)$) {\reftext{Harr95}\cite{harris1995} (  -- $\mid$ M , -- , -- $\mid$ M , --  )};
\draw (harris1995.west) -| ++(-\dy,\fy*\dy);
\coordinate (harris1995C) at ($(harris1995.west)+(\dxStart+\dy,0)$);
\node[ ref] (perez-tomas2006) at ($(harris1995C |- 0,-21.500000*\dy)$) {\reftext{Pere06}\cite{perez-tomas2006} (  0.38 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (perez-tomas2006.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (itoh1995) at ($(harris1995.west |- 0,-22.500000*\dy)$) {\reftext{Itoh95}\cite{itoh1995} (  0.20 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (itoh1995.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (arpatzanis2006) at ($(itoh1995.west |- 0,-23.500000*\dy)$) {\reftext{Arpa06}\cite{arpatzanis2006} (  0.20 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (arpatzanis2006.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (rodrigues2021) at ($(arpatzanis2006.west |- 0,-24.500000*\dy)$) {\reftext{Rodr21}\cite{rodrigues2021} (  -- $\mid$ 0.18 , -- , -- $\mid$ 0.22 , --  )};
\draw (rodrigues2021.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-26.500000*\dy) {\citeauthor{son1994}};
\node[no4H, ref] (son1994) at (0,-27.500000*\dy) {\reftext{Son94}\cite{son1994} (  -- $\mid$ -- , -- , -- $\mid$ -- , --  )};
\coordinate (son1994C) at ($(son1994.west)+(\dxStart+\dy,0)$);
\node[ ref] (bechstedt1998) at ($(son1994C |- 0,-28.500000*\dy)$) {\reftext{Bech98}\cite{bechstedt1998} (  -- $\mid$ -- , M , M $\mid$ -- , M  )};
\draw (bechstedt1998.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-30.500000*\dy) {\citeauthor{harima1995}};
\node[fund, ref] (harima1995) at (0,-31.500000*\dy) {\reftext{Hari95}\cite{harima1995} (  -- $\mid$ 0.3 , -- , -- $\mid$ 0.48 , --  )};
\coordinate (harima1995C) at ($(harima1995.west)+(\dxStart+\dy,0)$);
\node[ ref] (nakashima1997) at ($(harima1995C |- 0,-32.500000*\dy)$) {\reftext{Naka97}\cite{nakashima1997} (  -- $\mid$ 0.3 , -- , -- $\mid$ 0.48 , --  )};
\draw (nakashima1997.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (harima1998) at ($(nakashima1997.west |- 0,-33.500000*\dy)$) {\reftext{Hari98}\cite{harima1998} (  -- $\mid$ -- , -- , -- $\mid$ 0.48 , --  )};
\draw (harima1998.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (gao2022a) at ($(harima1998.west |- 0,-34.500000*\dy)$) {\reftext{Gao22a}\cite{gao2022a} (  -- $\mid$ -- , -- , -- $\mid$ 0.48 , --  )};
\draw (gao2022a.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-36.500000*\dy) {\citeauthor{karch1995}};
\node[fund, ref] (karch1995) at (0,-37.500000*\dy) {\reftext{Karc95}\cite{karch1995} (  -- $\mid$ -- , 0.66 , 0.31 $\mid$ -- , 0.3  )};
\coordinate (karch1995C) at ($(karch1995.west)+(\dxStart+\dy,0)$);
\node[ ref] (bechstedt1998) at ($(karch1995C |- 0,-38.500000*\dy)$) {\reftext{Bech98}\cite{bechstedt1998} (  -- $\mid$ -- , M , M $\mid$ -- , M  )};
\draw (bechstedt1998.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (pensl2005) at ($(bechstedt1998.west |- 0,-39.500000*\dy)$) {\reftext{Pens05}\cite{pensl2005} (  -- $\mid$ -- , M , M $\mid$ -- , M  )};
\draw (pensl2005.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-41.500000*\dy) {\citeauthor{lambrecht1995}};
\node[fund, ref] (lambrecht1995) at (0,-42.500000*\dy) {\reftext{Lamb95}\cite{lambrecht1995} (  -- $\mid$ 0.4 , 0.58 , 0.28 $\mid$ 0.27 , 0.31  )};
\coordinate (lambrecht1995C) at ($(lambrecht1995.west)+(\dxStart+\dy,0)$);
\node[ ref] (lambrecht1997) at ($(lambrecht1995C |- 0,-43.500000*\dy)$) {\reftext{Lamb97}\cite{lambrecht1997} (  -- $\mid$ -- , 0.58 , 0.28 $\mid$ -- , 0.31  )};
\draw (lambrecht1997.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (bechstedt1998) at ($(lambrecht1997.west |- 0,-44.500000*\dy)$) {\reftext{Bech98}\cite{bechstedt1998} (  -- $\mid$ -- , M , M $\mid$ -- , M  )};
\draw (bechstedt1998.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (pennington2004) at ($(bechstedt1998.west |- 0,-45.500000*\dy)$) {\reftext{Penn04}\cite{pennington2004} (  0.41 $\mid$ -- , 0.58 , 0.29 $\mid$ -- , 0.33  )};
\draw (pennington2004.west) -| ++(-\dy,\fy*\dy);
\coordinate (pennington2004C) at ($(pennington2004.west)+(\dxStart+\dy,0)$);
\node[ ref] (tilak2007) at ($(pennington2004C |- 0,-46.500000*\dy)$) {\reftext{Tila07}\cite{tilak2007} (  0.41 $\mid$ 0.42 , -- , -- $\mid$ -- , --  )};
\draw (tilak2007.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,0.000000*\dy) {\citeauthor{son1995}};
\node[fund, ref] (son1995) at (\xSepOne,-1.000000*\dy) {\reftext{Son95}\cite{son1995} (  -- $\mid$ 0.42 , -- , -- $\mid$ 0.29 , --  )};
\coordinate (son1995C) at ($(son1995.west)+(\dxStart+\dy,0)$);
\node[ ref] (joshi1995) at ($(son1995C |- 0,-2.000000*\dy)$) {\reftext{Josh95}\cite{joshi1995} (  -- $\mid$ 0.42 , -- , -- $\mid$ 0.29 , --  )};
\draw (joshi1995.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (ivanov2000) at ($(joshi1995.west |- 0,-3.000000*\dy)$) {\reftext{Ivan00}\cite{ivanov2000} (  0.37 $\mid$ 0.42 , -- , -- $\mid$ 0.29 , --  )};
\draw (ivanov2000.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (levinshtein2001) at ($(ivanov2000.west |- 0,-4.000000*\dy)$) {\reftext{Levi01}\cite{levinshtein2001} (  0.37 $\mid$ 0.42 , -- , -- $\mid$ 0.29 , --  )};
\draw (levinshtein2001.west) -| ++(-\dy,\fy*\dy);
\coordinate (levinshtein2001C) at ($(levinshtein2001.west)+(\dxStart+\dy,0)$);
\node[ ref] (tamaki2008a) at ($(levinshtein2001C |- 0,-5.000000*\dy)$) {\reftext{Tama08a}\cite{tamaki2008a} (  0.3713 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (tamaki2008a.west) -| ++(-\dy,\fy*\dy);
\coordinate (tamaki2008aC) at ($(tamaki2008a.west)+(\dxStart+\dy,0)$);
\node[ ref] (song2012) at ($(tamaki2008aC |- 0,-6.000000*\dy)$) {\reftext{Song12}\cite{song2012} (  0.3713 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (song2012.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (albanese2010) at ($(levinshtein2001.west |- 0,-7.000000*\dy)$) {\reftext{Alba10}\cite{albanese2010} (  0.37 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (albanese2010.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (yang2019) at ($(albanese2010.west |- 0,-8.000000*\dy)$) {\reftext{Yang19}\cite{yang2019} (  0.36 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (yang2019.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (ioffe2023) at ($(yang2019.west |- 0,-9.000000*\dy)$) {\reftext{Ioff23}\cite{ioffe2023} (  0.37 $\mid$ 0.42 , -- , -- $\mid$ 0.29 , --  )};
\draw (ioffe2023.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-11.000000*\dy) {\citeauthor{wenzien1995}};
\node[fund, ref] (wenzien1995) at (\xSepOne,-12.000000*\dy) {\reftext{Wenz95}\cite{wenzien1995} (  -- $\mid$ -- , 0.6 , 0.28 $\mid$ -- , 0.19  )};
\coordinate (wenzien1995C) at ($(wenzien1995.west)+(\dxStart+\dy,0)$);
\node[ ref] (bechstedt1998) at ($(wenzien1995C |- 0,-13.000000*\dy)$) {\reftext{Bech98}\cite{bechstedt1998} (  -- $\mid$ -- , M , M $\mid$ -- , M  )};
\draw (bechstedt1998.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-15.000000*\dy) {\citeauthor{nilsson1996}};
\node[fund, ref] (nilsson1996) at (\xSepOne,-16.000000*\dy) {\reftext{Nils96}\cite{nilsson1996} (  -- $\mid$ -- , M , M $\mid$ -- , M  )};
\coordinate (nilsson1996C) at ($(nilsson1996.west)+(\dxStart+\dy,0)$);
\node[ ref] (mickevicius1998) at ($(nilsson1996C |- 0,-17.000000*\dy)$) {\reftext{Mick98}\cite{mickevicius1998} (  -- $\mid$ 0.42 , -- , -- $\mid$ 0.28 , --  )};
\draw (mickevicius1998.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (mickevicius1998a) at ($(mickevicius1998.west |- 0,-18.000000*\dy)$) {\reftext{Mick98a}\cite{mickevicius1998a} (  -- $\mid$ 0.42 , -- , -- $\mid$ 0.28 , --  )};
\draw (mickevicius1998a.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-20.000000*\dy) {\citeauthor{persson1996}};
\node[fund, ref] (persson1996) at (\xSepOne,-21.000000*\dy) {\reftext{Pers96}\cite{persson1996} (  -- $\mid$ -- , 0.57 , 0.28 $\mid$ -- , 0.31  )};
\coordinate (persson1996C) at ($(persson1996.west)+(\dxStart+\dy,0)$);
\node[ ref] (bakowski1997) at ($(persson1996C |- 0,-22.000000*\dy)$) {\reftext{Bako97}\cite{bakowski1997} (  0.37 $\mid$ -- , 0.57 , 0.28 $\mid$ -- , 0.31  )};
\draw (bakowski1997.west) -| ++(-\dy,\fy*\dy);
\coordinate (bakowski1997C) at ($(bakowski1997.west)+(\dxStart+\dy,0)$);
\node[ ref] (huang1998) at ($(bakowski1997C |- 0,-23.000000*\dy)$) {\reftext{Huan98}\cite{huang1998} (  0.37 $\mid$ -- , 0.57 , 0.28 $\mid$ -- , 0.31  )};
\draw (huang1998.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (shah1998) at ($(huang1998.west |- 0,-24.000000*\dy)$) {\reftext{Shah98}\cite{shah1998} (  0.37 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (shah1998.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (lee2002) at ($(shah1998.west |- 0,-25.000000*\dy)$) {\reftext{Lee02}\cite{lee2002} (  0.37 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (lee2002.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (bechstedt1998) at ($(bakowski1997.west |- 0,-26.000000*\dy)$) {\reftext{Bech98}\cite{bechstedt1998} (  -- $\mid$ -- , M , M $\mid$ -- , M  )};
\draw (bechstedt1998.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (kinoshita1998) at ($(bechstedt1998.west |- 0,-27.000000*\dy)$) {\reftext{Kino98}\cite{kinoshita1998} (  -- $\mid$ -- , 0.57 , 0.28 $\mid$ -- , 0.31  )};
\draw (kinoshita1998.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (persson1999a) at ($(kinoshita1998.west |- 0,-28.000000*\dy)$) {\reftext{Pers99a}\cite{persson1999a} (  -- $\mid$ -- , 0.57 , 0.28 $\mid$ -- , 0.31  )};
\draw (persson1999a.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (persson1999b) at ($(persson1999a.west |- 0,-29.000000*\dy)$) {\reftext{Pers99b}\cite{persson1999b} (  -- $\mid$ -- , 0.57 , 0.28 $\mid$ -- , 0.31  )};
\draw (persson1999b.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (pensl2005) at ($(persson1999b.west |- 0,-30.000000*\dy)$) {\reftext{Pens05}\cite{pensl2005} (  -- $\mid$ -- , M , M $\mid$ -- , M  )};
\draw (pensl2005.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-32.000000*\dy) {\citeauthor{volm1996}};
\node[fund, ref] (volm1996) at (\xSepOne,-33.000000*\dy) {\reftext{Volm96}\cite{volm1996} (  -- $\mid$ -- , 0.58 , 0.31 $\mid$ -- , 0.33  )};
\coordinate (volm1996C) at ($(volm1996.west)+(\dxStart+\dy,0)$);
\node[ ref] (devaty1997) at ($(volm1996C |- 0,-34.000000*\dy)$) {\reftext{Deva97}\cite{devaty1997} (  -- $\mid$ -- , 0.58 , 0.31 $\mid$ -- , 0.33  )};
\draw (devaty1997.west) -| ++(-\dy,\fy*\dy);
\coordinate (devaty1997C) at ($(devaty1997.west)+(\dxStart+\dy,0)$);
\node[ ref] (camassel2008) at ($(devaty1997C |- 0,-35.000000*\dy)$) {\reftext{Cama08}\cite{camassel2008} (  -- $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (camassel2008.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (galeckas1997) at ($(devaty1997.west |- 0,-36.000000*\dy)$) {\reftext{Gale97}\cite{galeckas1997} (  -- $\mid$ -- , 0.58 , -- $\mid$ -- , --  )};
\draw (galeckas1997.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (hemmingsson1997) at ($(galeckas1997.west |- 0,-37.000000*\dy)$) {\reftext{Hemm97}\cite{hemmingsson1997} (  0.37 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (hemmingsson1997.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (bechstedt1998) at ($(hemmingsson1997.west |- 0,-38.000000*\dy)$) {\reftext{Bech98}\cite{bechstedt1998} (  -- $\mid$ -- , M , M $\mid$ -- , M  )};
\draw (bechstedt1998.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (chen2000) at ($(bechstedt1998.west |- 0,-39.000000*\dy)$) {\reftext{Chen00}\cite{chen2000} (  -- $\mid$ -- , 0.58 , 0.31 $\mid$ -- , 0.33  )};
\draw (chen2000.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (ladesmartin2000) at ($(chen2000.west |- 0,-40.000000*\dy)$) {\reftext{Lade00}\cite{ladesmartin2000} (  0.39 $\mid$ -- , 0.58 , 0.31 $\mid$ -- , 0.33  )};
\draw (ladesmartin2000.west) -| ++(-\dy,\fy*\dy);
\coordinate (ladesmartin2000C) at ($(ladesmartin2000.west)+(\dxStart+\dy,0)$);
\node[ ref] (rakheja2020) at ($(ladesmartin2000C |- 0,-41.000000*\dy)$) {\reftext{Rakh20}\cite{rakheja2020} (  -- $\mid$ -- , 0.58 , 0.31 $\mid$ -- , 0.33  )};
\draw (rakheja2020.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (pernot2000) at ($(ladesmartin2000.west |- 0,-42.000000*\dy)$) {\reftext{Pern00}\cite{pernot2000} (  -- $\mid$ -- , 0.58 , 0.31 $\mid$ -- , 0.33  )};
\draw (pernot2000.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (ivanov2003a) at ($(pernot2000.west |- 0,-43.000000*\dy)$) {\reftext{Ivan03a}\cite{ivanov2003a} (  -- $\mid$ -- , 0.58 , 0.31 $\mid$ -- , 0.33  )};
\draw (ivanov2003a.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (ayalew2004) at ($(ivanov2003a.west |- 0,-44.000000*\dy)$) {\reftext{Ayal04}\cite{ayalew2004} (  0.39 $\mid$ -- , 0.58 , 0.31 $\mid$ -- , 0.33  )};
\draw (ayalew2004.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (feng2004a) at ($(ayalew2004.west |- 0,-45.000000*\dy)$) {\reftext{Feng04a}\cite{feng2004a} (  -- $\mid$ -- , 0.58 , 0.31 $\mid$ -- , 0.33  )};
\draw (feng2004a.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (negoro2004a) at ($(feng2004a.west |- 0,-46.000000*\dy)$) {\reftext{Nego04a}\cite{negoro2004a} (  0.39 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (negoro2004a.west) -| ++(-\dy,\fy*\dy);
\coordinate (negoro2004aC) at ($(negoro2004a.west)+(\dxStart+\dy,0)$);
\node[ ref] (kim2024) at ($(negoro2004aC |- 0,-47.000000*\dy)$) {\reftext{Kim24}\cite{kim2024} (  0.20 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (kim2024.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (pensl2005) at ($(negoro2004a.west |- 0,-48.000000*\dy)$) {\reftext{Pens05}\cite{pensl2005} (  -- $\mid$ -- , M , M $\mid$ -- , M  )};
\draw (pensl2005.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (kimoto2014a) at ($(pensl2005.west |- 0,-49.000000*\dy)$) {\reftext{Kimo14a}\cite{kimoto2014a} (  -- $\mid$ 0.42 , 0.58 , 0.31 $\mid$ 0.33 , 0.33  )};
\draw (kimoto2014a.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (klahold2020) at ($(kimoto2014a.west |- 0,-50.000000*\dy)$) {\reftext{Klah20}\cite{klahold2020} (  -- $\mid$ -- , 0.58 , 0.31 $\mid$ -- , 0.33  )};
\draw (klahold2020.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (ishikawa2021) at ($(klahold2020.west |- 0,-51.000000*\dy)$) {\reftext{Ishi21}\cite{ishikawa2021} (  -- $\mid$ -- , 0.58 , 0.31 $\mid$ -- , 0.33  )};
\draw (ishikawa2021.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (khanna2023) at ($(ishikawa2021.west |- 0,-52.000000*\dy)$) {\reftext{Khan23}\cite{khanna2023} (  0.39 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (khanna2023.west) -| ++(-\dy,\fy*\dy);
\coordinate (khanna2023C) at ($(khanna2023.west)+(\dxStart+\dy,0)$);
\node[ ref] (nouketcha2020) at ($(khanna2023C |- 0,-53.000000*\dy)$) {\reftext{Nouk20}\cite{nouketcha2020} (  0.39 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (nouketcha2020.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (maximenko2023) at ($(khanna2023.west |- 0,-54.000000*\dy)$) {\reftext{Maxi23}\cite{maximenko2023} (  0.39 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (maximenko2023.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (pearton2023) at ($(maximenko2023.west |- 0,-55.000000*\dy)$) {\reftext{Pear23}\cite{pearton2023} (  0.39 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (pearton2023.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,0.000000*\dy) {\citeauthor{persson1997}};
\node[fund, ref] (persson1997) at (\xSepOne + \xSepTwo,-1.000000*\dy) {\reftext{Pers97}\cite{persson1997} (  -- $\mid$ -- , M , M $\mid$ -- , M  )};
\coordinate (persson1997C) at ($(persson1997.west)+(\dxStart+\dy,0)$);
\node[ ref] (lindefelt1998) at ($(persson1997C |- 0,-2.000000*\dy)$) {\reftext{Lind98}\cite{lindefelt1998} (  -- $\mid$ -- , 0.58 , 0.28 $\mid$ -- , 0.31  )};
\draw (lindefelt1998.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (persson1998a) at ($(lindefelt1998.west |- 0,-3.000000*\dy)$) {\reftext{Pers98a}\cite{persson1998a} (  M $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (persson1998a.west) -| ++(-\dy,\fy*\dy);
\coordinate (persson1998aC) at ($(persson1998a.west)+(\dxStart+\dy,0)$);
\node[ ref] (scajev2013a) at ($(persson1998aC |- 0,-4.000000*\dy)$) {\reftext{Scaj13a}\cite{scajev2013a} (  0.37 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (scajev2013a.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (iwata2000) at ($(persson1998a.west |- 0,-5.000000*\dy)$) {\reftext{Iwat00}\cite{iwata2000} (  -- $\mid$ -- , 0.57 , 0.28 $\mid$ -- , 0.31  )};
\draw (iwata2000.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (iwata2000a) at ($(iwata2000.west |- 0,-6.000000*\dy)$) {\reftext{Iwat00a}\cite{iwata2000a} (  -- $\mid$ -- , 0.57 , 0.28 $\mid$ -- , 0.31  )};
\draw (iwata2000a.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (iwata2001) at ($(iwata2000a.west |- 0,-7.000000*\dy)$) {\reftext{Iwat01}\cite{iwata2001} (  -- $\mid$ -- , 0.57 , 0.28 $\mid$ -- , 0.31  )};
\draw (iwata2001.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (son2004) at ($(iwata2001.west |- 0,-8.000000*\dy)$) {\reftext{Son04}\cite{son2004} (  -- $\mid$ -- , M , M $\mid$ -- , M  )};
\draw (son2004.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (persson2005) at ($(son2004.west |- 0,-9.000000*\dy)$) {\reftext{Pers05}\cite{persson2005} (  -- $\mid$ -- , M , M $\mid$ -- , M  )};
\draw (persson2005.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (reshanov2005) at ($(persson2005.west |- 0,-10.000000*\dy)$) {\reftext{Resh05}\cite{reshanov2005} (  0.37 $\mid$ -- , 0.58 , 0.28 $\mid$ -- , 0.31  )};
\draw (reshanov2005.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (janzen2008) at ($(reshanov2005.west |- 0,-11.000000*\dy)$) {\reftext{Janz08}\cite{janzen2008} (  -- $\mid$ -- , 0.61 , 0.29 $\mid$ -- , 0.33  )};
\draw (janzen2008.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (raynaud2010) at ($(janzen2008.west |- 0,-12.000000*\dy)$) {\reftext{Rayn10}\cite{raynaud2010} (  0.37 $\mid$ -- , 0.57 , 0.28 $\mid$ -- , 0.31  )};
\draw (raynaud2010.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (biondo2012) at ($(raynaud2010.west |- 0,-13.000000*\dy)$) {\reftext{Bion12}\cite{biondo2012} (  0.8 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (biondo2012.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-15.000000*\dy) {\citeauthor{wellenhofer1997}};
\node[fund, ref] (wellenhofer1997) at (\xSepOne + \xSepTwo,-16.000000*\dy) {\reftext{Well97}\cite{wellenhofer1997} (  0.394 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\coordinate (wellenhofer1997C) at ($(wellenhofer1997.west)+(\dxStart+\dy,0)$);
\node[ ref] (sridhara1998a) at ($(wellenhofer1997C |- 0,-17.000000*\dy)$) {\reftext{Srid98a}\cite{sridhara1998a} (  -- $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (sridhara1998a.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (scaburri2011a) at ($(sridhara1998a.west |- 0,-18.000000*\dy)$) {\reftext{Scab11a}\cite{scaburri2011a} (  0.394 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (scaburri2011a.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (hatakeyama2013) at ($(scaburri2011a.west |- 0,-19.000000*\dy)$) {\reftext{Hata13}\cite{hatakeyama2013} (  0.394 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (hatakeyama2013.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (sozzi2019) at ($(hatakeyama2013.west |- 0,-20.000000*\dy)$) {\reftext{Sozz19}\cite{sozzi2019} (  0.40 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (sozzi2019.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (luo2020) at ($(sozzi2019.west |- 0,-21.000000*\dy)$) {\reftext{Luo20}\cite{luo2020} (  0.4 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (luo2020.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (yang2022) at ($(luo2020.west |- 0,-22.000000*\dy)$) {\reftext{Yang22}\cite{yang2022} (  -- $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (yang2022.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-24.000000*\dy) {\citeauthor{son2000}};
\node[fund, ref] (son2000) at (\xSepOne + \xSepTwo,-25.000000*\dy) {\reftext{Son00}\cite{son2000} (  -- $\mid$ 0.45 , -- , -- $\mid$ 0.30 , --  )};
\coordinate (son2000C) at ($(son2000.west)+(\dxStart+\dy,0)$);
\node[ ref] (kohlscheen2003) at ($(son2000C |- 0,-26.000000*\dy)$) {\reftext{Kohl03}\cite{kohlscheen2003} (  -- $\mid$ 0.45 , -- , -- $\mid$ 0.3 , --  )};
\draw (kohlscheen2003.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-28.000000*\dy) {\citeauthor{ng2010}};
\node[fund, ref] (ng2010) at (\xSepOne + \xSepTwo,-29.000000*\dy) {\reftext{Ng10}\cite{ng2010} (  -- $\mid$ -- , 0.66 , 0.31 $\mid$ -- , 0.34  )};
\coordinate (ng2010C) at ($(ng2010.west)+(\dxStart+\dy,0)$);
\node[ ref] (ng2011) at ($(ng2010C |- 0,-30.000000*\dy)$) {\reftext{Ng11}\cite{ng2011} (  -- $\mid$ -- , 0.66 , 0.31 $\mid$ -- , 0.34  )};
\draw (ng2011.west) -| ++(-\dy,\fy*\dy);


==> data/dos_ref_chain_h.tex <==
\node[desc] at (0,0.000000*\dy) {Hole ($\mdh$ $\mid$ $\mdhperp$, $\mhgm$, $\mhgk$ $\mid$ $\mdhpara$, $\mhga$)};
\node[author] at (0,-1.500000*\dy) {\citeauthor{vandaal1963}};
\node[no4H, ref] (vandaal1963) at (0,-2.500000*\dy) {\reftext{Vand63}\cite{vandaal1963} (  1 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\coordinate (vandaal1963C) at ($(vandaal1963.west)+(\dxStart+\dy,0)$);
\node[ ref] (pensl1993) at ($(vandaal1963C |- 0,-3.500000*\dy)$) {\reftext{Pens93}\cite{pensl1993} (  1 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (pensl1993.west) -| ++(-\dy,\fy*\dy);
\coordinate (pensl1993C) at ($(pensl1993.west)+(\dxStart+\dy,0)$);
\node[ ref] (kuznetsov1995) at ($(pensl1993C |- 0,-4.500000*\dy)$) {\reftext{Kuzn95}\cite{kuznetsov1995} (  1 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (kuznetsov1995.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-6.500000*\dy) {\citeauthor{kackell1994}};
\node[fund, ref] (kackell1994) at (0,-7.500000*\dy) {\reftext{Kack94}\cite{kackell1994} (  -- $\mid$ -- , M , M $\mid$ -- , M  )};
\coordinate (kackell1994C) at ($(kackell1994.west)+(\dxStart+\dy,0)$);
\node[ ref] (kaeckell1996) at ($(kackell1994C |- 0,-8.500000*\dy)$) {\reftext{Kaec96}\cite{kaeckell1996} (  -- $\mid$ -- , M , M $\mid$ -- , M  )};
\draw (kaeckell1996.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (galeckas1997) at ($(kaeckell1996.west |- 0,-9.500000*\dy)$) {\reftext{Gale97}\cite{galeckas1997} (  -- $\mid$ -- , 4.2 , -- $\mid$ -- , --  )};
\draw (galeckas1997.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-11.500000*\dy) {\citeauthor{harris1995}};
\node[ ref] (harris1995) at (0,-12.500000*\dy) {\reftext{Harr95}\cite{harris1995} (  -- $\mid$ -- , -- , -- $\mid$ -- , --  )};
\coordinate (harris1995C) at ($(harris1995.west)+(\dxStart+\dy,0)$);
\node[ ref] (perez-tomas2006) at ($(harris1995C |- 0,-13.500000*\dy)$) {\reftext{Pere06}\cite{perez-tomas2006} (  1.2 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (perez-tomas2006.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-15.500000*\dy) {\citeauthor{bakowski1997}};
\node[fund, ref] (bakowski1997) at (0,-16.500000*\dy) {\reftext{Bako97}\cite{bakowski1997} (  M $\mid$ -- , -- , -- $\mid$ -- , --  )};
\coordinate (bakowski1997C) at ($(bakowski1997.west)+(\dxStart+\dy,0)$);
\node[ ref] (huang1998) at ($(bakowski1997C |- 0,-17.500000*\dy)$) {\reftext{Huan98}\cite{huang1998} (  1.2 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (huang1998.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (shah1998) at ($(huang1998.west |- 0,-18.500000*\dy)$) {\reftext{Shah98}\cite{shah1998} (  1.2 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (shah1998.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (lee2002) at ($(shah1998.west |- 0,-19.500000*\dy)$) {\reftext{Lee02}\cite{lee2002} (  1.2 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (lee2002.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,0.000000*\dy) {\citeauthor{persson1997}};
\node[fund, ref] (persson1997) at (\xSepOne,-1.000000*\dy) {\reftext{Pers97}\cite{persson1997} (  -- $\mid$ M , -- , -- $\mid$ M , --  )};
\coordinate (persson1997C) at ($(persson1997.west)+(\dxStart+\dy,0)$);
\node[guess, ref] (ladesmartin2000) at ($(persson1997C |- 0,-2.000000*\dy)$) {\reftext{Lade00}\cite{ladesmartin2000} (  0.82 $\mid$ 0.59 , -- , -- $\mid$ 1.6 , --  )};
\draw (ladesmartin2000.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (zhao2000) at ($(ladesmartin2000.west |- 0,-3.000000*\dy)$) {\reftext{Zhao00}\cite{zhao2000} (  -- $\mid$ M , -- , -- $\mid$ M , --  )};
\draw (zhao2000.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (flores2003) at ($(zhao2000.west |- 0,-4.000000*\dy)$) {\reftext{Flor03}\cite{flores2003} (  -- $\mid$ 0.59 , -- , -- $\mid$ 1.6 , --  )};
\draw (flores2003.west) -| ++(-\dy,\fy*\dy);
\coordinate (flores2003C) at ($(flores2003.west)+(\dxStart+\dy,0)$);
\node[ ref] (vasconcelos2019) at ($(flores2003C |- 0,-5.000000*\dy)$) {\reftext{Vasc19}\cite{vasconcelos2019} (  -- $\mid$ 0.59 , -- , -- $\mid$ 1.6 , --  )};
\draw (vasconcelos2019.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (ayalew2004) at ($(flores2003.west |- 0,-6.000000*\dy)$) {\reftext{Ayal04}\cite{ayalew2004} (  0.82 $\mid$ 0.59 , -- , -- $\mid$ 1.6 , --  )};
\draw (ayalew2004.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (janzen2008) at ($(ayalew2004.west |- 0,-7.000000*\dy)$) {\reftext{Janz08}\cite{janzen2008} (  -- $\mid$ 0.59 , -- , -- $\mid$ 1.6 , --  )};
\draw (janzen2008.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (biondo2012) at ($(janzen2008.west |- 0,-8.000000*\dy)$) {\reftext{Bion12}\cite{biondo2012} (  1.2 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (biondo2012.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (khanna2023) at ($(biondo2012.west |- 0,-9.000000*\dy)$) {\reftext{Khan23}\cite{khanna2023} (  0.82 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (khanna2023.west) -| ++(-\dy,\fy*\dy);
\coordinate (khanna2023C) at ($(khanna2023.west)+(\dxStart+\dy,0)$);
\node[ ref] (nouketcha2020) at ($(khanna2023C |- 0,-10.000000*\dy)$) {\reftext{Nouk20}\cite{nouketcha2020} (  0.82 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (nouketcha2020.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (maximenko2023) at ($(khanna2023.west |- 0,-11.000000*\dy)$) {\reftext{Maxi23}\cite{maximenko2023} (  0.82 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (maximenko2023.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (pearton2023) at ($(maximenko2023.west |- 0,-12.000000*\dy)$) {\reftext{Pear23}\cite{pearton2023} (  0.82 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (pearton2023.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-14.000000*\dy) {\citeauthor{schadt1997}};
\node[ ref] (schadt1997) at (\xSepOne,-15.000000*\dy) {\reftext{Scha97}\cite{schadt1997} (  -- $\mid$ -- , -- , -- $\mid$ -- , --  )};
\coordinate (schadt1997C) at ($(schadt1997.west)+(\dxStart+\dy,0)$);
\node[ ref] (troffer1998) at ($(schadt1997C |- 0,-16.000000*\dy)$) {\reftext{Trof98}\cite{troffer1998} (  1 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (troffer1998.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-18.000000*\dy) {\citeauthor{wellenhofer1997}};
\node[ ref] (wellenhofer1997) at (\xSepOne,-19.000000*\dy) {\reftext{Well97}\cite{wellenhofer1997} (  -- $\mid$ -- , -- , -- $\mid$ -- , --  )};
\coordinate (wellenhofer1997C) at ($(wellenhofer1997.west)+(\dxStart+\dy,0)$);
\node[ ref] (hatakeyama2013) at ($(wellenhofer1997C |- 0,-20.000000*\dy)$) {\reftext{Hata13}\cite{hatakeyama2013} (  2.64 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (hatakeyama2013.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (sozzi2019) at ($(hatakeyama2013.west |- 0,-21.000000*\dy)$) {\reftext{Sozz19}\cite{sozzi2019} (  2.6 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (sozzi2019.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (luo2020) at ($(sozzi2019.west |- 0,-22.000000*\dy)$) {\reftext{Luo20}\cite{luo2020} (  2.64 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (luo2020.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (yang2022) at ($(luo2020.west |- 0,-23.000000*\dy)$) {\reftext{Yang22}\cite{yang2022} (  -- $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (yang2022.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,0.000000*\dy) {\citeauthor{persson1998a}};
\node[fund, ref] (persson1998a) at (\xSepOne + \xSepTwo,-1.000000*\dy) {\reftext{Pers98a}\cite{persson1998a} (  M $\mid$ -- , M , M $\mid$ -- , M  )};
\coordinate (persson1998aC) at ($(persson1998a.west)+(\dxStart+\dy,0)$);
\node[ ref] (pernot2005) at ($(persson1998aC |- 0,-2.000000*\dy)$) {\reftext{Pern05}\cite{pernot2005} (  M $\mid$ M , -- , -- $\mid$ M , --  )};
\draw (pernot2005.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (scajev2013a) at ($(pernot2005.west |- 0,-3.000000*\dy)$) {\reftext{Scaj13a}\cite{scajev2013a} (  0.94 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (scajev2013a.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-5.000000*\dy) {\citeauthor{persson1999b}};
\node[fund, ref] (persson1999b) at (\xSepOne + \xSepTwo,-6.000000*\dy) {\reftext{Pers99b}\cite{persson1999b} (  -- $\mid$ M , -- , -- $\mid$ M , --  )};
\coordinate (persson1999bC) at ($(persson1999b.west)+(\dxStart+\dy,0)$);
\node[ ref] (son2004) at ($(persson1999bC |- 0,-7.000000*\dy)$) {\reftext{Son04}\cite{son2004} (  -- $\mid$ M , -- , -- $\mid$ M , --  )};
\draw (son2004.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (persson2005) at ($(son2004.west |- 0,-8.000000*\dy)$) {\reftext{Pers05}\cite{persson2005} (  -- $\mid$ M , -- , -- $\mid$ M , --  )};
\draw (persson2005.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-10.000000*\dy) {\citeauthor{son2000}};
\node[fund, ref] (son2000) at (\xSepOne + \xSepTwo,-11.000000*\dy) {\reftext{Son00}\cite{son2000} (  -- $\mid$ 0.66 , -- , -- $\mid$ 1.75 , --  )};
\coordinate (son2000C) at ($(son2000.west)+(\dxStart+\dy,0)$);
\node[ ref] (kohlscheen2003) at ($(son2000C |- 0,-12.000000*\dy)$) {\reftext{Kohl03}\cite{kohlscheen2003} (  -- $\mid$ 0.66 , -- , -- $\mid$ 1.75 , --  )};
\draw (kohlscheen2003.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (feng2004a) at ($(kohlscheen2003.west |- 0,-13.000000*\dy)$) {\reftext{Feng04a}\cite{feng2004a} (  -- $\mid$ 0.66 , -- , -- $\mid$ 1.75 , --  )};
\draw (feng2004a.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (pensl2005) at ($(feng2004a.west |- 0,-14.000000*\dy)$) {\reftext{Pens05}\cite{pensl2005} (  -- $\mid$ 0.66 , -- , -- $\mid$ 1.75 , --  )};
\draw (pensl2005.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (reshanov2005) at ($(pensl2005.west |- 0,-15.000000*\dy)$) {\reftext{Resh05}\cite{reshanov2005} (  1.26 $\mid$ 0.66 , -- , -- $\mid$ 1.75 , --  )};
\draw (reshanov2005.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (albanese2010) at ($(reshanov2005.west |- 0,-16.000000*\dy)$) {\reftext{Alba10}\cite{albanese2010} (  1.2 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (albanese2010.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (kimoto2014a) at ($(albanese2010.west |- 0,-17.000000*\dy)$) {\reftext{Kimo14a}\cite{kimoto2014a} (  -- $\mid$ 0.66 , -- , -- $\mid$ 1.75 , --  )};
\draw (kimoto2014a.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (yang2019) at ($(kimoto2014a.west |- 0,-18.000000*\dy)$) {\reftext{Yang19}\cite{yang2019} (  1.2 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (yang2019.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (klahold2020) at ($(yang2019.west |- 0,-19.000000*\dy)$) {\reftext{Klah20}\cite{klahold2020} (  -- $\mid$ 0.66 , -- , -- $\mid$ 1.75 , --  )};
\draw (klahold2020.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (rakheja2020) at ($(klahold2020.west |- 0,-20.000000*\dy)$) {\reftext{Rakh20}\cite{rakheja2020} (  -- $\mid$ 0.66 , -- , -- $\mid$ 1.75 , --  )};
\draw (rakheja2020.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (ishikawa2024) at ($(rakheja2020.west |- 0,-21.000000*\dy)$) {\reftext{Ishi24}\cite{ishikawa2024} (  -- $\mid$ 0.66 , -- , -- $\mid$ 1.75 , --  )};
\draw (ishikawa2024.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-23.000000*\dy) {\citeauthor{levinshtein2001}};
\node[ ref] (levinshtein2001) at (\xSepOne + \xSepTwo,-24.000000*\dy) {\reftext{Levi01}\cite{levinshtein2001} (  1 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\coordinate (levinshtein2001C) at ($(levinshtein2001.west)+(\dxStart+\dy,0)$);
\node[ ref] (tamaki2008a) at ($(levinshtein2001C |- 0,-25.000000*\dy)$) {\reftext{Tama08a}\cite{tamaki2008a} (  1.0001 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (tamaki2008a.west) -| ++(-\dy,\fy*\dy);
\coordinate (tamaki2008aC) at ($(tamaki2008a.west)+(\dxStart+\dy,0)$);
\node[ ref] (song2012) at ($(tamaki2008aC |- 0,-26.000000*\dy)$) {\reftext{Song12}\cite{song2012} (  1.0001 $\mid$ -- , -- , -- $\mid$ -- , --  )};
\draw (song2012.west) -| ++(-\dy,\fy*\dy);


==> data/mobility_figure_CT_doping_elec.tex <==
\pgfplotsset{cycle list name=CT}
\addplot+[samples=\sampleCount, domain=\xMinDop:\xMaxDop] {CTZero(20,380,4.50E+17,0.45)}; 
\addlegendentry{\reftext{Ruff94}\cite{ruff1994}  }
\addplot+[samples=\sampleCount, domain=1.00E+16:1.00E+20] {CT(0,947,1.94E+17,0.61)}; 
\addlegendentry{\reftext{Scha94}\cite{schaffer1994} $\perp$ H}
\addplot+[samples=\sampleCount, domain=1.00E+16:1.00E+19] {CT(0,1071,1.94E+17,0.4)}; 
\addlegendentry{\reftext{Mick98}\cite{mickevicius1998}  C}
\addplot+[samples=\sampleCount, domain=\xMinDop:\xMaxDop] {CT(40,800,4.00E+17,0.44)}; 
\addlegendentry{\reftext{Rosc98}\cite{roschke1998}  }
\addplot+[samples=\sampleCount, domain=\xMinDop:\xMaxDop] {CT(0,947,1.94E+17,0.61)}; 
\addlegendentry{\reftext{Shah98}\cite{shah1998}  }
\addplot+[samples=\sampleCount, domain=\xMinDop:\xMaxDop] {CTZero(88,970,1.43E+17,1)}; 
\addlegendentry{\reftext{Wrig98}\cite{wright1998}  }
\addplot+[samples=\sampleCount, domain=\xMinDop:\xMaxDop] {CT(79.8,855,2.00E+17,1)}; 
\addlegendentry{\reftext{Levi01a}\cite{levinshtein2001a}  }
\addplot+[samples=\sampleCount, domain=3.00E+15:7.00E+19] {CT(30,880,2.00E+17,0.67)}; 
\addlegendentry{\reftext{Mnat01}\cite{mnatsakanov2001}  C}
\addplot+[samples=\sampleCount, domain=1.00E+14:1.00E+20] {CT(0,1141,1.94E+17,0.61)}; 
\addlegendentry{\reftext{Mori01}\cite{morisette2001} $\parallel$ C}
\addplot+[samples=\sampleCount, domain=8.00E+14:5.00E+19] {CT(40,950,2.00E+17,0.76)}; 
\addlegendentry{\reftext{Rosc01}\cite{roschke2001} $\perp$ }
\addplot+[samples=\sampleCount, domain=2.00E+15:8.00E+18] {CT(0,954,1.28E+17,0.61)}; 
\addlegendentry{\reftext{Hata03}\cite{hatakeyama2003}  H}
\addplot+[samples=\sampleCount, domain=4.00E+14:1.00E+20] {CT(0,977,1.17E+17,0.49)}; 
\addlegendentry{\reftext{Kaga04}\cite{kagamihara2004}  H}
\addplot+[samples=\sampleCount, domain=\xMinDop:\xMaxDop] {CT(0,1400,1.00E+17,0.5)}; 
\addlegendentry{\reftext{Adac05}\cite{adachi2005}  }
\addplot+[samples=\sampleCount, domain=\xMinDop:\xMaxDop] {CT(40,950,2.00E+17,0.73)}; 
\addlegendentry{\reftext{Bala05}\cite{balachandran2005}  }
\addplot+[samples=\sampleCount, domain=\xMinDop:\xMaxDop] {CT(33,771,2.00E+17,0.76)}; 
\addlegendentry{\reftext{Werb07}\cite{werber2007}  C}
\addplot+[samples=\sampleCount, domain=\xMinDop:\xMaxDop] {CT(0,950,1.90E+17,0.6)}; 
\addlegendentry{\reftext{Cha08}\cite{cha2008}  }
\addplot+[samples=\sampleCount, domain=\xMinDop:\xMaxDop] {CT(6,200,1.00E+16,1)}; 
\addlegendentry{\reftext{Pezz08}\cite{pezzimenti2008}  C}
\addplot+[samples=\sampleCount, domain=1.00E+14:1.00E+20] {CTZero(40,910,2.00E+17,0.76)}; 
\addlegendentry{\reftext{Habi11}\cite{habib2011}  }
\addplot+[samples=\sampleCount, domain=1.00E+14:3.00E+19] {CT(5,1010,1.25E+17,0.65)}; 
\addlegendentry{\reftext{Hata13}\cite{hatakeyama2013}  }
\addplot+[samples=\sampleCount, domain=1.00E+15:1.00E+20] {CT(28,950,1.94E+17,0.61)}; 
\addlegendentry{\reftext{Stef14}\cite{stefanakis2014} $\perp$ }
\addplot+[samples=\sampleCount, domain=\xMinDop:\xMaxDop] {CT(40,947,1.94E+17,0.61)}; 
\addlegendentry{\reftext{Shar15}\cite{sharma2015} $\parallel$ C}
\addplot+[samples=\sampleCount, domain=\xMinDop:\xMaxDop] {CT(40,950,1.94E+17,0.61)}; 
\addlegendentry{\reftext{Arva17}\cite{arvanitopoulos2017}  }
\addplot+[samples=\sampleCount, domain=3.00E+18:2.50E+19] {CT(20,950,2.00E+17,0.8)}; 
\addlegendentry{\reftext{Vasi17}\cite{vasilevskiy2017}  H}
\addplot+[samples=\sampleCount, domain=2.00E+15:3.00E+18] {CTZero(40,970,2.4e17,0.7)}; 
\addlegendentry{\reftext{Ishi21}\cite{ishikawa2021} $\perp$ H}
\addplot+[samples=\sampleCount, domain=2.00E+15:3.00E+18] {CTZero(60,1120,2.3e17,0.74)}; 
\addlegendentry{\reftext{Ishi21}\cite{ishikawa2021} $\parallel$ H}
\addplot+[samples=\sampleCount, domain=1.00E+14:1.00E+19] {CTZero(15.48,1415.4,1.80E+17,0.560723)}; 
\addlegendentry{\reftext{Lech21}\cite{lechner2021} $\parallel$ }
\addplot+[samples=\sampleCount, domain=\xMinDop:\xMaxDop] {CT(40,950,2.00E+17,0.76)}; 
\addlegendentry{\reftext{Rao22}\cite{rao2022}  }
\addplot+[samples=\sampleCount, domain=5.00E+14:3.00E+18] {CTZero(40,1000,2.2e17,0.68)}; 
\addlegendentry{\reftext{Ishi23}\cite{ishikawa2023} $\perp$ H}
\addplot+[samples=\sampleCount, domain=5.00E+14:3.00E+18] {CTZero(20,1240,2e17,0.64)}; 
\addlegendentry{\reftext{Ishi23}\cite{ishikawa2023} $\parallel$ H}


==> data/mobility_figure_CT_doping_hole.tex <==
\pgfplotsset{cycle list name=CT}
\addplot+[samples=\sampleCount, domain=\xMinDop:\xMaxDop] {CTZero(5,70,1.00E+19,0.5)}; 
\addlegendentry{\reftext{Ruff94}\cite{ruff1994}  }
\addplot+[samples=\sampleCount, domain=1.00E+16:1.00E+20] {CT(15.9,124,1.76E+19,0.34)}; 
\addlegendentry{\reftext{Scha94}\cite{schaffer1994} $\perp$ H}
\addplot+[samples=\sampleCount, domain=\xMinDop:\xMaxDop] {CT(25.9,128.1,1.00E+19,0.24)}; 
\addlegendentry{\reftext{Shah98}\cite{shah1998}  }
\addplot+[samples=\sampleCount, domain=\xMinDop:\xMaxDop] {CTZero(74,43,1.43E+17,1)}; 
\addlegendentry{\reftext{Wrig98}\cite{wright1998}  }
\addplot+[samples=\sampleCount, domain=\xMinDop:\xMaxDop] {CT(65,114,5.00E+17,1)}; 
\addlegendentry{\reftext{Levi01a}\cite{levinshtein2001a}  }
\addplot+[samples=\sampleCount, domain=3.00E+15:7.00E+19] {CT(33,117,1.00E+19,0.5)}; 
\addlegendentry{\reftext{Mnat01}\cite{mnatsakanov2001}  C}
\addplot+[samples=\sampleCount, domain=2.00E+15:8.00E+18] {CT(15.9,120,1.80E+18,0.65)}; 
\addlegendentry{\reftext{Hata03}\cite{hatakeyama2003}  H}
\addplot+[samples=\sampleCount, domain=1.00E+15:1.00E+19] {CT(37.6,106,2.97E+18,0.356)}; 
\addlegendentry{\reftext{Mats04}\cite{matsuura2004}  H}
\addplot+[samples=\sampleCount, domain=\xMinDop:\xMaxDop] {CT(53.3,105.4,2.20E+18,0.7)}; 
\addlegendentry{\reftext{Bala05}\cite{balachandran2005}  }
\addplot+[samples=\sampleCount, domain=\xMinDop:\xMaxDop] {CTZero(10,81,1.00E+19,0.5)}; 
\addlegendentry{\reftext{Werb07}\cite{werber2007}  C}
\addplot+[samples=\sampleCount, domain=\xMinDop:\xMaxDop] {CT(16,140,1.70E+19,0.34)}; 
\addlegendentry{\reftext{Cha08}\cite{cha2008}  }
\addplot+[samples=\sampleCount, domain=\xMinDop:\xMaxDop] {CT(2,20,1.00E+16,1)}; 
\addlegendentry{\reftext{Pezz08}\cite{pezzimenti2008}  C}
\addplot+[samples=\sampleCount, domain=1.00E+15:1.00E+20] {CT(0,114.1,5.38E+18,0.66)}; 
\addlegendentry{\reftext{Koiz09}\cite{koizumi2009}  H}
\addplot+[samples=\sampleCount, domain=1.00E+14:1.00E+20] {CTZero(40,82,6.30E+18,0.55)}; 
\addlegendentry{\reftext{Habi11}\cite{habib2011}  }
\addplot+[samples=\sampleCount, domain=1.00E+14:3.00E+19] {CT(0,113.5,2.40E+18,0.69)}; 
\addlegendentry{\reftext{Hata13}\cite{hatakeyama2013}  }
\addplot+[samples=\sampleCount, domain=1.00E+16:1.00E+20] {CT(0,75,2.00E+19,0.7)}; 
\addlegendentry{\reftext{Liau15}\cite{liaugaudas2015}  C}
\addplot+[samples=\sampleCount, domain=\xMinDop:\xMaxDop] {CT(15.9,124,1.76E+19,0.34)}; 
\addlegendentry{\reftext{Shar15}\cite{sharma2015} $\parallel$ C}
\addplot+[samples=\sampleCount, domain=8.00E+14:1.00E+19] {CT(0,110,3e18,0.6)}; 
\addlegendentry{\reftext{Tana18}\cite{tanaka2018}  H}
\addplot+[samples=\sampleCount, domain=8.00E+14:1.00E+19] {CT(0,95,1e19,0.7)}; 
\addlegendentry{\reftext{Tana18}\cite{tanaka2018}  C}
\addplot+[samples=\sampleCount, domain=1.00E+14:1.00E+19] {CTZero(2.529,469.42607,1.28E+19,0.332645)}; 
\addlegendentry{\reftext{Lech21}\cite{lechner2021}  }
\addplot+[samples=\sampleCount, domain=\xMinDop:\xMaxDop] {CT(15.9,125,1.76E+19,0.76)}; 
\addlegendentry{\reftext{Rao22}\cite{rao2022}  }
\addplot+[samples=\sampleCount, domain=8.00E+15:9.00E+18] {CTZero(20,74,6.2e18,0.72)}; 
\addlegendentry{\reftext{Ishi24}\cite{ishikawa2024} $\perp$ H}
\addplot+[samples=\sampleCount, domain=8.00E+15:9.00E+18] {CTZero(20,63,6.4e18,0.83)}; 
\addlegendentry{\reftext{Ishi24}\cite{ishikawa2024} $\parallel$ H}


==> data/mobility_figure_CT_temp_elec.tex <==
\pgfplotsset{cycle list name=CT}
\addplot+[samples=\sampleCount, domain=\xMin:\xMax] {CTZero(20,380,4.50E+17,0.45,0,-3,0,0,0)}; 
\addlegendentry{\reftext{Ruff94}\cite{ruff1994}  }
\addplot+[samples=\sampleCount, domain=80:600] {CT(0,947,1.94E+17,0.61,0,-2.15,0,0,0)}; 
\addlegendentry{\reftext{Scha94}\cite{schaffer1994} $\perp$ H}
\addplot+[samples=\sampleCount, domain=\xMin:\xMax] {CTZero(88,970,1.43E+17,1,-0.57,-2.7,2.55,0,0)}; 
\addlegendentry{\reftext{Wrig98}\cite{wright1998}  }
\addplot+[samples=\sampleCount, domain=200:700] {CT(40,950,2.00E+17,0.76,-0.5,-2.4,1,0,0)}; 
\addlegendentry{\reftext{Rosc01}\cite{roschke2001} $\perp$ }
\addplot+[samples=\sampleCount, domain=\xMin:\xMax] {CT(40,950,2.00E+17,0.73,0,-2.4,0,0,-0.76)}; 
\addlegendentry{\reftext{Bala05}\cite{balachandran2005}  }
\addplot+[samples=\sampleCount, domain=\xMin:\xMax] {CT(0,950,1.90E+17,0.6,1,-2.15,0,0,0.05)}; 
\addlegendentry{\reftext{Cha08}\cite{cha2008}  }
\addplot+[samples=\sampleCount, domain=250:1000] {CTZero(40,910,2.00E+17,0.76,-1.538,-2.397,0.75,0.722,0)}; 
\addlegendentry{\reftext{Habi11}\cite{habib2011}  }
\addplot+[samples=\sampleCount, domain=300:600] {CT(5,1010,1.25E+17,0.65,-0.57,-2.6,2.4,-0.146,0)}; 
\addlegendentry{\reftext{Hata13}\cite{hatakeyama2013}  }
\addplot+[samples=\sampleCount, domain=50:900] {CT(28,950,1.94E+17,0.61,0,-2.4,0,0,0.73)}; 
\addlegendentry{\reftext{Stef14}\cite{stefanakis2014} $\perp$ }
\addplot+[samples=\sampleCount, domain=\xMin:\xMax] {CT(40,947,1.94E+17,0.61,-0.5,-2.9,0,0,2.4)}; 
\addlegendentry{\reftext{Shar15}\cite{sharma2015} $\parallel$ C}
\addplot+[samples=\sampleCount, domain=\xMin:\xMax] {CT(40,950,1.94E+17,0.61,-1.536,-2.4,0,0,0)}; 
\addlegendentry{\reftext{Arva17}\cite{arvanitopoulos2017}  }
\addplot+[samples=\sampleCount, domain=300:600] {CTZero(40,970,2.4e17,0.7,0,-2.58,0,0,0)}; 
\addlegendentry{\reftext{Ishi21}\cite{ishikawa2021} $\perp$ H}
\addplot+[samples=\sampleCount, domain=300:600] {CTZero(60,1120,2.3e17,0.74,0,-2.67,0,0,0)}; 
\addlegendentry{\reftext{Ishi21}\cite{ishikawa2021} $\parallel$ H}
\addplot+[samples=\sampleCount, domain=\xMin:\xMax] {CTZero(15.48,1415.4,1.80E+17,0.560723,0,-2.5,0,0,0)}; 
\addlegendentry{\reftext{Lech21}\cite{lechner2021} $\parallel$ }
\addplot+[samples=\sampleCount, domain=\xMin:\xMax] {CT(40,950,2.00E+17,0.76,-0.5,-2.15,0,0,-0.76)}; 
\addlegendentry{\reftext{Rao22}\cite{rao2022}  }
\addplot+[samples=\sampleCount, domain=300:600] {CTZero(40,1000,2.2e17,0.68,-0.7,-2.9,0,0,-2.5)}; 
\addlegendentry{\reftext{Ishi23}\cite{ishikawa2023} $\perp$ H}
\addplot+[samples=\sampleCount, domain=300:600] {CTZero(20,1240,2e17,0.64,0.3,-3.2,0,0,-2.7)}; 
\addlegendentry{\reftext{Ishi23}\cite{ishikawa2023} $\parallel$ H}


==> data/mobility_figure_CT_temp_hole.tex <==
\pgfplotsset{cycle list name=CT}
\addplot+[samples=\sampleCount, domain=\xMin:\xMax] {CTZero(5,70,1.00E+19,0.5,0,-3,0,0,0)}; 
\addlegendentry{\reftext{Ruff94}\cite{ruff1994}  }
\addplot+[samples=\sampleCount, domain=\xMin:\xMax] {CTZero(74,43,1.43E+17,1,-0.57,-2.7,2.55,0,0)}; 
\addlegendentry{\reftext{Wrig98}\cite{wright1998}  }
\addplot+[samples=\sampleCount, domain=\xMin:\xMax] {CT(53.3,105.4,2.20E+18,0.7,0,-2.1,0,0,0)}; 
\addlegendentry{\reftext{Bala05}\cite{balachandran2005}  }
\addplot+[samples=\sampleCount, domain=\xMin:\xMax] {CT(16,140,1.70E+19,0.34,-1.6,-2.14,0,0,0.17)}; 
\addlegendentry{\reftext{Cha08}\cite{cha2008}  }
\addplot+[samples=\sampleCount, domain=\xMin:\xMax] {CT(0,114.1,5.38E+18,0.66,0,-2.72,0,-0.35,2.44)}; 
\addlegendentry{\reftext{Koiz09}\cite{koizumi2009}  H}
\addplot+[samples=\sampleCount, domain=250:1000] {CTZero(40,82,6.30E+18,0.55,-1.538,-2.2397,0.75,0.722,0)}; 
\addlegendentry{\reftext{Habi11}\cite{habib2011}  }
\addplot+[samples=\sampleCount, domain=300:600] {CT(0,113.5,2.40E+18,0.69,-0.57,-2.6,2.9,-0.2,0)}; 
\addlegendentry{\reftext{Hata13}\cite{hatakeyama2013}  }
\addplot+[samples=\sampleCount, domain=\xMin:\xMax] {CT(15.9,124,1.76E+19,0.34,-0.5,-2.9,0,0,2.3)}; 
\addlegendentry{\reftext{Shar15}\cite{sharma2015} $\parallel$ C}
\addplot+[samples=\sampleCount, domain=298:700] {CT(0,110,3e18,0.6,0,-3,0,0,-1.8)}; 
\addlegendentry{\reftext{Tana18}\cite{tanaka2018}  H}
\addplot+[samples=\sampleCount, domain=298:700] {CT(0,95,1e19,0.7,0,-2.1,0,0,-1.5)}; 
\addlegendentry{\reftext{Tana18}\cite{tanaka2018}  C}
\addplot+[samples=\sampleCount, domain=\xMin:\xMax] {CTZero(2.529,469.42607,1.28E+19,0.332645,0,-2,0,0,0)}; 
\addlegendentry{\reftext{Lech21}\cite{lechner2021}  }
\addplot+[samples=\sampleCount, domain=\xMin:\xMax] {CT(15.9,125,1.76E+19,0.76,-0.5,-2.15,0,0,-0.76)}; 
\addlegendentry{\reftext{Rao22}\cite{rao2022}  }
\addplot+[samples=\sampleCount, domain=300:600] {CTZero(20,74,6.2e18,0.72,-2.2,-2.3,0,0,-0.9)}; 
\addlegendentry{\reftext{Ishi24}\cite{ishikawa2024} $\perp$ H}
\addplot+[samples=\sampleCount, domain=300:600] {CTZero(20,63,6.4e18,0.83,-2.2,-2.3,0,0,-0.9)}; 
\addlegendentry{\reftext{Ishi24}\cite{ishikawa2024} $\parallel$ H}


==> data/mobility_figure_mob_values.tex <==


\node[symbol] (elec) at (0,0) {$\mun$};
\coordinate (elec0) at (elec.north);
\node[ref, lwelec] (elec1) at (elec0.north west) {\tikz \node[paper, fund] {\reftext{Main24}\cite{mainali2024}};};
\node[value, scale=1.100000] (elecvalue1) at (elec1.west) {\num{39+-2}};
\node[ref, lwelec] (elec2) at (elec1.north west) {\tikz \node[paper, fund] {\reftext{Neim06}\cite{neimontas2006}}; \tikz \node[paper, fund] {\reftext{Scha94a}\cite{schadt1994a}};};
\node[value, scale=1.200000] (elecvalue2) at (elec2.west) {\num{116}};
\node[ref, lwelec] (elec3) at (elec2.north west) {\tikz \node[paper, fund] {\reftext{Khan98}\cite{khan1998}};};
\node[value, scale=1.100000] (elecvalue3) at (elec3.west) {\num{400}};
\node[ref, lwelec] (elec4) at (elec3.north west) {\tikz \node[paper, fund] {\reftext{Scho94}\cite{schoner1994}};};
\node[value, scale=1.100000] (elecvalue4) at (elec4.west) {\num{417}};
\node[ref, lwelec] (elec5) at (elec4.north west) {\tikz \node[paper] {\reftext{Kimo19}\cite{kimoto2019}}; \tikz \node[paper] {\reftext{Kimo14a}\cite{kimoto2014a}}; \tikz \node[paper] {\reftext{Khan00b}\cite{khan2000b}};};
\node[value, scale=1.300000] (elecvalue5) at (elec5.west) {\num{450}};
\node[ref, lwelec] (elec6) at (elec5.north west) {\tikz \node[paper] {\reftext{Sand11}\cite{sandeep2011}};};
\node[value, scale=1.100000] (elecvalue6) at (elec6.west) {\num{460}};
\node[ref, lwelec] (elec7) at (elec6.north west) {\tikz \node[paper] {\reftext{Will06}\cite{willander2006}}; \tikz \node[paper] {\reftext{Elas03}\cite{elasser2003}}; \tikz \node[paper] {\reftext{Trew02}\cite{trew2002}}; \tikz \node[paper] {\reftext{Elas00}\cite{elasser2000}}; \tikz \node[paper] {\reftext{Trew97}\cite{trew1997}}; \tikz \node[paper] {\reftext{Neub71}\cite{neuberger1971}};};
\node[value, scale=1.600000] (elecvalue7) at (elec7.west) {\num{500}};
\node[ref, lwelec] (elec8) at (elec7.north west) {\tikz \node[paper, fund] {\reftext{Chen22}\cite{cheng2022}};};
\node[value, scale=1.100000] (elecvalue8) at (elec8.west) {\num{615}};
\node[ref, lwelec] (elec9) at (elec8.north west) {\tikz \node[paper] {\reftext{Kaji15}\cite{kaji2015}}; \tikz \node[paper] {\reftext{Pank14}\cite{pankove2014}}; \tikz \node[paper] {\reftext{Mani11}\cite{manikam2011}}; \tikz \node[paper] {\reftext{Hudg03}\cite{hudgins2003}}; \tikz \node[paper] {\reftext{Zhan02}\cite{zhang2002}}; \tikz \node[paper] {\reftext{Keme02}\cite{kemerley2002}}; \tikz \node[paper] {\reftext{Pacc00}\cite{pacchioni2000}}; \tikz \node[paper] {\reftext{Afan00}\cite{afanasev2000}}; \tikz \node[paper] {\reftext{Choy74}\cite{choyke1974}}; \tikz \node[paper, fund] {\reftext{Loma72}\cite{lomakina1972}};};
\node[value, scale=2.000000] (elecvalue9) at (elec9.west) {\num{700}};
\node[ref, lwelec] (elec10) at (elec9.north west) {\tikz \node[paper] {\reftext{Su10}\cite{su2010}}; \tikz \node[paper] {\reftext{Alba10}\cite{albanese2010}}; \tikz \node[paper] {\reftext{Masr02}\cite{masri2002}}; \tikz \node[paper] {\reftext{Lee02}\cite{lee2002}}; \tikz \node[paper] {\reftext{Itoh96}\cite{itoh1996}}; \tikz \node[paper] {\reftext{Itoh95}\cite{itoh1995}}; \tikz \node[paper, fund] {\reftext{Itoh94}\cite{itoh1994}};};
\node[value, scale=1.700000] (elecvalue10) at (elec10.west) {\num{720}};
\node[ref, lwelec] (elec11) at (elec10.north west) {\tikz \node[paper, fund] {\reftext{Lavi05}\cite{lavia2005}}; \tikz \node[paper] {\reftext{Kimo97}\cite{kimoto1997}};};
\node[value, scale=1.200000] (elecvalue11) at (elec11.west) {\num{724}};
\node[ref, lwelec] (elec12) at (elec11.north west) {\tikz \node[paper] {\reftext{Sole19}\cite{soler2019}};};
\node[value, scale=1.100000] (elecvalue12) at (elec12.west) {\num{750}};
\node[ref, lwelec] (elec13) at (elec12.north west) {\tikz \node[paper] {\reftext{Dena22}\cite{denapoli2022}}; \tikz \node[paper] {\reftext{Bela22}\cite{belas2022}}; \tikz \node[paper] {\reftext{Jiya20}\cite{jiya2020}}; \tikz \node[paper] {\reftext{Hass18}\cite{hassan2018}}; \tikz \node[paper] {\reftext{Ryba17}\cite{rybalka2017}}; \tikz \node[paper] {\reftext{Arvi17}\cite{arvinte2017}}; \tikz \node[paper] {\reftext{Choi16}\cite{choi2016}}; \tikz \node[paper] {\reftext{Neud13}\cite{neudeck2013}}; \tikz \node[paper] {\reftext{Mant13}\cite{mantooth2013}}; \tikz \node[paper] {\reftext{Nava08}\cite{nava2008}}; \tikz \node[paper] {\reftext{Sze07}\cite{sze2007}}; \tikz \node[paper] {\reftext{Zhao06}\cite{zhao2006}}; \tikz \node[paper] {\reftext{Levi04}\cite{levinshtein2004}}; \tikz \node[paper] {\reftext{Ng03}\cite{ng2003}}; \tikz \node[paper] {\reftext{Lebe99}\cite{lebedev1999}}; \tikz \node[paper] {\reftext{Burk99}\cite{burk1999}}; \tikz \node[paper] {\reftext{Agar99}\cite{agarwal1999}}; \tikz \node[paper] {\reftext{Chel97}\cite{chelnokov1997}}; \tikz \node[paper] {\reftext{Agar96}\cite{agarwal1996}}; \tikz \node[paper] {\reftext{Neud95}\cite{neudeck1995}};};
\node[value, scale=3.000000] (elecvalue13) at (elec13.west) {\num{800}};
\node[ref, lwelec] (elec14) at (elec13.north west) {\tikz \node[paper] {\reftext{Schr06}\cite{schroeder2006}}; \tikz \node[paper] {\reftext{Saks00}\cite{saks2000}};};
\node[value, scale=1.200000] (elecvalue14) at (elec14.west) {\num{900}};
\node[ref, lwelec] (elec15) at (elec14.north west) {\tikz \node[paper] {\reftext{Codr00}\cite{codreanu2000}};};
\node[value, scale=1.100000] (elecvalue15) at (elec15.west) {\num{947}};
\node[ref, lwelec] (elec16) at (elec15.north west) {\tikz \node[paper, fund] {\reftext{Choy97d}\cite{choyke1997d}};};
\node[value, scale=1.100000] (elecvalue16) at (elec16.west) {\num{948}};
\node[ref, lwelec] (elec17) at (elec16.north west) {\tikz \node[paper] {\reftext{Chou21}\cite{choudhary2021}}; \tikz \node[paper] {\reftext{Supr20}\cite{suproniuk2020}}; \tikz \node[paper] {\reftext{Luo20}\cite{luo2020}}; \tikz \node[paper] {\reftext{Cabe18}\cite{cabello2018}}; \tikz \node[paper] {\reftext{Fuji15}\cite{fujita2015}}; \tikz \node[paper] {\reftext{Kami14}\cite{kaminski2014}}; \tikz \node[paper] {\reftext{Pell13}\cite{pellish2013}}; \tikz \node[paper] {\reftext{Ostl11a}\cite{ostling2011a}}; \tikz \node[paper] {\reftext{Ostl11}\cite{ostling2011}}; \tikz \node[paper] {\reftext{Meno11}\cite{menon2011}}; \tikz \node[paper] {\reftext{Butt11}\cite{buttay2011}}; \tikz \node[paper] {\reftext{Kami09}\cite{kaminski2009}}; \tikz \node[paper] {\reftext{Mill07}\cite{millan2007}}; \tikz \node[paper, fund] {\reftext{Gale02}\cite{galeckas2002}};};
\node[value, scale=2.400000] (elecvalue17) at (elec17.west) {\num{950}};
\node[ref, lwelec] (elec18) at (elec17.north west) {\tikz \node[paper, fund] {\reftext{Jais24}\cite{jaiswal2024}};};
\node[value, scale=1.100000] (elecvalue18) at (elec18.west) {\num{952}};
\node[ref, lwelec] (elec19) at (elec18.north west) {\tikz \node[paper] {\reftext{Mori01}\cite{morisette2001}};};
\node[value, scale=1.100000] (elecvalue19) at (elec19.west) {\num{975}};
\node[ref, lwelec] (elec20) at (elec19.north west) {\tikz \node[paper] {\reftext{Guo19}\cite{guo2019}}; \tikz \node[paper] {\reftext{Tsao18}\cite{tsao2018}};};
\node[value, scale=1.200000] (elecvalue20) at (elec20.west) {\num{980}};
\node[ref, lwelec] (elec21) at (elec20.north west) {\tikz \node[paper, fund] {\reftext{Mats04a}\cite{matsunami2004a}}; \tikz \node[paper, fund] {\reftext{Kimo01}\cite{kimoto2001}};};
\node[value, scale=1.200000] (elecvalue21) at (elec21.west) {\num{981}};
\node[ref, lwelec] (elec22) at (elec21.north west) {\tikz \node[paper] {\reftext{Pear23}\cite{pearton2023}}; \tikz \node[paper] {\reftext{Lech21}\cite{lechner2021}}; \tikz \node[paper] {\reftext{Bane21}\cite{banerjee2021}}; \tikz \node[paper] {\reftext{Zhen20}\cite{zheng2020}}; \tikz \node[paper] {\reftext{Bisw20}\cite{biswas2020}}; \tikz \node[paper] {\reftext{Trip19}\cite{tripathi2019}}; \tikz \node[paper] {\reftext{Pear18}\cite{pearton2018}}; \tikz \node[paper] {\reftext{Lutz18}\cite{lutz2018}}; \tikz \node[paper] {\reftext{Uhne15}\cite{uhnevionak2015}}; \tikz \node[paper] {\reftext{Higa14}\cite{higashiwaki2014}}; \tikz \node[paper] {\reftext{Neil12}\cite{neilainglesias2012}}; \tikz \node[paper] {\reftext{Lutz11}\cite{lutz2011}}; \tikz \node[paper] {\reftext{Gerh11}\cite{gerhardt2011}}; \tikz \node[paper] {\reftext{Ozpi04}\cite{ozpineci2004}}; \tikz \node[paper] {\reftext{Powe02}\cite{powell2002}}; \tikz \node[paper] {\reftext{Wern01}\cite{werner2001}}; \tikz \node[paper] {\reftext{Evwa96}\cite{evwaraye1996}}; \tikz \node[paper] {\reftext{Casa96}\cite{casady1996}};};
\node[value, scale=2.800000] (elecvalue22) at (elec22.west) {\num{1000}};
\node[ref, lwelec] (elec23) at (elec22.north west) {\tikz \node[paper] {\reftext{Elah17}\cite{elahipanah2017}};};
\node[value, scale=1.100000] (elecvalue23) at (elec23.west) {\num{1020}};
\node[ref, lwelec] (elec24) at (elec23.north west) {\tikz \node[paper] {\reftext{Yode96}\cite{yoder1996}};};
\node[value, scale=1.100000] (elecvalue24) at (elec24.west) {\num{1140}};


\node[symbol] (elecperp) at (0+ \dxelec,0) {$\munperp$};
\coordinate (elecperp0) at (elecperp.north);
\node[ref, lwelecperp] (elecperp1) at (elecperp0.north west) {\tikz \node[paper, fund] {\reftext{Arda05}\cite{ardaravicius2005}};};
\node[value, scale=1.100000] (elecperpvalue1) at (elecperp1.west) {\num{275+-25}};
\node[ref, lwelecperp] (elecperp2) at (elecperp1.north west) {\tikz \node[paper, fund] {\reftext{Bert04}\cite{bertilsson2004}};};
\node[value, scale=1.100000] (elecperpvalue2) at (elecperp2.west) {\num{610}};
\node[ref, lwelecperp] (elecperp3) at (elecperp2.north west) {\tikz \node[paper] {\reftext{Naug17}\cite{naugarhiya2017}};};
\node[value, scale=1.100000] (elecperpvalue3) at (elecperp3.west) {\num{650}};
\node[ref, lwelecperp] (elecperp4) at (elecperp3.north west) {\tikz \node[paper] {\reftext{Loma74}\cite{lomakina1974}};};
\node[value, scale=1.100000] (elecperpvalue4) at (elecperp4.west) {\num{700}};
\node[ref, lwelecperp] (elecperp5) at (elecperp4.north west) {\tikz \node[paper] {\reftext{Chow17}\cite{chow2017}}; \tikz \node[paper] {\reftext{Dhan10}\cite{dhanaraj2010}}; \tikz \node[paper] {\reftext{Klei09}\cite{klein2009}}; \tikz \node[paper] {\reftext{Cole04}\cite{cole2004}}; \tikz \node[paper] {\reftext{Chow04}\cite{chow2004}}; \tikz \node[paper] {\reftext{Elas02}\cite{elasser2002}}; \tikz \node[paper] {\reftext{Dmit00}\cite{dmitriev2000}}; \tikz \node[paper] {\reftext{Chow00a}\cite{chow2000a}}; \tikz \node[paper] {\reftext{Chow00}\cite{chow2000}}; \tikz \node[paper] {\reftext{Chow97}\cite{chow1997}}; \tikz \node[paper] {\reftext{Chow96}\cite{chow1996}};};
\node[value, scale=2.100000] (elecperpvalue5) at (elecperp5.west) {\num{720}};
\node[ref, lwelecperp] (elecperp6) at (elecperp5.north west) {\tikz \node[paper] {\reftext{Mukh23}\cite{mukherjee2023}}; \tikz \node[paper] {\reftext{Mukh20a}\cite{mukherjee2020a}}; \tikz \node[paper] {\reftext{Wije11}\cite{wijesundara2011}}; \tikz \node[paper] {\reftext{Zhu08}\cite{zhu2008}}; \tikz \node[paper] {\reftext{Neud06}\cite{neudeck2006}}; \tikz \node[paper] {\reftext{Ayal04}\cite{ayalew2004}}; \tikz \node[paper] {\reftext{Neud01}\cite{neudeck2001}}; \tikz \node[paper] {\reftext{Weit98}\cite{weitzel1998}}; \tikz \node[paper] {\reftext{Srir97}\cite{sriram1997}}; \tikz \node[paper] {\reftext{Weit96}\cite{weitzel1996}};};
\node[value, scale=2.000000] (elecperpvalue6) at (elecperp6.west) {\num{800}};
\node[ref, lwelecperp] (elecperp7) at (elecperp6.north west) {\tikz \node[paper, fund] {\reftext{Mats97}\cite{matsunami1997}};};
\node[value, scale=1.100000] (elecperpvalue7) at (elecperp7.west) {\num{851}};
\node[ref, lwelecperp] (elecperp8) at (elecperp7.north west) {\tikz \node[paper] {\reftext{Rakh20}\cite{rakheja2020}}; \tikz \node[paper] {\reftext{Zett02}\cite{zetterling2002}}; \tikz \node[paper] {\reftext{Palm97}\cite{palmour1997}};};
\node[value, scale=1.300000] (elecperpvalue8) at (elecperp8.west) {\num{950}};
\node[ref, lwelecperp] (elecperp9) at (elecperp8.north west) {\tikz \node[paper] {\reftext{Lade00}\cite{ladesmartin2000}};};
\node[value, scale=1.100000] (elecperpvalue9) at (elecperp9.west) {\num{1000}};
\node[ref, lwelecperp] (elecperp10) at (elecperp9.north west) {\tikz \node[paper] {\reftext{Ostl24}\cite{ostling2024}}; \tikz \node[paper] {\reftext{Capa22}\cite{capan2022}}; \tikz \node[paper] {\reftext{Bere21}\cite{berens2021}}; \tikz \node[paper] {\reftext{Resc18}\cite{rescher2018}}; \tikz \node[paper] {\reftext{Kimo15}\cite{kimoto2015}};};
\node[value, scale=1.500000] (elecperpvalue10) at (elecperp10.west) {\num{1020}};


\node[symbol] (elecpara) at (0+ \dxelec+ \dxelecperp,0) {$\munpara$};
\coordinate (elecpara0) at (elecpara.north);
\node[ref, lwelecpara] (elecpara1) at (elecpara0.north west) {\tikz \node[paper] {\reftext{Chow17}\cite{chow2017}}; \tikz \node[paper] {\reftext{Dhan10}\cite{dhanaraj2010}}; \tikz \node[paper] {\reftext{Klei09}\cite{klein2009}}; \tikz \node[paper] {\reftext{Cole04}\cite{cole2004}}; \tikz \node[paper] {\reftext{Chow04}\cite{chow2004}}; \tikz \node[paper] {\reftext{Elas02}\cite{elasser2002}}; \tikz \node[paper] {\reftext{Dmit00}\cite{dmitriev2000}}; \tikz \node[paper] {\reftext{Chow00a}\cite{chow2000a}}; \tikz \node[paper] {\reftext{Chow00}\cite{chow2000}}; \tikz \node[paper] {\reftext{Chow97}\cite{chow1997}}; \tikz \node[paper] {\reftext{Chow96}\cite{chow1996}};};
\node[value, scale=2.100000] (elecparavalue1) at (elecpara1.west) {\num{650}};
\node[ref, lwelecpara] (elecpara2) at (elecpara1.north west) {\tikz \node[paper, fund] {\reftext{Bert04}\cite{bertilsson2004}};};
\node[value, scale=1.100000] (elecparavalue2) at (elecpara2.west) {\num{730}};
\node[ref, lwelecpara] (elecpara3) at (elecpara2.north west) {\tikz \node[paper] {\reftext{Mukh23}\cite{mukherjee2023}}; \tikz \node[paper] {\reftext{Mukh20a}\cite{mukherjee2020a}}; \tikz \node[paper] {\reftext{Naug17}\cite{naugarhiya2017}}; \tikz \node[paper] {\reftext{Wije11}\cite{wijesundara2011}}; \tikz \node[paper] {\reftext{Neud06}\cite{neudeck2006}}; \tikz \node[paper] {\reftext{Neud01}\cite{neudeck2001}}; \tikz \node[paper] {\reftext{Srir97}\cite{sriram1997}};};
\node[value, scale=1.700000] (elecparavalue3) at (elecpara3.west) {\num{800}};
\node[ref, lwelecpara] (elecpara4) at (elecpara3.north west) {\tikz \node[paper] {\reftext{Lang22}\cite{langpoklakpam2022}}; \tikz \node[paper] {\reftext{Liu15}\cite{liu2015}}; \tikz \node[paper] {\reftext{Zhu08}\cite{zhu2008}}; \tikz \node[paper] {\reftext{Ayal04}\cite{ayalew2004}};};
\node[value, scale=1.400000] (elecparavalue4) at (elecpara4.west) {\num{900}};
\node[ref, lwelecpara] (elecpara5) at (elecpara4.north west) {\tikz \node[paper] {\reftext{Palm97}\cite{palmour1997}};};
\node[value, scale=1.100000] (elecparavalue5) at (elecpara5.west) {\num{1140}};
\node[ref, lwelecpara] (elecpara6) at (elecpara5.north west) {\tikz \node[paper] {\reftext{Rakh20}\cite{rakheja2020}}; \tikz \node[paper] {\reftext{Zett02}\cite{zetterling2002}};};
\node[value, scale=1.200000] (elecparavalue6) at (elecpara6.west) {\num{1150}};
\node[ref, lwelecpara] (elecpara7) at (elecpara6.north west) {\tikz \node[paper] {\reftext{Ostl24}\cite{ostling2024}}; \tikz \node[paper] {\reftext{Capa22}\cite{capan2022}}; \tikz \node[paper] {\reftext{Bere21}\cite{berens2021}}; \tikz \node[paper] {\reftext{Resc18}\cite{rescher2018}}; \tikz \node[paper] {\reftext{Kimo15}\cite{kimoto2015}};};
\node[value, scale=1.500000] (elecparavalue7) at (elecpara7.west) {\num{1200}};


\node[symbol] (hole) at (0+ \dxelec+ \dxelecperp+ \dxelecpara,0) {$\mup$};
\coordinate (hole0) at (hole.north);
\node[ref, lwhole] (hole1) at (hole0.north west) {\tikz \node[paper] {\reftext{Trip19}\cite{tripathi2019}}; \tikz \node[paper] {\reftext{Neil12}\cite{neilainglesias2012}}; \tikz \node[paper] {\reftext{Will06}\cite{willander2006}}; \tikz \node[paper] {\reftext{Elas03}\cite{elasser2003}}; \tikz \node[paper] {\reftext{Wern01}\cite{werner2001}}; \tikz \node[paper] {\reftext{Elas00}\cite{elasser2000}}; \tikz \node[paper] {\reftext{Trew97}\cite{trew1997}}; \tikz \node[paper] {\reftext{Yode96}\cite{yoder1996}};};
\node[value, scale=1.800000] (holevalue1) at (hole1.west) {\num{50}};
\node[ref, lwhole] (hole2) at (hole1.north west) {\tikz \node[paper, fund] {\reftext{Neim06}\cite{neimontas2006}};};
\node[value, scale=1.100000] (holevalue2) at (hole2.west) {\num{52}};
\node[ref, lwhole] (hole3) at (hole2.north west) {\tikz \node[paper] {\reftext{Kaji15}\cite{kaji2015}}; \tikz \node[paper] {\reftext{Pank14}\cite{pankove2014}}; \tikz \node[paper] {\reftext{Sand11}\cite{sandeep2011}}; \tikz \node[paper] {\reftext{Lebe99}\cite{lebedev1999}};};
\node[value, scale=1.400000] (holevalue3) at (hole3.west) {\num{60}};
\node[ref, lwhole] (hole4) at (hole3.north west) {\tikz \node[paper, fund] {\reftext{Mats20}\cite{matsunami2020}};};
\node[value, scale=1.100000] (holevalue4) at (hole4.west) {\num{67}};
\node[ref, lwhole] (hole5) at (hole4.north west) {\tikz \node[paper] {\reftext{Pens03}\cite{pensl2003}};};
\node[value, scale=1.100000] (holevalue5) at (hole5.west) {\num{80}};
\node[ref, lwhole] (hole6) at (hole5.north west) {\tikz \node[paper] {\reftext{Bane21}\cite{banerjee2021}}; \tikz \node[paper] {\reftext{Sole19}\cite{soler2019}}; \tikz \node[paper, fund] {\reftext{Mats04}\cite{matsuura2004}}; \tikz \node[paper] {\reftext{Ng03}\cite{ng2003}};};
\node[value, scale=1.400000] (holevalue6) at (hole6.west) {\num{100}};
\node[ref, lwhole] (hole7) at (hole6.north west) {\tikz \node[paper, fund] {\reftext{Mart02}\cite{martinez2002}};};
\node[value, scale=1.100000] (holevalue7) at (hole7.west) {\num{107}};
\node[ref, lwhole] (hole8) at (hole7.north west) {\tikz \node[paper] {\reftext{Dena22}\cite{denapoli2022}}; \tikz \node[paper] {\reftext{Lech21}\cite{lechner2021}}; \tikz \node[paper] {\reftext{Jiya20}\cite{jiya2020}}; \tikz \node[paper] {\reftext{Lutz18}\cite{lutz2018}}; \tikz \node[paper] {\reftext{Hass18}\cite{hassan2018}}; \tikz \node[paper] {\reftext{Ryba17}\cite{rybalka2017}}; \tikz \node[paper] {\reftext{Arvi17}\cite{arvinte2017}}; \tikz \node[paper] {\reftext{Choi16}\cite{choi2016}}; \tikz \node[paper] {\reftext{Fuji15}\cite{fujita2015}}; \tikz \node[paper] {\reftext{Neud13}\cite{neudeck2013}}; \tikz \node[paper] {\reftext{Mant13}\cite{mantooth2013}}; \tikz \node[paper] {\reftext{Lutz11}\cite{lutz2011}}; \tikz \node[paper] {\reftext{Gerh11}\cite{gerhardt2011}}; \tikz \node[paper] {\reftext{Butt11}\cite{buttay2011}}; \tikz \node[paper] {\reftext{Nava08}\cite{nava2008}}; \tikz \node[paper] {\reftext{Mill07}\cite{millan2007}}; \tikz \node[paper] {\reftext{Schr06}\cite{schroeder2006}}; \tikz \node[paper] {\reftext{Ozpi04}\cite{ozpineci2004}}; \tikz \node[paper] {\reftext{Ragh98a}\cite{raghunathan1998a}}; \tikz \node[paper] {\reftext{Chel97}\cite{chelnokov1997}}; \tikz \node[paper] {\reftext{Casa96}\cite{casady1996}}; \tikz \node[paper] {\reftext{Neud95}\cite{neudeck1995}};};
\node[value, scale=3.200000] (holevalue8) at (hole8.west) {\num{115}};
\node[ref, lwhole] (hole9) at (hole8.north west) {\tikz \node[paper] {\reftext{Guo19}\cite{guo2019}}; \tikz \node[paper] {\reftext{Cabe18}\cite{cabello2018}}; \tikz \node[paper] {\reftext{Elah17}\cite{elahipanah2017}}; \tikz \node[paper] {\reftext{Pell13}\cite{pellish2013}}; \tikz \node[paper] {\reftext{Ostl11a}\cite{ostling2011a}}; \tikz \node[paper] {\reftext{Ostl11}\cite{ostling2011}}; \tikz \node[paper] {\reftext{Alba10}\cite{albanese2010}}; \tikz \node[paper] {\reftext{Zhao06}\cite{zhao2006}}; \tikz \node[paper] {\reftext{Levi04}\cite{levinshtein2004}}; \tikz \node[paper] {\reftext{Lee02}\cite{lee2002}};};
\node[value, scale=2.000000] (holevalue9) at (hole9.west) {\num{120}};
\node[ref, lwhole] (hole10) at (hole9.north west) {\tikz \node[paper] {\reftext{Meno11}\cite{menon2011}};};
\node[value, scale=1.100000] (holevalue10) at (hole10.west) {\num{124}};
\node[ref, lwhole] (hole11) at (hole10.north west) {\tikz \node[paper] {\reftext{Chou21}\cite{choudhary2021}}; \tikz \node[paper] {\reftext{Mori01}\cite{morisette2001}};};
\node[value, scale=1.200000] (holevalue11) at (hole11.west) {\num{125}};
\node[ref, lwhole] (hole12) at (hole11.north west) {\tikz \node[paper] {\reftext{Agar99}\cite{agarwal1999}}; \tikz \node[paper] {\reftext{Agar96}\cite{agarwal1996}};};
\node[value, scale=1.200000] (holevalue12) at (hole12.west) {\num{140}};
\node[ref, lwhole] (hole13) at (hole12.north west) {\tikz \node[paper] {\reftext{Supr20}\cite{suproniuk2020}};};
\node[value, scale=1.100000] (holevalue13) at (hole13.west) {\num{150}};


\node[symbol] (holeperp) at (0+ \dxelec+ \dxelecperp+ \dxelecpara+ \dxhole,0) {$\mupperp$};
\coordinate (holeperp0) at (holeperp.north);
\node[ref, lwholeperp] (holeperp1) at (holeperp0.north west) {\tikz \node[paper, fund] {\reftext{Cont06}\cite{contreras2006}};};
\node[value, scale=1.100000] (holeperpvalue1) at (holeperp1.west) {\num{37}};
\node[ref, lwholeperp] (holeperp2) at (holeperp1.north west) {\tikz \node[paper, fund] {\reftext{Bell99}\cite{bellotti1999}};};
\node[value, scale=1.100000] (holeperpvalue2) at (holeperp2.west) {\num{97}};
\node[ref, lwholeperp] (holeperp3) at (holeperp2.north west) {\tikz \node[paper] {\reftext{Mukh23}\cite{mukherjee2023}}; \tikz \node[paper] {\reftext{Mukh20a}\cite{mukherjee2020a}}; \tikz \node[paper] {\reftext{Naug17}\cite{naugarhiya2017}}; \tikz \node[paper] {\reftext{Wije11}\cite{wijesundara2011}}; \tikz \node[paper] {\reftext{Zhu08}\cite{zhu2008}}; \tikz \node[paper] {\reftext{Neud06}\cite{neudeck2006}}; \tikz \node[paper] {\reftext{Neud01}\cite{neudeck2001}}; \tikz \node[paper] {\reftext{Lade00}\cite{ladesmartin2000}};};
\node[value, scale=1.800000] (holeperpvalue3) at (holeperp3.west) {\num{115}};
\node[ref, lwholeperp] (holeperp4) at (holeperp3.north west) {\tikz \node[paper] {\reftext{Ostl24}\cite{ostling2024}}; \tikz \node[paper] {\reftext{Rakh20}\cite{rakheja2020}}; \tikz \node[paper] {\reftext{Resc18}\cite{rescher2018}}; \tikz \node[paper] {\reftext{Zett02}\cite{zetterling2002}}; \tikz \node[paper] {\reftext{Weit98}\cite{weitzel1998}}; \tikz \node[paper] {\reftext{Weit96}\cite{weitzel1996}};};
\node[value, scale=1.600000] (holeperpvalue4) at (holeperp4.west) {\num{120}};


\node[symbol] (holepara) at (0+ \dxelec+ \dxelecperp+ \dxelecpara+ \dxhole+ \dxholeperp,0) {$\muppara$};
\coordinate (holepara0) at (holepara.north);
\node[ref, lwholepara] (holepara1) at (holepara0.north west) {\tikz \node[paper] {\reftext{Chow96}\cite{chow1996}};};
\node[value, scale=1.100000] (holeparavalue1) at (holepara1.west) {\num{50}};
\node[ref, lwholepara] (holepara2) at (holepara1.north west) {\tikz \node[paper, fund] {\reftext{Vasc19}\cite{vasconcelos2019}};};
\node[value, scale=1.100000] (holeparavalue2) at (holepara2.west) {\num{54.1}};
\node[ref, lwholepara] (holepara3) at (holepara2.north west) {\tikz \node[paper, fund] {\reftext{Bell99}\cite{bellotti1999}};};
\node[value, scale=1.100000] (holeparavalue3) at (holepara3.west) {\num{73}};
\node[ref, lwholepara] (holepara4) at (holepara3.north west) {\tikz \node[paper] {\reftext{Ayal04}\cite{ayalew2004}};};
\node[value, scale=1.100000] (holeparavalue4) at (holepara4.west) {\num{115}};
\node[ref, lwholepara] (holepara5) at (holepara4.north west) {\tikz \node[paper] {\reftext{Capa22}\cite{capan2022}}; \tikz \node[paper] {\reftext{Bere21}\cite{berens2021}}; \tikz \node[paper] {\reftext{Kimo15}\cite{kimoto2015}};};
\node[value, scale=1.300000] (holeparavalue5) at (holepara5.west) {\num{120}};


==> data/mobility_figure_ratio.tex <==


\node[symbol] (elec) at (0,0) {$\munperp/\munpara$};
\coordinate (elec0) at (elec.north);
\node[ref, lwelec] (elec1) at (elec0.north west) {\tikz \node[paper, fund] {\reftext{Chen20}\cite{cheng2020}};};
\node[value, scale=1.100000] (elecvalue1) at (elec1.west) {\num{0.69}};
\node[ref, lwelec] (elec2) at (elec1.north west) {\tikz \node[paper, fund] {\reftext{Iwat00}\cite{iwata2000}}; \tikz \node[paper, fund] {\reftext{Son95}\cite{son1995}};};
\node[value, scale=1.200000] (elecvalue2) at (elec2.west) {\num{0.7}};
\node[ref, lwelec] (elec3) at (elec2.north west) {\tikz \node[paper, fund] {\reftext{Josh95}\cite{joshi1995}};};
\node[value, scale=1.100000] (elecvalue3) at (elec3.west) {\num{0.75}};
\node[ref, lwelec] (elec4) at (elec3.north west) {\tikz \node[paper] {\reftext{Casa96}\cite{casady1996}};};
\node[value, scale=1.100000] (elecvalue4) at (elec4.west) {\num{0.76}};
\node[ref, lwelec] (elec5) at (elec4.north west) {\tikz \node[paper, fund] {\reftext{Mick98}\cite{mickevicius1998}};};
\node[value, scale=1.100000] (elecvalue5) at (elec5.west) {\num{0.79}};
\node[ref, lwelec] (elec6) at (elec5.north west) {\tikz \node[paper] {\reftext{Neil12}\cite{neilainglesias2012}}; \tikz \node[paper] {\reftext{Alba10}\cite{albanese2010}}; \tikz \node[paper] {\reftext{Ayal04}\cite{ayalew2004}}; \tikz \node[paper] {\reftext{Rosc01}\cite{roschke2001}}; \tikz \node[paper] {\reftext{Lade00}\cite{ladesmartin2000}};};
\node[value, scale=1.500000] (elecvalue6) at (elec6.west) {\num{0.8}};
\node[ref, lwelec] (elec7) at (elec6.north west) {\tikz \node[paper, fund] {\reftext{Nils96}\cite{nilsson1996}};};
\node[value, scale=1.100000] (elecvalue7) at (elec7.west) {\num{0.82}};
\node[ref, lwelec] (elec8) at (elec7.north west) {\tikz \node[paper] {\reftext{Jin24}\cite{jin2024}}; \tikz \node[paper] {\reftext{Rakh20}\cite{rakheja2020}}; \tikz \node[paper] {\reftext{Joha19}\cite{johannesson2019}}; \tikz \node[paper] {\reftext{Arva19}\cite{arvanitopoulos2019}}; \tikz \node[paper] {\reftext{Lutz18}\cite{lutz2018}}; \tikz \node[paper] {\reftext{Naug17}\cite{naugarhiya2017}}; \tikz \node[paper] {\reftext{Chen15}\cite{chen2015}}; \tikz \node[paper] {\reftext{Stef14}\cite{stefanakis2014}}; \tikz \node[paper] {\reftext{Hata13}\cite{hatakeyama2013}}; \tikz \node[paper] {\reftext{Lutz11}\cite{lutz2011}}; \tikz \node[paper] {\reftext{Schr06}\cite{schroeder2006}}; \tikz \node[paper] {\reftext{Bert04a}\cite{bertilsson2004a}}; \tikz \node[paper] {\reftext{Line03}\cite{linewih2003}}; \tikz \node[paper, fund] {\reftext{Hata03}\cite{hatakeyama2003}}; \tikz \node[paper] {\reftext{Zett02}\cite{zetterling2002}}; \tikz \node[paper] {\reftext{Lee02}\cite{lee2002}}; \tikz \node[paper] {\reftext{Mick98a}\cite{mickevicius1998a}}; \tikz \node[paper] {\reftext{Palm97}\cite{palmour1997}}; \tikz \node[paper, fund] {\reftext{Mats97}\cite{matsunami1997}}; \tikz \node[paper] {\reftext{Bako97}\cite{bakowski1997}}; \tikz \node[paper, fund] {\reftext{Scha94}\cite{schaffer1994}}; \tikz \node[paper, fund] {\reftext{Scha94a}\cite{schadt1994a}};};
\node[value, scale=3.200000] (elecvalue8) at (elec8.west) {\num{0.83}};
\node[ref, lwelec] (elec9) at (elec8.north west) {\tikz \node[paper] {\reftext{Bert04}\cite{bertilsson2004}};};
\node[value, scale=1.100000] (elecvalue9) at (elec9.west) {\num{0.84}};
\node[ref, lwelec] (elec10) at (elec9.north west) {\tikz \node[paper] {\reftext{Ostl24}\cite{ostling2024}}; \tikz \node[paper] {\reftext{Capa22}\cite{capan2022}}; \tikz \node[paper, fund] {\reftext{Ishi21}\cite{ishikawa2021}}; \tikz \node[paper] {\reftext{Bere21}\cite{berens2021}}; \tikz \node[paper] {\reftext{Kimo19}\cite{kimoto2019}}; \tikz \node[paper] {\reftext{Resc18}\cite{rescher2018}}; \tikz \node[paper] {\reftext{Kimo15}\cite{kimoto2015}}; \tikz \node[paper] {\reftext{Kimo14a}\cite{kimoto2014a}}; \tikz \node[paper, fund] {\reftext{Bert01}\cite{bertilsson2001}};};
\node[value, scale=1.900000] (elecvalue10) at (elec10.west) {\num{0.85}};
\node[ref, lwelec] (elec11) at (elec10.north west) {\tikz \node[paper, fund] {\reftext{Choy97d}\cite{choyke1997d}};};
\node[value, scale=1.100000] (elecvalue11) at (elec11.west) {\num{0.86}};
\node[ref, lwelec] (elec12) at (elec11.north west) {\tikz \node[paper] {\reftext{Zhu08}\cite{zhu2008}};};
\node[value, scale=1.100000] (elecvalue12) at (elec12.west) {\num{0.89}};
\node[ref, lwelec] (elec13) at (elec12.north west) {\tikz \node[paper] {\reftext{Mukh23}\cite{mukherjee2023}}; \tikz \node[paper] {\reftext{Wije11}\cite{wijesundara2011}}; \tikz \node[paper] {\reftext{Neud06}\cite{neudeck2006}}; \tikz \node[paper] {\reftext{Neud01}\cite{neudeck2001}}; \tikz \node[paper] {\reftext{Srir97}\cite{sriram1997}};};
\node[value, scale=1.500000] (elecvalue13) at (elec13.west) {\num{1}};
\node[ref, lwelec] (elec14) at (elec13.north west) {\tikz \node[paper] {\reftext{Chow17}\cite{chow2017}}; \tikz \node[paper] {\reftext{Dhan10}\cite{dhanaraj2010}}; \tikz \node[paper] {\reftext{Klei09}\cite{klein2009}}; \tikz \node[paper] {\reftext{Cole04}\cite{cole2004}}; \tikz \node[paper] {\reftext{Chow04}\cite{chow2004}}; \tikz \node[paper] {\reftext{Elas02}\cite{elasser2002}}; \tikz \node[paper] {\reftext{Chow00a}\cite{chow2000a}}; \tikz \node[paper] {\reftext{Chow00}\cite{chow2000}}; \tikz \node[paper] {\reftext{Chow97}\cite{chow1997}}; \tikz \node[paper] {\reftext{Chow96}\cite{chow1996}};};
\node[value, scale=2.000000] (elecvalue14) at (elec14.west) {\num{1.11}};
\node[ref, lwelec] (elec15) at (elec14.north west) {\tikz \node[paper] {\reftext{Dena22}\cite{denapoli2022}}; \tikz \node[paper] {\reftext{Naka97}\cite{nakashima1997}}; \tikz \node[paper, fund] {\reftext{Hari95}\cite{harima1995}};};
\node[value, scale=1.300000] (elecvalue15) at (elec15.west) {\num{1.2}};


\node[symbol] (hole) at (0+ \dxelec,0) {$\mupperp/\muppara$};
\coordinate (hole0) at (hole.north);
\node[ref, lwhole] (hole1) at (hole0.north west) {\tikz \node[paper] {\reftext{Alba10}\cite{albanese2010}};};
\node[value, scale=1.100000] (holevalue1) at (hole1.west) {\num{0.8}};
\node[ref, lwhole] (hole2) at (hole1.north west) {\tikz \node[paper] {\reftext{Arva19}\cite{arvanitopoulos2019}}; \tikz \node[paper] {\reftext{Ayal04}\cite{ayalew2004}}; \tikz \node[paper] {\reftext{Bako97}\cite{bakowski1997}};};
\node[value, scale=1.300000] (holevalue2) at (hole2.west) {\num{1}};
\node[ref, lwhole] (hole3) at (hole2.north west) {\tikz \node[paper, fund] {\reftext{Ishi24}\cite{ishikawa2024}};};
\node[value, scale=1.100000] (holevalue3) at (hole3.west) {\num{1.11}};
\node[ref, lwhole] (hole4) at (hole3.north west) {\tikz \node[paper] {\reftext{Joha19}\cite{johannesson2019}}; \tikz \node[paper] {\reftext{Naug17}\cite{naugarhiya2017}}; \tikz \node[paper] {\reftext{Stef14}\cite{stefanakis2014}}; \tikz \node[paper] {\reftext{Pari13}\cite{parisini2013}}; \tikz \node[paper] {\reftext{Hata13}\cite{hatakeyama2013}}; \tikz \node[paper, fund] {\reftext{Hata03}\cite{hatakeyama2003}};};
\node[value, scale=1.600000] (holevalue4) at (hole4.west) {\num{1.15}};
\node[ref, lwhole] (hole5) at (hole4.north west) {\tikz \node[paper] {\reftext{Kimo19}\cite{kimoto2019}};};
\node[value, scale=1.100000] (holevalue5) at (hole5.west) {\num{1.18}};
\node[ref, lwhole] (hole6) at (hole5.north west) {\tikz \node[paper, fund] {\reftext{Bell99}\cite{bellotti1999}};};
\node[value, scale=1.100000] (holevalue6) at (hole6.west) {\num{1.33}};


==> data/mobility_figure_vsat_field_elec.tex <==
\pgfplotsset{cycle list name=CT}
\addplot+[samples=\sampleCount, domain=1.00E+04:3.00E+05] {vsat(2.08E+07,0.825)}; 
\addlegendentry{\reftext{Khan98}\cite{khan1998} $\perp$}
\addplot+[samples=\sampleCount, domain=1.00E+04:1.00E+06] {vsat(2.00E+07,1)}; 
\addlegendentry{\reftext{Mick98}\cite{mickevicius1998} $\perp$}
\addplot+[samples=\sampleCount, domain=1.00E+04:1.00E+06] {vsat(2.50E+07,1)}; 
\addlegendentry{\reftext{Mick98}\cite{mickevicius1998} $\parallel$}
\addplot+[samples=\sampleCount, domain=3.00E+03:5.00E+05] {vsat(2.2e7,1.2)}; 
\addlegendentry{\reftext{Khan00}\cite{khan2000} $\perp$}
\addplot+[samples=\sampleCount, domain=3.00E+03:5.00E+05] {vsat(1.6e7,2.2)}; 
\addlegendentry{\reftext{Khan00}\cite{khan2000} $\perp$}
\addplot+[samples=\sampleCount, domain=2.00E+03:3.00E+06] {vsat(2.10E+07,0.84/1.1)}; 
\addlegendentry{\reftext{Bert01}\cite{bertilsson2001} $\perp$}
\addplot+[samples=\sampleCount, domain=2.00E+03:3.00E+06] {vsat(1.70E+07,0.84/1.1)}; 
\addlegendentry{\reftext{Bert01}\cite{bertilsson2001} $\parallel$}
\addplot+[samples=\sampleCount, domain=3.00E+03:1.00E+06] {vsat(2.40E+07,0.85)}; 
\addlegendentry{\reftext{Rosc01}\cite{roschke2001}}
\addplot+[samples=\sampleCount, domain=2.00E+03:2.00E+06] {vsat(2.00E+07,0.9/1.1)}; 
\addlegendentry{\reftext{Bert04a}\cite{bertilsson2004a} $\perp$}
\addplot+[samples=\sampleCount, domain=2.00E+03:2.00E+06] {vsat(1.70E+07,0.9/1.1)}; 
\addlegendentry{\reftext{Bert04a}\cite{bertilsson2004a} $\parallel$}
\addplot+[samples=\sampleCount, domain=\xMin:\xMax] {vsat(2.00E+07,1)}; 
\addlegendentry{\reftext{Das15}\cite{das2015}}
\addplot+[samples=\sampleCount, domain=\xMin:\xMax] {vsat(8.70E+06,2)}; 
\addlegendentry{\reftext{Bela22}\cite{belas2022}}


==> data/mobility_figure_vsat_values_elec.tex <==


\node[symbol] (elecvsat) at (0,0) {$\vsat$};
\coordinate (elecvsat0) at (elecvsat.north);
\node[ref, lwelecvsat] (elecvsat1) at (elecvsat0.north west) {\tikz \node[paper] {\reftext{Ostl24}\cite{ostling2024}}; \tikz \node[paper] {\reftext{Elah17}\cite{elahipanah2017}};};
\node[value, scale=1.200000] (elecvsatvalue1) at (elecvsat1.west) {\num{2}};
\node[ref, lwelecvsat] (elecvsat2) at (elecvsat1.north west) {\tikz \node[paper, fund] {\reftext{Sank00}\cite{sankin2000}};};
\node[value, scale=1.100000] (elecvsatvalue2) at (elecvsat2.west) {\num{3.30E+06}};
\node[ref, lwelecvsat] (elecvsat3) at (elecvsat2.north west) {\tikz \node[paper] {\reftext{Zhan08}\cite{zhang2008}};};
\node[value, scale=1.100000] (elecvsatvalue3) at (elecvsat3.west) {\num{8.00E+06}};
\node[ref, lwelecvsat] (elecvsat4) at (elecvsat3.north west) {\tikz \node[paper, fund] {\reftext{Bela22}\cite{belas2022}};};
\node[value, scale=1.100000] (elecvsatvalue4) at (elecvsat4.west) {\num{8.70E+06}};
\node[ref, lwelecvsat] (elecvsat5) at (elecvsat4.north west) {\tikz \node[paper] {\reftext{Nawa10}\cite{nawaz2010}};};
\node[value, scale=1.100000] (elecvsatvalue5) at (elecvsat5.west) {\num{1.50E+07}};
\node[ref, lwelecvsat] (elecvsat6) at (elecvsat5.north west) {\tikz \node[paper, fund] {\reftext{Aktu09}\cite{akturk2009}};};
\node[value, scale=1.100000] (elecvsatvalue6) at (elecvsat6.west) {\num{1.60E+07}};
\node[ref, lwelecvsat] (elecvsat7) at (elecvsat6.north west) {\tikz \node[paper] {\reftext{Liu21}\cite{liu2021}}; \tikz \node[paper, fund] {\reftext{Sun10}\cite{sun2010}};};
\node[value, scale=1.200000] (elecvsatvalue7) at (elecvsat7.west) {\num{1.80E+07}};
\node[ref, lwelecvsat] (elecvsat8) at (elecvsat7.north west) {\tikz \node[paper, fund] {\reftext{Jais24}\cite{jaiswal2024}}; \tikz \node[paper] {\reftext{Pear23}\cite{pearton2023}}; \tikz \node[paper] {\reftext{Mukh23}\cite{mukherjee2023}}; \tikz \node[paper] {\reftext{Lang22}\cite{langpoklakpam2022}}; \tikz \node[paper] {\reftext{Dena22}\cite{denapoli2022}}; \tikz \node[paper] {\reftext{Zegh20}\cite{zeghdar2020}}; \tikz \node[paper] {\reftext{Mukh20a}\cite{mukherjee2020a}}; \tikz \node[paper] {\reftext{Mats20}\cite{matsunami2020}}; \tikz \node[paper] {\reftext{Sole19}\cite{soler2019}}; \tikz \node[paper] {\reftext{Guo19}\cite{guo2019}}; \tikz \node[paper] {\reftext{Pear18}\cite{pearton2018}}; \tikz \node[paper] {\reftext{Lutz18}\cite{lutz2018}}; \tikz \node[paper] {\reftext{Hass18}\cite{hassan2018}}; \tikz \node[paper] {\reftext{Lebe17}\cite{lebedev2017}}; \tikz \node[paper] {\reftext{Chow17}\cite{chow2017}}; \tikz \node[paper] {\reftext{Arvi17}\cite{arvinte2017}}; \tikz \node[paper] {\reftext{Uhne15}\cite{uhnevionak2015}}; \tikz \node[paper, no4H] {\reftext{Mant15}\cite{mantooth2015}}; \tikz \node[paper] {\reftext{Fuji15}\cite{fujita2015}}; \tikz \node[paper, fund] {\reftext{Das15}\cite{das2015}}; \tikz \node[paper] {\reftext{Chen15}\cite{chen2015}}; \tikz \node[paper] {\reftext{Usma14}\cite{usman2014}}; \tikz \node[paper] {\reftext{Pezz13}\cite{pezzimenti2013}}; \tikz \node[paper] {\reftext{Pell13}\cite{pellish2013}}; \tikz \node[paper] {\reftext{Neud13}\cite{neudeck2013}}; \tikz \node[paper] {\reftext{Mant13}\cite{mantooth2013}}; \tikz \node[paper] {\reftext{Neil12}\cite{neilainglesias2012}}; \tikz \node[paper] {\reftext{Khal12}\cite{khalid2012}}; \tikz \node[paper] {\reftext{Bion12}\cite{biondo2012}}; \tikz \node[paper] {\reftext{Wije11}\cite{wijesundara2011}}; \tikz \node[paper] {\reftext{Ostl11a}\cite{ostling2011a}}; \tikz \node[paper] {\reftext{Ostl11}\cite{ostling2011}}; \tikz \node[paper] {\reftext{Lutz11}\cite{lutz2011}}; \tikz \node[paper] {\reftext{Gerh11}\cite{gerhardt2011}}; \tikz \node[paper] {\reftext{Butt11}\cite{buttay2011}}; \tikz \node[paper] {\reftext{Beye11}\cite{beyer2011}}; \tikz \node[paper] {\reftext{Zhan10}\cite{zhang2010}}; \tikz \node[paper] {\reftext{Su10}\cite{su2010}}; \tikz \node[paper] {\reftext{Dhan10}\cite{dhanaraj2010}}; \tikz \node[paper] {\reftext{Alba10}\cite{albanese2010}}; \tikz \node[paper] {\reftext{Zhan09}\cite{zhang2009}}; \tikz \node[paper] {\reftext{Zhu08}\cite{zhu2008}}; \tikz \node[paper] {\reftext{Pezz08}\cite{pezzimenti2008}}; \tikz \node[paper] {\reftext{Cha08}\cite{cha2008}}; \tikz \node[paper] {\reftext{Sze07}\cite{sze2007}}; \tikz \node[paper] {\reftext{Mill07}\cite{millan2007}}; \tikz \node[paper] {\reftext{Zhao06}\cite{zhao2006}}; \tikz \node[paper] {\reftext{Will06}\cite{willander2006}}; \tikz \node[paper] {\reftext{Neud06}\cite{neudeck2006}}; \tikz \node[paper] {\reftext{Resh05}\cite{reshanov2005}}; \tikz \node[paper] {\reftext{Pens05}\cite{pensl2005}}; \tikz \node[paper] {\reftext{Bhat05}\cite{bhatnagar2005}}; \tikz \node[paper] {\reftext{Ozpi04}\cite{ozpineci2004}}; \tikz \node[paper] {\reftext{Mats04a}\cite{matsunami2004a}}; \tikz \node[paper] {\reftext{Cole04}\cite{cole2004}}; \tikz \node[paper] {\reftext{Chow04}\cite{chow2004}}; \tikz \node[paper] {\reftext{Hudg03}\cite{hudgins2003}}; \tikz \node[paper] {\reftext{Han03}\cite{han2003}}; \tikz \node[paper] {\reftext{Elas03}\cite{elasser2003}}; \tikz \node[paper] {\reftext{Doga03}\cite{dogan2003}}; \tikz \node[paper] {\reftext{Zhan02}\cite{zhang2002}}; \tikz \node[paper] {\reftext{Zett02}\cite{zetterling2002}}; \tikz \node[paper] {\reftext{Trew02}\cite{trew2002}}; \tikz \node[paper] {\reftext{Powe02}\cite{powell2002}}; \tikz \node[paper] {\reftext{Masr02}\cite{masri2002}}; \tikz \node[paper] {\reftext{Lee02}\cite{lee2002}}; \tikz \node[paper] {\reftext{Elas02}\cite{elasser2002}}; \tikz \node[paper] {\reftext{Neud01}\cite{neudeck2001}}; \tikz \node[paper] {\reftext{Nall00}\cite{nallet2000}}; \tikz \node[paper] {\reftext{Elas00}\cite{elasser2000}}; \tikz \node[paper] {\reftext{Dmit00}\cite{dmitriev2000}}; \tikz \node[paper] {\reftext{Codr00}\cite{codreanu2000}}; \tikz \node[paper] {\reftext{Chow00a}\cite{chow2000a}}; \tikz \node[paper] {\reftext{Chow00}\cite{chow2000}}; \tikz \node[paper] {\reftext{Nall99}\cite{nallet1999}}; \tikz \node[paper] {\reftext{Lebe99}\cite{lebedev1999}}; \tikz \node[paper] {\reftext{Burk99}\cite{burk1999}}; \tikz \node[paper] {\reftext{Bell99}\cite{bellotti1999}}; \tikz \node[paper] {\reftext{Agar99}\cite{agarwal1999}}; \tikz \node[paper] {\reftext{Wrig98}\cite{wright1998}}; \tikz \node[paper] {\reftext{Weit98}\cite{weitzel1998}}; \tikz \node[paper] {\reftext{Shah98}\cite{shah1998}}; \tikz \node[paper] {\reftext{Rosc98}\cite{roschke1998}}; \tikz \node[paper] {\reftext{Trew97}\cite{trew1997}}; \tikz \node[paper] {\reftext{Srir97}\cite{sriram1997}}; \tikz \node[paper] {\reftext{Chow97}\cite{chow1997}}; \tikz \node[paper] {\reftext{Chel97}\cite{chelnokov1997}}; \tikz \node[paper] {\reftext{Yode96}\cite{yoder1996}}; \tikz \node[paper] {\reftext{Wrig96}\cite{wright1996}}; \tikz \node[paper] {\reftext{Weit96}\cite{weitzel1996}}; \tikz \node[paper] {\reftext{Chow96}\cite{chow1996}}; \tikz \node[paper] {\reftext{Agar96}\cite{agarwal1996}}; \tikz \node[paper] {\reftext{Neud95}\cite{neudeck1995}}; \tikz \node[paper] {\reftext{Weit94}\cite{weitzel1994}}; \tikz \node[paper, no4H] {\reftext{Ruff94}\cite{ruff1994}}; \tikz \node[paper] {\reftext{Gotz93}\cite{gotz1993}}; \tikz \node[paper, no4H] {\reftext{Bhat93}\cite{bhatnagar1993}}; \tikz \node[paper, no4H] {\reftext{Powe89}\cite{powell1989}}; \tikz \node[paper, no4H] {\reftext{V.mu77a}\cite{v.muench1977a}};};
\node[value, scale=7.000000] (elecvsatvalue8) at (elecvsat8.west) {\num{2.00E+07}};
\node[ref, lwelecvsat] (elecvsat9) at (elecvsat8.north west) {\tikz \node[paper] {\reftext{Bane21}\cite{banerjee2021}};};
\node[value, scale=1.100000] (elecvsatvalue9) at (elecvsat9.west) {\num{2.12E+07}};
\node[ref, lwelecvsat] (elecvsat10) at (elecvsat9.north west) {\tikz \node[paper] {\reftext{Lech21}\cite{lechner2021}}; \tikz \node[paper] {\reftext{Chou21}\cite{choudhary2021}}; \tikz \node[paper] {\reftext{Bere21}\cite{berens2021}}; \tikz \node[paper] {\reftext{Rakh20}\cite{rakheja2020}}; \tikz \node[paper] {\reftext{Jiya20}\cite{jiya2020}}; \tikz \node[paper] {\reftext{Trip19}\cite{tripathi2019}}; \tikz \node[paper] {\reftext{Joha19}\cite{johannesson2019}}; \tikz \node[paper] {\reftext{Bali19}\cite{baliga2019}}; \tikz \node[paper] {\reftext{Resc18}\cite{rescher2018}}; \tikz \node[paper] {\reftext{Arva17}\cite{arvanitopoulos2017}}; \tikz \node[paper] {\reftext{Kimo15}\cite{kimoto2015}}; \tikz \node[paper] {\reftext{Kimo14a}\cite{kimoto2014a}}; \tikz \node[paper] {\reftext{Schr06}\cite{schroeder2006}}; \tikz \node[paper] {\reftext{Bros04}\cite{brosselard2004}};};
\node[value, scale=2.400000] (elecvsatvalue10) at (elecvsat10.west) {\num{2.20E+07}};
\node[ref, lwelecvsat] (elecvsat11) at (elecvsat10.north west) {\tikz \node[paper, fund] {\reftext{Rosc01}\cite{roschke2001}};};
\node[value, scale=1.100000] (elecvsatvalue11) at (elecvsat11.west) {\num{2.40E+07}};
\node[ref, lwelecvsat] (elecvsat12) at (elecvsat11.north west) {\tikz \node[paper] {\reftext{Wang99}\cite{wang1999}}; \tikz \node[paper] {\reftext{Itoh96}\cite{itoh1996}};};
\node[value, scale=1.200000] (elecvsatvalue12) at (elecvsat12.west) {\num{2.70E+07}};


\node[symbol] (elecvsatperp) at (0+ \dxelecvsat,0) {$\vsperp$};
\coordinate (elecvsatperp0) at (elecvsatperp.north);
\node[ref, lwelecvsatperp] (elecvsatperp1) at (elecvsatperp0.north west) {\tikz \node[paper, fund] {\reftext{Tana24}\cite{tanaka2024}}; \tikz \node[paper, fund] {\reftext{Arda05}\cite{ardaravicius2005}};};
\node[value, scale=1.200000] (elecvsatperpvalue1) at (elecvsatperp1.west) {\num{1.40E+07}};
\node[ref, lwelecvsatperp] (elecvsatperp2) at (elecvsatperp1.north west) {\tikz \node[paper, fund] {\reftext{Donn09}\cite{donnarumma2009}};};
\node[value, scale=1.100000] (elecvsatperpvalue2) at (elecvsatperp2.west) {\num{1.85e7}};
\node[ref, lwelecvsatperp] (elecvsatperp3) at (elecvsatperp2.north west) {\tikz \node[paper, fund] {\reftext{Bert04a}\cite{bertilsson2004a}}; \tikz \node[paper, fund] {\reftext{Mick98}\cite{mickevicius1998}};};
\node[value, scale=1.200000] (elecvsatperpvalue3) at (elecvsatperp3.west) {\num{2.00E+07}};
\node[ref, lwelecvsatperp] (elecvsatperp4) at (elecvsatperp3.north west) {\tikz \node[paper, fund] {\reftext{Khan98}\cite{khan1998}};};
\node[value, scale=1.100000] (elecvsatperpvalue4) at (elecvsatperp4.west) {\num{2.08E+07}};
\node[ref, lwelecvsatperp] (elecvsatperp5) at (elecvsatperp4.north west) {\tikz \node[paper, fund] {\reftext{Bert01}\cite{bertilsson2001}}; \tikz \node[paper, fund] {\reftext{Nils96}\cite{nilsson1996}}; \tikz \node[paper, fund] {\reftext{Josh95}\cite{joshi1995}};};
\node[value, scale=1.300000] (elecvsatperpvalue5) at (elecvsatperp5.west) {\num{2.10E+07}};
\node[ref, lwelecvsatperp] (elecvsatperp6) at (elecvsatperp5.north west) {\tikz \node[paper, fund] {\reftext{Hjel03}\cite{hjelm2003}};};
\node[value, scale=1.100000] (elecvsatperpvalue6) at (elecvsatperp6.west) {\num{2.12E+07}};
\node[ref, lwelecvsatperp] (elecvsatperp7) at (elecvsatperp6.north west) {\tikz \node[paper] {\reftext{Khan00b}\cite{khan2000b}}; \tikz \node[paper, fund] {\reftext{Khan00}\cite{khan2000}};};
\node[value, scale=1.200000] (elecvsatperpvalue7) at (elecvsatperp7.west) {\num{2.2e7}};
\node[ref, lwelecvsatperp] (elecvsatperp8) at (elecvsatperp7.north west) {\tikz \node[paper] {\reftext{Jin24}\cite{jin2024}}; \tikz \node[paper] {\reftext{Chen20}\cite{cheng2020}}; \tikz \node[paper] {\reftext{Kimo19}\cite{kimoto2019}}; \tikz \node[paper] {\reftext{Arva19}\cite{arvanitopoulos2019}}; \tikz \node[paper] {\reftext{Loph18}\cite{lophitis2018}}; \tikz \node[paper] {\reftext{Naug17}\cite{naugarhiya2017}}; \tikz \node[paper, fund] {\reftext{Hata13}\cite{hatakeyama2013}}; \tikz \node[paper] {\reftext{Ayal04}\cite{ayalew2004}}; \tikz \node[paper, fund] {\reftext{Lade00}\cite{ladesmartin2000}};};
\node[value, scale=1.900000] (elecvsatperpvalue8) at (elecvsatperp8.west) {\num{2.20E+07}};
\node[ref, lwelecvsatperp] (elecvsatperp9) at (elecvsatperp8.north west) {\tikz \node[paper, fund] {\reftext{Nils00}\cite{nilsson2000}};};
\node[value, scale=1.100000] (elecvsatperpvalue9) at (elecvsatperp9.west) {\num{2.26E+07}};


\node[symbol] (elecvsatpara) at (0+ \dxelecvsat+ \dxelecvsatperp,0) {$\vspara$};
\coordinate (elecvsatpara0) at (elecvsatpara.north);
\node[ref, lwelecvsatpara] (elecvsatpara1) at (elecvsatpara0.north west) {\tikz \node[paper, fund] {\reftext{Vass00}\cite{vassilevski2000}};};
\node[value, scale=1.100000] (elecvsatparavalue1) at (elecvsatpara1.west) {\num{8e6}};
\node[ref, lwelecvsatpara] (elecvsatpara2) at (elecvsatpara1.north west) {\tikz \node[paper] {\reftext{Naug17}\cite{naugarhiya2017}};};
\node[value, scale=1.100000] (elecvsatparavalue2) at (elecvsatpara2.west) {\num{1.20E+07}};
\node[ref, lwelecvsatpara] (elecvsatpara3) at (elecvsatpara2.north west) {\tikz \node[paper] {\reftext{Jin24}\cite{jin2024}};};
\node[value, scale=1.100000] (elecvsatparavalue3) at (elecvsatpara3.west) {\num{1.32E+07}};
\node[ref, lwelecvsatpara] (elecvsatpara4) at (elecvsatpara3.north west) {\tikz \node[paper, fund] {\reftext{Hjel03}\cite{hjelm2003}};};
\node[value, scale=1.100000] (elecvsatparavalue4) at (elecvsatpara4.west) {\num{1.58E+07}};
\node[ref, lwelecvsatpara] (elecvsatpara5) at (elecvsatpara4.north west) {\tikz \node[paper, fund] {\reftext{Nils00}\cite{nilsson2000}};};
\node[value, scale=1.100000] (elecvsatparavalue5) at (elecvsatpara5.west) {\num{1.64E+07}};
\node[ref, lwelecvsatpara] (elecvsatpara6) at (elecvsatpara5.north west) {\tikz \node[paper, fund] {\reftext{Bert04a}\cite{bertilsson2004a}}; \tikz \node[paper, fund] {\reftext{Bert01}\cite{bertilsson2001}};};
\node[value, scale=1.200000] (elecvsatparavalue6) at (elecvsatpara6.west) {\num{1.70E+07}};
\node[ref, lwelecvsatpara] (elecvsatpara7) at (elecvsatpara6.north west) {\tikz \node[paper, fund] {\reftext{Nils96}\cite{nilsson1996}};};
\node[value, scale=1.100000] (elecvsatparavalue7) at (elecvsatpara7.west) {\num{1.80E+07}};
\node[ref, lwelecvsatpara] (elecvsatpara8) at (elecvsatpara7.north west) {\tikz \node[paper, fund] {\reftext{Zhao00}\cite{zhao2000}};};
\node[value, scale=1.100000] (elecvsatparavalue8) at (elecvsatpara8.west) {\num{1.83E+07}};
\node[ref, lwelecvsatpara] (elecvsatpara9) at (elecvsatpara8.north west) {\tikz \node[paper] {\reftext{Loph18}\cite{lophitis2018}};};
\node[value, scale=1.100000] (elecvsatparavalue9) at (elecvsatpara9.west) {\num{1.90E+07}};
\node[ref, lwelecvsatpara] (elecvsatpara10) at (elecvsatpara9.north west) {\tikz \node[paper] {\reftext{Nava08}\cite{nava2008}}; \tikz \node[paper, no4H] {\reftext{Pers05}\cite{persson2005}}; \tikz \node[paper] {\reftext{Casa96}\cite{casady1996}};};
\node[value, scale=1.300000] (elecvsatparavalue10) at (elecvsatpara10.west) {\num{2.00E+07}};
\node[ref, lwelecvsatpara] (elecvsatpara11) at (elecvsatpara10.north west) {\tikz \node[paper, fund] {\reftext{Mick98}\cite{mickevicius1998}};};
\node[value, scale=1.100000] (elecvsatparavalue11) at (elecvsatpara11.west) {\num{2.50E+07}};
\node[ref, lwelecvsatpara] (elecvsatpara12) at (elecvsatpara11.north west) {\tikz \node[paper, fund] {\reftext{Josh95}\cite{joshi1995}};};
\node[value, scale=1.100000] (elecvsatparavalue12) at (elecvsatpara12.west) {\num{2.70E+07}};


==> data/mobility_figure_vsat_values_hole.tex <==


\node[symbol] (holevsat) at (0,0) {$\vsat$};
\coordinate (holevsat0) at (holevsat.north);
\node[ref, lwholevsat] (holevsat1) at (holevsat0.north west) {\tikz \node[paper] {\reftext{Shah98}\cite{shah1998}};};
\node[value, scale=1.100000] (holevsatvalue1) at (holevsat1.west) {\num{1.00E+06}};
\node[ref, lwholevsat] (holevsat2) at (holevsat1.north west) {\tikz \node[paper] {\reftext{Liu21}\cite{liu2021}};};
\node[value, scale=1.100000] (holevsatvalue2) at (holevsat2.west) {\num{8.00E+06}};
\node[ref, lwholevsat] (holevsat3) at (holevsat2.north west) {\tikz \node[paper, fund] {\reftext{Guo25}\cite{guo2025}}; \tikz \node[paper] {\reftext{Nawa10}\cite{nawaz2010}}; \tikz \node[paper, fund] {\reftext{Aktu09}\cite{akturk2009}};};
\node[value, scale=1.300000] (holevsatvalue3) at (holevsat3.west) {\num{1.00E+07}};
\node[ref, lwholevsat] (holevsat4) at (holevsat3.north west) {\tikz \node[paper] {\reftext{Bane21}\cite{banerjee2021}};};
\node[value, scale=1.100000] (holevsatvalue4) at (holevsat4.west) {\num{1.08E+07}};
\node[ref, lwholevsat] (holevsat5) at (holevsat4.north west) {\tikz \node[paper] {\reftext{Kimo19}\cite{kimoto2019}}; \tikz \node[paper] {\reftext{Bali19}\cite{baliga2019}}; \tikz \node[paper] {\reftext{Kimo15}\cite{kimoto2015}}; \tikz \node[paper, fund] {\reftext{Kimo14a}\cite{kimoto2014a}};};
\node[value, scale=1.400000] (holevsatvalue5) at (holevsat5.west) {\num{1.30E+07}};
\node[ref, lwholevsat] (holevsat6) at (holevsat5.north west) {\tikz \node[paper] {\reftext{Zegh20}\cite{zeghdar2020}}; \tikz \node[paper, fund] {\reftext{Das15}\cite{das2015}}; \tikz \node[paper] {\reftext{Chen15}\cite{chen2015}}; \tikz \node[paper] {\reftext{Usma14}\cite{usman2014}}; \tikz \node[paper] {\reftext{Pezz13}\cite{pezzimenti2013}}; \tikz \node[paper] {\reftext{Khal12}\cite{khalid2012}}; \tikz \node[paper] {\reftext{Bion12}\cite{biondo2012}}; \tikz \node[paper] {\reftext{Beye11}\cite{beyer2011}}; \tikz \node[paper] {\reftext{Zhan10}\cite{zhang2010}}; \tikz \node[paper] {\reftext{Zhan09}\cite{zhang2009}}; \tikz \node[paper] {\reftext{Cha08}\cite{cha2008}}; \tikz \node[paper] {\reftext{Bhat05}\cite{bhatnagar2005}}; \tikz \node[paper] {\reftext{Keme02}\cite{kemerley2002}}; \tikz \node[paper] {\reftext{Nall99}\cite{nallet1999}}; \tikz \node[paper] {\reftext{Wrig98}\cite{wright1998}}; \tikz \node[paper] {\reftext{Wrig96}\cite{wright1996}}; \tikz \node[paper, no4H] {\reftext{Ruff94}\cite{ruff1994}};};
\node[value, scale=2.700000] (holevsatvalue6) at (holevsat6.west) {\num{2.00E+07}};
\node[ref, lwholevsat] (holevsat7) at (holevsat6.north west) {\tikz \node[paper] {\reftext{Lech21}\cite{lechner2021}}; \tikz \node[paper] {\reftext{Chou21}\cite{choudhary2021}}; \tikz \node[paper] {\reftext{Rakh20}\cite{rakheja2020}}; \tikz \node[paper] {\reftext{Loph18}\cite{lophitis2018}}; \tikz \node[paper] {\reftext{Arva17}\cite{arvanitopoulos2017}};};
\node[value, scale=1.500000] (holevsatvalue7) at (holevsat7.west) {\num{2.20E+07}};
\node[ref, lwholevsat] (holevsat8) at (holevsat7.north west) {\tikz \node[paper] {\reftext{Wang99}\cite{wang1999}};};
\node[value, scale=1.100000] (holevsatvalue8) at (holevsat8.west) {\num{2.70E+07}};


\node[symbol] (holevsatperp) at (0+ \dxholevsat,0) {$\vsperp$};
\coordinate (holevsatperp0) at (holevsatperp.north);
\node[ref, lwholevsatperp] (holevsatperp1) at (holevsatperp0.north west) {\tikz \node[paper] {\reftext{Naug17}\cite{naugarhiya2017}}; \tikz \node[paper] {\reftext{Hata13}\cite{hatakeyama2013}};};
\node[value, scale=1.200000] (holevsatperpvalue1) at (holevsatperp1.west) {\num{1.00E+07}};
\node[ref, lwholevsatperp] (holevsatperp2) at (holevsatperp1.north west) {\tikz \node[paper, fund] {\reftext{Hjel03}\cite{hjelm2003}};};
\node[value, scale=1.100000] (holevsatperpvalue2) at (holevsatperp2.west) {\num{1.08E+07}};
\node[ref, lwholevsatperp] (holevsatperp3) at (holevsatperp2.north west) {\tikz \node[paper, fund] {\reftext{Nils00}\cite{nilsson2000}};};
\node[value, scale=1.100000] (holevsatperpvalue3) at (holevsatperp3.west) {\num{1.10E+07}};
\node[ref, lwholevsatperp] (holevsatperp4) at (holevsatperp3.north west) {\tikz \node[paper] {\reftext{Arva19}\cite{arvanitopoulos2019}};};
\node[value, scale=1.100000] (holevsatperpvalue4) at (holevsatperp4.west) {\num{2.20E+07}};


\node[symbol] (holevsatpara) at (0+ \dxholevsat+ \dxholevsatperp,0) {$\vspara$};
\coordinate (holevsatpara0) at (holevsatpara.north);
\node[ref, lwholevsatpara] (holevsatpara1) at (holevsatpara0.north west) {\tikz \node[paper, fund] {\reftext{Nils00}\cite{nilsson2000}};};
\node[value, scale=1.100000] (holevsatparavalue1) at (holevsatpara1.west) {\num{6.50E+06}};
\node[ref, lwholevsatpara] (holevsatpara2) at (holevsatpara1.north west) {\tikz \node[paper, fund] {\reftext{Hjel03}\cite{hjelm2003}};};
\node[value, scale=1.100000] (holevsatparavalue2) at (holevsatpara2.west) {\num{7.30E+06}};
\node[ref, lwholevsatpara] (holevsatpara3) at (holevsatpara2.north west) {\tikz \node[paper] {\reftext{Naug17}\cite{naugarhiya2017}};};
\node[value, scale=1.100000] (holevsatparavalue3) at (holevsatpara3.west) {\num{8.00E+06}};
\node[ref, lwholevsatpara] (holevsatpara4) at (holevsatpara3.north west) {\tikz \node[paper, fund] {\reftext{Zhao00}\cite{zhao2000}};};
\node[value, scale=1.100000] (holevsatparavalue4) at (holevsatpara4.west) {\num{8.60E+06}};


==> data/mobility_ref_chain.tex <==
\node[desc] at (0,0.000000*\dy) {Mobility ($\munperp$, $\munpara$) ($\mupperp$, $\muppara$)};
\node[author] at (0,-1.500000*\dy) {\citeauthor{barrett1967}};
\node[fund, ref] (barrett1967) at (0,-2.500000*\dy) {\reftext{Barr67}\cite{barrett1967}  ( \num{456} ) ( -- )};
\coordinate (barrett1967C) at ($(barrett1967.west)+(\dxStart+\dy,0)$);
\node[ ref] (neuberger1971) at ($(barrett1967C |- 0,-3.500000*\dy)$) {\reftext{Neub71}\cite{neuberger1971}  ( \num{500} ) ( -- )};
\draw (neuberger1971.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-5.500000*\dy) {\citeauthor{lomakina1972}};
\node[fund, ref] (lomakina1972) at (0,-6.500000*\dy) {\reftext{Loma72}\cite{lomakina1972}  ( \num{700} ) ( -- )};
\coordinate (lomakina1972C) at ($(lomakina1972.west)+(\dxStart+\dy,0)$);
\node[ ref] (choyke1974) at ($(lomakina1972C |- 0,-7.500000*\dy)$) {\reftext{Choy74}\cite{choyke1974}  ( \num{700} ) ( -- )};
\draw (choyke1974.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (lomakina1974) at ($(choyke1974.west |- 0,-8.500000*\dy)$) {\reftext{Loma74}\cite{lomakina1974}  ( \num{700} ) ( -- )};
\draw (lomakina1974.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (pankove2014) at ($(lomakina1974.west |- 0,-9.500000*\dy)$) {\reftext{Pank14}\cite{pankove2014}  ( \num{700} ) ( \num{60} )};
\draw (pankove2014.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-11.500000*\dy) {\citeauthor{marshall1974}};
\node[ ref] (marshall1974) at (0,-12.500000*\dy) {\reftext{Mars74}\cite{marshall1974}  ( -- ) ( -- )};
\coordinate (marshall1974C) at ($(marshall1974.west)+(\dxStart+\dy,0)$);
\node[ ref] (hudgins2003) at ($(marshall1974C |- 0,-13.500000*\dy)$) {\reftext{Hudg03}\cite{hudgins2003}  ( \num{700} ) ( -- )};
\draw (hudgins2003.west) -| ++(-\dy,\fy*\dy);
\coordinate (hudgins2003C) at ($(hudgins2003.west)+(\dxStart+\dy,0)$);
\node[ ref] (manikam2011) at ($(hudgins2003C |- 0,-14.500000*\dy)$) {\reftext{Mani11}\cite{manikam2011}  ( \num{700} ) ( -- )};
\draw (manikam2011.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-16.500000*\dy) {\citeauthor{itoh1994}};
\node[fund, ref] (itoh1994) at (0,-17.500000*\dy) {\reftext{Itoh94}\cite{itoh1994}  ( \num{720} ) ( -- )};
\coordinate (itoh1994C) at ($(itoh1994.west)+(\dxStart+\dy,0)$);
\node[ ref] (itoh1995) at ($(itoh1994C |- 0,-18.500000*\dy)$) {\reftext{Itoh95}\cite{itoh1995}  ( \num{720} ) ( -- )};
\draw (itoh1995.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (itoh1996) at ($(itoh1995.west |- 0,-19.500000*\dy)$) {\reftext{Itoh96}\cite{itoh1996}  ( \num{720} ) ( -- )};
\draw (itoh1996.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (kimoto1997) at ($(itoh1996.west |- 0,-20.500000*\dy)$) {\reftext{Kimo97}\cite{kimoto1997}  ( \num{724} ) ( -- )};
\draw (kimoto1997.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-22.500000*\dy) {\citeauthor{larkin1994a}};
\node[no4H, ref] (larkin1994a) at (0,-23.500000*\dy) {\reftext{Lark94a}\cite{larkin1994a}  ( -- ) ( -- )};
\coordinate (larkin1994aC) at ($(larkin1994a.west)+(\dxStart+\dy,0)$);
\node[ ref] (casady1996) at ($(larkin1994aC |- 0,-24.500000*\dy)$) {\reftext{Casa96}\cite{casady1996}  ( \num{1000} ) ( \num{115} )};
\draw (casady1996.west) -| ++(-\dy,\fy*\dy);
\coordinate (casady1996C) at ($(casady1996.west)+(\dxStart+\dy,0)$);
\node[ ref] (gerhardt2011) at ($(casady1996C |- 0,-25.500000*\dy)$) {\reftext{Gerh11}\cite{gerhardt2011}  ( \num{1000} ) ( \num{115} )};
\draw (gerhardt2011.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-27.500000*\dy) {\citeauthor{schaffer1994}};
\node[ ref] (schaffer1994) at (0,-28.500000*\dy) {\reftext{Scha94}\cite{schaffer1994}  ( M ) ( -- )};
\coordinate (schaffer1994C) at ($(schaffer1994.west)+(\dxStart+\dy,0)$);
\node[ ref] (son1995) at ($(schaffer1994C |- 0,-29.500000*\dy)$) {\reftext{Son95}\cite{son1995}  ( \numrange{800}{1000} ) ( -- )};
\draw (son1995.west) -| ++(-\dy,\fy*\dy);
\coordinate (son1995C) at ($(son1995.west)+(\dxStart+\dy,0)$);
\node[ ref] (evwaraye1996) at ($(son1995C |- 0,-30.500000*\dy)$) {\reftext{Evwa96}\cite{evwaraye1996}  ( \num{1000} ) ( -- )};
\draw (evwaraye1996.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (casady1996) at ($(son1995.west |- 0,-31.500000*\dy)$) {\reftext{Casa96}\cite{casady1996}  ( \num{1000} ) ( \num{115} )};
\draw (casady1996.west) -| ++(-\dy,\fy*\dy);
\coordinate (casady1996C) at ($(casady1996.west)+(\dxStart+\dy,0)$);
\node[ ref] (gerhardt2011) at ($(casady1996C |- 0,-32.500000*\dy)$) {\reftext{Gerh11}\cite{gerhardt2011}  ( \num{1000} ) ( \num{115} )};
\draw (gerhardt2011.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (palmour1997) at ($(casady1996.west |- 0,-33.500000*\dy)$) {\reftext{Palm97}\cite{palmour1997} ( \num{950} , \num{1140} ) ( -- )};
\draw (palmour1997.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (raghunathan1998a) at ($(palmour1997.west |- 0,-34.500000*\dy)$) {\reftext{Ragh98a}\cite{raghunathan1998a}  ( -- ) ( \num{115} )};
\draw (raghunathan1998a.west) -| ++(-\dy,\fy*\dy);
\coordinate (raghunathan1998aC) at ($(raghunathan1998a.west)+(\dxStart+\dy,0)$);
\node[ ref] (neudeck2001) at ($(raghunathan1998aC |- 0,-35.500000*\dy)$) {\reftext{Neud01}\cite{neudeck2001} ( \num{800} , \num{800} ) ( \num{115} )};
\draw (neudeck2001.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-37.500000*\dy) {\citeauthor{roschke1998}};
\node[ ref] (roschke1998) at (0,-38.500000*\dy) {\reftext{Rosc98}\cite{roschke1998}  ( -- ) ( -- )};
\coordinate (roschke1998C) at ($(roschke1998.west)+(\dxStart+\dy,0)$);
\node[ ref] (mukherjee2020a) at ($(roschke1998C |- 0,-39.500000*\dy)$) {\reftext{Mukh20a}\cite{mukherjee2020a} ( \num{800} , \num{800} ) ( \num{115} )};
\draw (mukherjee2020a.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-41.500000*\dy) {\citeauthor{weitzel1998}};
\node[ ref] (weitzel1998) at (0,-42.500000*\dy) {\reftext{Weit98}\cite{weitzel1998}  ( \num{800} ) ( \num{120} )};
\coordinate (weitzel1998C) at ($(weitzel1998.west)+(\dxStart+\dy,0)$);
\node[ ref] (neudeck2001) at ($(weitzel1998C |- 0,-43.500000*\dy)$) {\reftext{Neud01}\cite{neudeck2001} ( \num{800} , \num{800} ) ( \num{115} )};
\draw (neudeck2001.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-45.500000*\dy) {\citeauthor{agarwal1999}};
\node[ ref] (agarwal1999) at (0,-46.500000*\dy) {\reftext{Agar99}\cite{agarwal1999}  ( \num{800} ) ( \num{140} )};
\coordinate (agarwal1999C) at ($(agarwal1999.west)+(\dxStart+\dy,0)$);
\node[ ref] (ng2003) at ($(agarwal1999C |- 0,-47.500000*\dy)$) {\reftext{Ng03}\cite{ng2003}  ( \num{800} ) ( \num{100} )};
\draw (ng2003.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-49.500000*\dy) {\citeauthor{siergiej1999}};
\node[ ref] (siergiej1999) at (0,-50.500000*\dy) {\reftext{Sier99}\cite{siergiej1999}  ( -- ) ( -- )};
\coordinate (siergiej1999C) at ($(siergiej1999.west)+(\dxStart+\dy,0)$);
\node[ ref] (belas2022) at ($(siergiej1999C |- 0,-51.500000*\dy)$) {\reftext{Bela22}\cite{belas2022}  ( \num{800} ) ( -- )};
\draw (belas2022.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-53.500000*\dy) {\citeauthor{afanasev2000}};
\node[ ref] (afanasev2000) at (0,-54.500000*\dy) {\reftext{Afan00}\cite{afanasev2000}  ( \num{700} ) ( -- )};
\coordinate (afanasev2000C) at ($(afanasev2000.west)+(\dxStart+\dy,0)$);
\node[ ref] (pacchioni2000) at ($(afanasev2000C |- 0,-55.500000*\dy)$) {\reftext{Pacc00}\cite{pacchioni2000}  ( \num{700} ) ( -- )};
\draw (pacchioni2000.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,0.000000*\dy) {\citeauthor{chow2000}};
\node[ ref] (chow2000) at (\xSepOne,-1.000000*\dy) {\reftext{Chow00}\cite{chow2000} ( \num{720} , \num{650} ) ( -- )};
\coordinate (chow2000C) at ($(chow2000.west)+(\dxStart+\dy,0)$);
\node[guess, ref] (dmitriev2000) at ($(chow2000C |- 0,-2.000000*\dy)$) {\reftext{Dmit00}\cite{dmitriev2000} ( \num{720} , \num{650} ) ( -- )};
\draw (dmitriev2000.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (elasser2002) at ($(dmitriev2000.west |- 0,-3.000000*\dy)$) {\reftext{Elas02}\cite{elasser2002} ( \num{720} , \num{650} ) ( -- )};
\draw (elasser2002.west) -| ++(-\dy,\fy*\dy);
\coordinate (elasser2002C) at ($(elasser2002.west)+(\dxStart+\dy,0)$);
\node[ ref] (su2010) at ($(elasser2002C |- 0,-4.000000*\dy)$) {\reftext{Su10}\cite{su2010}  ( \num{720} ) ( -- )};
\draw (su2010.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (dhanaraj2010) at ($(elasser2002.west |- 0,-5.000000*\dy)$) {\reftext{Dhan10}\cite{dhanaraj2010} ( \num{720} , \num{650} ) ( -- )};
\draw (dhanaraj2010.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-7.000000*\dy) {\citeauthor{khan2000}};
\node[fund, ref] (khan2000) at (\xSepOne,-8.000000*\dy) {\reftext{Khan00}\cite{khan2000}  ( \num{450} ) ( -- )};
\coordinate (khan2000C) at ($(khan2000.west)+(\dxStart+\dy,0)$);
\node[ ref] (khan2000b) at ($(khan2000C |- 0,-9.000000*\dy)$) {\reftext{Khan00b}\cite{khan2000b}  ( \num{450} ) ( -- )};
\draw (khan2000b.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (kimoto2019) at ($(khan2000b.west |- 0,-10.000000*\dy)$) {\reftext{Kimo19}\cite{kimoto2019}  ( \num{450} ) ( -- )};
\draw (kimoto2019.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-12.000000*\dy) {\citeauthor{ladesmartin2000}};
\node[ ref] (ladesmartin2000) at (\xSepOne,-13.000000*\dy) {\reftext{Lade00}\cite{ladesmartin2000}  ( \num{1000} ) ( \num{115} )};
\coordinate (ladesmartin2000C) at ($(ladesmartin2000.west)+(\dxStart+\dy,0)$);
\node[ ref] (rakheja2020) at ($(ladesmartin2000C |- 0,-14.000000*\dy)$) {\reftext{Rakh20}\cite{rakheja2020} ( \num{950} , \num{1150} ) ( \num{120} )};
\draw (rakheja2020.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (lechner2021) at ($(rakheja2020.west |- 0,-15.000000*\dy)$) {\reftext{Lech21}\cite{lechner2021}  ( \num{1000} ) ( \num{115} )};
\draw (lechner2021.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-17.000000*\dy) {\citeauthor{levinshtein2001}};
\node[ ref] (levinshtein2001) at (\xSepOne,-18.000000*\dy) {\reftext{Levi01}\cite{levinshtein2001}  ( \num{<900} ) ( \num{<120} )};
\coordinate (levinshtein2001C) at ($(levinshtein2001.west)+(\dxStart+\dy,0)$);
\node[ ref] (levinshtein2004) at ($(levinshtein2001C |- 0,-19.000000*\dy)$) {\reftext{Levi04}\cite{levinshtein2004}  ( \num{800} ) ( \num{120} )};
\draw (levinshtein2004.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-21.000000*\dy) {\citeauthor{roschke2001}};
\node[ ref] (roschke2001) at (\xSepOne,-22.000000*\dy) {\reftext{Rosc01}\cite{roschke2001}  ( -- ) ( -- )};
\coordinate (roschke2001C) at ($(roschke2001.west)+(\dxStart+\dy,0)$);
\node[ ref] (luo2020) at ($(roschke2001C |- 0,-23.000000*\dy)$) {\reftext{Luo20}\cite{luo2020}  ( \num{950} ) ( -- )};
\draw (luo2020.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-25.000000*\dy) {\citeauthor{zetterling2002}};
\node[ ref] (zetterling2002) at (\xSepOne,-26.000000*\dy) {\reftext{Zett02}\cite{zetterling2002} ( \num{950} , \num{1150} ) ( \num{120} )};
\coordinate (zetterling2002C) at ($(zetterling2002.west)+(\dxStart+\dy,0)$);
\node[ ref] (ostling2011a) at ($(zetterling2002C |- 0,-27.000000*\dy)$) {\reftext{Ostl11a}\cite{ostling2011a}  ( \num{950} ) ( \num{120} )};
\draw (ostling2011a.west) -| ++(-\dy,\fy*\dy);
\coordinate (ostling2011aC) at ($(ostling2011a.west)+(\dxStart+\dy,0)$);
\node[ ref] (ostling2011) at ($(ostling2011aC |- 0,-28.000000*\dy)$) {\reftext{Ostl11}\cite{ostling2011}  ( \num{950} ) ( \num{120} )};
\draw (ostling2011.west) -| ++(-\dy,\fy*\dy);
\coordinate (ostling2011C) at ($(ostling2011.west)+(\dxStart+\dy,0)$);
\node[ ref] (pellish2013) at ($(ostling2011C |- 0,-29.000000*\dy)$) {\reftext{Pell13}\cite{pellish2013}  ( \num{950} ) ( \num{120} )};
\draw (pellish2013.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-31.000000*\dy) {\citeauthor{ozpineci2004}};
\node[ ref] (ozpineci2004) at (\xSepOne,-32.000000*\dy) {\reftext{Ozpi04}\cite{ozpineci2004}  ( \num{1000} ) ( \num{115} )};
\coordinate (ozpineci2004C) at ($(ozpineci2004.west)+(\dxStart+\dy,0)$);
\node[ ref] (uhnevionak2015) at ($(ozpineci2004C |- 0,-33.000000*\dy)$) {\reftext{Uhne15}\cite{uhnevionak2015}  ( \num{1000} ) ( -- )};
\draw (uhnevionak2015.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-35.000000*\dy) {\citeauthor{bhatnagar2005}};
\node[ ref] (bhatnagar2005) at (\xSepOne,-36.000000*\dy) {\reftext{Bhat05}\cite{bhatnagar2005}  ( -- ) ( -- )};
\coordinate (bhatnagar2005C) at ($(bhatnagar2005.west)+(\dxStart+\dy,0)$);
\node[ ref] (codreanu2000) at ($(bhatnagar2005C |- 0,-37.000000*\dy)$) {\reftext{Codr00}\cite{codreanu2000}  ( \num{947} ) ( -- )};
\draw (codreanu2000.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-39.000000*\dy) {\citeauthor{neudeck2006}};
\node[ ref] (neudeck2006) at (\xSepOne,-40.000000*\dy) {\reftext{Neud06}\cite{neudeck2006} ( \num{800} , \num{800} ) ( \num{115} )};
\coordinate (neudeck2006C) at ($(neudeck2006.west)+(\dxStart+\dy,0)$);
\node[ ref] (wijesundara2011) at ($(neudeck2006C |- 0,-41.000000*\dy)$) {\reftext{Wije11}\cite{wijesundara2011} ( \num{800} , \num{800} ) ( \num{115} )};
\draw (wijesundara2011.west) -| ++(-\dy,\fy*\dy);
\coordinate (wijesundara2011C) at ($(wijesundara2011.west)+(\dxStart+\dy,0)$);
\node[ ref] (langpoklakpam2022) at ($(wijesundara2011C |- 0,-42.000000*\dy)$) {\reftext{Lang22}\cite{langpoklakpam2022}  ( \num{900} ) ( -- )};
\draw (langpoklakpam2022.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (arvinte2017) at ($(wijesundara2011.west |- 0,-43.000000*\dy)$) {\reftext{Arvi17}\cite{arvinte2017}  ( \num{800} ) ( \num{115} )};
\draw (arvinte2017.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (mukherjee2023) at ($(arvinte2017.west |- 0,-44.000000*\dy)$) {\reftext{Mukh23}\cite{mukherjee2023} ( \num{800} , \num{800} ) ( \num{115} )};
\draw (mukherjee2023.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-46.000000*\dy) {\citeauthor{sze2007}};
\node[ ref] (sze2007) at (\xSepOne,-47.000000*\dy) {\reftext{Sze07}\cite{sze2007}  ( \num{800} ) ( -- )};
\coordinate (sze2007C) at ($(sze2007.west)+(\dxStart+\dy,0)$);
\node[ ref] (neudeck1995) at ($(sze2007C |- 0,-48.000000*\dy)$) {\reftext{Neud95}\cite{neudeck1995}  ( \num{800} ) ( \num{115} )};
\draw (neudeck1995.west) -| ++(-\dy,\fy*\dy);
\coordinate (neudeck1995C) at ($(neudeck1995.west)+(\dxStart+\dy,0)$);
\node[ ref] (zhu2008) at ($(neudeck1995C |- 0,-49.000000*\dy)$) {\reftext{Zhu08}\cite{zhu2008} ( \num{800} , \num{900} ) ( \num{115} )};
\draw (zhu2008.west) -| ++(-\dy,\fy*\dy);
\coordinate (zhu2008C) at ($(zhu2008.west)+(\dxStart+\dy,0)$);
\node[ ref] (liu2015) at ($(zhu2008C |- 0,-50.000000*\dy)$) {\reftext{Liu15}\cite{liu2015}  ( \num{900} ) ( -- )};
\draw (liu2015.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (suproniuk2020) at ($(neudeck1995.west |- 0,-51.000000*\dy)$) {\reftext{Supr20}\cite{suproniuk2020}  ( \num{950} ) ( \num{150} )};
\draw (suproniuk2020.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-53.000000*\dy) {\citeauthor{kaminski2009}};
\node[ ref] (kaminski2009) at (\xSepOne,-54.000000*\dy) {\reftext{Kami09}\cite{kaminski2009}  ( \num{950} ) ( -- )};
\coordinate (kaminski2009C) at ($(kaminski2009.west)+(\dxStart+\dy,0)$);
\node[ ref] (kaminski2014) at ($(kaminski2009C |- 0,-55.000000*\dy)$) {\reftext{Kami14}\cite{kaminski2014}  ( \num{950} ) ( -- )};
\draw (kaminski2014.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,0.000000*\dy) {\citeauthor{buttay2011}};
\node[ ref] (buttay2011) at (\xSepOne + \xSepTwo,-1.000000*\dy) {\reftext{Butt11}\cite{buttay2011}  ( \num{950} ) ( \num{115} )};
\coordinate (buttay2011C) at ($(buttay2011.west)+(\dxStart+\dy,0)$);
\node[ ref] (fujita2015) at ($(buttay2011C |- 0,-2.000000*\dy)$) {\reftext{Fuji15}\cite{fujita2015}  ( \num{950} ) ( \num{115} )};
\draw (fujita2015.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-4.000000*\dy) {\citeauthor{hatakeyama2013}};
\node[ ref] (hatakeyama2013) at (\xSepOne + \xSepTwo,-5.000000*\dy) {\reftext{Hata13}\cite{hatakeyama2013}  ( -- ) ( -- )};
\coordinate (hatakeyama2013C) at ($(hatakeyama2013.west)+(\dxStart+\dy,0)$);
\node[ ref] (naugarhiya2017) at ($(hatakeyama2013C |- 0,-6.000000*\dy)$) {\reftext{Naug17}\cite{naugarhiya2017} ( \num{650} , \num{800} ) ( \num{115} )};
\draw (naugarhiya2017.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-8.000000*\dy) {\citeauthor{neudeck2013}};
\node[ ref] (neudeck2013) at (\xSepOne + \xSepTwo,-9.000000*\dy) {\reftext{Neud13}\cite{neudeck2013}  ( \num{800} ) ( \num{115} )};
\coordinate (neudeck2013C) at ($(neudeck2013.west)+(\dxStart+\dy,0)$);
\node[ ref] (mantooth2013) at ($(neudeck2013C |- 0,-10.000000*\dy)$) {\reftext{Mant13}\cite{mantooth2013}  ( \num{800} ) ( \num{115} )};
\draw (mantooth2013.west) -| ++(-\dy,\fy*\dy);
\coordinate (mantooth2013C) at ($(mantooth2013.west)+(\dxStart+\dy,0)$);
\node[ ref] (hassan2018) at ($(mantooth2013C |- 0,-11.000000*\dy)$) {\reftext{Hass18}\cite{hassan2018}  ( \num{800} ) ( \num{115} )};
\draw (hassan2018.west) -| ++(-\dy,\fy*\dy);
\coordinate (hassan2018C) at ($(hassan2018.west)+(\dxStart+\dy,0)$);
\node[ ref] (jiya2020) at ($(hassan2018C |- 0,-12.000000*\dy)$) {\reftext{Jiya20}\cite{jiya2020}  ( \num{800} ) ( \num{115} )};
\draw (jiya2020.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-14.000000*\dy) {\citeauthor{bellone2014}};
\node[ ref] (bellone2014) at (\xSepOne + \xSepTwo,-15.000000*\dy) {\reftext{Bell14}\cite{bellone2014}  ( -- ) ( -- )};
\coordinate (bellone2014C) at ($(bellone2014.west)+(\dxStart+\dy,0)$);
\node[ ref] (dibenedetto2014) at ($(bellone2014C |- 0,-16.000000*\dy)$) {\reftext{Dibe14}\cite{dibenedetto2014}  ( -- ) ( -- )};
\draw (dibenedetto2014.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-18.000000*\dy) {\citeauthor{higashiwaki2014}};
\node[ ref] (higashiwaki2014) at (\xSepOne + \xSepTwo,-19.000000*\dy) {\reftext{Higa14}\cite{higashiwaki2014}  ( \num{1000} ) ( -- )};
\coordinate (higashiwaki2014C) at ($(higashiwaki2014.west)+(\dxStart+\dy,0)$);
\node[ ref] (zheng2020) at ($(higashiwaki2014C |- 0,-20.000000*\dy)$) {\reftext{Zhen20}\cite{zheng2020}  ( \num{1000} ) ( -- )};
\draw (zheng2020.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-22.000000*\dy) {\citeauthor{kimoto2014a}};
\node[ ref] (kimoto2014a) at (\xSepOne + \xSepTwo,-23.000000*\dy) {\reftext{Kimo14a}\cite{kimoto2014a}  ( \num{450} ) ( -- )};
\coordinate (kimoto2014aC) at ($(kimoto2014a.west)+(\dxStart+\dy,0)$);
\node[ ref] (kaji2015) at ($(kimoto2014aC |- 0,-24.000000*\dy)$) {\reftext{Kaji15}\cite{kaji2015}  ( \num{700} ) ( \num{60} )};
\draw (kaji2015.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (elahipanah2017) at ($(kaji2015.west |- 0,-25.000000*\dy)$) {\reftext{Elah17}\cite{elahipanah2017}  ( \num{1020} ) ( \num{120} )};
\draw (elahipanah2017.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (rescher2018) at ($(elahipanah2017.west |- 0,-26.000000*\dy)$) {\reftext{Resc18}\cite{rescher2018} ( \num{1020} , \num{1200} ) ( \num{120} )};
\draw (rescher2018.west) -| ++(-\dy,\fy*\dy);
\coordinate (rescher2018C) at ($(rescher2018.west)+(\dxStart+\dy,0)$);
\node[ ref] (berens2021) at ($(rescher2018C |- 0,-27.000000*\dy)$) {\reftext{Bere21}\cite{berens2021} ( \num{1020} , \num{1200} ) ( \num{120} )};
\draw (berens2021.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (capan2022) at ($(rescher2018.west |- 0,-28.000000*\dy)$) {\reftext{Capa22}\cite{capan2022} ( \num{1020} , \num{1200} ) ( \num{120} )};
\draw (capan2022.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-30.000000*\dy) {\citeauthor{kimoto2015}};
\node[ ref] (kimoto2015) at (\xSepOne + \xSepTwo,-31.000000*\dy) {\reftext{Kimo15}\cite{kimoto2015} ( \num{1020} , \num{1200} ) ( \num{120} )};
\coordinate (kimoto2015C) at ($(kimoto2015.west)+(\dxStart+\dy,0)$);
\node[ ref] (ostling2024) at ($(kimoto2015C |- 0,-32.000000*\dy)$) {\reftext{Ostl24}\cite{ostling2024} ( \num{1020} , \num{1200} ) ( \num{120} )};
\draw (ostling2024.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-34.000000*\dy) {\citeauthor{choi2016}};
\node[ ref] (choi2016) at (\xSepOne + \xSepTwo,-35.000000*\dy) {\reftext{Choi16}\cite{choi2016}  ( \num{800} ) ( \num{115} )};
\coordinate (choi2016C) at ($(choi2016.west)+(\dxStart+\dy,0)$);
\node[ ref] (naugarhiya2017) at ($(choi2016C |- 0,-36.000000*\dy)$) {\reftext{Naug17}\cite{naugarhiya2017} ( \num{650} , \num{800} ) ( \num{115} )};
\draw (naugarhiya2017.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-38.000000*\dy) {\citeauthor{arvanitopoulos2017}};
\node[ ref] (arvanitopoulos2017) at (\xSepOne + \xSepTwo,-39.000000*\dy) {\reftext{Arva17}\cite{arvanitopoulos2017}  ( -- ) ( -- )};
\coordinate (arvanitopoulos2017C) at ($(arvanitopoulos2017.west)+(\dxStart+\dy,0)$);
\node[ ref] (choudhary2021) at ($(arvanitopoulos2017C |- 0,-40.000000*\dy)$) {\reftext{Chou21}\cite{choudhary2021}  ( \num{950} ) ( \num{125} )};
\draw (choudhary2021.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-42.000000*\dy) {\citeauthor{baliga2019}};
\node[ ref] (baliga2019) at (\xSepOne + \xSepTwo,-43.000000*\dy) {\reftext{Bali19}\cite{baliga2019}  ( -- ) ( -- )};
\coordinate (baliga2019C) at ($(baliga2019.west)+(\dxStart+\dy,0)$);
\node[ ref] (tsao2018) at ($(baliga2019C |- 0,-44.000000*\dy)$) {\reftext{Tsao18}\cite{tsao2018}  ( \num{980} ) ( -- )};
\draw (tsao2018.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-46.000000*\dy) {\citeauthor{ioffe2023}};
\node[ ref] (ioffe2023) at (\xSepOne + \xSepTwo,-47.000000*\dy) {\reftext{Ioff23}\cite{ioffe2023}  ( \num{<900} ) ( \num{<120} )};
\coordinate (ioffe2023C) at ($(ioffe2023.west)+(\dxStart+\dy,0)$);
\node[ ref] (banerjee2021) at ($(ioffe2023C |- 0,-48.000000*\dy)$) {\reftext{Bane21}\cite{banerjee2021}  ( \num{1000} ) ( \num{100} )};
\draw (banerjee2021.west) -| ++(-\dy,\fy*\dy);


==> data/mobility_ref_chain_low_elec.tex <==
\node[desc] at (0,0.000000*\dy) {Electron (dir) ($\mumin$, $\mumax$, $\mu_0$, $\nref$, $\delta$) ($\gmin$, $\gmax$, $\gamma_0$, $\gref$, $\gdelta$, $\gNNref$)};
\node[author] at (0,-1.500000*\dy) {\citeauthor{ruff1993}};
\node[no4H, ref] (ruff1993) at (0,-2.500000*\dy) {\reftext{Ruff93}\cite{ruff1993} ( -- ) ( -- , -- , -- , -- , -- ) ( -- , -- , -- , -- , -- , -- )};
\coordinate (ruff1993C) at ($(ruff1993.west)+(\dxStart+\dy,0)$);
\node[ ref] (biondo2012) at ($(ruff1993C |- 0,-3.500000*\dy)$) {\reftext{Bion12}\cite{biondo2012} ( -- ) ( -- , -- , \num{870} , \num{2.00E+17} , \num{0.55} ) ( -- , -- , \num{-2} , -- , -- , -- )};
\draw (biondo2012.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-5.500000*\dy) {\citeauthor{ruff1994}};
\node[no4H, ref] (ruff1994) at (0,-6.500000*\dy) {\reftext{Ruff94}\cite{ruff1994} ( -- ) ( \num{20} , -- , \num{380} , \num{4.50E+17} , \num{0.45} ) ( -- , -- , \num{-3} , -- , -- , -- )};
\coordinate (ruff1994C) at ($(ruff1994.west)+(\dxStart+\dy,0)$);
\node[ ref] (nallet1999) at ($(ruff1994C |- 0,-7.500000*\dy)$) {\reftext{Nall99}\cite{nallet1999} ( -- ) ( \num{20} , -- , \num{700} , \num{4.50E+17} , \num{0.45} ) ( -- , -- , \num{-3} , -- , -- , -- )};
\draw (nallet1999.west) -| ++(-\dy,\fy*\dy);
\coordinate (nallet1999C) at ($(nallet1999.west)+(\dxStart+\dy,0)$);
\node[ ref] (nallet2000) at ($(nallet1999C |- 0,-8.500000*\dy)$) {\reftext{Nall00}\cite{nallet2000} ( -- ) ( \num{20} , -- , \num{700} , \num{4.50E+17} , \num{0.45} ) ( -- , -- , \num{-3} , -- , -- , -- )};
\draw (nallet2000.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-10.500000*\dy) {\citeauthor{schaffer1994}};
\node[fund, ref] (schaffer1994) at (0,-11.500000*\dy) {\reftext{Scha94}\cite{schaffer1994} ( $\perp$ ) ( \num{0} , \num{947} , -- , \num{1.94E+17} , \num{0.61} ) ( -- , \num{-2.15} , -- , -- , -- , -- )};
\coordinate (schaffer1994C) at ($(schaffer1994.west)+(\dxStart+\dy,0)$);
\node[ ref] (bakowski1997) at ($(schaffer1994C |- 0,-12.500000*\dy)$) {\reftext{Bako97}\cite{bakowski1997} ( -- ) ( \num{0} , -- , \num{947} , \num{1.94E+17} , \num{0.61} ) ( -- , -- , \num{-2.15} , -- , -- , -- )};
\draw (bakowski1997.west) -| ++(-\dy,\fy*\dy);
\coordinate (bakowski1997C) at ($(bakowski1997.west)+(\dxStart+\dy,0)$);
\node[ ref] (codreanu2000) at ($(bakowski1997C |- 0,-13.500000*\dy)$) {\reftext{Codr00}\cite{codreanu2000} ( -- ) ( \num{0} , -- , \num{947} , \num{1.94E+17} , \num{0.61} ) ( -- , -- , \num{-2.15} , -- , -- , -- )};
\draw (codreanu2000.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (mcnutt2004) at ($(codreanu2000.west |- 0,-14.500000*\dy)$) {\reftext{Mcnu04}\cite{mcnutt2004} ( -- ) ( -- , -- , \num{947} , \num{1.94E+17} , \num{0.61} ) ( -- , -- , \num{-2.15} , -- , -- , -- )};
\draw (mcnutt2004.west) -| ++(-\dy,\fy*\dy);
\coordinate (mcnutt2004C) at ($(mcnutt2004.west)+(\dxStart+\dy,0)$);
\node[ ref] (mcnutt2013) at ($(mcnutt2004C |- 0,-15.500000*\dy)$) {\reftext{Mcnu13}\cite{mcnutt2013} ( -- ) ( -- , -- , \num{947} , \num{1.94E+17} , \num{0.61} ) ( -- , -- , \num{-2.15} , -- , -- , -- )};
\draw (mcnutt2013.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (dibenedetto2014) at ($(mcnutt2004.west |- 0,-16.500000*\dy)$) {\reftext{Dibe14}\cite{dibenedetto2014} ( -- ) ( -- , -- , -- , -- , -- ) ( -- , -- , \num{-2.15} , -- , -- , -- )};
\draw (dibenedetto2014.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (wang1998) at ($(bakowski1997.west |- 0,-17.500000*\dy)$) {\reftext{Wang98}\cite{wang1998} ( -- ) ( -- , \num{947} , -- , \num{1.94E+17} , \num{0.61} ) ( -- , \num{-2} , -- , -- , -- , -- )};
\draw (wang1998.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (wang1999) at ($(wang1998.west |- 0,-18.500000*\dy)$) {\reftext{Wang99}\cite{wang1999} ( -- ) ( -- , \num{947} , -- , \num{1.94E+17} , \num{0.61} ) ( -- , \num{-2} , -- , -- , -- , -- )};
\draw (wang1999.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (ladesmartin2000) at ($(wang1999.west |- 0,-19.500000*\dy)$) {\reftext{Lade00}\cite{ladesmartin2000} ( -- ) ( \num{0} , \num{947} , -- , \num{1.94E+17} , \num{0.61} ) ( -- , -- , -- , -- , -- , -- )};
\draw (ladesmartin2000.west) -| ++(-\dy,\fy*\dy);
\coordinate (ladesmartin2000C) at ($(ladesmartin2000.west)+(\dxStart+\dy,0)$);
\node[ ref] (cheng2020) at ($(ladesmartin2000C |- 0,-20.500000*\dy)$) {\reftext{Chen20}\cite{cheng2020} ( $\parallel$ ) ( \num{0} , \num{947} , -- , \num{1.94E+17} , \num{0.61} ) ( -- , -- , -- , -- , -- , -- )};
\draw (cheng2020.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (lee2002) at ($(ladesmartin2000.west |- 0,-21.500000*\dy)$) {\reftext{Lee02}\cite{lee2002} ( $\parallel/\perp$ ) ( \num{0} , -- , \num{1136}/\num{947} , \num{1.94E+17} , \num{0.61} ) ( \num{-2.4}/\num{-2.15} , \num{-2.4}/\num{-2.15} , -- , -- , -- , -- )};
\draw (lee2002.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (li2003) at ($(lee2002.west |- 0,-22.500000*\dy)$) {\reftext{Li03}\cite{li2003} ( -- ) ( -- , -- , \num{947} , \num{1.94E+17} , \num{0.61} ) ( -- , -- , \num{-2} , -- , -- , -- )};
\draw (li2003.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (zhao2003) at ($(li2003.west |- 0,-23.500000*\dy)$) {\reftext{Zhao03}\cite{zhao2003} ( -- ) ( -- , -- , \num{947} , \num{1.94E+17} , \num{0.61} ) ( -- , -- , \num{-2} , -- , -- , -- )};
\draw (zhao2003.west) -| ++(-\dy,\fy*\dy);
\coordinate (zhao2003C) at ($(zhao2003.west)+(\dxStart+\dy,0)$);
\node[ ref] (das2015) at ($(zhao2003C |- 0,-24.500000*\dy)$) {\reftext{Das15}\cite{das2015} ( -- ) ( \num{0} , -- , \num{947} , \num{1.94E+17} , \num{0.61} ) ( -- , -- , \num{-2} , -- , -- , -- )};
\draw (das2015.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (ayalew2004) at ($(zhao2003.west |- 0,-25.500000*\dy)$) {\reftext{Ayal04}\cite{ayalew2004} ( $\perp$ ) ( \num{40} , \num{950} , -- , \num{1.94E+17} , \num{0.61} ) ( \num{-0.5} , \num{-2.4} , -- , -- , -- , -- )};
\draw (ayalew2004.west) -| ++(-\dy,\fy*\dy);
\coordinate (ayalew2004C) at ($(ayalew2004.west)+(\dxStart+\dy,0)$);
\node[ ref] (maximenko2023) at ($(ayalew2004C |- 0,-26.500000*\dy)$) {\reftext{Maxi23}\cite{maximenko2023} ( -- ) ( \num{40} , \num{950} , -- , \num{1.94E+17} , \num{0.61} ) ( \num{-0.5} , \num{-2.4} , -- , -- , -- , -- )};
\draw (maximenko2023.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (brosselard2004) at ($(ayalew2004.west |- 0,-27.500000*\dy)$) {\reftext{Bros04}\cite{brosselard2004} ( -- ) ( \num{0} , \num{947} , -- , \num{1.94E+17} , \num{0.61} ) ( \num{0} , \num{-2.15} , -- , -- , -- , \num{0} )};
\draw (brosselard2004.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (schroeder2006) at ($(brosselard2004.west |- 0,-28.500000*\dy)$) {\reftext{Schr06}\cite{schroeder2006} ( -- ) ( \num{0} , \num{947} , -- , \num{1.94E+17} , \num{0.61} ) ( -- , -- , -- , -- , -- , -- )};
\draw (schroeder2006.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (zhang2009) at ($(schroeder2006.west |- 0,-29.500000*\dy)$) {\reftext{Zhan09}\cite{zhang2009} ( -- ) ( -- , -- , \num{947} , \num{1.94E+17} , \num{0.61} ) ( -- , -- , \num{-2} , -- , -- , -- )};
\draw (zhang2009.west) -| ++(-\dy,\fy*\dy);
\coordinate (zhang2009C) at ($(zhang2009.west)+(\dxStart+\dy,0)$);
\node[ ref] (khalid2012) at ($(zhang2009C |- 0,-30.500000*\dy)$) {\reftext{Khal12}\cite{khalid2012} ( -- ) ( -- , \num{947} , -- , \num{1.94E+17} , \num{0.61} ) ( -- , \num{-2} , -- , -- , -- , -- )};
\draw (khalid2012.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (zhang2010) at ($(zhang2009.west |- 0,-31.500000*\dy)$) {\reftext{Zhan10}\cite{zhang2010} ( -- ) ( -- , -- , \num{947} , \num{1.94E+17} , \num{0.61} ) ( -- , -- , \num{-2} , -- , -- , -- )};
\draw (zhang2010.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (lutz2011) at ($(zhang2010.west |- 0,-32.500000*\dy)$) {\reftext{Lutz11}\cite{lutz2011} ( -- ) ( \num{0} , \num{947} , -- , \num{1.94E+17} , \num{0.61} ) ( -- , \num{-2.15} , -- , -- , -- , -- )};
\draw (lutz2011.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (buono2012) at ($(lutz2011.west |- 0,-33.500000*\dy)$) {\reftext{Buon12}\cite{buono2012} ( -- ) ( -- , -- , \num{950} , \num{1.94E+17} , \num{0.61} ) ( -- , -- , \num{-2.15} , -- , -- , -- )};
\draw (buono2012.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (chen2015) at ($(buono2012.west |- 0,-34.500000*\dy)$) {\reftext{Chen15}\cite{chen2015} ( $\parallel/\perp$ ) ( \num{0} , -- , \num{1136}/\num{947} , \num{1.94E+17} , \num{0.61} ) ( \num{-2.4}/\num{-2.15} , -- , \num{-2.4}/\num{-2.15} , -- , -- , -- )};
\draw (chen2015.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (johannesson2016) at ($(chen2015.west |- 0,-35.500000*\dy)$) {\reftext{Joha16}\cite{johannesson2016} ( -- ) ( \num{0} , \num{947} , -- , \num{1.94E+17} , \num{0.61} ) ( -- , \num{-2.15} , -- , -- , -- , -- )};
\draw (johannesson2016.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (lutz2018) at ($(johannesson2016.west |- 0,-36.500000*\dy)$) {\reftext{Lutz18}\cite{lutz2018} ( -- ) ( \num{0} , \num{947} , -- , \num{1.94E+17} , \num{0.61} ) ( -- , \num{-2.15} , -- , -- , -- , -- )};
\draw (lutz2018.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (arvanitopoulos2019) at ($(lutz2018.west |- 0,-37.500000*\dy)$) {\reftext{Arva19}\cite{arvanitopoulos2019} ( $\perp$ ) ( \num{40} , \num{950} , -- , \num{1.94E+17} , \num{0.61} ) ( -- , -- , -- , -- , -- , -- )};
\draw (arvanitopoulos2019.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (johannesson2019) at ($(arvanitopoulos2019.west |- 0,-38.500000*\dy)$) {\reftext{Joha19}\cite{johannesson2019} ( -- ) ( -- , \num{940} , -- , -- , -- ) ( -- , -- , -- , -- , -- , -- )};
\draw (johannesson2019.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (yang2022) at ($(johannesson2019.west |- 0,-39.500000*\dy)$) {\reftext{Yang22}\cite{yang2022} ( -- ) ( -- , -- , -- , -- , -- ) ( -- , -- , -- , -- , -- , -- )};
\draw (yang2022.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-41.500000*\dy) {\citeauthor{mickevicius1998}};
\node[fund, ref] (mickevicius1998) at (0,-42.500000*\dy) {\reftext{Mick98}\cite{mickevicius1998} ( -- ) ( -- , \num{1071} , -- , \num{1.94E+17} , \num{0.4} ) ( -- , -- , -- , -- , -- , -- )};
\coordinate (mickevicius1998C) at ($(mickevicius1998.west)+(\dxStart+\dy,0)$);
\node[ ref] (tilak2007) at ($(mickevicius1998C |- 0,-43.500000*\dy)$) {\reftext{Tila07}\cite{tilak2007} ( -- ) ( -- , \num{1071} , -- , \num{1.94E+17} , \num{0.4} ) ( -- , \num{2.4} , -- , -- , -- , -- )};
\draw (tilak2007.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-45.500000*\dy) {\citeauthor{wright1998}};
\node[fund, ref] (wright1998) at (0,-46.500000*\dy) {\reftext{Wrig98}\cite{wright1998} ( -- ) ( \num{88} , -- , \num{970} , \num{1.43E+17} , \num{1} ) ( \num{-0.57} , -- , \num{-2.7} , \num{2.55} , -- , -- )};
\coordinate (wright1998C) at ($(wright1998.west)+(\dxStart+\dy,0)$);
\node[ ref] (baliga2006) at ($(wright1998C |- 0,-47.500000*\dy)$) {\reftext{Bali06}\cite{baliga2006} ( -- ) ( -- , \num{1140} , -- , -- , -- ) ( -- , \num{-2.7} , -- , -- , -- , -- )};
\draw (baliga2006.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (baliga2019) at ($(baliga2006.west |- 0,-48.500000*\dy)$) {\reftext{Bali19}\cite{baliga2019} ( -- ) ( -- , \num{1140} , -- , -- , -- ) ( -- , \num{-2.7} , -- , -- , -- , -- )};
\draw (baliga2019.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-50.500000*\dy) {\citeauthor{mnatsakanov2001}};
\node[fund, ref] (mnatsakanov2001) at (0,-51.500000*\dy) {\reftext{Mnat01}\cite{mnatsakanov2001} ( -- ) ( \num{30} , \num{880} , -- , \num{2.00E+17} , \num{0.67} ) ( -- , -- , -- , -- , -- , -- )};
\coordinate (mnatsakanov2001C) at ($(mnatsakanov2001.west)+(\dxStart+\dy,0)$);
\node[ ref] (mnatsakanov2002) at ($(mnatsakanov2001C |- 0,-52.500000*\dy)$) {\reftext{Mnat02}\cite{mnatsakanov2002} ( -- ) ( \num{30} , \num{880} , -- , \num{2.00E+17} , \num{0.67} ) ( -- , -- , -- , -- , -- , -- )};
\draw (mnatsakanov2002.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,0.000000*\dy) {\citeauthor{roschke2001}};
\node[fund, ref] (roschke2001) at (\xSepOne,-1.000000*\dy) {\reftext{Rosc01}\cite{roschke2001} ( $\perp$ ) ( \num{40} , \num{950} , -- , \num{2.00E+17} , \num{0.76} ) ( \num{-0.5} , \num{-2.4} , -- , \num{1} , -- , -- )};
\coordinate (roschke2001C) at ($(roschke2001.west)+(\dxStart+\dy,0)$);
\node[ ref] (linewih2003) at ($(roschke2001C |- 0,-2.000000*\dy)$) {\reftext{Line03}\cite{linewih2003} ( -- ) ( \num{40} , \num{950} , -- , \num{2.00E+17} , \num{0.76} ) ( -- , -- , -- , -- , -- , -- )};
\draw (linewih2003.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (bertilsson2004) at ($(linewih2003.west |- 0,-3.000000*\dy)$) {\reftext{Bert04}\cite{bertilsson2004} ( $\perp$ ) ( \num{40} , \num{950} , -- , \num{2.00E+17} , \num{0.76} ) ( -- , \num{-2.4} , -- , -- , -- , \num{-0.76} )};
\draw (bertilsson2004.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (bertilsson2004a) at ($(bertilsson2004.west |- 0,-4.000000*\dy)$) {\reftext{Bert04a}\cite{bertilsson2004a} ( $\perp$ ) ( \num{40} , \num{950} , -- , \num{2.00E+17} , \num{0.76} ) ( -- , \num{-2.4} , -- , -- , -- , \num{-0.76} )};
\draw (bertilsson2004a.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (lv2004) at ($(bertilsson2004a.west |- 0,-5.000000*\dy)$) {\reftext{Lv04}\cite{lv2004} ( -- ) ( \num{40} , \num{950} , -- , \num{2.00E+17} , \num{0.76} ) ( -- , \num{-2.4} , -- , -- , -- , \num{1.05} )};
\draw (lv2004.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (perez-tomas2006) at ($(lv2004.west |- 0,-6.000000*\dy)$) {\reftext{Pere06}\cite{perez-tomas2006} ( -- ) ( \num{40} , \num{950} , -- , \num{2.00E+17} , \num{0.76} ) ( -- , \num{-2} , -- , -- , -- , -- )};
\draw (perez-tomas2006.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (tamaki2008a) at ($(perez-tomas2006.west |- 0,-7.000000*\dy)$) {\reftext{Tama08a}\cite{tamaki2008a} ( -- ) ( -- , \num{950} , -- , \num{2.00E+17} , \num{0.76} ) ( -- , \num{-2.8} , -- , -- , -- , -- )};
\draw (tamaki2008a.west) -| ++(-\dy,\fy*\dy);
\coordinate (tamaki2008aC) at ($(tamaki2008a.west)+(\dxStart+\dy,0)$);
\node[guess, ref] (song2012) at ($(tamaki2008aC |- 0,-8.000000*\dy)$) {\reftext{Song12}\cite{song2012} ( -- ) ( \num{0} , \num{950} , -- , \num{2.00E+17} , \num{0.76} ) ( -- , \num{-2.8} , -- , -- , -- , -- )};
\draw (song2012.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (liu2021) at ($(song2012.west |- 0,-9.000000*\dy)$) {\reftext{Liu21}\cite{liu2021} ( -- ) ( -- , \num{950} , -- , \num{2.00E+17} , \num{0.76} ) ( -- , \num{-2.9} , -- , -- , -- , -- )};
\draw (liu2021.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (albanese2010) at ($(tamaki2008a.west |- 0,-10.000000*\dy)$) {\reftext{Alba10}\cite{albanese2010} ( -- ) ( \num{40} , \num{950} , -- , \num{2.00E+17} , \num{0.76} ) ( \num{-0.5} , \num{-2.4} , -- , -- , -- , \num{-0.76} )};
\draw (albanese2010.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (bellone2011) at ($(albanese2010.west |- 0,-11.000000*\dy)$) {\reftext{Bell11}\cite{bellone2011} ( -- ) ( \num{40} , \num{950} , -- , \num{2.00E+17} , \num{0.76} ) ( \num{-0.5} , \num{-2.4} , -- , -- , -- , \num{-0.76} )};
\draw (bellone2011.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (neilainglesias2012) at ($(bellone2011.west |- 0,-12.000000*\dy)$) {\reftext{Neil12}\cite{neilainglesias2012} ( -- ) ( \num{40} , \num{950} , -- , \num{2.00E+17} , \num{0.76} ) ( \num{-0.5} , \num{-2.4} , -- , \num{1} , \num{0} , -- )};
\draw (neilainglesias2012.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (pezzimenti2013) at ($(neilainglesias2012.west |- 0,-13.000000*\dy)$) {\reftext{Pezz13}\cite{pezzimenti2013} ( -- ) ( \num{40} , \num{950} , -- , \num{2.00E+17} , \num{0.76} ) ( \num{-0.5} , \num{-2.4} , -- , -- , -- , \num{-0.76} )};
\draw (pezzimenti2013.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (megherbi2015) at ($(pezzimenti2013.west |- 0,-14.000000*\dy)$) {\reftext{Megh15}\cite{megherbi2015} ( -- ) ( \num{40} , \num{950} , -- , \num{2.00E+17} , \num{0.76} ) ( \num{-0.5} , \num{-2.4} , -- , -- , -- , \num{-0.76} )};
\draw (megherbi2015.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (zhou2016) at ($(megherbi2015.west |- 0,-15.000000*\dy)$) {\reftext{Zhou16}\cite{zhou2016} ( -- ) ( \num{40} , \num{950} , -- , \num{2.00E+17} , \num{1} ) ( -- , -- , -- , -- , -- , -- )};
\draw (zhou2016.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (megherbi2018) at ($(zhou2016.west |- 0,-16.000000*\dy)$) {\reftext{Megh18}\cite{megherbi2018} ( -- ) ( \num{40} , \num{950} , -- , -- , -- ) ( -- , -- , -- , -- , -- , -- )};
\draw (megherbi2018.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (megherbi2018a) at ($(megherbi2018.west |- 0,-17.000000*\dy)$) {\reftext{Megh18a}\cite{megherbi2018a} ( -- ) ( \num{40} , \num{950} , -- , \num{2.00E+17} , -- ) ( -- , -- , -- , -- , -- , -- )};
\draw (megherbi2018a.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (zeghdar2019) at ($(megherbi2018a.west |- 0,-18.000000*\dy)$) {\reftext{Zegh19}\cite{zeghdar2019} ( -- ) ( \num{40} , \num{950} , -- , \num{2.00E+17} , \num{0.76} ) ( \num{-0.5} , \num{-2.4} , -- , -- , -- , \num{-0.76} )};
\draw (zeghdar2019.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (zeghdar2020) at ($(zeghdar2019.west |- 0,-19.000000*\dy)$) {\reftext{Zegh20}\cite{zeghdar2020} ( -- ) ( \num{40} , \num{950} , -- , \num{2.00E+17} , \num{0.76} ) ( \num{0.5} , \num{2.4} , -- , -- , -- , \num{0.76} )};
\draw (zeghdar2020.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-21.000000*\dy) {\citeauthor{hatakeyama2003}};
\node[fund, ref] (hatakeyama2003) at (\xSepOne,-22.000000*\dy) {\reftext{Hata03}\cite{hatakeyama2003} ( -- ) ( \num{0} , \num{954} , -- , \num{1.28E+17} , \num{0.61} ) ( -- , -- , -- , -- , -- , -- )};
\coordinate (hatakeyama2003C) at ($(hatakeyama2003.west)+(\dxStart+\dy,0)$);
\node[ ref] (nipoti2016a) at ($(hatakeyama2003C |- 0,-23.000000*\dy)$) {\reftext{Nipo16a}\cite{nipoti2016a} ( -- ) ( -- , -- , -- , -- , -- ) ( -- , -- , -- , -- , -- , -- )};
\draw (nipoti2016a.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-25.000000*\dy) {\citeauthor{balachandran2005}};
\node[fund, ref] (balachandran2005) at (\xSepOne,-26.000000*\dy) {\reftext{Bala05}\cite{balachandran2005} ( -- ) ( \num{40} , \num{950} , -- , \num{2.00E+17} , \num{0.73} ) ( -- , \num{-2.4} , -- , -- , -- , \num{-0.76} )};
\coordinate (balachandran2005C) at ($(balachandran2005.west)+(\dxStart+\dy,0)$);
\node[guess, ref] (nawaz2010) at ($(balachandran2005C |- 0,-27.000000*\dy)$) {\reftext{Nawa10}\cite{nawaz2010} ( -- ) ( \num{40} , \num{950} , -- , \num{2.00E+17} , \num{0.73} ) ( \num{0} , \num{-2.4} , -- , -- , -- , \num{-0.76} )};
\draw (nawaz2010.west) -| ++(-\dy,\fy*\dy);
\coordinate (nawaz2010C) at ($(nawaz2010.west)+(\dxStart+\dy,0)$);
\node[ ref] (usman2014) at ($(nawaz2010C |- 0,-28.000000*\dy)$) {\reftext{Usma14}\cite{usman2014} ( -- ) ( \num{40} , \num{950} , -- , \num{2.00E+17} , \num{0.73} ) ( \num{0} , \num{-2.4} , -- , -- , -- , \num{-0.76} )};
\draw (usman2014.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-30.000000*\dy) {\citeauthor{habib2011}};
\node[fund, ref] (habib2011) at (\xSepOne,-31.000000*\dy) {\reftext{Habi11}\cite{habib2011} ( -- ) ( \num{40} , -- , \num{910} , \num{2.00E+17} , \num{0.76} ) ( \num{-1.538} , -- , \num{-2.397} , \num{0.75} , \num{0.722} , -- )};
\coordinate (habib2011C) at ($(habib2011.west)+(\dxStart+\dy,0)$);
\node[guess, ref] (lophitis2018) at ($(habib2011C |- 0,-32.000000*\dy)$) {\reftext{Loph18}\cite{lophitis2018} ( $\perp/\parallel$ ) ( \num{40} , \num{910}/\num{1100} , -- , \num{2.00E+17} , \num{0.76} ) ( \num{-1.536} , \num{-2.4} , -- , \num{0.75} , \num{0.722} , -- )};
\draw (lophitis2018.west) -| ++(-\dy,\fy*\dy);
\coordinate (lophitis2018C) at ($(lophitis2018.west)+(\dxStart+\dy,0)$);
\node[ ref] (rakheja2020) at ($(lophitis2018C |- 0,-33.000000*\dy)$) {\reftext{Rakh20}\cite{rakheja2020} ( -- ) ( -- , \num{699.4} , -- , -- , -- ) ( -- , -- , -- , -- , -- , -- )};
\draw (rakheja2020.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-35.000000*\dy) {\citeauthor{hatakeyama2013}};
\node[fund, ref] (hatakeyama2013) at (\xSepOne,-36.000000*\dy) {\reftext{Hata13}\cite{hatakeyama2013} ( -- ) ( \num{5} , \num{1010} , -- , \num{1.25E+17} , \num{0.65} ) ( \num{-0.57} , \num{-2.6} , -- , \num{2.4} , \num{-0.146} , -- )};
\coordinate (hatakeyama2013C) at ($(hatakeyama2013.west)+(\dxStart+\dy,0)$);
\node[ ref] (naugarhiya2017) at ($(hatakeyama2013C |- 0,-37.000000*\dy)$) {\reftext{Naug17}\cite{naugarhiya2017} ( $\perp$ ) ( \num{5} , \num{1010} , -- , \num{1.25E+17} , \num{0.65} ) ( \num{-0.57} , \num{-2.6} , -- , \num{2.4} , \num{-0.146} , -- )};
\draw (naugarhiya2017.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (jin2024) at ($(naugarhiya2017.west |- 0,-38.000000*\dy)$) {\reftext{Jin24}\cite{jin2024} ( -- ) ( \num{5} , \num{1010} , -- , \num{1.25E+17} , \num{0.65} ) ( -- , -- , -- , -- , -- , -- )};
\draw (jin2024.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-40.000000*\dy) {\citeauthor{kimoto2014a}};
\node[ ref] (kimoto2014a) at (\xSepOne,-41.000000*\dy) {\reftext{Kimo14a}\cite{kimoto2014a} ( $\perp$ ) ( -- , \num{1020} , -- , \num{1.80E+17} , \num{0.6} ) ( -- , \numrange{-1.8}{-2.8} , -- , -- , -- , -- )};
\coordinate (kimoto2014aC) at ($(kimoto2014a.west)+(\dxStart+\dy,0)$);
\node[ ref] (fujihara2017) at ($(kimoto2014aC |- 0,-42.000000*\dy)$) {\reftext{Fuji17}\cite{fujihara2017} ( -- ) ( -- , -- , -- , -- , -- ) ( -- , -- , -- , -- , -- , -- )};
\draw (fujihara2017.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (kimoto2019) at ($(fujihara2017.west |- 0,-43.000000*\dy)$) {\reftext{Kimo19}\cite{kimoto2019} ( $\perp$ ) ( -- , \num{1020} , -- , \num{1.80E+17} , \num{0.6} ) ( -- , \numrange{-1.8}{-2.8} , -- , -- , -- , -- )};
\draw (kimoto2019.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-45.000000*\dy) {\citeauthor{stefanakis2014}};
\node[fund, ref] (stefanakis2014) at (\xSepOne,-46.000000*\dy) {\reftext{Stef14}\cite{stefanakis2014} ( $\perp$ ) ( \num{28} , \num{950} , -- , \num{1.94E+17} , \num{0.61} ) ( \num{0} , \num{-2.4} , -- , -- , -- , \num{0.73} )};
\coordinate (stefanakis2014C) at ($(stefanakis2014.west)+(\dxStart+\dy,0)$);
\node[ ref] (tripathi2019) at ($(stefanakis2014C |- 0,-47.000000*\dy)$) {\reftext{Trip19}\cite{tripathi2019} ( -- ) ( \num{28} , \num{950} , -- , \num{1.94E+17} , \num{0.61} ) ( \num{0} , \num{-2.4} , -- , -- , -- , \num{0.73} )};
\draw (tripathi2019.west) -| ++(-\dy,\fy*\dy);


==> data/mobility_ref_chain_low_hole.tex <==
\node[desc] at (0,0.000000*\dy) {Hole (dir) ($\mumin$, $\mumax$, $\mu_0$, $\nref$, $\delta$) ($\gmin$, $\gmax$, $\gamma_0$, $\gref$, $\gdelta$, $\gNNref$)};
\node[author] at (0,-1.500000*\dy) {\citeauthor{ruff1993}};
\node[no4H, ref] (ruff1993) at (0,-2.500000*\dy) {\reftext{Ruff93}\cite{ruff1993} ( -- ) ( -- , -- , -- , -- , -- ) ( -- , -- , -- , -- , -- , -- )};
\coordinate (ruff1993C) at ($(ruff1993.west)+(\dxStart+\dy,0)$);
\node[ ref] (biondo2012) at ($(ruff1993C |- 0,-3.500000*\dy)$) {\reftext{Bion12}\cite{biondo2012} ( -- ) ( -- , -- , \num{120} , \num{2.00E+17} , \num{0.3} ) ( -- , -- , \num{-2} , -- , -- , -- )};
\draw (biondo2012.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-5.500000*\dy) {\citeauthor{ruff1994}};
\node[no4H, ref] (ruff1994) at (0,-6.500000*\dy) {\reftext{Ruff94}\cite{ruff1994} ( -- ) ( \num{5} , -- , \num{70} , \num{1.00E+19} , \num{0.5} ) ( -- , -- , \num{-3} , -- , -- , -- )};
\coordinate (ruff1994C) at ($(ruff1994.west)+(\dxStart+\dy,0)$);
\node[ ref] (nallet1999) at ($(ruff1994C |- 0,-7.500000*\dy)$) {\reftext{Nall99}\cite{nallet1999} ( -- ) ( \num{20} , \num{350} , -- , \num{1.00E+19} , \num{0.5} ) ( -- , -- , \num{-3} , -- , -- , -- )};
\draw (nallet1999.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-9.500000*\dy) {\citeauthor{schaffer1994}};
\node[fund, ref] (schaffer1994) at (0,-10.500000*\dy) {\reftext{Scha94}\cite{schaffer1994} ( $\perp$ ) ( \num{15.9} , \num{124} , -- , \num{1.76E+19} , \num{0.34} ) ( -- , -- , -- , -- , -- , -- )};
\coordinate (schaffer1994C) at ($(schaffer1994.west)+(\dxStart+\dy,0)$);
\node[ ref] (bakowski1997) at ($(schaffer1994C |- 0,-11.500000*\dy)$) {\reftext{Bako97}\cite{bakowski1997} ( -- ) ( \num{15.9} , -- , \num{108.1} , \num{1.76E+19} , \num{0.34} ) ( -- , -- , \num{-2.15} , -- , -- , -- )};
\draw (bakowski1997.west) -| ++(-\dy,\fy*\dy);
\coordinate (bakowski1997C) at ($(bakowski1997.west)+(\dxStart+\dy,0)$);
\node[ ref] (mcnutt2004) at ($(bakowski1997C |- 0,-12.500000*\dy)$) {\reftext{Mcnu04}\cite{mcnutt2004} ( -- ) ( \num{15.9} , -- , \num{108.9} , \num{1.76E+19} , \num{0.34} ) ( -- , -- , \num{-2.15} , -- , -- , -- )};
\draw (mcnutt2004.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (chen2015) at ($(mcnutt2004.west |- 0,-13.500000*\dy)$) {\reftext{Chen15}\cite{chen2015} ( $\parallel/\perp$ ) ( \num{15.9} , -- , \num{124} , \num{1.76E+19} , \num{0.34} ) ( \num{-2.15} , -- , \num{-2.15} , -- , -- , -- )};
\draw (chen2015.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (wang1998) at ($(bakowski1997.west |- 0,-14.500000*\dy)$) {\reftext{Wang98}\cite{wang1998} ( -- ) ( \num{15.9} , -- , \num{124} , \num{1.76E+19} , \num{0.34} ) ( -- , \num{-2.5} , -- , -- , -- , -- )};
\draw (wang1998.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (wang1999) at ($(wang1998.west |- 0,-15.500000*\dy)$) {\reftext{Wang99}\cite{wang1999} ( -- ) ( \num{15.9} , -- , \num{124} , \num{1.76E+19} , \num{0.34} ) ( -- , \num{-2.5} , -- , -- , -- , -- )};
\draw (wang1999.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (ladesmartin2000) at ($(wang1999.west |- 0,-16.500000*\dy)$) {\reftext{Lade00}\cite{ladesmartin2000} ( -- ) ( \num{15.9} , \num{124} , -- , \num{1.76E+19} , \num{0.34} ) ( -- , \numrange{-1.8}{-2.2} , -- , -- , -- , -- )};
\draw (ladesmartin2000.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (morisette2001) at ($(ladesmartin2000.west |- 0,-17.500000*\dy)$) {\reftext{Mori01}\cite{morisette2001} ( -- ) ( \num{15.9} , \num{124} , -- , \num{1.76E+19} , \num{0.34} ) ( -- , -- , -- , -- , -- , -- )};
\draw (morisette2001.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (lee2002) at ($(morisette2001.west |- 0,-18.500000*\dy)$) {\reftext{Lee02}\cite{lee2002} ( $\perp$ ) ( \num{15.9} , -- , \num{124} , \num{1.76E+19} , \num{0.34} ) ( -- , \num{-2.15} , -- , -- , -- , -- )};
\draw (lee2002.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (li2003) at ($(lee2002.west |- 0,-19.500000*\dy)$) {\reftext{Li03}\cite{li2003} ( -- ) ( \num{15.9} , -- , \num{124} , \num{1.76E+19} , \num{0.34} ) ( -- , -- , \num{-2} , -- , -- , -- )};
\draw (li2003.west) -| ++(-\dy,\fy*\dy);
\coordinate (li2003C) at ($(li2003.west)+(\dxStart+\dy,0)$);
\node[ ref] (megherbi2018) at ($(li2003C |- 0,-20.500000*\dy)$) {\reftext{Megh18}\cite{megherbi2018} ( -- ) ( \num{15.9} , \num{125} , -- , -- , -- ) ( -- , -- , -- , -- , -- , -- )};
\draw (megherbi2018.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (megherbi2018a) at ($(megherbi2018.west |- 0,-21.500000*\dy)$) {\reftext{Megh18a}\cite{megherbi2018a} ( -- ) ( \num{15.9} , \num{125} , -- , \num{1.76E+19} , -- ) ( -- , -- , -- , -- , -- , -- )};
\draw (megherbi2018a.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (zeghdar2019) at ($(megherbi2018a.west |- 0,-22.500000*\dy)$) {\reftext{Zegh19}\cite{zeghdar2019} ( -- ) ( \num{15.9} , \num{125} , -- , \num{1.76E+19} , \num{0.34} ) ( \num{-0.5} , \num{-2.15} , -- , -- , -- , \num{-0.34} )};
\draw (zeghdar2019.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (zeghdar2020) at ($(zeghdar2019.west |- 0,-23.500000*\dy)$) {\reftext{Zegh20}\cite{zeghdar2020} ( -- ) ( \num{15.9} , \num{125} , -- , \num{1.76E+19} , \num{0.34} ) ( \num{0.5} , \num{2.15} , -- , -- , -- , \num{0.34} )};
\draw (zeghdar2020.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (zhao2003) at ($(li2003.west |- 0,-24.500000*\dy)$) {\reftext{Zhao03}\cite{zhao2003} ( -- ) ( \num{15.9} , -- , \num{124} , \num{1.76E+19} , \num{0.34} ) ( -- , -- , \num{-2} , -- , -- , -- )};
\draw (zhao2003.west) -| ++(-\dy,\fy*\dy);
\coordinate (zhao2003C) at ($(zhao2003.west)+(\dxStart+\dy,0)$);
\node[ ref] (das2015) at ($(zhao2003C |- 0,-25.500000*\dy)$) {\reftext{Das15}\cite{das2015} ( -- ) ( \num{15.9} , -- , \num{124} , \num{1.76E+19} , \num{0.34} ) ( -- , -- , \num{-2} , -- , -- , -- )};
\draw (das2015.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (ayalew2004) at ($(zhao2003.west |- 0,-26.500000*\dy)$) {\reftext{Ayal04}\cite{ayalew2004} ( -- ) ( \num{15.9} , \num{125} , -- , \num{1.76E+19} , \num{0.34} ) ( \num{-0.5} , \num{-2.15} , -- , -- , -- , -- )};
\draw (ayalew2004.west) -| ++(-\dy,\fy*\dy);
\coordinate (ayalew2004C) at ($(ayalew2004.west)+(\dxStart+\dy,0)$);
\node[ ref] (maximenko2023) at ($(ayalew2004C |- 0,-27.500000*\dy)$) {\reftext{Maxi23}\cite{maximenko2023} ( -- ) ( \num{15.9} , \num{125} , -- , \num{1.76E+19} , \num{0.34} ) ( \num{-0.5} , \num{-2.15} , -- , -- , -- , -- )};
\draw (maximenko2023.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (brosselard2004) at ($(ayalew2004.west |- 0,-28.500000*\dy)$) {\reftext{Bros04}\cite{brosselard2004} ( -- ) ( \num{15.9} , \num{124} , -- , \num{1.76E+19} , \num{0.34} ) ( \num{0} , \num{-2.15} , -- , -- , -- , \num{0} )};
\draw (brosselard2004.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (adachi2005) at ($(brosselard2004.west |- 0,-29.500000*\dy)$) {\reftext{Adac05}\cite{adachi2005} ( -- ) ( \num{15.9} , \num{124} , -- , \num{1.76E+19} , \num{0.34} ) ( -- , -- , -- , -- , -- , -- )};
\draw (adachi2005.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (schroeder2006) at ($(adachi2005.west |- 0,-30.500000*\dy)$) {\reftext{Schr06}\cite{schroeder2006} ( -- ) ( \num{15.9} , \num{124} , -- , \num{1.76E+19} , \num{0.34} ) ( -- , -- , -- , -- , -- , -- )};
\draw (schroeder2006.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (tamaki2008a) at ($(schroeder2006.west |- 0,-31.500000*\dy)$) {\reftext{Tama08a}\cite{tamaki2008a} ( -- ) ( -- , \num{124} , -- , \num{1.76E+19} , \num{0.34} ) ( -- , \num{-2.8} , -- , -- , -- , -- )};
\draw (tamaki2008a.west) -| ++(-\dy,\fy*\dy);
\coordinate (tamaki2008aC) at ($(tamaki2008a.west)+(\dxStart+\dy,0)$);
\node[ ref] (liu2021) at ($(tamaki2008aC |- 0,-32.500000*\dy)$) {\reftext{Liu21}\cite{liu2021} ( -- ) ( -- , \num{125} , -- , \num{1.76E+17} , \num{0.34} ) ( -- , \num{-2.8} , -- , -- , -- , -- )};
\draw (liu2021.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (zhang2009) at ($(tamaki2008a.west |- 0,-33.500000*\dy)$) {\reftext{Zhan09}\cite{zhang2009} ( -- ) ( \num{15.9} , -- , \num{124} , \num{1.76E+19} , \num{0.34} ) ( -- , -- , \num{-2} , -- , -- , -- )};
\draw (zhang2009.west) -| ++(-\dy,\fy*\dy);
\coordinate (zhang2009C) at ($(zhang2009.west)+(\dxStart+\dy,0)$);
\node[ ref] (khalid2012) at ($(zhang2009C |- 0,-34.500000*\dy)$) {\reftext{Khal12}\cite{khalid2012} ( -- ) ( \num{15.9} , \num{124} , -- , \num{1.76E+17} , \num{0.34} ) ( -- , \num{-2} , -- , -- , -- , -- )};
\draw (khalid2012.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (albanese2010) at ($(zhang2009.west |- 0,-35.500000*\dy)$) {\reftext{Alba10}\cite{albanese2010} ( -- ) ( \num{15.9} , \num{125} , -- , \num{1.76E+17} , \num{0.34} ) ( \num{-0.5} , \num{-2.15} , -- , -- , -- , \num{-0.34} )};
\draw (albanese2010.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (zhang2010) at ($(albanese2010.west |- 0,-36.500000*\dy)$) {\reftext{Zhan10}\cite{zhang2010} ( -- ) ( \num{15.9} , -- , \num{124} , \num{1.76E+19} , \num{0.34} ) ( -- , -- , \num{-2} , -- , -- , -- )};
\draw (zhang2010.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (bellone2011) at ($(zhang2010.west |- 0,-37.500000*\dy)$) {\reftext{Bell11}\cite{bellone2011} ( -- ) ( \num{15.9} , \num{125} , -- , \num{1.76E+19} , \num{0.34} ) ( \num{-0.5} , \num{-2.15} , -- , -- , -- , \num{-0.34} )};
\draw (bellone2011.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (lutz2011) at ($(bellone2011.west |- 0,-38.500000*\dy)$) {\reftext{Lutz11}\cite{lutz2011} ( -- ) ( \num{15.9} , \num{124} , -- , \num{1.76E+19} , \num{0.34} ) ( -- , \num{-2.15} , -- , -- , -- , -- )};
\draw (lutz2011.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (buono2012) at ($(lutz2011.west |- 0,-39.500000*\dy)$) {\reftext{Buon12}\cite{buono2012} ( -- ) ( -- , -- , \num{108.1} , \num{1.76E+19} , \num{0.34} ) ( -- , -- , \num{-2.15} , -- , -- , -- )};
\draw (buono2012.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (song2012) at ($(buono2012.west |- 0,-40.500000*\dy)$) {\reftext{Song12}\cite{song2012} ( -- ) ( \num{0} , \num{124} , -- , \num{1.76E+19} , \num{0.34} ) ( -- , \num{-2.8} , -- , -- , -- , -- )};
\draw (song2012.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (pezzimenti2013) at ($(song2012.west |- 0,-41.500000*\dy)$) {\reftext{Pezz13}\cite{pezzimenti2013} ( -- ) ( \num{15.9} , \num{125} , -- , \num{1.76E+19} , \num{0.34} ) ( \num{-0.5} , \num{-2.15} , -- , -- , -- , \num{-0.34} )};
\draw (pezzimenti2013.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (chen2015) at ($(pezzimenti2013.west |- 0,-42.500000*\dy)$) {\reftext{Chen15}\cite{chen2015} ( $\parallel/\perp$ ) ( \num{15.9} , -- , \num{124} , \num{1.76E+19} , \num{0.34} ) ( \num{-2.15} , -- , \num{-2.15} , -- , -- , -- )};
\draw (chen2015.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (megherbi2015) at ($(chen2015.west |- 0,-43.500000*\dy)$) {\reftext{Megh15}\cite{megherbi2015} ( -- ) ( \num{15.9} , \num{124} , -- , \num{1.76E+17} , \num{0.34} ) ( \num{-0.5} , \num{-2.15} , -- , -- , -- , \num{-0.34} )};
\draw (megherbi2015.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (johannesson2016) at ($(megherbi2015.west |- 0,-44.500000*\dy)$) {\reftext{Joha16}\cite{johannesson2016} ( -- ) ( \num{15.9} , \num{124} , -- , \num{1.76E+19} , \num{0.34} ) ( -- , \num{-2.15} , -- , -- , -- , -- )};
\draw (johannesson2016.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (arvanitopoulos2017) at ($(johannesson2016.west |- 0,-45.500000*\dy)$) {\reftext{Arva17}\cite{arvanitopoulos2017} ( -- ) ( \num{15.9} , \num{125} , -- , \num{1.76E+19} , \num{0.34} ) ( \num{-0.57} , \num{-2.15} , -- , -- , -- , -- )};
\draw (arvanitopoulos2017.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (lutz2018) at ($(arvanitopoulos2017.west |- 0,-46.500000*\dy)$) {\reftext{Lutz18}\cite{lutz2018} ( -- ) ( \num{15.9} , \num{124} , -- , \num{1.76E+19} , \num{0.34} ) ( -- , \num{-2.15} , -- , -- , -- , -- )};
\draw (lutz2018.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (arvanitopoulos2019) at ($(lutz2018.west |- 0,-47.500000*\dy)$) {\reftext{Arva19}\cite{arvanitopoulos2019} ( $\perp$ ) ( \num{16} , \num{125} , -- , \num{1.76E+19} , \num{0.34} ) ( -- , -- , -- , -- , -- , -- )};
\draw (arvanitopoulos2019.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (johannesson2019) at ($(arvanitopoulos2019.west |- 0,-48.500000*\dy)$) {\reftext{Joha19}\cite{johannesson2019} ( -- ) ( -- , \num{20} , -- , -- , -- ) ( -- , -- , -- , -- , -- , -- )};
\draw (johannesson2019.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (yang2022) at ($(johannesson2019.west |- 0,-49.500000*\dy)$) {\reftext{Yang22}\cite{yang2022} ( -- ) ( -- , -- , -- , -- , -- ) ( -- , -- , -- , -- , -- , -- )};
\draw (yang2022.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,0.000000*\dy) {\citeauthor{wright1998}};
\node[fund, ref] (wright1998) at (\xSepOne,-1.000000*\dy) {\reftext{Wrig98}\cite{wright1998} ( -- ) ( \num{74} , -- , \num{43} , \num{1.43E+17} , \num{1} ) ( \num{-0.57} , -- , \num{-2.7} , \num{2.55} , -- , -- )};
\coordinate (wright1998C) at ($(wright1998.west)+(\dxStart+\dy,0)$);
\node[ ref] (baliga2019) at ($(wright1998C |- 0,-2.000000*\dy)$) {\reftext{Bali19}\cite{baliga2019} ( -- ) ( -- , \num{120} , -- , -- , -- ) ( -- , \num{-3.4} , -- , -- , -- , -- )};
\draw (baliga2019.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-4.000000*\dy) {\citeauthor{mnatsakanov2001}};
\node[fund, ref] (mnatsakanov2001) at (\xSepOne,-5.000000*\dy) {\reftext{Mnat01}\cite{mnatsakanov2001} ( -- ) ( \num{33} , \num{117} , -- , \num{1.00E+19} , \num{0.5} ) ( -- , -- , -- , -- , -- , -- )};
\coordinate (mnatsakanov2001C) at ($(mnatsakanov2001.west)+(\dxStart+\dy,0)$);
\node[ ref] (mnatsakanov2002) at ($(mnatsakanov2001C |- 0,-6.000000*\dy)$) {\reftext{Mnat02}\cite{mnatsakanov2002} ( -- ) ( \num{33} , \num{117} , -- , \num{1.00E+19} , \num{0.5} ) ( -- , -- , -- , -- , -- , -- )};
\draw (mnatsakanov2002.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-8.000000*\dy) {\citeauthor{hatakeyama2003}};
\node[fund, ref] (hatakeyama2003) at (\xSepOne,-9.000000*\dy) {\reftext{Hata03}\cite{hatakeyama2003} ( -- ) ( \num{15.9} , \num{120} , -- , \num{1.80E+18} , \num{0.65} ) ( -- , -- , -- , -- , -- , -- )};
\coordinate (hatakeyama2003C) at ($(hatakeyama2003.west)+(\dxStart+\dy,0)$);
\node[ ref] (negoro2004) at ($(hatakeyama2003C |- 0,-10.000000*\dy)$) {\reftext{Nego04}\cite{negoro2004} ( -- ) ( \num{16} , \num{120} , -- , \num{1.80E+18} , \num{0.65} ) ( -- , -- , -- , -- , -- , -- )};
\draw (negoro2004.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (nipoti2016a) at ($(negoro2004.west |- 0,-11.000000*\dy)$) {\reftext{Nipo16a}\cite{nipoti2016a} ( -- ) ( -- , -- , -- , -- , -- ) ( -- , -- , -- , -- , -- , -- )};
\draw (nipoti2016a.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-13.000000*\dy) {\citeauthor{balachandran2005}};
\node[fund, ref] (balachandran2005) at (\xSepOne,-14.000000*\dy) {\reftext{Bala05}\cite{balachandran2005} ( -- ) ( \num{53.3} , \num{105.4} , -- , \num{2.20E+18} , \num{0.7} ) ( -- , \num{-2.1} , -- , -- , -- , -- )};
\coordinate (balachandran2005C) at ($(balachandran2005.west)+(\dxStart+\dy,0)$);
\node[ ref] (nawaz2010) at ($(balachandran2005C |- 0,-15.000000*\dy)$) {\reftext{Nawa10}\cite{nawaz2010} ( -- ) ( \num{53.3} , \num{105.4} , -- , \num{2.20E+18} , \num{0.7} ) ( \num{0} , \num{-2.1} , -- , \num{0} , -- , -- )};
\draw (nawaz2010.west) -| ++(-\dy,\fy*\dy);
\coordinate (nawaz2010C) at ($(nawaz2010.west)+(\dxStart+\dy,0)$);
\node[ ref] (usman2014) at ($(nawaz2010C |- 0,-16.000000*\dy)$) {\reftext{Usma14}\cite{usman2014} ( -- ) ( \num{53.3} , \num{105.4} , -- , \num{2.20E+18} , \num{0.7} ) ( \num{0} , \num{-2.1} , -- , -- , -- , \num{0} )};
\draw (usman2014.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-18.000000*\dy) {\citeauthor{koizumi2009}};
\node[fund, ref] (koizumi2009) at (\xSepOne,-19.000000*\dy) {\reftext{Koiz09}\cite{koizumi2009} ( -- ) ( \num{0} , \num{114.1} , -- , \num{5.38E+18} , \num{0.66} ) ( \num{0} , \num{-2.72} , -- , -- , \num{-0.35} , \num{2.44} )};
\coordinate (koizumi2009C) at ($(koizumi2009.west)+(\dxStart+\dy,0)$);
\node[ ref] (stefanakis2014) at ($(koizumi2009C |- 0,-20.000000*\dy)$) {\reftext{Stef14}\cite{stefanakis2014} ( $\perp$ ) ( \num{0} , \num{114} , -- , \num{5.38E+18} , \num{0.66} ) ( \num{0} , \num{-2.72} , -- , -- , \num{-0.35} , \num{2.44} )};
\draw (stefanakis2014.west) -| ++(-\dy,\fy*\dy);
\coordinate (stefanakis2014C) at ($(stefanakis2014.west)+(\dxStart+\dy,0)$);
\node[ ref] (tripathi2019) at ($(stefanakis2014C |- 0,-21.000000*\dy)$) {\reftext{Trip19}\cite{tripathi2019} ( -- ) ( \num{0} , \num{114} , -- , \num{1.00E+16} , \num{0.7} ) ( \num{0} , \num{-2.72} , -- , -- , -- , \num{2.44} )};
\draw (tripathi2019.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-23.000000*\dy) {\citeauthor{hatakeyama2013}};
\node[fund, ref] (hatakeyama2013) at (\xSepOne,-24.000000*\dy) {\reftext{Hata13}\cite{hatakeyama2013} ( -- ) ( \num{0} , \num{113.5} , -- , \num{2.40E+18} , \num{0.69} ) ( \num{-0.57} , \num{-2.6} , -- , \num{2.9} , \num{-0.2} , -- )};
\coordinate (hatakeyama2013C) at ($(hatakeyama2013.west)+(\dxStart+\dy,0)$);
\node[ ref] (naugarhiya2017) at ($(hatakeyama2013C |- 0,-25.000000*\dy)$) {\reftext{Naug17}\cite{naugarhiya2017} ( $\perp$ ) ( \num{0} , \num{113.5} , -- , \num{2.40E+18} , \num{0.69} ) ( \num{-0.57} , \num{-2.6} , -- , \num{2.9} , \num{-0.2} , -- )};
\draw (naugarhiya2017.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (lophitis2018) at ($(naugarhiya2017.west |- 0,-26.000000*\dy)$) {\reftext{Loph18}\cite{lophitis2018} ( $\parallel/\perp$ ) ( \num{0} , \num{114} , -- , \num{2.40E+18} , \num{0.69} ) ( \num{-0.57} , \num{-2.6} , -- , \num{2.9} , \num{-0.2} , -- )};
\draw (lophitis2018.west) -| ++(-\dy,\fy*\dy);
\coordinate (lophitis2018C) at ($(lophitis2018.west)+(\dxStart+\dy,0)$);
\node[ ref] (rakheja2020) at ($(lophitis2018C |- 0,-27.000000*\dy)$) {\reftext{Rakh20}\cite{rakheja2020} ( -- ) ( -- , \num{105.6} , -- , -- , -- ) ( -- , -- , -- , -- , -- , -- )};
\draw (rakheja2020.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (guo2025) at ($(lophitis2018.west |- 0,-28.000000*\dy)$) {\reftext{Guo25}\cite{guo2025} ( -- ) ( -- , \num{113.5} , -- , \num{2.40E+18} , \num{0.69} ) ( -- , -- , -- , -- , -- , -- )};
\draw (guo2025.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-30.000000*\dy) {\citeauthor{kimoto2014a}};
\node[ ref] (kimoto2014a) at (\xSepOne,-31.000000*\dy) {\reftext{Kimo14a}\cite{kimoto2014a} ( $\perp$ ) ( -- , \num{118} , -- , \num{2.20E+18} , \num{0.7} ) ( -- , \numrange{-1.8}{-2.5} , -- , -- , -- , -- )};
\coordinate (kimoto2014aC) at ($(kimoto2014a.west)+(\dxStart+\dy,0)$);
\node[ ref] (fujihara2017) at ($(kimoto2014aC |- 0,-32.000000*\dy)$) {\reftext{Fuji17}\cite{fujihara2017} ( -- ) ( -- , -- , -- , -- , -- ) ( -- , -- , -- , -- , -- , -- )};
\draw (fujihara2017.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (kimoto2019) at ($(fujihara2017.west |- 0,-33.000000*\dy)$) {\reftext{Kimo19}\cite{kimoto2019} ( -- ) ( -- , \num{118} , -- , \num{2.20E+18} , \num{0.7} ) ( -- , -- , -- , -- , -- , -- )};
\draw (kimoto2019.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (huang2022b) at ($(kimoto2019.west |- 0,-34.000000*\dy)$) {\reftext{Huan22b}\cite{huang2022b} ( -- ) ( \num{0} , \num{118} , -- , \num{2.20E+18} , \num{0.7} ) ( -- , -- , -- , -- , -- , -- )};
\draw (huang2022b.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-36.000000*\dy) {\citeauthor{tanaka2018}};
\node[fund, ref] (tanaka2018) at (\xSepOne,-37.000000*\dy) {\reftext{Tana18}\cite{tanaka2018} ( -- ) ( \num{0} , \num{110}/\num{95} , -- , \num{3e18}/\num{1e19} , \num{0.6}/\num{0.7} ) ( \num{0} , \num{-3}/\num{-2.1} , -- , -- , -- , \num{-1.8}/\num{-1.5} )};
\coordinate (tanaka2018C) at ($(tanaka2018.west)+(\dxStart+\dy,0)$);
\node[ ref] (kajikawa2021) at ($(tanaka2018C |- 0,-38.000000*\dy)$) {\reftext{Kaji21}\cite{kajikawa2021} ( -- ) ( -- , \num{95} , -- , \num{1.00E+19} , \num{0.71} ) ( -- , \num{-2.1} , -- , -- , -- , \num{-1.5} )};
\draw (kajikawa2021.west) -| ++(-\dy,\fy*\dy);


==> data/mobility_vsat_ref_chain_elec.tex <==
\node[desc] at (0,0.000000*\dy) {Electron ($\vs$, $\vsperp$, $\vspara$) ($\gsat$, $\beta$, $\gbeta$, $\Tsat$)};
\node[author] at (0,-1.500000*\dy) {\citeauthor{powell1989}};
\node[no4H, ref] (powell1989) at (0,-2.500000*\dy) {\reftext{Powe89}\cite{powell1989}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\coordinate (powell1989C) at ($(powell1989.west)+(\dxStart+\dy,0)$);
\node[ ref] (gotz1993) at ($(powell1989C |- 0,-3.500000*\dy)$) {\reftext{Gotz93}\cite{gotz1993}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\draw (gotz1993.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-5.500000*\dy) {\citeauthor{ruff1994}};
\node[no4H, ref] (ruff1994) at (0,-6.500000*\dy) {\reftext{Ruff94}\cite{ruff1994}  ( \num{2.00E+07} , -- , -- ) ( -- , \num{2} , -- , -- )};
\coordinate (ruff1994C) at ($(ruff1994.west)+(\dxStart+\dy,0)$);
\node[ ref] (nallet1999) at ($(ruff1994C |- 0,-7.500000*\dy)$) {\reftext{Nall99}\cite{nallet1999}  ( \num{2.00E+07} , -- , -- ) ( \num{-0.5} , \num{2} , -- , -- )};
\draw (nallet1999.west) -| ++(-\dy,\fy*\dy);
\coordinate (nallet1999C) at ($(nallet1999.west)+(\dxStart+\dy,0)$);
\node[ ref] (nallet2000) at ($(nallet1999C |- 0,-8.500000*\dy)$) {\reftext{Nall00}\cite{nallet2000}  ( \num{2.00E+07} , -- , -- ) ( \num{-0.5} , \num{2} , -- , -- )};
\draw (nallet2000.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (cha2008) at ($(nallet2000.west |- 0,-9.500000*\dy)$) {\reftext{Cha08}\cite{cha2008}  ( \num{2.00E+07} , -- , -- ) ( \num{-0.5} , \num{2} , -- , -- )};
\draw (cha2008.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-11.500000*\dy) {\citeauthor{weitzel1994}};
\node[ ref] (weitzel1994) at (0,-12.500000*\dy) {\reftext{Weit94}\cite{weitzel1994}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\coordinate (weitzel1994C) at ($(weitzel1994.west)+(\dxStart+\dy,0)$);
\node[ ref] (wright1996) at ($(weitzel1994C |- 0,-13.500000*\dy)$) {\reftext{Wrig96}\cite{wright1996}  ( \num{2.00E+07} , -- , -- ) ( -- , \num{2} , -- , -- )};
\draw (wright1996.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-15.500000*\dy) {\citeauthor{harris1995}};
\node[ ref] (harris1995) at (0,-16.500000*\dy) {\reftext{Harr95}\cite{harris1995}  ( -- , -- , -- ) ( -- , -- , -- , -- )};
\coordinate (harris1995C) at ($(harris1995.west)+(\dxStart+\dy,0)$);
\node[ ref] (bellotti1999) at ($(harris1995C |- 0,-17.500000*\dy)$) {\reftext{Bell99}\cite{bellotti1999}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\draw (bellotti1999.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-19.500000*\dy) {\citeauthor{joshi1995}};
\node[fund, ref] (joshi1995) at (0,-20.500000*\dy) {\reftext{Josh95}\cite{joshi1995}  ( -- , \num{2.70E+07} , \num{2.10E+07} ) ( -- , -- , -- , \num{300} )};
\coordinate (joshi1995C) at ($(joshi1995.west)+(\dxStart+\dy,0)$);
\node[ ref] (itoh1996) at ($(joshi1995C |- 0,-21.500000*\dy)$) {\reftext{Itoh96}\cite{itoh1996}  ( \num{2.70E+07} , -- , -- ) ( -- , -- , -- , -- )};
\draw (itoh1996.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (wang1999) at ($(itoh1996.west |- 0,-22.500000*\dy)$) {\reftext{Wang99}\cite{wang1999}  ( \num{2.70E+07} , -- , -- ) ( -- , \num{2} , -- , -- )};
\draw (wang1999.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-24.500000*\dy) {\citeauthor{casady1996}};
\node[ ref] (casady1996) at (0,-25.500000*\dy) {\reftext{Casa96}\cite{casady1996}  ( -- , \num{2.00E+07} , -- ) ( -- , -- , -- , -- )};
\coordinate (casady1996C) at ($(casady1996.west)+(\dxStart+\dy,0)$);
\node[ ref] (gerhardt2011) at ($(casady1996C |- 0,-26.500000*\dy)$) {\reftext{Gerh11}\cite{gerhardt2011}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\draw (gerhardt2011.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-28.500000*\dy) {\citeauthor{chow1996}};
\node[ ref] (chow1996) at (0,-29.500000*\dy) {\reftext{Chow96}\cite{chow1996}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\coordinate (chow1996C) at ($(chow1996.west)+(\dxStart+\dy,0)$);
\node[ ref] (hudgins2003) at ($(chow1996C |- 0,-30.500000*\dy)$) {\reftext{Hudg03}\cite{hudgins2003}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\draw (hudgins2003.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-32.500000*\dy) {\citeauthor{yoder1996}};
\node[ ref] (yoder1996) at (0,-33.500000*\dy) {\reftext{Yode96}\cite{yoder1996}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\coordinate (yoder1996C) at ($(yoder1996.west)+(\dxStart+\dy,0)$);
\node[ ref] (neilainglesias2012) at ($(yoder1996C |- 0,-34.500000*\dy)$) {\reftext{Neil12}\cite{neilainglesias2012}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\draw (neilainglesias2012.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-36.500000*\dy) {\citeauthor{sriram1997}};
\node[ ref] (sriram1997) at (0,-37.500000*\dy) {\reftext{Srir97}\cite{sriram1997}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\coordinate (sriram1997C) at ($(sriram1997.west)+(\dxStart+\dy,0)$);
\node[ ref] (han2003) at ($(sriram1997C |- 0,-38.500000*\dy)$) {\reftext{Han03}\cite{han2003}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\draw (han2003.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-40.500000*\dy) {\citeauthor{trew1997}};
\node[ ref] (trew1997) at (0,-41.500000*\dy) {\reftext{Trew97}\cite{trew1997}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\coordinate (trew1997C) at ($(trew1997.west)+(\dxStart+\dy,0)$);
\node[ ref] (codreanu2000) at ($(trew1997C |- 0,-42.500000*\dy)$) {\reftext{Codr00}\cite{codreanu2000}  ( \num{2.00E+07} , -- , -- ) ( -- , \num{1} , -- , -- )};
\draw (codreanu2000.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-44.500000*\dy) {\citeauthor{roschke1998}};
\node[ ref] (roschke1998) at (0,-45.500000*\dy) {\reftext{Rosc98}\cite{roschke1998}  ( \num{2.00E+07} , -- , -- ) ( -- , \num{2} , -- , -- )};
\coordinate (roschke1998C) at ($(roschke1998.west)+(\dxStart+\dy,0)$);
\node[ ref] (mukherjee2020a) at ($(roschke1998C |- 0,-46.500000*\dy)$) {\reftext{Mukh20a}\cite{mukherjee2020a}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\draw (mukherjee2020a.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-48.500000*\dy) {\citeauthor{weitzel1998}};
\node[ ref] (weitzel1998) at (0,-49.500000*\dy) {\reftext{Weit98}\cite{weitzel1998}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\coordinate (weitzel1998C) at ($(weitzel1998.west)+(\dxStart+\dy,0)$);
\node[ ref] (neudeck2001) at ($(weitzel1998C |- 0,-50.500000*\dy)$) {\reftext{Neud01}\cite{neudeck2001}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\draw (neudeck2001.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (neudeck2006) at ($(neudeck2001.west |- 0,-51.500000*\dy)$) {\reftext{Neud06}\cite{neudeck2006}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\draw (neudeck2006.west) -| ++(-\dy,\fy*\dy);
\coordinate (neudeck2006C) at ($(neudeck2006.west)+(\dxStart+\dy,0)$);
\node[ ref] (wijesundara2011) at ($(neudeck2006C |- 0,-52.500000*\dy)$) {\reftext{Wije11}\cite{wijesundara2011}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\draw (wijesundara2011.west) -| ++(-\dy,\fy*\dy);
\coordinate (wijesundara2011C) at ($(wijesundara2011.west)+(\dxStart+\dy,0)$);
\node[ ref] (langpoklakpam2022) at ($(wijesundara2011C |- 0,-53.500000*\dy)$) {\reftext{Lang22}\cite{langpoklakpam2022}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\draw (langpoklakpam2022.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (arvinte2017) at ($(wijesundara2011.west |- 0,-54.500000*\dy)$) {\reftext{Arvi17}\cite{arvinte2017}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\draw (arvinte2017.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (mukherjee2023) at ($(arvinte2017.west |- 0,-55.500000*\dy)$) {\reftext{Mukh23}\cite{mukherjee2023}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\draw (mukherjee2023.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,0.000000*\dy) {\citeauthor{wright1998}};
\node[ ref] (wright1998) at (\xSepOne,-1.000000*\dy) {\reftext{Wrig98}\cite{wright1998}  ( \num{2.00E+07} , -- , -- ) ( -- , \num{2} , -- , -- )};
\coordinate (wright1998C) at ($(wright1998.west)+(\dxStart+\dy,0)$);
\node[ ref] (baliga2019) at ($(wright1998C |- 0,-2.000000*\dy)$) {\reftext{Bali19}\cite{baliga2019}  ( \num{2.20E+07} , -- , -- ) ( -- , \num{1.25} , -- , -- )};
\draw (baliga2019.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-4.000000*\dy) {\citeauthor{chow2000}};
\node[ ref] (chow2000) at (\xSepOne,-5.000000*\dy) {\reftext{Chow00}\cite{chow2000}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\coordinate (chow2000C) at ($(chow2000.west)+(\dxStart+\dy,0)$);
\node[guess, ref] (dmitriev2000) at ($(chow2000C |- 0,-6.000000*\dy)$) {\reftext{Dmit00}\cite{dmitriev2000}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\draw (dmitriev2000.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (elasser2002) at ($(dmitriev2000.west |- 0,-7.000000*\dy)$) {\reftext{Elas02}\cite{elasser2002}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\draw (elasser2002.west) -| ++(-\dy,\fy*\dy);
\coordinate (elasser2002C) at ($(elasser2002.west)+(\dxStart+\dy,0)$);
\node[ ref] (su2010) at ($(elasser2002C |- 0,-8.000000*\dy)$) {\reftext{Su10}\cite{su2010}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\draw (su2010.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (dhanaraj2010) at ($(elasser2002.west |- 0,-9.000000*\dy)$) {\reftext{Dhan10}\cite{dhanaraj2010}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\draw (dhanaraj2010.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-11.000000*\dy) {\citeauthor{khan2000}};
\node[fund, ref] (khan2000) at (\xSepOne,-12.000000*\dy) {\reftext{Khan00}\cite{khan2000}  ( -- , -- , \num{2.2e7}/\num{1.6e7} ) ( -- , \num{1.2}/\num{2.2} , -- , \num{296}/\num{593} )};
\coordinate (khan2000C) at ($(khan2000.west)+(\dxStart+\dy,0)$);
\node[ ref] (khan2000b) at ($(khan2000C |- 0,-13.000000*\dy)$) {\reftext{Khan00b}\cite{khan2000b}  ( -- , -- , \num{2.2e7}/\num{1.6e7} ) ( -- , \num{1.2}/\num{2.2} , -- , \num{296}/\num{593} )};
\draw (khan2000b.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (biondo2012) at ($(khan2000b.west |- 0,-14.000000*\dy)$) {\reftext{Bion12}\cite{biondo2012}  ( \num{2.00E+07} , -- , -- ) ( -- , \num{2} , -- , -- )};
\draw (biondo2012.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (kimoto2019) at ($(biondo2012.west |- 0,-15.000000*\dy)$) {\reftext{Kimo19}\cite{kimoto2019}  ( -- , -- , \num{2.20E+07} ) ( -- , -- , -- , -- )};
\draw (kimoto2019.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (cheng2020) at ($(kimoto2019.west |- 0,-16.000000*\dy)$) {\reftext{Chen20}\cite{cheng2020}  ( -- , -- , \num{2.20E+07} ) ( -- , \num{1.2} , -- , -- )};
\draw (cheng2020.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-18.000000*\dy) {\citeauthor{ladesmartin2000}};
\node[fund, ref] (ladesmartin2000) at (\xSepOne,-19.000000*\dy) {\reftext{Lade00}\cite{ladesmartin2000}  ( -- , -- , \num{2.20E+07} ) ( \num{-0.44} , \num{1.2} , \num{1} , -- )};
\coordinate (ladesmartin2000C) at ($(ladesmartin2000.west)+(\dxStart+\dy,0)$);
\node[guess, ref] (ayalew2004) at ($(ladesmartin2000C |- 0,-20.000000*\dy)$) {\reftext{Ayal04}\cite{ayalew2004}  ( -- , -- , \num{2.20E+07} ) ( \num{-0.44} , \num{1.2} , \num{1} , -- )};
\draw (ayalew2004.west) -| ++(-\dy,\fy*\dy);
\coordinate (ayalew2004C) at ($(ayalew2004.west)+(\dxStart+\dy,0)$);
\node[ ref] (lechner2021) at ($(ayalew2004C |- 0,-21.000000*\dy)$) {\reftext{Lech21}\cite{lechner2021}  ( \num{2.20E+07} , -- , -- ) ( \num{0.44} , \num{1.2} , \num{1} , -- )};
\draw (lechner2021.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (schroeder2006) at ($(ayalew2004.west |- 0,-22.000000*\dy)$) {\reftext{Schr06}\cite{schroeder2006}  ( \num{2.20E+07} , -- , -- ) ( \num{-0.44} , \num{1.2} , \num{1} , -- )};
\draw (schroeder2006.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (arvanitopoulos2017) at ($(schroeder2006.west |- 0,-23.000000*\dy)$) {\reftext{Arva17}\cite{arvanitopoulos2017}  ( \num{2.20E+07} , -- , -- ) ( \num{0.44} , \num{1.2} , \num{1} , -- )};
\draw (arvanitopoulos2017.west) -| ++(-\dy,\fy*\dy);
\coordinate (arvanitopoulos2017C) at ($(arvanitopoulos2017.west)+(\dxStart+\dy,0)$);
\node[ ref] (arvanitopoulos2019) at ($(arvanitopoulos2017C |- 0,-24.000000*\dy)$) {\reftext{Arva19}\cite{arvanitopoulos2019}  ( -- , -- , \num{2.20E+07} ) ( -- , \num{1.2} , -- , -- )};
\draw (arvanitopoulos2019.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (choudhary2021) at ($(arvanitopoulos2019.west |- 0,-25.000000*\dy)$) {\reftext{Chou21}\cite{choudhary2021}  ( \num{2.20E+07} , -- , -- ) ( -- , -- , -- , -- )};
\draw (choudhary2021.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (lophitis2018) at ($(arvanitopoulos2017.west |- 0,-26.000000*\dy)$) {\reftext{Loph18}\cite{lophitis2018}  ( -- , \num{1.90E+07} , \num{2.20E+07} ) ( \num{-0.44} , \num{1.2} , \num{1} , -- )};
\draw (lophitis2018.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (rakheja2020) at ($(lophitis2018.west |- 0,-27.000000*\dy)$) {\reftext{Rakh20}\cite{rakheja2020}  ( \num{2.20E+07} , -- , -- ) ( -- , -- , \numrange{1.2}{2} , -- )};
\draw (rakheja2020.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-29.000000*\dy) {\citeauthor{nilsson2000}};
\node[fund, ref] (nilsson2000) at (\xSepOne,-30.000000*\dy) {\reftext{Nils00}\cite{nilsson2000}  ( -- , \num{1.64E+07} , \num{2.26E+07} ) ( -- , -- , -- , -- )};
\coordinate (nilsson2000C) at ($(nilsson2000.west)+(\dxStart+\dy,0)$);
\node[ ref] (biondo2012) at ($(nilsson2000C |- 0,-31.000000*\dy)$) {\reftext{Bion12}\cite{biondo2012}  ( \num{2.00E+07} , -- , -- ) ( -- , \num{2} , -- , -- )};
\draw (biondo2012.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-33.000000*\dy) {\citeauthor{vassilevski2000}};
\node[fund, ref] (vassilevski2000) at (\xSepOne,-34.000000*\dy) {\reftext{Vass00}\cite{vassilevski2000}  ( -- , \num{8e6}/\num{7.5e6} , -- ) ( -- , -- , -- , \num{300}/\num{460} )};
\coordinate (vassilevski2000C) at ($(vassilevski2000.west)+(\dxStart+\dy,0)$);
\node[ ref] (zhang2008) at ($(vassilevski2000C |- 0,-35.000000*\dy)$) {\reftext{Zhan08}\cite{zhang2008}  ( \num{8.00E+06} , -- , -- ) ( -- , -- , -- , -- )};
\draw (zhang2008.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-37.000000*\dy) {\citeauthor{zhao2000}};
\node[fund, ref] (zhao2000) at (\xSepOne,-38.000000*\dy) {\reftext{Zhao00}\cite{zhao2000}  ( -- , \num{1.83E+07} , -- ) ( -- , -- , -- , -- )};
\coordinate (zhao2000C) at ($(zhao2000.west)+(\dxStart+\dy,0)$);
\node[guess, ref] (liu2021) at ($(zhao2000C |- 0,-39.000000*\dy)$) {\reftext{Liu21}\cite{liu2021}  ( \num{1.80E+07} , -- , -- ) ( -- , \num{2} , -- , -- )};
\draw (liu2021.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-41.000000*\dy) {\citeauthor{zetterling2002}};
\node[ ref] (zetterling2002) at (\xSepOne,-42.000000*\dy) {\reftext{Zett02}\cite{zetterling2002}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\coordinate (zetterling2002C) at ($(zetterling2002.west)+(\dxStart+\dy,0)$);
\node[ ref] (ostling2011a) at ($(zetterling2002C |- 0,-43.000000*\dy)$) {\reftext{Ostl11a}\cite{ostling2011a}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\draw (ostling2011a.west) -| ++(-\dy,\fy*\dy);
\coordinate (ostling2011aC) at ($(ostling2011a.west)+(\dxStart+\dy,0)$);
\node[ ref] (ostling2011) at ($(ostling2011aC |- 0,-44.000000*\dy)$) {\reftext{Ostl11}\cite{ostling2011}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\draw (ostling2011.west) -| ++(-\dy,\fy*\dy);
\coordinate (ostling2011C) at ($(ostling2011.west)+(\dxStart+\dy,0)$);
\node[ ref] (pellish2013) at ($(ostling2011C |- 0,-45.000000*\dy)$) {\reftext{Pell13}\cite{pellish2013}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\draw (pellish2013.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-47.000000*\dy) {\citeauthor{zhang2002}};
\node[ ref] (zhang2002) at (\xSepOne,-48.000000*\dy) {\reftext{Zhan02}\cite{zhang2002}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\coordinate (zhang2002C) at ($(zhang2002.west)+(\dxStart+\dy,0)$);
\node[ ref] (trew2002) at ($(zhang2002C |- 0,-49.000000*\dy)$) {\reftext{Trew02}\cite{trew2002}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\draw (trew2002.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-51.000000*\dy) {\citeauthor{hjelm2003}};
\node[fund, ref] (hjelm2003) at (\xSepOne,-52.000000*\dy) {\reftext{Hjel03}\cite{hjelm2003}  ( -- , \num{1.58E+07} , \num{2.12E+07} ) ( -- , -- , -- , -- )};
\coordinate (hjelm2003C) at ($(hjelm2003.west)+(\dxStart+\dy,0)$);
\node[guess, ref] (banerjee2021) at ($(hjelm2003C |- 0,-53.000000*\dy)$) {\reftext{Bane21}\cite{banerjee2021}  ( \num{2.12E+07} , -- , -- ) ( -- , \num{1.2} , -- , -- )};
\draw (banerjee2021.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,0.000000*\dy) {\citeauthor{li2003}};
\node[ ref] (li2003) at (\xSepOne + \xSepTwo,-1.000000*\dy) {\reftext{Li03}\cite{li2003}  ( -- , -- , -- ) ( -- , -- , -- , -- )};
\coordinate (li2003C) at ($(li2003.west)+(\dxStart+\dy,0)$);
\node[ ref] (zeghdar2020) at ($(li2003C |- 0,-2.000000*\dy)$) {\reftext{Zegh20}\cite{zeghdar2020}  ( \num{2.00E+07} , -- , -- ) ( -- , \num{2} , -- , -- )};
\draw (zeghdar2020.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-4.000000*\dy) {\citeauthor{ozpineci2004}};
\node[ ref] (ozpineci2004) at (\xSepOne + \xSepTwo,-5.000000*\dy) {\reftext{Ozpi04}\cite{ozpineci2004}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\coordinate (ozpineci2004C) at ($(ozpineci2004.west)+(\dxStart+\dy,0)$);
\node[ ref] (uhnevionak2015) at ($(ozpineci2004C |- 0,-6.000000*\dy)$) {\reftext{Uhne15}\cite{uhnevionak2015}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\draw (uhnevionak2015.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-8.000000*\dy) {\citeauthor{baliga2006}};
\node[ ref] (baliga2006) at (\xSepOne + \xSepTwo,-9.000000*\dy) {\reftext{Bali06}\cite{baliga2006}  ( -- , -- , -- ) ( -- , -- , -- , -- )};
\coordinate (baliga2006C) at ($(baliga2006.west)+(\dxStart+\dy,0)$);
\node[no4H, ref] (mantooth2015) at ($(baliga2006C |- 0,-10.000000*\dy)$) {\reftext{Mant15}\cite{mantooth2015}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\draw (mantooth2015.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-12.000000*\dy) {\citeauthor{sze2007}};
\node[ ref] (sze2007) at (\xSepOne + \xSepTwo,-13.000000*\dy) {\reftext{Sze07}\cite{sze2007}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\coordinate (sze2007C) at ($(sze2007.west)+(\dxStart+\dy,0)$);
\node[ ref] (neudeck1995) at ($(sze2007C |- 0,-14.000000*\dy)$) {\reftext{Neud95}\cite{neudeck1995}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\draw (neudeck1995.west) -| ++(-\dy,\fy*\dy);
\coordinate (neudeck1995C) at ($(neudeck1995.west)+(\dxStart+\dy,0)$);
\node[ ref] (dogan2003) at ($(neudeck1995C |- 0,-15.000000*\dy)$) {\reftext{Doga03}\cite{dogan2003}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\draw (dogan2003.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (zhu2008) at ($(dogan2003.west |- 0,-16.000000*\dy)$) {\reftext{Zhu08}\cite{zhu2008}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\draw (zhu2008.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-18.000000*\dy) {\citeauthor{zhang2009}};
\node[ ref] (zhang2009) at (\xSepOne + \xSepTwo,-19.000000*\dy) {\reftext{Zhan09}\cite{zhang2009}  ( \num{2.00E+07} , -- , -- ) ( -- , \num{2} , -- , -- )};
\coordinate (zhang2009C) at ($(zhang2009.west)+(\dxStart+\dy,0)$);
\node[ ref] (khalid2012) at ($(zhang2009C |- 0,-20.000000*\dy)$) {\reftext{Khal12}\cite{khalid2012}  ( \num{2.00E+07} , -- , -- ) ( -- , \num{2} , -- , -- )};
\draw (khalid2012.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-22.000000*\dy) {\citeauthor{buttay2011}};
\node[ ref] (buttay2011) at (\xSepOne + \xSepTwo,-23.000000*\dy) {\reftext{Butt11}\cite{buttay2011}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\coordinate (buttay2011C) at ($(buttay2011.west)+(\dxStart+\dy,0)$);
\node[ ref] (fujita2015) at ($(buttay2011C |- 0,-24.000000*\dy)$) {\reftext{Fuji15}\cite{fujita2015}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\draw (fujita2015.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-26.000000*\dy) {\citeauthor{hatakeyama2013}};
\node[fund, ref] (hatakeyama2013) at (\xSepOne + \xSepTwo,-27.000000*\dy) {\reftext{Hata13}\cite{hatakeyama2013}  ( -- , -- , \num{2.20E+07} ) ( \num{-0.46} , \num{1.2} , \num{0.88} , -- )};
\coordinate (hatakeyama2013C) at ($(hatakeyama2013.west)+(\dxStart+\dy,0)$);
\node[ ref] (naugarhiya2017) at ($(hatakeyama2013C |- 0,-28.000000*\dy)$) {\reftext{Naug17}\cite{naugarhiya2017}  ( -- , \num{1.20E+07} , \num{2.20E+07} ) ( -- , -- , -- , -- )};
\draw (naugarhiya2017.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (johannesson2019) at ($(naugarhiya2017.west |- 0,-29.000000*\dy)$) {\reftext{Joha19}\cite{johannesson2019}  ( \num{2.20E+07} , -- , -- ) ( -- , \num{1.2} , -- , -- )};
\draw (johannesson2019.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (jin2024) at ($(johannesson2019.west |- 0,-30.000000*\dy)$) {\reftext{Jin24}\cite{jin2024}  ( -- , \num{1.32E+07} , \num{2.20E+07} ) ( -- , \num{1.2} , -- , -- )};
\draw (jin2024.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-32.000000*\dy) {\citeauthor{neudeck2013}};
\node[ ref] (neudeck2013) at (\xSepOne + \xSepTwo,-33.000000*\dy) {\reftext{Neud13}\cite{neudeck2013}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\coordinate (neudeck2013C) at ($(neudeck2013.west)+(\dxStart+\dy,0)$);
\node[ ref] (mantooth2013) at ($(neudeck2013C |- 0,-34.000000*\dy)$) {\reftext{Mant13}\cite{mantooth2013}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\draw (mantooth2013.west) -| ++(-\dy,\fy*\dy);
\coordinate (mantooth2013C) at ($(mantooth2013.west)+(\dxStart+\dy,0)$);
\node[ ref] (hassan2018) at ($(mantooth2013C |- 0,-35.000000*\dy)$) {\reftext{Hass18}\cite{hassan2018}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\draw (hassan2018.west) -| ++(-\dy,\fy*\dy);
\coordinate (hassan2018C) at ($(hassan2018.west)+(\dxStart+\dy,0)$);
\node[ ref] (jiya2020) at ($(hassan2018C |- 0,-36.000000*\dy)$) {\reftext{Jiya20}\cite{jiya2020}  ( \num{2.20E+07} , -- , -- ) ( -- , -- , -- , -- )};
\draw (jiya2020.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-38.000000*\dy) {\citeauthor{kimoto2014a}};
\node[ ref] (kimoto2014a) at (\xSepOne + \xSepTwo,-39.000000*\dy) {\reftext{Kimo14a}\cite{kimoto2014a}  ( \num{2.20E+07} , -- , -- ) ( -- , -- , -- , -- )};
\coordinate (kimoto2014aC) at ($(kimoto2014a.west)+(\dxStart+\dy,0)$);
\node[ ref] (elahipanah2017) at ($(kimoto2014aC |- 0,-40.000000*\dy)$) {\reftext{Elah17}\cite{elahipanah2017}  ( \num{2} , -- , -- ) ( -- , -- , -- , -- )};
\draw (elahipanah2017.west) -| ++(-\dy,\fy*\dy);
\coordinate (elahipanah2017C) at ($(elahipanah2017.west)+(\dxStart+\dy,0)$);
\node[ ref] (ostling2024) at ($(elahipanah2017C |- 0,-41.000000*\dy)$) {\reftext{Ostl24}\cite{ostling2024}  ( \num{2} , -- , -- ) ( -- , -- , -- , -- )};
\draw (ostling2024.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (rescher2018) at ($(elahipanah2017.west |- 0,-42.000000*\dy)$) {\reftext{Resc18}\cite{rescher2018}  ( \num{2.20E+07} , -- , -- ) ( -- , -- , -- , -- )};
\draw (rescher2018.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (berens2021) at ($(rescher2018.west |- 0,-43.000000*\dy)$) {\reftext{Bere21}\cite{berens2021}  ( \num{2.20E+07} , -- , -- ) ( -- , -- , -- , -- )};
\draw (berens2021.west) -| ++(-\dy,\fy*\dy);


==> data/mobility_vsat_ref_chain_hole.tex <==
\node[desc] at (0,0.000000*\dy) {Hole ($\vs$, $\vsperp$, $\vspara$) ($\gsat$, $\beta$, $\gbeta$, $\Tsat$)};
\node[author] at (0,-1.500000*\dy) {\citeauthor{ruff1994}};
\node[no4H, ref] (ruff1994) at (0,-2.500000*\dy) {\reftext{Ruff94}\cite{ruff1994}  ( \num{2.00E+07} , -- , -- ) ( -- , -- , -- , -- )};
\coordinate (ruff1994C) at ($(ruff1994.west)+(\dxStart+\dy,0)$);
\node[ ref] (nallet1999) at ($(ruff1994C |- 0,-3.500000*\dy)$) {\reftext{Nall99}\cite{nallet1999}  ( \num{2.00E+07} , -- , -- ) ( \num{-0.5} , \num{2} , -- , -- )};
\draw (nallet1999.west) -| ++(-\dy,\fy*\dy);
\coordinate (nallet1999C) at ($(nallet1999.west)+(\dxStart+\dy,0)$);
\node[ ref] (cha2008) at ($(nallet1999C |- 0,-4.500000*\dy)$) {\reftext{Cha08}\cite{cha2008}  ( \num{2.00E+07} , -- , -- ) ( -- , \num{2} , \num{-0.5} , -- )};
\draw (cha2008.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-6.500000*\dy) {\citeauthor{weitzel1994}};
\node[ ref] (weitzel1994) at (0,-7.500000*\dy) {\reftext{Weit94}\cite{weitzel1994}  ( -- , -- , -- ) ( -- , -- , -- , -- )};
\coordinate (weitzel1994C) at ($(weitzel1994.west)+(\dxStart+\dy,0)$);
\node[ ref] (wright1996) at ($(weitzel1994C |- 0,-8.500000*\dy)$) {\reftext{Wrig96}\cite{wright1996}  ( \num{2.00E+07} , -- , -- ) ( -- , \num{1} , -- , -- )};
\draw (wright1996.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-10.500000*\dy) {\citeauthor{wright1998}};
\node[ ref] (wright1998) at (0,-11.500000*\dy) {\reftext{Wrig98}\cite{wright1998}  ( \num{2.00E+07} , -- , -- ) ( -- , \num{1} , -- , -- )};
\coordinate (wright1998C) at ($(wright1998.west)+(\dxStart+\dy,0)$);
\node[ ref] (baliga2019) at ($(wright1998C |- 0,-12.500000*\dy)$) {\reftext{Bali19}\cite{baliga2019}  ( \num{1.30E+07} , -- , -- ) ( -- , \num{1.2} , -- , -- )};
\draw (baliga2019.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-14.500000*\dy) {\citeauthor{khan2000}};
\node[ ref] (khan2000) at (0,-15.500000*\dy) {\reftext{Khan00}\cite{khan2000}  ( -- , -- , -- ) ( -- , -- , -- , -- )};
\coordinate (khan2000C) at ($(khan2000.west)+(\dxStart+\dy,0)$);
\node[ ref] (biondo2012) at ($(khan2000C |- 0,-16.500000*\dy)$) {\reftext{Bion12}\cite{biondo2012}  ( \num{2.00E+07} , -- , -- ) ( -- , \num{2.00E+00} , -- , -- )};
\draw (biondo2012.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-18.500000*\dy) {\citeauthor{ladesmartin2000}};
\node[ ref] (ladesmartin2000) at (0,-19.500000*\dy) {\reftext{Lade00}\cite{ladesmartin2000}  ( -- , -- , -- ) ( -- , -- , -- , -- )};
\coordinate (ladesmartin2000C) at ($(ladesmartin2000.west)+(\dxStart+\dy,0)$);
\node[ ref] (rakheja2020) at ($(ladesmartin2000C |- 0,-20.500000*\dy)$) {\reftext{Rakh20}\cite{rakheja2020}  ( \num{2.20E+07} , -- , -- ) ( -- , \numrange{1.2}{2} , -- , -- )};
\draw (rakheja2020.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-22.500000*\dy) {\citeauthor{nilsson2000}};
\node[fund, ref] (nilsson2000) at (0,-23.500000*\dy) {\reftext{Nils00}\cite{nilsson2000}  ( -- , \num{6.50E+06} , \num{1.10E+07} ) ( -- , -- , -- , -- )};
\coordinate (nilsson2000C) at ($(nilsson2000.west)+(\dxStart+\dy,0)$);
\node[ ref] (biondo2012) at ($(nilsson2000C |- 0,-24.500000*\dy)$) {\reftext{Bion12}\cite{biondo2012}  ( \num{2.00E+07} , -- , -- ) ( -- , \num{2.00E+00} , -- , -- )};
\draw (biondo2012.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-26.500000*\dy) {\citeauthor{zhao2000}};
\node[fund, ref] (zhao2000) at (0,-27.500000*\dy) {\reftext{Zhao00}\cite{zhao2000}  ( -- , \num{8.60E+06} , -- ) ( -- , -- , -- , -- )};
\coordinate (zhao2000C) at ($(zhao2000.west)+(\dxStart+\dy,0)$);
\node[guess, ref] (liu2021) at ($(zhao2000C |- 0,-28.500000*\dy)$) {\reftext{Liu21}\cite{liu2021}  ( \num{8.00E+06} , -- , -- ) ( -- , \num{1.2} , -- , -- )};
\draw (liu2021.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,0.000000*\dy) {\citeauthor{hjelm2003}};
\node[fund, ref] (hjelm2003) at (\xSepOne,-1.000000*\dy) {\reftext{Hjel03}\cite{hjelm2003}  ( -- , \num{7.30E+06} , \num{1.08E+07} ) ( -- , -- , -- , -- )};
\coordinate (hjelm2003C) at ($(hjelm2003.west)+(\dxStart+\dy,0)$);
\node[ ref] (hatakeyama2013) at ($(hjelm2003C |- 0,-2.000000*\dy)$) {\reftext{Hata13}\cite{hatakeyama2013}  ( -- , -- , \num{1.00E+07} ) ( -- , -- , -- , -- )};
\draw (hatakeyama2013.west) -| ++(-\dy,\fy*\dy);
\coordinate (hatakeyama2013C) at ($(hatakeyama2013.west)+(\dxStart+\dy,0)$);
\node[ ref] (naugarhiya2017) at ($(hatakeyama2013C |- 0,-3.000000*\dy)$) {\reftext{Naug17}\cite{naugarhiya2017}  ( -- , \num{8.00E+06} , \num{1.00E+07} ) ( -- , -- , -- , -- )};
\draw (naugarhiya2017.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (banerjee2021) at ($(hatakeyama2013.west |- 0,-4.000000*\dy)$) {\reftext{Bane21}\cite{banerjee2021}  ( \num{1.08E+07} , -- , -- ) ( -- , \num{1.2} , -- , -- )};
\draw (banerjee2021.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-6.000000*\dy) {\citeauthor{li2003}};
\node[ ref] (li2003) at (\xSepOne,-7.000000*\dy) {\reftext{Li03}\cite{li2003}  ( -- , -- , -- ) ( -- , -- , -- , -- )};
\coordinate (li2003C) at ($(li2003.west)+(\dxStart+\dy,0)$);
\node[ ref] (zeghdar2020) at ($(li2003C |- 0,-8.000000*\dy)$) {\reftext{Zegh20}\cite{zeghdar2020}  ( \num{2.00E+07} , -- , -- ) ( -- , \num{1} , -- , -- )};
\draw (zeghdar2020.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-10.000000*\dy) {\citeauthor{ayalew2004}};
\node[ ref] (ayalew2004) at (\xSepOne,-11.000000*\dy) {\reftext{Ayal04}\cite{ayalew2004}  ( -- , -- , -- ) ( -- , -- , -- , -- )};
\coordinate (ayalew2004C) at ($(ayalew2004.west)+(\dxStart+\dy,0)$);
\node[ ref] (lechner2021) at ($(ayalew2004C |- 0,-12.000000*\dy)$) {\reftext{Lech21}\cite{lechner2021}  ( \num{2.20E+07} , -- , -- ) ( \num{0.44} , \num{1.2} , \num{1} , -- )};
\draw (lechner2021.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-14.000000*\dy) {\citeauthor{zhang2009}};
\node[ ref] (zhang2009) at (\xSepOne,-15.000000*\dy) {\reftext{Zhan09}\cite{zhang2009}  ( \num{2.00E+07} , -- , -- ) ( -- , \num{1} , -- , -- )};
\coordinate (zhang2009C) at ($(zhang2009.west)+(\dxStart+\dy,0)$);
\node[ ref] (khalid2012) at ($(zhang2009C |- 0,-16.000000*\dy)$) {\reftext{Khal12}\cite{khalid2012}  ( \num{2.00E+07} , -- , -- ) ( -- , \num{1} , -- , -- )};
\draw (khalid2012.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-18.000000*\dy) {\citeauthor{kimoto2014a}};
\node[fund, ref] (kimoto2014a) at (\xSepOne,-19.000000*\dy) {\reftext{Kimo14a}\cite{kimoto2014a}  ( \num{1.30E+07} , -- , -- ) ( -- , -- , -- , -- )};
\coordinate (kimoto2014aC) at ($(kimoto2014a.west)+(\dxStart+\dy,0)$);
\node[guess, ref] (kimoto2015) at ($(kimoto2014aC |- 0,-20.000000*\dy)$) {\reftext{Kimo15}\cite{kimoto2015}  ( \num{1.30E+07} , -- , -- ) ( -- , -- , -- , -- )};
\draw (kimoto2015.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (kimoto2019) at ($(kimoto2015.west |- 0,-21.000000*\dy)$) {\reftext{Kimo19}\cite{kimoto2019}  ( \num{1.30E+07} , -- , -- ) ( -- , -- , -- , -- )};
\draw (kimoto2019.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-23.000000*\dy) {\citeauthor{arvanitopoulos2017}};
\node[ ref] (arvanitopoulos2017) at (\xSepOne,-24.000000*\dy) {\reftext{Arva17}\cite{arvanitopoulos2017}  ( \num{2.20E+07} , -- , -- ) ( \num{0.44} , \num{1.20E+00} , \num{1} , -- )};
\coordinate (arvanitopoulos2017C) at ($(arvanitopoulos2017.west)+(\dxStart+\dy,0)$);
\node[ ref] (lophitis2018) at ($(arvanitopoulos2017C |- 0,-25.000000*\dy)$) {\reftext{Loph18}\cite{lophitis2018}  ( \num{2.20E+07} , -- , -- ) ( \num{-0.44} , \num{1.2} , \num{1} , -- )};
\draw (lophitis2018.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (arvanitopoulos2019) at ($(lophitis2018.west |- 0,-26.000000*\dy)$) {\reftext{Arva19}\cite{arvanitopoulos2019}  ( -- , -- , \num{2.20E+07} ) ( -- , \num{1.2} , -- , -- )};
\draw (arvanitopoulos2019.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (choudhary2021) at ($(arvanitopoulos2019.west |- 0,-27.000000*\dy)$) {\reftext{Chou21}\cite{choudhary2021}  ( \num{2.20E+07} , -- , -- ) ( -- , -- , -- , -- )};
\draw (choudhary2021.west) -| ++(-\dy,\fy*\dy);


==> data/mobility_vsat_stat_elec.tex <==
\addplot+ [ boxplot prepared = { lower whisker=7.5000e+06, lower quartile=1.3850e+07, median=1.7000e+07, upper quartile=1.9975e+07, upper whisker=2.7000e+07},] coordinates {} node[mean,anchor=west] at (boxplot box cs: \boxplotvalue{median},0.5) {\pgfmathfloatparsenumber{\boxplotvalue{median}}\pgfmathfloattomacro{\pgfmathresult}{\F}{\M}{\E}\M};
\addplot+ [ boxplot prepared = { lower whisker=1.4000e+07, lower quartile=1.6625e+07, median=2.0900e+07, upper quartile=2.1800e+07, upper whisker=2.2600e+07},] coordinates {} node[mean,anchor=east] at (boxplot box cs: \boxplotvalue{median},0.5) {\pgfmathfloatparsenumber{\boxplotvalue{median}}\pgfmathfloattomacro{\pgfmathresult}{\F}{\M}{\E}\M};
\addplot+ [ boxplot prepared = { lower whisker=3.3000e+06, lower quartile=8.7000e+06, median=1.8000e+07, upper quartile=2.0000e+07, upper whisker=2.4000e+07},] coordinates {} node[mean,anchor=east] at (boxplot box cs: \boxplotvalue{median},0.5) {\pgfmathfloatparsenumber{\boxplotvalue{median}}\pgfmathfloattomacro{\pgfmathresult}{\F}{\M}{\E}\M};


==> data/permittivity_eps.tex <==


\node[symbol] (epsperp) at (0,0) {$\espe$};
\coordinate (epsperp0) at (epsperp.north);
\node[ref, lwepsperp] (epsperp1) at (epsperp0.north west) {\tikz \node[paper] {\reftext{Janz08}\cite{janzen2008}};};
\node[value, scale=1.100000] (epsperpvalue1) at (epsperp1.west) {\num{9.55}};
\node[ref, lwepsperp] (epsperp2) at (epsperp1.north west) {\tikz \node[paper] {\reftext{Yode96}\cite{yoder1996}};};
\node[value, scale=1.100000] (epsperpvalue2) at (epsperp2.west) {\num{9.6}};
\node[ref, lwepsperp] (epsperp3) at (epsperp2.north west) {\tikz \node[paper, fund] {\reftext{Pers05}\cite{persson2005}};};
\node[value, scale=1.100000] (epsperpvalue3) at (epsperp3.west) {\num{9.63}};
\node[ref, lwepsperp] (epsperp4) at (epsperp3.north west) {\tikz \node[paper] {\reftext{Ioff23}\cite{ioffe2023}}; \tikz \node[paper] {\reftext{Naug17}\cite{naugarhiya2017}}; \tikz \node[paper] {\reftext{Hata13}\cite{hatakeyama2013}}; \tikz \node[paper] {\reftext{Koiz09}\cite{koizumi2009}}; \tikz \node[paper] {\reftext{Son04}\cite{son2004}}; \tikz \node[paper] {\reftext{Levi01}\cite{levinshtein2001}}; \tikz \node[paper] {\reftext{Lade00}\cite{ladesmartin2000}}; \tikz \node[paper] {\reftext{Pers99}\cite{persson1999}}; \tikz \node[paper] {\reftext{Lind98}\cite{lindefelt1998}}; \tikz \node[paper] {\reftext{Pers97}\cite{persson1997}}; \tikz \node[paper] {\reftext{Bako97}\cite{bakowski1997}}; \tikz \node[paper, no4H] {\reftext{Patr70}\cite{patrick1970}};};
\node[value, scale=2.200000] (epsperpvalue4) at (epsperp4.west) {\num{9.66}};
\node[ref, lwepsperp] (epsperp5) at (epsperp4.north west) {\tikz \node[paper] {\reftext{Yosh18}\cite{yoshioka2018}};};
\node[value, scale=1.100000] (epsperpvalue5) at (epsperp5.west) {\num{9.7}};
\node[ref, lwepsperp] (epsperp6) at (epsperp5.north west) {\tikz \node[paper] {\reftext{Kimo19}\cite{kimoto2019}}; \tikz \node[paper] {\reftext{Kimo14a}\cite{kimoto2014a}}; \tikz \node[paper] {\reftext{Resh05}\cite{reshanov2005}}; \tikz \node[paper] {\reftext{Pens05}\cite{pensl2005}}; \tikz \node[paper] {\reftext{Ayal04}\cite{ayalew2004}}; \tikz \node[paper] {\reftext{Trof98}\cite{troffer1998}}; \tikz \node[paper] {\reftext{Scha97}\cite{schadt1997}}; \tikz \node[paper, no4H] {\reftext{Nino94}\cite{ninomiya1994}}; \tikz \node[paper, fund] {\reftext{Iked80}\cite{ikeda1980}};};
\node[value, scale=1.900000] (epsperpvalue6) at (epsperp6.west) {\num{9.76}};
\node[ref, lwepsperp] (epsperp7) at (epsperp6.north west) {\tikz \node[paper, fund] {\reftext{Li24b}\cite{li2024b}};};
\node[value, scale=1.100000] (epsperpvalue7) at (epsperp7.west) {\num{9.77}};
\node[ref, lwepsperp] (epsperp8) at (epsperp7.north west) {\tikz \node[paper] {\reftext{Torr22}\cite{torres2022}}; \tikz \node[paper, fund] {\reftext{Cout17}\cite{coutinho2017}};};
\node[value, scale=1.200000] (epsperpvalue8) at (epsperp8.west) {\num{9.88}};
\node[ref, lwepsperp] (epsperp9) at (epsperp8.north west) {\tikz \node[paper, fund] {\reftext{Naft16}\cite{naftaly2016}};};
\node[value, scale=1.100000] (epsperpvalue9) at (epsperp9.west) {\num{9.91}};
\node[ref, lwepsperp] (epsperp10) at (epsperp9.north west) {\tikz \node[paper, fund] {\reftext{Chen22}\cite{cheng2022}};};
\node[value, scale=1.100000] (epsperpvalue10) at (epsperp10.west) {\num{9.97}};
\node[ref, lwepsperp] (epsperp11) at (epsperp10.north west) {\tikz \node[paper, fund] {\reftext{Karc96}\cite{karch1996}};};
\node[value, scale=1.100000] (epsperpvalue11) at (epsperp11.west) {\num{10.352}};


\node[symbol] (eps) at (0+ \dxepsperp,0) {$\es$};
\coordinate (eps0) at (eps.north);
\node[ref, lweps] (eps1) at (eps0.north west) {\tikz \node[paper] {\reftext{Bane21}\cite{banerjee2021}}; \tikz \node[paper] {\reftext{Acha17}\cite{acharyya2017}};};
\node[value, scale=1.200000] (epsvalue1) at (eps1.west) {\num{8.5884}};
\node[ref, lweps] (eps2) at (eps1.north west) {\tikz \node[paper, fund] {\reftext{Jone11}\cite{jones2011}};};
\node[value, scale=1.100000] (epsvalue2) at (eps2.west) {\num{9.60}};
\node[ref, lweps] (eps3) at (eps2.north west) {\tikz \node[paper] {\reftext{Rao22}\cite{rao2022}}; \tikz \node[paper] {\reftext{Zatk21}\cite{zatko2021}}; \tikz \node[paper] {\reftext{Lech21}\cite{lechner2021}}; \tikz \node[paper] {\reftext{Chou21}\cite{choudhary2021}}; \tikz \node[paper] {\reftext{Trip19}\cite{tripathi2019}}; \tikz \node[paper] {\reftext{Sozz19}\cite{sozzi2019}}; \tikz \node[paper] {\reftext{Micc19}\cite{miccoli2019}}; \tikz \node[paper] {\reftext{Arva17}\cite{arvanitopoulos2017}}; \tikz \node[paper] {\reftext{Nipo16}\cite{nipoti2016}}; \tikz \node[paper] {\reftext{Usma14}\cite{usman2014}}; \tikz \node[paper] {\reftext{Pezz13}\cite{pezzimenti2013}}; \tikz \node[paper] {\reftext{Sand11}\cite{sandeep2011}}; \tikz \node[paper] {\reftext{Bell11}\cite{bellone2011}}; \tikz \node[paper] {\reftext{Pezz08}\cite{pezzimenti2008}}; \tikz \node[paper] {\reftext{Schr06}\cite{schroeder2006}};};
\node[value, scale=2.500000] (epsvalue3) at (eps3.west) {\num{9.66}};
\node[ref, lweps] (eps4) at (eps3.north west) {\tikz \node[paper] {\reftext{Kova20}\cite{kovalchuk2020}};};
\node[value, scale=1.100000] (epsvalue4) at (eps4.west) {\num{9.67}};
\node[ref, lweps] (eps5) at (eps4.north west) {\tikz \node[paper] {\reftext{Kim24}\cite{kim2024}}; \tikz \node[paper] {\reftext{Dong24}\cite{dong2024}}; \tikz \node[paper] {\reftext{Yang23}\cite{yang2023}}; \tikz \node[paper] {\reftext{Pear23}\cite{pearton2023}}; \tikz \node[paper] {\reftext{Yang22}\cite{yang2022}}; \tikz \node[paper] {\reftext{Dena22}\cite{denapoli2022}}; \tikz \node[paper] {\reftext{Zhen20}\cite{zheng2020}}; \tikz \node[paper] {\reftext{Jiya20}\cite{jiya2020}}; \tikz \node[paper] {\reftext{Bisw20}\cite{biswas2020}}; \tikz \node[paper] {\reftext{Sole19}\cite{soler2019}}; \tikz \node[paper] {\reftext{Bali19}\cite{baliga2019}}; \tikz \node[paper] {\reftext{Tsao18}\cite{tsao2018}}; \tikz \node[paper] {\reftext{Pear18}\cite{pearton2018}}; \tikz \node[paper] {\reftext{Hass18}\cite{hassan2018}}; \tikz \node[paper] {\reftext{Cabe18}\cite{cabello2018}}; \tikz \node[paper] {\reftext{Ryba17}\cite{rybalka2017}}; \tikz \node[paper] {\reftext{Arvi17}\cite{arvinte2017}}; \tikz \node[paper] {\reftext{Liu15}\cite{liu2015}}; \tikz \node[paper] {\reftext{Chen15}\cite{chen2015}}; \tikz \node[paper] {\reftext{Kami14}\cite{kaminski2014}}; \tikz \node[paper] {\reftext{Higa14}\cite{higashiwaki2014}}; \tikz \node[paper] {\reftext{Neud13}\cite{neudeck2013}}; \tikz \node[paper] {\reftext{Mant13}\cite{mantooth2013}}; \tikz \node[paper] {\reftext{Alba10}\cite{albanese2010}}; \tikz \node[paper] {\reftext{Kami09}\cite{kaminski2009}}; \tikz \node[paper] {\reftext{Donn09}\cite{donnarumma2009}}; \tikz \node[paper] {\reftext{Aktu09}\cite{akturk2009}}; \tikz \node[paper] {\reftext{Zhu08}\cite{zhu2008}}; \tikz \node[paper] {\reftext{Nava08}\cite{nava2008}}; \tikz \node[paper] {\reftext{Neud06}\cite{neudeck2006}}; \tikz \node[paper] {\reftext{Bali06}\cite{baliga2006}}; \tikz \node[paper] {\reftext{Choi05}\cite{choi2005}}; \tikz \node[paper] {\reftext{Bhat05}\cite{bhatnagar2005}}; \tikz \node[paper] {\reftext{Cole04}\cite{cole2004}}; \tikz \node[paper] {\reftext{Hjel03}\cite{hjelm2003}}; \tikz \node[paper] {\reftext{Han03}\cite{han2003}}; \tikz \node[paper] {\reftext{Neud01}\cite{neudeck2001}}; \tikz \node[paper] {\reftext{Mori01}\cite{morisette2001}}; \tikz \node[paper] {\reftext{Iwat01}\cite{iwata2001}}; \tikz \node[paper] {\reftext{Zhao00}\cite{zhao2000}}; \tikz \node[paper] {\reftext{Iwat00a}\cite{iwata2000a}}; \tikz \node[paper] {\reftext{Iwat00}\cite{iwata2000}}; \tikz \node[paper] {\reftext{Codr00}\cite{codreanu2000}}; \tikz \node[paper] {\reftext{Egil99}\cite{egilsson1999}}; \tikz \node[paper] {\reftext{Burk99}\cite{burk1999}}; \tikz \node[paper] {\reftext{Wrig98}\cite{wright1998}}; \tikz \node[paper] {\reftext{Weit98}\cite{weitzel1998}}; \tikz \node[paper] {\reftext{Mick98}\cite{mickevicius1998}}; \tikz \node[paper] {\reftext{Huan98}\cite{huang1998}}; \tikz \node[paper] {\reftext{Srir97}\cite{sriram1997}}; \tikz \node[paper] {\reftext{Wrig96}\cite{wright1996}}; \tikz \node[paper] {\reftext{Weit96}\cite{weitzel1996}}; \tikz \node[paper] {\reftext{Nils96}\cite{nilsson1996}};};
\node[value, scale=6.300000] (epsvalue5) at (eps5.west) {\num{9.7}};
\node[ref, lweps] (eps6) at (eps5.north west) {\tikz \node[paper] {\reftext{Neil12}\cite{neilainglesias2012}};};
\node[value, scale=1.100000] (epsvalue6) at (eps6.west) {\num{9.72}};
\node[ref, lweps] (eps7) at (eps6.north west) {\tikz \node[paper] {\reftext{Darm19}\cite{darmody2019}}; \tikz \node[paper] {\reftext{Zipp11}\cite{zippelius2011}};};
\node[value, scale=1.200000] (epsvalue7) at (eps7.west) {\num{9.76}};
\node[ref, lweps] (eps8) at (eps7.north west) {\tikz \node[paper, fund] {\reftext{Hart11}\cite{hartnett2011}};};
\node[value, scale=1.100000] (epsvalue8) at (eps8.west) {\num{9.77}};
\node[ref, lweps] (eps9) at (eps8.north west) {\tikz \node[paper] {\reftext{Scab11a}\cite{scaburri2011a}}; \tikz \node[paper] {\reftext{Pern05}\cite{pernot2005}}; \tikz \node[paper] {\reftext{Pern01}\cite{pernot2001}}; \tikz \node[paper] {\reftext{Lind98}\cite{lindefelt1998}};};
\node[value, scale=1.400000] (epsvalue9) at (eps9.west) {\num{9.78}};
\node[ref, lweps] (eps10) at (eps9.north west) {\tikz \node[paper] {\reftext{Kimo15}\cite{kimoto2015}}; \tikz \node[paper] {\reftext{Zhao03}\cite{zhao2003}}; \tikz \node[paper] {\reftext{Elas03}\cite{elasser2003}}; \tikz \node[paper] {\reftext{Elas00}\cite{elasser2000}}; \tikz \node[paper] {\reftext{Chel97}\cite{chelnokov1997}}; \tikz \node[paper] {\reftext{Scho94}\cite{schoner1994}};};
\node[value, scale=1.600000] (epsvalue10) at (eps10.west) {\num{9.8}};
\node[ref, lweps] (eps11) at (eps10.north west) {\tikz \node[paper, fund] {\reftext{Ivan06}\cite{ivanov2006}};};
\node[value, scale=1.100000] (epsvalue11) at (eps11.west) {\num{9.93}};
\node[ref, lweps] (eps12) at (eps11.north west) {\tikz \node[paper] {\reftext{Chow93}\cite{chow1993}};};
\node[value, scale=1.100000] (epsvalue12) at (eps12.west) {\num{9.945}};
\node[ref, lweps] (eps13) at (eps12.north west) {\tikz \node[paper] {\reftext{Tana18}\cite{tanaka2018}};};
\node[value, scale=1.100000] (epsvalue13) at (eps13.west) {\num{9.95}};
\node[ref, lweps] (eps14) at (eps13.north west) {\tikz \node[paper, fund] {\reftext{Dutt06}\cite{dutta2006}};};
\node[value, scale=1.100000] (epsvalue14) at (eps14.west) {\num{9.97}};
\node[ref, lweps] (eps15) at (eps14.north west) {\tikz \node[paper] {\reftext{Ostl24}\cite{ostling2024}}; \tikz \node[paper] {\reftext{Rodr21}\cite{rodrigues2021}}; \tikz \node[paper] {\reftext{Nouk20}\cite{nouketcha2020}}; \tikz \node[paper] {\reftext{Klah20}\cite{klahold2020}}; \tikz \node[paper] {\reftext{Vasc19}\cite{vasconcelos2019}}; \tikz \node[paper] {\reftext{Lebe17}\cite{lebedev2017}}; \tikz \node[paper] {\reftext{Elah17}\cite{elahipanah2017}}; \tikz \node[paper] {\reftext{Chow17}\cite{chow2017}}; \tikz \node[paper] {\reftext{Fuji15}\cite{fujita2015}}; \tikz \node[paper] {\reftext{Pell13}\cite{pellish2013}}; \tikz \node[paper] {\reftext{Wije11}\cite{wijesundara2011}}; \tikz \node[paper] {\reftext{Ostl11}\cite{ostling2011}}; \tikz \node[paper] {\reftext{Butt11}\cite{buttay2011}}; \tikz \node[paper] {\reftext{Su10}\cite{su2010}}; \tikz \node[paper] {\reftext{Dhan10}\cite{dhanaraj2010}}; \tikz \node[paper] {\reftext{Sze07}\cite{sze2007}}; \tikz \node[paper] {\reftext{Mill07}\cite{millan2007}}; \tikz \node[paper] {\reftext{Pere06}\cite{perez-tomas2006}}; \tikz \node[paper] {\reftext{Arpa06}\cite{arpatzanis2006}}; \tikz \node[paper] {\reftext{Chow04}\cite{chow2004}}; \tikz \node[paper] {\reftext{Zhan02}\cite{zhang2002}}; \tikz \node[paper] {\reftext{Zett02}\cite{zetterling2002}}; \tikz \node[paper] {\reftext{Trew02}\cite{trew2002}}; \tikz \node[paper] {\reftext{Lee02}\cite{lee2002}}; \tikz \node[paper] {\reftext{Keme02}\cite{kemerley2002}}; \tikz \node[paper] {\reftext{Elas02}\cite{elasser2002}}; \tikz \node[paper] {\reftext{Dmit00}\cite{dmitriev2000}}; \tikz \node[paper] {\reftext{Chow00a}\cite{chow2000a}}; \tikz \node[paper] {\reftext{Chow00}\cite{chow2000}}; \tikz \node[paper] {\reftext{Bell00}\cite{bellotti2000}}; \tikz \node[paper] {\reftext{Bell99}\cite{bellotti1999}}; \tikz \node[paper] {\reftext{Zett98}\cite{zetterling1998}}; \tikz \node[paper] {\reftext{Shah98}\cite{shah1998}}; \tikz \node[paper] {\reftext{Rosc98}\cite{roschke1998}}; \tikz \node[paper] {\reftext{Dani98}\cite{danielsson1998}}; \tikz \node[paper] {\reftext{Chow97}\cite{chow1997}}; \tikz \node[paper] {\reftext{Chow96}\cite{chow1996}};};
\node[value, scale=4.700000] (epsvalue15) at (eps15.west) {\num{10}};
\node[ref, lweps] (eps16) at (eps15.north west) {\tikz \node[paper] {\reftext{Ozpi04}\cite{ozpineci2004}};};
\node[value, scale=1.100000] (epsvalue16) at (eps16.west) {\num{10.1}};
\node[ref, lweps] (eps17) at (eps16.north west) {\tikz \node[paper, fund] {\reftext{Yang22a}\cite{yang2022a}};};
\node[value, scale=1.100000] (epsvalue17) at (eps17.west) {\num{10.21}};


\node[symbol] (epspara) at (0+ \dxepsperp+ \dxeps,0) {$\espa$};
\coordinate (epspara0) at (epspara.north);
\node[ref, lwepspara] (epspara1) at (epspara0.north west) {\tikz \node[paper, fund] {\reftext{Pers05}\cite{persson2005}};};
\node[value, scale=1.100000] (epsparavalue1) at (epspara1.west) {\num{9.94}};
\node[ref, lwepspara] (epspara2) at (epspara1.north west) {\tikz \node[paper] {\reftext{Ayal04}\cite{ayalew2004}}; \tikz \node[paper, no4H] {\reftext{Nino94}\cite{ninomiya1994}};};
\node[value, scale=1.200000] (epsparavalue2) at (epspara2.west) {\num{9.98}};
\node[ref, lwepspara] (epspara3) at (epspara2.north west) {\tikz \node[paper] {\reftext{Yode96}\cite{yoder1996}};};
\node[value, scale=1.100000] (epsparavalue3) at (epspara3.west) {\num{10}};
\node[ref, lwepspara] (epspara4) at (epspara3.north west) {\tikz \node[paper] {\reftext{Ioff23}\cite{ioffe2023}}; \tikz \node[paper] {\reftext{Naug17}\cite{naugarhiya2017}}; \tikz \node[paper] {\reftext{Hata13}\cite{hatakeyama2013}}; \tikz \node[paper] {\reftext{Koiz09}\cite{koizumi2009}}; \tikz \node[paper] {\reftext{Son04}\cite{son2004}}; \tikz \node[paper] {\reftext{Levi01}\cite{levinshtein2001}}; \tikz \node[paper] {\reftext{Lade00}\cite{ladesmartin2000}}; \tikz \node[paper] {\reftext{Pers99}\cite{persson1999}}; \tikz \node[paper] {\reftext{Lind98}\cite{lindefelt1998}}; \tikz \node[paper] {\reftext{Pers97}\cite{persson1997}}; \tikz \node[paper] {\reftext{Bako97}\cite{bakowski1997}}; \tikz \node[paper, no4H] {\reftext{Patr70}\cite{patrick1970}};};
\node[value, scale=2.200000] (epsparavalue4) at (epspara4.west) {\num{10.03}};
\node[ref, lwepspara] (epspara5) at (epspara4.north west) {\tikz \node[paper, fund] {\reftext{Li24b}\cite{li2024b}}; \tikz \node[paper] {\reftext{Niwa15}\cite{niwa2015}};};
\node[value, scale=1.200000] (epsparavalue5) at (epspara5.west) {\num{10.2}};
\node[ref, lwepspara] (epspara6) at (epspara5.north west) {\tikz \node[paper] {\reftext{Li23a}\cite{li2023a}}; \tikz \node[paper, fund] {\reftext{Li23}\cite{li2023}};};
\node[value, scale=1.200000] (epsparavalue6) at (epspara6.west) {\num{10.27}};
\node[ref, lwepspara] (epspara7) at (epspara6.north west) {\tikz \node[paper] {\reftext{Kimo19}\cite{kimoto2019}}; \tikz \node[paper] {\reftext{Kimo14a}\cite{kimoto2014a}}; \tikz \node[paper] {\reftext{Resh05}\cite{reshanov2005}}; \tikz \node[paper] {\reftext{Pens05}\cite{pensl2005}}; \tikz \node[paper] {\reftext{Trof98}\cite{troffer1998}}; \tikz \node[paper] {\reftext{Scha97}\cite{schadt1997}}; \tikz \node[paper, fund] {\reftext{Iked80}\cite{ikeda1980}};};
\node[value, scale=1.700000] (epsparavalue7) at (epspara7.west) {\num{10.32}};
\node[ref, lwepspara] (epspara8) at (epspara7.north west) {\tikz \node[paper] {\reftext{Janz08}\cite{janzen2008}};};
\node[value, scale=1.100000] (epsparavalue8) at (epspara8.west) {\num{10.36}};
\node[ref, lwepspara] (epspara9) at (epspara8.north west) {\tikz \node[paper, fund] {\reftext{Naft16}\cite{naftaly2016}};};
\node[value, scale=1.100000] (epsparavalue9) at (epspara9.west) {\num{10.53}};
\node[ref, lwepspara] (epspara10) at (epspara9.north west) {\tikz \node[paper] {\reftext{Torr22}\cite{torres2022}}; \tikz \node[paper, fund] {\reftext{Cout17}\cite{coutinho2017}};};
\node[value, scale=1.200000] (epsparavalue10) at (epspara10.west) {\num{10.65}};
\node[ref, lwepspara] (epspara11) at (epspara10.north west) {\tikz \node[paper, fund] {\reftext{Karc96}\cite{karch1996}};};
\node[value, scale=1.100000] (epsparavalue11) at (epspara11.west) {\num{10.9}};


==> data/permittivity_fundFigure.tex <==
\addplot[forget plot, epspara, error bars/.cd, y dir=both, y explicit] coordinates {(1,10.03)};
\addplot[forget plot, epsperp, error bars/.cd, y dir=both, y explicit] coordinates {(1,9.66)};
\addplot[forget plot, hfpara, error bars/.cd, y dir=both, y explicit] coordinates {(1,6.7)};
\addplot[forget plot, hfperp, error bars/.cd, y dir=both, y explicit] coordinates {(1,6.52)};
\addplot[forget plot, epspara, error bars/.cd, y dir=both, y explicit] coordinates {(2,10.32)};
\addplot[forget plot, epsperp, error bars/.cd, y dir=both, y explicit] coordinates {(2,9.76)};
\addplot[forget plot, hfpara, error bars/.cd, y dir=both, y explicit] coordinates {(3,7.20)};
\addplot[forget plot, hfperp, error bars/.cd, y dir=both, y explicit] coordinates {(3,6.96)};
\addplot[forget plot, epspara, error bars/.cd, y dir=both, y explicit] coordinates {(4,9.98)};
\addplot[forget plot, epsperp, error bars/.cd, y dir=both, y explicit] coordinates {(4,9.76)};
\addplot[forget plot, hfpara, error bars/.cd, y dir=both, y explicit] coordinates {(4,6.67)};
\addplot[forget plot, hfperp, error bars/.cd, y dir=both, y explicit] coordinates {(4,6.59)};
\addplot[forget plot, hfpara, error bars/.cd, y dir=both, y explicit] coordinates {(5,6.78)};
\addplot[forget plot, hfperp, error bars/.cd, y dir=both, y explicit] coordinates {(5,6.56)};
\addplot[forget plot, epspara, error bars/.cd, y dir=both, y explicit] coordinates {(6,10.9)};
\addplot[forget plot, epsperp, error bars/.cd, y dir=both, y explicit] coordinates {(6,10.352)};
\addplot[forget plot, hfpara, error bars/.cd, y dir=both, y explicit] coordinates {(6,7.169)};
\addplot[forget plot, hfperp, error bars/.cd, y dir=both, y explicit] coordinates {(6,6.946)};
\addplot[forget plot, hfpara, error bars/.cd, y dir=both, y explicit] coordinates {(7,7.17)};
\addplot[forget plot, hfperp, error bars/.cd, y dir=both, y explicit] coordinates {(7,6.95)};
\addplot[forget plot, hfpara, error bars/.cd, y dir=both, y explicit] coordinates {(8,7.61)};
\addplot[forget plot, hfperp, error bars/.cd, y dir=both, y explicit] coordinates {(8,7.54)};
\addplot[forget plot, hfpara, error bars/.cd, y dir=both, y explicit] coordinates {(9,7.47)};
\addplot[forget plot, hfperp, error bars/.cd, y dir=both, y explicit] coordinates {(9,6.94)};
\addplot[forget plot, hfpara, error bars/.cd, y dir=both, y explicit] coordinates {(10,6.44)};
\addplot[forget plot, hfperp, error bars/.cd, y dir=both, y explicit] coordinates {(10,6.25)};
\addplot[forget plot, epspara, error bars/.cd, y dir=both, y explicit] coordinates {(11,9.94)};
\addplot[forget plot, epsperp, error bars/.cd, y dir=both, y explicit] coordinates {(11,9.63)};
\addplot[forget plot, hfpara, error bars/.cd, y dir=both, y explicit] coordinates {(11,6.62)};
\addplot[forget plot, hfperp, error bars/.cd, y dir=both, y explicit] coordinates {(11,6.40)};
\addplot[forget plot, hf, error bars/.cd, y dir=both, y explicit] coordinates {(12,6.81)};
\addplot[forget plot, eps, error bars/.cd, y dir=both, y explicit] coordinates {(13,9.97) +- (0,0.02)};
\addplot[forget plot, eps, error bars/.cd, y dir=both, y explicit] coordinates {(14,9.93) +- (0,0.01)};
\addplot[forget plot, eps, error bars/.cd, y dir=both, y explicit] coordinates {(15,9.77)};
\addplot[forget plot, eps, error bars/.cd, y dir=both, y explicit] coordinates {(16,9.60)};
\addplot[forget plot, epspara, error bars/.cd, y dir=both, y explicit] coordinates {(17,10.53)};
\addplot[forget plot, epsperp, error bars/.cd, y dir=both, y explicit] coordinates {(17,9.91)};
\addplot[forget plot, epspara, error bars/.cd, y dir=both, y explicit] coordinates {(18,10.65)};
\addplot[forget plot, epsperp, error bars/.cd, y dir=both, y explicit] coordinates {(18,9.88)};
\addplot[forget plot, hf, error bars/.cd, y dir=both, y explicit] coordinates {(19,6.587) +- (0,0.003)};
\addplot[forget plot, epsperp, error bars/.cd, y dir=both, y explicit] coordinates {(20,9.97)};
\addplot[forget plot, hf, error bars/.cd, y dir=both, y explicit] coordinates {(21,6.51)};
\addplot[forget plot, eps, error bars/.cd, y dir=both, y explicit] coordinates {(22,10.21)};
\addplot[forget plot, epspara, error bars/.cd, y dir=both, y explicit] coordinates {(23,10.27) +- (0,0.03)};
\addplot[forget plot, epspara, error bars/.cd, y dir=both, y explicit] coordinates {(24,10.2) +- (0,0.05)};
\addplot[forget plot, epsperp, error bars/.cd, y dir=both, y explicit] coordinates {(24,9.77) +- (0,0.01)};
\addplot[forget plot, hfperp, error bars/.cd, y dir=both, y explicit] coordinates {(25,6.40) +- (0,0.2)};


==> data/permittivity_hf.tex <==


\node[symbol] (hfperp) at (0,0) {$\eipe$};
\coordinate (hfperp0) at (hfperp.north);
\node[ref, lwhfperp] (hfperp1) at (hfperp0.north west) {\tikz \node[paper, fund] {\reftext{Peng04}\cite{peng-shou2004}};};
\node[value, scale=1.100000] (hfperpvalue1) at (hfperp1.west) {\num{6.25}};
\node[ref, lwhfperp] (hfperp2) at (hfperp1.north west) {\tikz \node[paper] {\reftext{Tiwa99}\cite{tiwald1999}};};
\node[value, scale=1.100000] (hfperpvalue2) at (hfperp2.west) {\num{6.4}};
\node[ref, lwhfperp] (hfperp3) at (hfperp2.north west) {\tikz \node[paper, fund] {\reftext{Main24}\cite{mainali2024}}; \tikz \node[paper, fund] {\reftext{Pers05}\cite{persson2005}};};
\node[value, scale=1.200000] (hfperpvalue3) at (hfperp3.west) {\num{6.40}};
\node[ref, lwhfperp] (hfperp4) at (hfperp3.north west) {\tikz \node[paper] {\reftext{Ioff23}\cite{ioffe2023}}; \tikz \node[paper] {\reftext{Koiz09}\cite{koizumi2009}}; \tikz \node[paper] {\reftext{Son04}\cite{son2004}}; \tikz \node[paper] {\reftext{Levi01}\cite{levinshtein2001}}; \tikz \node[paper] {\reftext{Pers99}\cite{persson1999}}; \tikz \node[paper] {\reftext{Pers97}\cite{persson1997}}; \tikz \node[paper] {\reftext{Wenz95}\cite{wenzien1995}}; \tikz \node[paper, no4H] {\reftext{Patr70}\cite{patrick1970}};};
\node[value, scale=1.800000] (hfperpvalue4) at (hfperp4.west) {\num{6.52}};
\node[ref, lwhfperp] (hfperp5) at (hfperp4.north west) {\tikz \node[paper, fund] {\reftext{Hari95}\cite{harima1995}};};
\node[value, scale=1.100000] (hfperpvalue5) at (hfperp5.west) {\num{6.56}};
\node[ref, lwhfperp] (hfperp6) at (hfperp5.north west) {\tikz \node[paper, no4H] {\reftext{Nino94}\cite{ninomiya1994}};};
\node[value, scale=1.100000] (hfperpvalue6) at (hfperp6.west) {\num{6.59}};
\node[ref, lwhfperp] (hfperp7) at (hfperp6.north west) {\tikz \node[paper, fund] {\reftext{Ahuj02}\cite{ahuja2002}};};
\node[value, scale=1.100000] (hfperpvalue7) at (hfperp7.west) {\num{6.94}};
\node[ref, lwhfperp] (hfperp8) at (hfperp7.north west) {\tikz \node[paper, fund] {\reftext{Karc96}\cite{karch1996}};};
\node[value, scale=1.100000] (hfperpvalue8) at (hfperp8.west) {\num{6.946}};
\node[ref, lwhfperp] (hfperp9) at (hfperp8.north west) {\tikz \node[paper, fund] {\reftext{Well96}\cite{wellenhofer1996}};};
\node[value, scale=1.100000] (hfperpvalue9) at (hfperp9.west) {\num{6.95}};
\node[ref, lwhfperp] (hfperp10) at (hfperp9.north west) {\tikz \node[paper] {\reftext{Bech97}\cite{bechstedt1997}}; \tikz \node[paper, fund] {\reftext{Chen94}\cite{chen1994}};};
\node[value, scale=1.200000] (hfperpvalue10) at (hfperp10.west) {\num{6.96}};
\node[ref, lwhfperp] (hfperp11) at (hfperp10.north west) {\tikz \node[paper, fund] {\reftext{Adol97}\cite{adolph1997}};};
\node[value, scale=1.100000] (hfperpvalue11) at (hfperp11.west) {\num{7.54}};


\node[symbol] (hf) at (0+ \dxhfperp,0) {$\ei$};
\coordinate (hf0) at (hf.north);
\node[ref, lwhf] (hf1) at (hf0.north west) {\tikz \node[paper] {\reftext{Kova20}\cite{kovalchuk2020}}; \tikz \node[paper] {\reftext{Donn09}\cite{donnarumma2009}}; \tikz \node[paper] {\reftext{Aktu09}\cite{akturk2009}}; \tikz \node[paper] {\reftext{Hjel03}\cite{hjelm2003}}; \tikz \node[paper] {\reftext{Iwat01}\cite{iwata2001}}; \tikz \node[paper] {\reftext{Zhao00}\cite{zhao2000}}; \tikz \node[paper] {\reftext{Iwat00a}\cite{iwata2000a}}; \tikz \node[paper] {\reftext{Iwat00}\cite{iwata2000}}; \tikz \node[paper] {\reftext{Mick98}\cite{mickevicius1998}}; \tikz \node[paper] {\reftext{Nils96}\cite{nilsson1996}};};
\node[value, scale=2.000000] (hfvalue1) at (hf1.west) {\num{6.5}};
\node[ref, lwhf] (hf2) at (hf1.north west) {\tikz \node[paper, fund] {\reftext{Gao22a}\cite{gao2022a}};};
\node[value, scale=1.100000] (hfvalue2) at (hf2.west) {\num{6.51}};
\node[ref, lwhf] (hf3) at (hf2.north west) {\tikz \node[paper] {\reftext{Kim24}\cite{kim2024}}; \tikz \node[paper] {\reftext{Arvi17}\cite{arvinte2017}};};
\node[value, scale=1.200000] (hfvalue3) at (hf3.west) {\num{6.52}};
\node[ref, lwhf] (hf4) at (hf3.north west) {\tikz \node[paper] {\reftext{Pern05}\cite{pernot2005}}; \tikz \node[paper] {\reftext{Pern01}\cite{pernot2001}};};
\node[value, scale=1.200000] (hfvalue4) at (hf4.west) {\num{6.58}};
\node[ref, lwhf] (hf5) at (hf4.north west) {\tikz \node[paper, fund] {\reftext{Tare19}\cite{tarekegne2019}};};
\node[value, scale=1.100000] (hfvalue5) at (hf5.west) {\num{6.587}};
\node[ref, lwhf] (hf6) at (hf5.north west) {\tikz \node[paper] {\reftext{Rodr21}\cite{rodrigues2021}}; \tikz \node[paper] {\reftext{Vasc19}\cite{vasconcelos2019}}; \tikz \node[paper] {\reftext{Torp01}\cite{torpo2001}}; \tikz \node[paper] {\reftext{Bell00}\cite{bellotti2000}}; \tikz \node[paper] {\reftext{Bell99}\cite{bellotti1999}};};
\node[value, scale=1.500000] (hfvalue6) at (hf6.west) {\num{6.7}};
\node[ref, lwhf] (hf7) at (hf6.north west) {\tikz \node[paper] {\reftext{Hari98}\cite{harima1998}};};
\node[value, scale=1.100000] (hfvalue7) at (hf7.west) {\num{6.8}};
\node[ref, lwhf] (hf8) at (hf7.north west) {\tikz \node[paper, fund] {\reftext{Chin06}\cite{ching2006}};};
\node[value, scale=1.100000] (hfvalue8) at (hf8.west) {\num{6.81}};


\node[symbol] (hfpara) at (0+ \dxhfperp+ \dxhf,0) {$\eipa$};
\coordinate (hfpara0) at (hfpara.north);
\node[ref, lwhfpara] (hfpara1) at (hfpara0.north west) {\tikz \node[paper, fund] {\reftext{Peng04}\cite{peng-shou2004}};};
\node[value, scale=1.100000] (hfparavalue1) at (hfpara1.west) {\num{6.44}};
\node[ref, lwhfpara] (hfpara2) at (hfpara1.north west) {\tikz \node[paper, fund] {\reftext{Pers05}\cite{persson2005}};};
\node[value, scale=1.100000] (hfparavalue2) at (hfpara2.west) {\num{6.62}};
\node[ref, lwhfpara] (hfpara3) at (hfpara2.north west) {\tikz \node[paper, no4H] {\reftext{Nino94}\cite{ninomiya1994}};};
\node[value, scale=1.100000] (hfparavalue3) at (hfpara3.west) {\num{6.67}};
\node[ref, lwhfpara] (hfpara4) at (hfpara3.north west) {\tikz \node[paper] {\reftext{Ioff23}\cite{ioffe2023}}; \tikz \node[paper] {\reftext{Koiz09}\cite{koizumi2009}}; \tikz \node[paper] {\reftext{Son04}\cite{son2004}}; \tikz \node[paper] {\reftext{Levi01}\cite{levinshtein2001}}; \tikz \node[paper] {\reftext{Pers99}\cite{persson1999}}; \tikz \node[paper] {\reftext{Pers97}\cite{persson1997}}; \tikz \node[paper, no4H] {\reftext{Patr70}\cite{patrick1970}};};
\node[value, scale=1.700000] (hfparavalue4) at (hfpara4.west) {\num{6.7}};
\node[ref, lwhfpara] (hfpara5) at (hfpara4.north west) {\tikz \node[paper, fund] {\reftext{Hari95}\cite{harima1995}};};
\node[value, scale=1.100000] (hfparavalue5) at (hfpara5.west) {\num{6.78}};
\node[ref, lwhfpara] (hfpara6) at (hfpara5.north west) {\tikz \node[paper, fund] {\reftext{Karc96}\cite{karch1996}};};
\node[value, scale=1.100000] (hfparavalue6) at (hfpara6.west) {\num{7.169}};
\node[ref, lwhfpara] (hfpara7) at (hfpara6.north west) {\tikz \node[paper, fund] {\reftext{Well96}\cite{wellenhofer1996}};};
\node[value, scale=1.100000] (hfparavalue7) at (hfpara7.west) {\num{7.17}};
\node[ref, lwhfpara] (hfpara8) at (hfpara7.north west) {\tikz \node[paper, fund] {\reftext{Chen94}\cite{chen1994}};};
\node[value, scale=1.100000] (hfparavalue8) at (hfpara8.west) {\num{7.20}};
\node[ref, lwhfpara] (hfpara9) at (hfpara8.north west) {\tikz \node[paper] {\reftext{Bech97}\cite{bechstedt1997}};};
\node[value, scale=1.100000] (hfparavalue9) at (hfpara9.west) {\num{7.2}};
\node[ref, lwhfpara] (hfpara10) at (hfpara9.north west) {\tikz \node[paper] {\reftext{Tiwa99}\cite{tiwald1999}};};
\node[value, scale=1.100000] (hfparavalue10) at (hfpara10.west) {\num{7.45}};
\node[ref, lwhfpara] (hfpara11) at (hfpara10.north west) {\tikz \node[paper, fund] {\reftext{Ahuj02}\cite{ahuja2002}};};
\node[value, scale=1.100000] (hfparavalue11) at (hfpara11.west) {\num{7.47}};
\node[ref, lwhfpara] (hfpara12) at (hfpara11.north west) {\tikz \node[paper, fund] {\reftext{Adol97}\cite{adolph1997}};};
\node[value, scale=1.100000] (hfparavalue12) at (hfpara12.west) {\num{7.61}};


==> data/permittivity_ref_chain.tex <==
\node[desc] at (0,0.000000*\dy) {Permittivity ($\espa$, $\espe$ / $\eipa$ , $\eipe$)};
\node[author] at (0,-1.500000*\dy) {\citeauthor{patrick1970}};
\node[no4H, ref] (patrick1970) at (0,-2.500000*\dy) {\reftext{Patr70}\cite{patrick1970} (  10.03 , 9.66 / 6.7 , 6.52  )};
\coordinate (patrick1970C) at ($(patrick1970.west)+(\dxStart+\dy,0)$);
\node[no4H, ref] (madelung1991) at ($(patrick1970C |- 0,-3.500000*\dy)$) {\reftext{Made91}\cite{madelung1991} (  10.03 , 9.66 / 6.7 , 6.52  )};
\draw (madelung1991.west) -| ++(-\dy,\fy*\dy);
\coordinate (madelung1991C) at ($(madelung1991.west)+(\dxStart+\dy,0)$);
\node[ ref] (wenzien1995) at ($(madelung1991C |- 0,-4.500000*\dy)$) {\reftext{Wenz95}\cite{wenzien1995} (  -- / -- , 6.52  )};
\draw (wenzien1995.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (persson1997) at ($(wenzien1995.west |- 0,-5.500000*\dy)$) {\reftext{Pers97}\cite{persson1997} (  10.03 , 9.66 / 6.7 , 6.52  )};
\draw (persson1997.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (persson1999) at ($(persson1997.west |- 0,-6.500000*\dy)$) {\reftext{Pers99}\cite{persson1999} (  10.03 , 9.66 / 6.7 , 6.52  )};
\draw (persson1999.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (son2004) at ($(persson1999.west |- 0,-7.500000*\dy)$) {\reftext{Son04}\cite{son2004} (  10.03 , 9.66 / 6.7 , 6.52  )};
\draw (son2004.west) -| ++(-\dy,\fy*\dy);
\node[no4H, ref] (harris1995) at ($(madelung1991.west |- 0,-8.500000*\dy)$) {\reftext{Harr95}\cite{harris1995} (  10.3 , 9.66 / 6.7 , 6.52  )};
\draw (harris1995.west) -| ++(-\dy,\fy*\dy);
\coordinate (harris1995C) at ($(harris1995.west)+(\dxStart+\dy,0)$);
\node[ ref] (neudeck2001) at ($(harris1995C |- 0,-9.500000*\dy)$) {\reftext{Neud01}\cite{neudeck2001} (  9.7 / --  )};
\draw (neudeck2001.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (choi2005) at ($(neudeck2001.west |- 0,-10.500000*\dy)$) {\reftext{Choi05}\cite{choi2005} (  9.7 / --  )};
\draw (choi2005.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (neudeck2006) at ($(choi2005.west |- 0,-11.500000*\dy)$) {\reftext{Neud06}\cite{neudeck2006} (  9.7 / --  )};
\draw (neudeck2006.west) -| ++(-\dy,\fy*\dy);
\coordinate (neudeck2006C) at ($(neudeck2006.west)+(\dxStart+\dy,0)$);
\node[ ref] (zhu2008) at ($(neudeck2006C |- 0,-12.500000*\dy)$) {\reftext{Zhu08}\cite{zhu2008} (  9.7 / --  )};
\draw (zhu2008.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (wijesundara2011) at ($(zhu2008.west |- 0,-13.500000*\dy)$) {\reftext{Wije11}\cite{wijesundara2011} (  10 / --  )};
\draw (wijesundara2011.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (arvinte2017) at ($(wijesundara2011.west |- 0,-14.500000*\dy)$) {\reftext{Arvi17}\cite{arvinte2017} (  9.7 / 6.52  )};
\draw (arvinte2017.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (pezzimenti2008) at ($(neudeck2006.west |- 0,-15.500000*\dy)$) {\reftext{Pezz08}\cite{pezzimenti2008} (  9.66 / --  )};
\draw (pezzimenti2008.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (pearton2023) at ($(pezzimenti2008.west |- 0,-16.500000*\dy)$) {\reftext{Pear23}\cite{pearton2023} (  9.7 / --  )};
\draw (pearton2023.west) -| ++(-\dy,\fy*\dy);
\node[no4H, ref] (casady1996) at ($(harris1995.west |- 0,-17.500000*\dy)$) {\reftext{Casa96}\cite{casady1996} (  9.66 / --  )};
\draw (casady1996.west) -| ++(-\dy,\fy*\dy);
\coordinate (casady1996C) at ($(casady1996.west)+(\dxStart+\dy,0)$);
\node[ ref] (huang1998) at ($(casady1996C |- 0,-18.500000*\dy)$) {\reftext{Huan98}\cite{huang1998} (  9.7 / --  )};
\draw (huang1998.west) -| ++(-\dy,\fy*\dy);
\node[no4H, ref] (madelung1996) at ($(casady1996.west |- 0,-19.500000*\dy)$) {\reftext{Made96}\cite{madelung1996} (  10.03 , 9.66 / 6.7 , 6.52  )};
\draw (madelung1996.west) -| ++(-\dy,\fy*\dy);
\coordinate (madelung1996C) at ($(madelung1996.west)+(\dxStart+\dy,0)$);
\node[ ref] (lindefelt1998) at ($(madelung1996C |- 0,-20.500000*\dy)$) {\reftext{Lind98}\cite{lindefelt1998} (  10.03 , 9.66 / --  )};
\draw (lindefelt1998.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (bakowski1997) at ($(madelung1996.west |- 0,-21.500000*\dy)$) {\reftext{Bako97}\cite{bakowski1997} (  10.03 , 9.66 / --  )};
\draw (bakowski1997.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (egilsson1999) at ($(bakowski1997.west |- 0,-22.500000*\dy)$) {\reftext{Egil99}\cite{egilsson1999} (  9.7 / --  )};
\draw (egilsson1999.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (ladesmartin2000) at ($(egilsson1999.west |- 0,-23.500000*\dy)$) {\reftext{Lade00}\cite{ladesmartin2000} (  10.03 , 9.66 / --  )};
\draw (ladesmartin2000.west) -| ++(-\dy,\fy*\dy);
\coordinate (ladesmartin2000C) at ($(ladesmartin2000.west)+(\dxStart+\dy,0)$);
\node[ ref] (lechner2021) at ($(ladesmartin2000C |- 0,-24.500000*\dy)$) {\reftext{Lech21}\cite{lechner2021} (  9.66 / --  )};
\draw (lechner2021.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (pernot2001) at ($(ladesmartin2000.west |- 0,-25.500000*\dy)$) {\reftext{Pern01}\cite{pernot2001} (  9.78 / 6.58  )};
\draw (pernot2001.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (pernot2005) at ($(pernot2001.west |- 0,-26.500000*\dy)$) {\reftext{Pern05}\cite{pernot2005} (  9.78 / 6.58  )};
\draw (pernot2005.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (arpatzanis2006) at ($(pernot2005.west |- 0,-27.500000*\dy)$) {\reftext{Arpa06}\cite{arpatzanis2006} (  10 / --  )};
\draw (arpatzanis2006.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (koizumi2009) at ($(arpatzanis2006.west |- 0,-28.500000*\dy)$) {\reftext{Koiz09}\cite{koizumi2009} (  10.03 , 9.66 / 6.7 , 6.52  )};
\draw (koizumi2009.west) -| ++(-\dy,\fy*\dy);
\coordinate (koizumi2009C) at ($(koizumi2009.west)+(\dxStart+\dy,0)$);
\node[ ref] (scaburri2011a) at ($(koizumi2009C |- 0,-29.500000*\dy)$) {\reftext{Scab11a}\cite{scaburri2011a} (  9.78 / --  )};
\draw (scaburri2011a.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (hatakeyama2013) at ($(koizumi2009.west |- 0,-30.500000*\dy)$) {\reftext{Hata13}\cite{hatakeyama2013} (  10.03 , 9.66 / --  )};
\draw (hatakeyama2013.west) -| ++(-\dy,\fy*\dy);
\coordinate (hatakeyama2013C) at ($(hatakeyama2013.west)+(\dxStart+\dy,0)$);
\node[ ref] (naugarhiya2017) at ($(hatakeyama2013C |- 0,-31.500000*\dy)$) {\reftext{Naug17}\cite{naugarhiya2017} (  10.03 , 9.66 / --  )};
\draw (naugarhiya2017.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (arvanitopoulos2017) at ($(hatakeyama2013.west |- 0,-32.500000*\dy)$) {\reftext{Arva17}\cite{arvanitopoulos2017} (  9.66 / --  )};
\draw (arvanitopoulos2017.west) -| ++(-\dy,\fy*\dy);
\coordinate (arvanitopoulos2017C) at ($(arvanitopoulos2017.west)+(\dxStart+\dy,0)$);
\node[ ref] (choudhary2021) at ($(arvanitopoulos2017C |- 0,-33.500000*\dy)$) {\reftext{Chou21}\cite{choudhary2021} (  9.66 / --  )};
\draw (choudhary2021.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (yoshioka2018) at ($(arvanitopoulos2017.west |- 0,-34.500000*\dy)$) {\reftext{Yosh18}\cite{yoshioka2018} (  -- , 9.7 / --  )};
\draw (yoshioka2018.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (miccoli2019) at ($(yoshioka2018.west |- 0,-35.500000*\dy)$) {\reftext{Micc19}\cite{miccoli2019} (  9.66 / --  )};
\draw (miccoli2019.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (tripathi2019) at ($(miccoli2019.west |- 0,-36.500000*\dy)$) {\reftext{Trip19}\cite{tripathi2019} (  9.66 / --  )};
\draw (tripathi2019.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (klahold2020) at ($(tripathi2019.west |- 0,-37.500000*\dy)$) {\reftext{Klah20}\cite{klahold2020} (  10 / --  )};
\draw (klahold2020.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (kovalchuk2020) at ($(klahold2020.west |- 0,-38.500000*\dy)$) {\reftext{Kova20}\cite{kovalchuk2020} (  9.67 / 6.5  )};
\draw (kovalchuk2020.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (zatko2021) at ($(kovalchuk2020.west |- 0,-39.500000*\dy)$) {\reftext{Zatk21}\cite{zatko2021} (  9.66 / --  )};
\draw (zatko2021.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (ioffe2023) at ($(zatko2021.west |- 0,-40.500000*\dy)$) {\reftext{Ioff23}\cite{ioffe2023} (  10.03 , 9.66 / 6.7 , 6.52  )};
\draw (ioffe2023.west) -| ++(-\dy,\fy*\dy);
\coordinate (ioffe2023C) at ($(ioffe2023.west)+(\dxStart+\dy,0)$);
\node[ ref] (acharyya2017) at ($(ioffe2023C |- 0,-41.500000*\dy)$) {\reftext{Acha17}\cite{acharyya2017} (  8.5884 / --  )};
\draw (acharyya2017.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (banerjee2021) at ($(acharyya2017.west |- 0,-42.500000*\dy)$) {\reftext{Bane21}\cite{banerjee2021} (  8.5884 / --  )};
\draw (banerjee2021.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (kim2024) at ($(ioffe2023.west |- 0,-43.500000*\dy)$) {\reftext{Kim24}\cite{kim2024} (  9.7 / 6.52  )};
\draw (kim2024.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-45.500000*\dy) {\citeauthor{bhatnagar1993}};
\node[no4H, ref] (bhatnagar1993) at (0,-46.500000*\dy) {\reftext{Bhat93}\cite{bhatnagar1993} (  9.7 / --  )};
\coordinate (bhatnagar1993C) at ($(bhatnagar1993.west)+(\dxStart+\dy,0)$);
\node[ ref] (codreanu2000) at ($(bhatnagar1993C |- 0,-47.500000*\dy)$) {\reftext{Codr00}\cite{codreanu2000} (  9.7 / --  )};
\draw (codreanu2000.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-49.500000*\dy) {\citeauthor{chow1993}};
\node[ ref] (chow1993) at (0,-50.500000*\dy) {\reftext{Chow93}\cite{chow1993} (  9.945 / --  )};
\coordinate (chow1993C) at ($(chow1993.west)+(\dxStart+\dy,0)$);
\node[ ref] (weitzel1996) at ($(chow1993C |- 0,-51.500000*\dy)$) {\reftext{Weit96}\cite{weitzel1996} (  9.7 / --  )};
\draw (weitzel1996.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,0.000000*\dy) {\citeauthor{chen1994}};
\node[fund, ref] (chen1994) at (\xSepOne,-1.000000*\dy) {\reftext{Chen94}\cite{chen1994} (  -- / 7.20 , 6.96  )};
\coordinate (chen1994C) at ($(chen1994.west)+(\dxStart+\dy,0)$);
\node[ ref] (bechstedt1997) at ($(chen1994C |- 0,-2.000000*\dy)$) {\reftext{Bech97}\cite{bechstedt1997} (  -- / 7.2 , 6.96  )};
\draw (bechstedt1997.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-4.000000*\dy) {\citeauthor{morkoc1994}};
\node[no4H, ref] (morkoc1994) at (\xSepOne,-5.000000*\dy) {\reftext{Mork94}\cite{morkoc1994} (  9.7 / --  )};
\coordinate (morkoc1994C) at ($(morkoc1994.west)+(\dxStart+\dy,0)$);
\node[ ref] (burk1999) at ($(morkoc1994C |- 0,-6.000000*\dy)$) {\reftext{Burk99}\cite{burk1999} (  9.7 / --  )};
\draw (burk1999.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-8.000000*\dy) {\citeauthor{ninomiya1994}};
\node[no4H, ref] (ninomiya1994) at (\xSepOne,-9.000000*\dy) {\reftext{Nino94}\cite{ninomiya1994} (  9.98 , 9.76 / 6.67 , 6.59  )};
\coordinate (ninomiya1994C) at ($(ninomiya1994.west)+(\dxStart+\dy,0)$);
\node[ ref] (ayalew2004) at ($(ninomiya1994C |- 0,-10.000000*\dy)$) {\reftext{Ayal04}\cite{ayalew2004} (  9.98 , 9.76 / --  )};
\draw (ayalew2004.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (kimoto2019) at ($(ayalew2004.west |- 0,-11.000000*\dy)$) {\reftext{Kimo19}\cite{kimoto2019} (  10.32 , 9.76 / --  )};
\draw (kimoto2019.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-13.000000*\dy) {\citeauthor{harima1995}};
\node[fund, ref] (harima1995) at (\xSepOne,-14.000000*\dy) {\reftext{Hari95}\cite{harima1995} (  -- / 6.78 , 6.56  )};
\coordinate (harima1995C) at ($(harima1995.west)+(\dxStart+\dy,0)$);
\node[ ref] (harima1998) at ($(harima1995C |- 0,-15.000000*\dy)$) {\reftext{Hari98}\cite{harima1998} (  -- / 6.8  )};
\draw (harima1998.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-17.000000*\dy) {\citeauthor{sriram1997}};
\node[ ref] (sriram1997) at (\xSepOne,-18.000000*\dy) {\reftext{Srir97}\cite{sriram1997} (  9.7 / --  )};
\coordinate (sriram1997C) at ($(sriram1997.west)+(\dxStart+\dy,0)$);
\node[ ref] (han2003) at ($(sriram1997C |- 0,-19.000000*\dy)$) {\reftext{Han03}\cite{han2003} (  9.7 / --  )};
\draw (han2003.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-21.000000*\dy) {\citeauthor{mickevicius1998}};
\node[ ref] (mickevicius1998) at (\xSepOne,-22.000000*\dy) {\reftext{Mick98}\cite{mickevicius1998} (  9.7 / 6.5  )};
\coordinate (mickevicius1998C) at ($(mickevicius1998.west)+(\dxStart+\dy,0)$);
\node[ ref] (zhao2000) at ($(mickevicius1998C |- 0,-23.000000*\dy)$) {\reftext{Zhao00}\cite{zhao2000} (  9.7 / 6.5  )};
\draw (zhao2000.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (akturk2009) at ($(zhao2000.west |- 0,-24.000000*\dy)$) {\reftext{Aktu09}\cite{akturk2009} (  9.7 / 6.5  )};
\draw (akturk2009.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-26.000000*\dy) {\citeauthor{troffer1998}};
\node[ ref] (troffer1998) at (\xSepOne,-27.000000*\dy) {\reftext{Trof98}\cite{troffer1998} (  10.32 , 9.76 / --  )};
\coordinate (troffer1998C) at ($(troffer1998.west)+(\dxStart+\dy,0)$);
\node[ ref] (zippelius2011) at ($(troffer1998C |- 0,-28.000000*\dy)$) {\reftext{Zipp11}\cite{zippelius2011} (  9.76 / --  )};
\draw (zippelius2011.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-30.000000*\dy) {\citeauthor{weitzel1998}};
\node[ ref] (weitzel1998) at (\xSepOne,-31.000000*\dy) {\reftext{Weit98}\cite{weitzel1998} (  9.7 / --  )};
\coordinate (weitzel1998C) at ($(weitzel1998.west)+(\dxStart+\dy,0)$);
\node[ ref] (nava2008) at ($(weitzel1998C |- 0,-32.000000*\dy)$) {\reftext{Nava08}\cite{nava2008} (  9.7 / --  )};
\draw (nava2008.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-34.000000*\dy) {\citeauthor{wright1998}};
\node[ ref] (wright1998) at (\xSepOne,-35.000000*\dy) {\reftext{Wrig98}\cite{wright1998} (  9.7 / --  )};
\coordinate (wright1998C) at ($(wright1998.west)+(\dxStart+\dy,0)$);
\node[ ref] (baliga2006) at ($(wright1998C |- 0,-36.000000*\dy)$) {\reftext{Bali06}\cite{baliga2006} (  9.7 / --  )};
\draw (baliga2006.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (baliga2019) at ($(baliga2006.west |- 0,-37.000000*\dy)$) {\reftext{Bali19}\cite{baliga2019} (  9.7 / --  )};
\draw (baliga2019.west) -| ++(-\dy,\fy*\dy);
\coordinate (baliga2019C) at ($(baliga2019.west)+(\dxStart+\dy,0)$);
\node[ ref] (tsao2018) at ($(baliga2019C |- 0,-38.000000*\dy)$) {\reftext{Tsao18}\cite{tsao2018} (  9.7 / --  )};
\draw (tsao2018.west) -| ++(-\dy,\fy*\dy);
\coordinate (tsao2018C) at ($(tsao2018.west)+(\dxStart+\dy,0)$);
\node[ ref] (jiya2020) at ($(tsao2018C |- 0,-39.000000*\dy)$) {\reftext{Jiya20}\cite{jiya2020} (  9.7 / --  )};
\draw (jiya2020.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-41.000000*\dy) {\citeauthor{nilsson1999}};
\node[ ref] (nilsson1999) at (\xSepOne,-42.000000*\dy) {\reftext{Nils99}\cite{nilsson1999} (  -- / --  )};
\coordinate (nilsson1999C) at ($(nilsson1999.west)+(\dxStart+\dy,0)$);
\node[ ref] (bellotti1999) at ($(nilsson1999C |- 0,-43.000000*\dy)$) {\reftext{Bell99}\cite{bellotti1999} (  10 / 6.7  )};
\draw (bellotti1999.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (bellotti2000) at ($(bellotti1999.west |- 0,-44.000000*\dy)$) {\reftext{Bell00}\cite{bellotti2000} (  10 / 6.7  )};
\draw (bellotti2000.west) -| ++(-\dy,\fy*\dy);
\coordinate (bellotti2000C) at ($(bellotti2000.west)+(\dxStart+\dy,0)$);
\node[ ref] (vasconcelos2019) at ($(bellotti2000C |- 0,-45.000000*\dy)$) {\reftext{Vasc19}\cite{vasconcelos2019} (  10 / 6.7  )};
\draw (vasconcelos2019.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (rodrigues2021) at ($(vasconcelos2019.west |- 0,-46.000000*\dy)$) {\reftext{Rodr21}\cite{rodrigues2021} (  10 / 6.7  )};
\draw (rodrigues2021.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-48.000000*\dy) {\citeauthor{chow2000}};
\node[ ref] (chow2000) at (\xSepOne,-49.000000*\dy) {\reftext{Chow00}\cite{chow2000} (  10 / --  )};
\coordinate (chow2000C) at ($(chow2000.west)+(\dxStart+\dy,0)$);
\node[ ref] (dhanaraj2010) at ($(chow2000C |- 0,-50.000000*\dy)$) {\reftext{Dhan10}\cite{dhanaraj2010} (  10 / --  )};
\draw (dhanaraj2010.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-52.000000*\dy) {\citeauthor{elasser2002}};
\node[ ref] (elasser2002) at (\xSepOne,-53.000000*\dy) {\reftext{Elas02}\cite{elasser2002} (  10 / --  )};
\coordinate (elasser2002C) at ($(elasser2002.west)+(\dxStart+\dy,0)$);
\node[ ref] (su2010) at ($(elasser2002C |- 0,-54.000000*\dy)$) {\reftext{Su10}\cite{su2010} (  10 / --  )};
\draw (su2010.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,0.000000*\dy) {\citeauthor{zetterling2002}};
\node[ ref] (zetterling2002) at (\xSepOne + \xSepTwo,-1.000000*\dy) {\reftext{Zett02}\cite{zetterling2002} (  10 / --  )};
\coordinate (zetterling2002C) at ($(zetterling2002.west)+(\dxStart+\dy,0)$);
\node[ ref] (ostling2011) at ($(zetterling2002C |- 0,-2.000000*\dy)$) {\reftext{Ostl11}\cite{ostling2011} (  10 / --  )};
\draw (ostling2011.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-4.000000*\dy) {\citeauthor{hjelm2003}};
\node[ ref] (hjelm2003) at (\xSepOne + \xSepTwo,-5.000000*\dy) {\reftext{Hjel03}\cite{hjelm2003} (  9.7 / 6.5  )};
\coordinate (hjelm2003C) at ($(hjelm2003.west)+(\dxStart+\dy,0)$);
\node[ ref] (kovalchuk2020) at ($(hjelm2003C |- 0,-6.000000*\dy)$) {\reftext{Kova20}\cite{kovalchuk2020} (  9.67 / 6.5  )};
\draw (kovalchuk2020.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-8.000000*\dy) {\citeauthor{agarwal2004}};
\node[no4H, ref] (agarwal2004) at (\xSepOne + \xSepTwo,-9.000000*\dy) {\reftext{Agar04}\cite{agarwal2004} (  10.007 / --  )};
\coordinate (agarwal2004C) at ($(agarwal2004.west)+(\dxStart+\dy,0)$);
\node[ ref] (ozpineci2004) at ($(agarwal2004C |- 0,-10.000000*\dy)$) {\reftext{Ozpi04}\cite{ozpineci2004} (  10.1 / --  )};
\draw (ozpineci2004.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-12.000000*\dy) {\citeauthor{ivanov2006}};
\node[fund, ref] (ivanov2006) at (\xSepOne + \xSepTwo,-13.000000*\dy) {\reftext{Ivan06}\cite{ivanov2006} (  9.93 / --  )};
\coordinate (ivanov2006C) at ($(ivanov2006.west)+(\dxStart+\dy,0)$);
\node[ ref] (janzen2008) at ($(ivanov2006C |- 0,-14.000000*\dy)$) {\reftext{Janz08}\cite{janzen2008} (  10.36 , 9.55 / --  )};
\draw (janzen2008.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-16.000000*\dy) {\citeauthor{kaminski2009}};
\node[ ref] (kaminski2009) at (\xSepOne + \xSepTwo,-17.000000*\dy) {\reftext{Kami09}\cite{kaminski2009} (  9.7 / --  )};
\coordinate (kaminski2009C) at ($(kaminski2009.west)+(\dxStart+\dy,0)$);
\node[ ref] (kaminski2014) at ($(kaminski2009C |- 0,-18.000000*\dy)$) {\reftext{Kami14}\cite{kaminski2014} (  9.7 / --  )};
\draw (kaminski2014.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-20.000000*\dy) {\citeauthor{buttay2011}};
\node[ ref] (buttay2011) at (\xSepOne + \xSepTwo,-21.000000*\dy) {\reftext{Butt11}\cite{buttay2011} (  10 / --  )};
\coordinate (buttay2011C) at ($(buttay2011.west)+(\dxStart+\dy,0)$);
\node[ ref] (fujita2015) at ($(buttay2011C |- 0,-22.000000*\dy)$) {\reftext{Fuji15}\cite{fujita2015} (  10 / --  )};
\draw (fujita2015.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-24.000000*\dy) {\citeauthor{neudeck2013}};
\node[ ref] (neudeck2013) at (\xSepOne + \xSepTwo,-25.000000*\dy) {\reftext{Neud13}\cite{neudeck2013} (  9.7 / --  )};
\coordinate (neudeck2013C) at ($(neudeck2013.west)+(\dxStart+\dy,0)$);
\node[ ref] (hassan2018) at ($(neudeck2013C |- 0,-26.000000*\dy)$) {\reftext{Hass18}\cite{hassan2018} (  9.7 / --  )};
\draw (hassan2018.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-28.000000*\dy) {\citeauthor{higashiwaki2014}};
\node[ ref] (higashiwaki2014) at (\xSepOne + \xSepTwo,-29.000000*\dy) {\reftext{Higa14}\cite{higashiwaki2014} (  9.7 / --  )};
\coordinate (higashiwaki2014C) at ($(higashiwaki2014.west)+(\dxStart+\dy,0)$);
\node[ ref] (liu2015) at ($(higashiwaki2014C |- 0,-30.000000*\dy)$) {\reftext{Liu15}\cite{liu2015} (  9.7 / --  )};
\draw (liu2015.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (zheng2020) at ($(liu2015.west |- 0,-31.000000*\dy)$) {\reftext{Zhen20}\cite{zheng2020} (  9.7 / --  )};
\draw (zheng2020.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-33.000000*\dy) {\citeauthor{kimoto2014a}};
\node[ ref] (kimoto2014a) at (\xSepOne + \xSepTwo,-34.000000*\dy) {\reftext{Kimo14a}\cite{kimoto2014a} (  10.32 , 9.76 / --  )};
\coordinate (kimoto2014aC) at ($(kimoto2014a.west)+(\dxStart+\dy,0)$);
\node[ ref] (elahipanah2017) at ($(kimoto2014aC |- 0,-35.000000*\dy)$) {\reftext{Elah17}\cite{elahipanah2017} (  10 / --  )};
\draw (elahipanah2017.west) -| ++(-\dy,\fy*\dy);
\coordinate (elahipanah2017C) at ($(elahipanah2017.west)+(\dxStart+\dy,0)$);
\node[ ref] (ostling2024) at ($(elahipanah2017C |- 0,-36.000000*\dy)$) {\reftext{Ostl24}\cite{ostling2024} (  10 / --  )};
\draw (ostling2024.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (rybalka2017) at ($(elahipanah2017.west |- 0,-37.000000*\dy)$) {\reftext{Ryba17}\cite{rybalka2017} (  9.7 / --  )};
\draw (rybalka2017.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (tanaka2018) at ($(rybalka2017.west |- 0,-38.000000*\dy)$) {\reftext{Tana18}\cite{tanaka2018} (  9.95 / --  )};
\draw (tanaka2018.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (darmody2019) at ($(tanaka2018.west |- 0,-39.000000*\dy)$) {\reftext{Darm19}\cite{darmody2019} (  9.76 / --  )};
\draw (darmody2019.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-41.000000*\dy) {\citeauthor{coutinho2017}};
\node[fund, ref] (coutinho2017) at (\xSepOne + \xSepTwo,-42.000000*\dy) {\reftext{Cout17}\cite{coutinho2017} (  10.65 , 9.88 / --  )};
\coordinate (coutinho2017C) at ($(coutinho2017.west)+(\dxStart+\dy,0)$);
\node[ ref] (torres2022) at ($(coutinho2017C |- 0,-43.000000*\dy)$) {\reftext{Torr22}\cite{torres2022} (  10.65 , 9.88 / --  )};
\draw (torres2022.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-45.000000*\dy) {\citeauthor{pearton2018}};
\node[ ref] (pearton2018) at (\xSepOne + \xSepTwo,-46.000000*\dy) {\reftext{Pear18}\cite{pearton2018} (  9.7 / --  )};
\coordinate (pearton2018C) at ($(pearton2018.west)+(\dxStart+\dy,0)$);
\node[ ref] (soler2019) at ($(pearton2018C |- 0,-47.000000*\dy)$) {\reftext{Sole19}\cite{soler2019} (  9.7 / --  )};
\draw (soler2019.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (kim2024) at ($(soler2019.west |- 0,-48.000000*\dy)$) {\reftext{Kim24}\cite{kim2024} (  9.7 / 6.52  )};
\draw (kim2024.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-50.000000*\dy) {\citeauthor{li2023}};
\node[fund, ref] (li2023) at (\xSepOne + \xSepTwo,-51.000000*\dy) {\reftext{Li23}\cite{li2023} (  10.27 , -- / --  )};
\coordinate (li2023C) at ($(li2023.west)+(\dxStart+\dy,0)$);
\node[ ref] (li2023a) at ($(li2023C |- 0,-52.000000*\dy)$) {\reftext{Li23a}\cite{li2023a} (  10.27 , -- / --  )};
\draw (li2023a.west) -| ++(-\dy,\fy*\dy);


==> data/regen_figure_auger.tex <==
\addplot+[domain=2e18:2e19, no marks, samples=\samp] {auger(5e-31)};
\addlegendentry{\reftext{Gale97}\cite{galeckas1997} $\cn$: (\num{5e-31})}
\addplot+[domain=2e18:2e19, no marks, samples=\samp] {auger(2e-31)};
\addlegendentry{\reftext{Gale97}\cite{galeckas1997} $\cp$: (\num{2e-31})}
\addplot+[domain=1e19:1e20, no marks, samples=\samp] {auger( 0.8e-31)};
\addlegendentry{\reftext{Scaj10}\cite{scajev2010} $C$: (\num{ 0.8e-31})}
\addplot+[domain=1e18:1e20, no marks, samples=\samp] {auger(scajev(5e-31,3.5e-9,7.8e16,300))};
\addlegendentry{\reftext{Scaj13}\cite{scajev2013} Eq. (\ref{eq:regen_auger_temp_indepth})}
\addplot+[domain=3e17:7e18, no marks, samples=\samp] {auger(1.6e-30)};
\addlegendentry{\reftext{Tawa16}\cite{tawara2016} $\cn$: (\num{1.6e-30})}
\addplot+[domain=1e18:1e20, no marks, samples=\samp] {auger(lophitis(6.7e-32, 2.45e-31, -2.2e-32, 300, 300, 3.47, 1e18))};
\addlegendentry{\reftext{Loph18}\cite{lophitis2018} Eq. (\ref{eq:regen_auger_temp_Si})}
\addplot+[domain=1e18:1e20, no marks, samples=\samp] {tanaka(7.4e-19)};
\addlegendentry{\reftext{Tana23}\cite{tanaka2023} \num{7.4e-19} $\DN^{-0.68}$}


==> data/regen_figure_bimolecular.tex <==
\addplot+[domain=1e16:1e19, no marks, samples=\samp] {bimolecular(1.50E-12)};
\addlegendentry{\reftext{Gale97}\cite{galeckas1997} $B$: (\num{1.5e-12})}
\addplot+[domain=1e16:2e19, no marks, samples=\samp] {bimolecular(3e-11)};
\addlegendentry{\reftext{Neim06}\cite{neimontas2006} $B$: (\num{3.0e-11})}
\addplot+[domain=4e14:1e16, no marks, samples=\samp] {bimolecular(1.3e-12)};
\addlegendentry{\reftext{Tawa16}\cite{tawara2016} $B$: (\num{1.3e-12})}
\addplot+[domain=4e14:1e16, no marks, samples=\samp] {bimolecular(0.94e-12)};
\addlegendentry{\reftext{Tawa16}\cite{tawara2016} $B$: (\num{9.4e-13})}


==> data/regen_figure_lifetime_dop_conc.tex <==
\addplot+[only marks, point meta=0, mark size=\mSizeMax]coordinates {(7.00E+14,6.00E-07)};
\addlegendentry{\reftext{Agar01}\cite{agarwal2001} $\taun$}
\addplot+[only marks, point meta=0, mark size=(\mSizeMax+\mSizeMin)/2]coordinates {(2.00E+17,6.60E-08)};
\addlegendentry{\reftext{Ivan06a}\cite{ivanov2006a} $\taun$}
\addplot+[only marks, point meta=0, mark size=(\mSizeMax+\mSizeMin)/2]coordinates {(2.04E+17,8.00E-09)};
\addlegendentry{\reftext{Alba10}\cite{albanese2010} $\taun$}
\addplot+[only marks, point meta=14.176091, mark size=(1-0.298119)*\mSizeMin+0.298119*\mSizeMax]coordinates {(9.00E+14,1.30E-06)};
\addlegendentry{\reftext{Haya11}\cite{hayashi2011} $\taun$}
\addplot+[only marks, point meta=14.176091, mark size=(1-0.298119)*\mSizeMin+0.298119*\mSizeMax]coordinates {(9.00E+14,1.60E-06)};
\addlegendentry{\reftext{Haya11a}\cite{hayashi2011a} $\taun$}
\addplot+[only marks, point meta=15.000000, mark size=(1-0.442690)*\mSizeMin+0.442690*\mSizeMax]coordinates {(5.60E+14,1.70E-06)};
\addlegendentry{\reftext{Haya12}\cite{hayashi2012} $\taun$}
\addplot+[only marks, point meta=15.959041, mark size=(1-0.610974)*\mSizeMin+0.610974*\mSizeMax]coordinates {(1.00E+18,3.10E-07)};
\addlegendentry{\reftext{Okud13a}\cite{okuda2013a} $\taun$}
\addplot+[only marks, point meta=16.556303, mark size=(1-0.715775)*\mSizeMin+0.715775*\mSizeMax]coordinates {(2.00E+14,1.00E-05)};
\addlegendentry{\reftext{Okud14}\cite{okuda2014} $\taun$}
\addplot+[only marks, point meta=0, mark size=\mSizeMax]coordinates {(1.00E+17,2.00E-08)};
\addlegendentry{\reftext{Liau15}\cite{liaugaudas2015} $\taun$}
\addplot+[only marks, point meta=14.556303, mark size=(1-0.364835)*\mSizeMin+0.364835*\mSizeMax]coordinates {(1.00E+15,1.20E-05)};
\addlegendentry{\reftext{Okud16}\cite{okuda2016} $\taun$}
\addplot+[only marks, point meta=0, mark size=(\mSizeMax+\mSizeMin)/2]coordinates {(8.00E+14,4.00E-07)};
\addlegendentry{\reftext{Hase17}\cite{hasegawa2017} $\taun$}
\addplot+[only marks, point meta=0, mark size=\mSizeMin]coordinates {(6.00E+14,1.20E-06)};
\addlegendentry{\reftext{Kato20}\cite{kato2020} $\taun$}
\addplot+[only marks, point meta=0, mark size=(\mSizeMax+\mSizeMin)/2]coordinates {(1.00E+19,1.30E-07)};
\addlegendentry{\reftext{Koya20}\cite{koyama2020} $\taun$}
\addplot+[only marks, point meta=0, mark size=(\mSizeMax+\mSizeMin)/2]coordinates {(2.00E+14,3.14E-06)};
\addlegendentry{\reftext{Zhan23a}\cite{zhang2023a} $\taun$}
\addlegendimage{empty legend}
\addlegendentry{}
\addlegendimage{empty legend}
\addlegendentry{}
\addplot+[only marks, point meta=0, mark size=\mSizeMax]coordinates {(5.00E+15,2.60E-07)};
\addlegendentry{\reftext{Gale97}\cite{galeckas1997} $\taup$}
\addplot+[only marks, point meta=0, mark size=(\mSizeMax+\mSizeMin)/2, error bars/.cd, x dir=both, x explicit]coordinates {(3e+16,7.00E-07) +- (1e+16,0)};
\addlegendentry{\reftext{Neud98}\cite{neudeck1998} $\taup$}
\addplot+[only marks, point meta=0, mark size=(\mSizeMax+\mSizeMin)/2]coordinates {(1e16,5.00E-07)};
\addlegendentry{\reftext{Gale99a}\cite{galeckas1999a} $\taup$}
\addplot+[only marks, point meta=0, mark size=(\mSizeMax+\mSizeMin)/2]coordinates {(5.00E+14,3.30E-07)};
\addlegendentry{\reftext{Kimo99}\cite{kimoto1999} $\taup$}
\addplot+[only marks, point meta=0, mark size=(\mSizeMax+\mSizeMin)/2, error bars/.cd, x dir=both, x explicit]coordinates {(1.75e+15,5.20E-08) +- (8.5e+14,0)};
\addlegendentry{\reftext{Udal00}\cite{udal2000} $\taup$}
\addplot+[only marks, point meta=0, mark size=(\mSizeMax+\mSizeMin)/2, error bars/.cd, x dir=both, x explicit]coordinates {(1.4e+16,1.00E-06) +- (4e+15,0)};
\addlegendentry{\reftext{Cheo03}\cite{cheong2003} $\taup$}
\addplot+[only marks, point meta=0, mark size=\mSizeMax]coordinates {(8.60E+15,3.50E-09)};
\addlegendentry{\reftext{Dome03}\cite{domeij2003} $\taup$}
\addplot+[only marks, point meta=0, mark size=(\mSizeMax+\mSizeMin)/2, error bars/.cd, x dir=both, x explicit]coordinates {(1.005e+16,3.00E-07) +- (9.95e+15,0)};
\addlegendentry{\reftext{Zhan03}\cite{zhang2003} $\taup$}
\addplot+[only marks, point meta=0, mark size=\mSizeMax]coordinates {(3.00E+14,1.55E-06)};
\addlegendentry{\reftext{Levi04}\cite{levinshtein2004} $\taup$}
\addplot+[only marks, point meta=0, mark size=(\mSizeMax+\mSizeMin)/2]coordinates {(7.00E+15,1.00E-06)};
\addlegendentry{\reftext{Resh05}\cite{reshanov2005} $\taup$}
\addplot+[only marks, point meta=13.000000, mark size=(1-0.091750)*\mSizeMin+0.091750*\mSizeMax]coordinates {(1.00E+14,5.00E-07)};
\addlegendentry{\reftext{Huh06}\cite{huh2006} $\taup$}
\addplot+[only marks, point meta=0, mark size=\mSizeMax]coordinates {(2.00E+14,3.70E-06)};
\addlegendentry{\reftext{Ivan06b}\cite{ivanov2006b} $\taup$}
\addplot+[only marks, point meta=0, mark size=(\mSizeMax+\mSizeMin)/2]coordinates {(5.00E+15,1.55E-05)};
\addlegendentry{\reftext{Jenn06}\cite{jenny2006} $\taup$}
\addplot+[only marks, point meta=0, mark size=(\mSizeMax+\mSizeMin)/2]coordinates {(1.00E+16,1.20E-08)};
\addlegendentry{\reftext{Neim06}\cite{neimontas2006} $\taup$}
\addplot+[only marks, point meta=16.801030, mark size=(1-0.758718)*\mSizeMin+0.758718*\mSizeMax]coordinates {(1.50E+15,2.50E-06)};
\addlegendentry{\reftext{Dann07}\cite{danno2007} $\taup$}
\addplot+[only marks, point meta=0, mark size=(\mSizeMax+\mSizeMin)/2]coordinates {(5.00E+15,2.18E-07)};
\addlegendentry{\reftext{Stor07}\cite{storasta2007} $\taup$}
\addplot+[only marks, point meta=0, mark size=(\mSizeMax+\mSizeMin)/2]coordinates {(7.00E+15,4.40E-09)};
\addlegendentry{\reftext{Udal07}\cite{udal2007} $\taup$}
\addplot+[only marks, point meta=12.698970, mark size=(1-0.038928)*\mSizeMin+0.038928*\mSizeMax, error bars/.cd, x dir=both, x explicit]coordinates {(1.5e+15,8.60E-06) +- (5e+14,0)};
\addlegendentry{\reftext{Kimo08}\cite{kimoto2008} $\taup$}
\addplot+[only marks, point meta=0, mark size=(\mSizeMax+\mSizeMin)/2]coordinates {(1.00E+14,9.90E-07)};
\addlegendentry{\reftext{Stor08}\cite{storasta2008} $\taup$}
\addplot+[only marks, point meta=16.801030, mark size=(1-0.758718)*\mSizeMin+0.758718*\mSizeMax, error bars/.cd, x dir=both, x explicit]coordinates {(3e+15,1.62E-06) +- (2e+15,0)};
\addlegendentry{\reftext{Hiyo09}\cite{hiyoshi2009} $\taup$}
\addplot+[only marks, point meta=0, mark size=\mSizeMax, error bars/.cd, x dir=both, x explicit]coordinates {(1.1e+15,2.13E-06) +- (1e+14,0)};
\addlegendentry{\reftext{Resh09}\cite{reshanov2009} $\taup$}
\addplot+[only marks, point meta=18.000000, mark size=(1-0.969101)*\mSizeMin+0.969101*\mSizeMax]coordinates {(4.00E+14,8.00E-07)};
\addlegendentry{\reftext{Jara10}\cite{jarasiunas2010} $\taup$}
\addplot+[only marks, point meta=16.198970, mark size=(1-0.653074)*\mSizeMin+0.653074*\mSizeMax, error bars/.cd, x dir=both, x explicit]coordinates {(9.5e+14,9.50E-06) +- (5e+13,0)};
\addlegendentry{\reftext{Kimo10}\cite{kimoto2010} $\taup$}
\addplot+[only marks, point meta=16.198970, mark size=(1-0.653074)*\mSizeMin+0.653074*\mSizeMax]coordinates {(7.00E+14,1.31E-05)};
\addlegendentry{\reftext{Kimo10a}\cite{kimoto2010a} $\taup$}
\addplot+[only marks, point meta=12.477121, mark size=(1-0.000000)*\mSizeMin+0.000000*\mSizeMax]coordinates {(7.00E+13,1.85E-05)};
\addlegendentry{\reftext{Miya10}\cite{miyazawa2010} $\taup$}
\addplot+[only marks, point meta=14.176091, mark size=(1-0.298119)*\mSizeMin+0.298119*\mSizeMax]coordinates {(1.20E+15,4.60E-06)};
\addlegendentry{\reftext{Haya11a}\cite{hayashi2011a} $\taup$}
\addplot+[only marks, point meta=0, mark size=(\mSizeMax+\mSizeMin)/2]coordinates {(1.00E+16,2.40E-07)};
\addlegendentry{\reftext{Donn12}\cite{donnarumma2012} $\taup$}
\addplot+[only marks, point meta=15.500000, mark size=(1-0.530425)*\mSizeMin+0.530425*\mSizeMax, error bars/.cd, x dir=both, x explicit]coordinates {(5.5e+14,3.32E-05) +- (2.5e+14,0)};
\addlegendentry{\reftext{Ichi12}\cite{ichikawa2012} $\taup$}
\addplot+[only marks, point meta=16.000000, mark size=(1-0.618161)*\mSizeMin+0.618161*\mSizeMax]coordinates {(1.00E+16,6.50E-06)};
\addlegendentry{\reftext{Kawa12}\cite{kawahara2012} $\taup$}
\addplot+[only marks, point meta=0, mark size=\mSizeMin]coordinates {(3.00E+15,1.60E-06)};
\addlegendentry{\reftext{Lilj13}\cite{lilja2013} $\taup$}
\addplot+[only marks, point meta=0, mark size=(\mSizeMax+\mSizeMin)/2, error bars/.cd, x dir=both, x explicit]coordinates {(2.5e+14,1.30E-05) +- (5e+13,0)};
\addlegendentry{\reftext{Miya13}\cite{miyazawa2013} $\taup$}
\addplot+[only marks, point meta=0, mark size=\mSizeMin]coordinates {(4.00E+14,5.50E-07)};
\addlegendentry{\reftext{Scaj13}\cite{scajev2013} $\taup$}
\addplot+[only marks, point meta=0, mark size=(\mSizeMax+\mSizeMin)/2]coordinates {(2.00E+14,1.30E-06)};
\addlegendentry{\reftext{Usma14}\cite{usman2014} $\taup$}
\addplot+[only marks, point meta=0, mark size=\mSizeMax]coordinates {(2.50E+14,2.50E-06)};
\addlegendentry{\reftext{Chow15}\cite{chowdhury2015} $\taup$}
\addplot+[only marks, point meta=14.000000, mark size=(1-0.267220)*\mSizeMin+0.267220*\mSizeMax]coordinates {(2.00E+14,2.16E-05)};
\addlegendentry{\reftext{Kaji15}\cite{kaji2015} $\taup$}
\addplot+[only marks, point meta=17.778151, mark size=(1-0.930173)*\mSizeMin+0.930173*\mSizeMax]coordinates {(8.00E+15,3.50E-07)};
\addlegendentry{\reftext{Suva15}\cite{suvanam2015} $\taup$}
\addplot+[only marks, point meta=0, mark size=(\mSizeMax+\mSizeMin)/2]coordinates {(3.00E+15,1.00E-06)};
\addlegendentry{\reftext{Puzz16}\cite{puzzanghera2016} $\taup$}
\addplot+[only marks, point meta=17.255273, mark size=(1-0.838424)*\mSizeMin+0.838424*\mSizeMax]coordinates {(1.00E+14,2.60E-05)};
\addlegendentry{\reftext{Sait16}\cite{saito2016} $\taup$}
\addplot+[only marks, point meta=0, mark size=(\mSizeMax+\mSizeMin)/2]coordinates {(1.50E+15,22.5e-9)};
\addlegendentry{\reftext{Stre16}\cite{strelchuk2016} $\taup$}
\addplot+[only marks, point meta=0, mark size=\mSizeMin]coordinates {(7.70E+17,3.00E-07)};
\addlegendentry{\reftext{Tawa16}\cite{tawara2016} $\taup$}
\addplot+[only marks, point meta=0, mark size=(\mSizeMax+\mSizeMin)/2]coordinates {(1.40E+14,2.60E-06)};
\addlegendentry{\reftext{Tsuc16}\cite{tsuchida2016} $\taup$}
\addplot+[only marks, point meta=0, mark size=(\mSizeMax+\mSizeMin)/2]coordinates {(1.00E+15,2.00E-05)};
\addlegendentry{\reftext{Ayed17}\cite{ayedh2017} $\taup$}
\addplot+[only marks, point meta=0, mark size=\mSizeMin]coordinates {(1.30E+15,3.50E-06)};
\addlegendentry{\reftext{Lilj17}\cite{lilja2017} $\taup$}
\addplot+[only marks, point meta=0, mark size=(\mSizeMax+\mSizeMin)/2]coordinates {(9.10E+18,11e-9)};
\addlegendentry{\reftext{Fang18}\cite{fang2018} $\taup$}
\addplot+[only marks, point meta=14.500000, mark size=(1-0.354955)*\mSizeMin+0.354955*\mSizeMax]coordinates {(1.00E+14,1.10E-04)};
\addlegendentry{\reftext{Kimo18}\cite{kimoto2018} $\taup$}
\addplot+[only marks, point meta=16.602060, mark size=(1-0.723804)*\mSizeMin+0.723804*\mSizeMax]coordinates {(2.00E+13,1.05E-06)};
\addlegendentry{\reftext{Cui19}\cite{cui2019} $\taup$}
\addplot+[only marks, point meta=0, mark size=\mSizeMin]coordinates {(1.00E+15,9.90E-06)};
\addlegendentry{\reftext{Mura19}\cite{murata2019} $\taup$}
\addplot+[only marks, point meta=0, mark size=\mSizeMin, error bars/.cd, x dir=both, x explicit]coordinates {(5.5e+15,7.00E-07) +- (4.5e+15,0)};
\addlegendentry{\reftext{Kato20}\cite{kato2020} $\taup$}
\addplot+[only marks, point meta=18.176091, mark size=(1-1.000000)*\mSizeMin+1.000000*\mSizeMax]coordinates {(1.00E+18,1.00E-05)};
\addlegendentry{\reftext{Naga20}\cite{nagaya2020} $\taup$}
\addplot+[only marks, point meta=0, mark size=\mSizeMax]coordinates {(1.00E+16,1.90E-05)};
\addlegendentry{\reftext{Sapi20}\cite{sapienza2020} $\taup$}
\addplot+[only marks, point meta=0, mark size=\mSizeMin, error bars/.cd, x dir=both, x explicit]coordinates {(7.5e+14,5.00E-06) +- (2.5e+14,0)};
\addlegendentry{\reftext{Erle21}\cite{erlekampf2021} $\taup$}
\addplot+[only marks, point meta=14.845098, mark size=(1-0.415510)*\mSizeMin+0.415510*\mSizeMax]coordinates {(2.00E+17,1.40E-07)};
\addlegendentry{\reftext{Mura21}\cite{murata2021} $\taup$}
\addplot+[only marks, point meta=17.767774, mark size=(1-0.928352)*\mSizeMin+0.928352*\mSizeMax]coordinates {(5.00E+13,1.63e-5)};
\addlegendentry{\reftext{Meli22a}\cite{meli2022a} $\taup$}
\addplot+[only marks, point meta=16.198970, mark size=(1-0.653074)*\mSizeMin+0.653074*\mSizeMax]coordinates {(1.00E+15,4.50E-06)};
\addlegendentry{\reftext{Kato24}\cite{kato2024} $\taup$}
\addplot+[only marks, point meta=17.602060, mark size=(1-0.899275)*\mSizeMin+0.899275*\mSizeMax]coordinates {(1.50E+14,6.09E-06)};
\addlegendentry{\reftext{Sozz24}\cite{sozzi2024} $\taup$}
\addlegendimage{empty legend}
\addlegendentry{}


==> data/regen_figure_lifetime_level_amount.tex <==
\addplot+[only marks, point meta=14.954243, mark size=(1-0.139012)*\mSizeMin+0.139012*\mSizeMax]coordinates {(1.5e14,1.30E-06)};
\addlegendentry{\reftext{Haya11}\cite{hayashi2011} $\taun$}
\addplot+[only marks, point meta=14.954243, mark size=(1-0.139012)*\mSizeMin+0.139012*\mSizeMax]coordinates {(1.5e14,1.60E-06)};
\addlegendentry{\reftext{Haya11a}\cite{hayashi2011a} $\taun$}
\addplot+[only marks, point meta=14.748188, mark size=(1-0.095161)*\mSizeMin+0.095161*\mSizeMax]coordinates {(1000000000000000,1.70E-06)};
\addlegendentry{\reftext{Haya12}\cite{hayashi2012} $\taun$}
\addplot+[only marks, point meta=18.000000, mark size=(1-0.787187)*\mSizeMin+0.787187*\mSizeMax]coordinates {(9.10000000000000E+15,3.10E-07)};
\addlegendentry{\reftext{Okud13a}\cite{okuda2013a} $\taun$}
\addplot+[only marks, point meta=14.301030, mark size=(1-0.000000)*\mSizeMin+0.000000*\mSizeMax]coordinates {(3.60000000000000E+16,1.00E-05)};
\addlegendentry{\reftext{Okud14}\cite{okuda2014} $\taun$}
\addplot+[only marks, point meta=15.000000, mark size=(1-0.148750)*\mSizeMin+0.148750*\mSizeMax]coordinates {(360000000000000,1.20E-05)};
\addlegendentry{\reftext{Okud16}\cite{okuda2016} $\taun$}
\addlegendimage{empty legend}
\addlegendentry{}
\addlegendimage{empty legend}
\addlegendentry{}
\addplot+[only marks, point meta=14.000000, mark size=(1-0.123536)*\mSizeMin+0.123536*\mSizeMax]coordinates {(1e13,5.00E-07)};
\addlegendentry{\reftext{Huh06}\cite{huh2006} $\taup$}
\addplot+[only marks, point meta=15.176091, mark size=(1-0.331399)*\mSizeMin+0.331399*\mSizeMax, error bars/.cd, x dir=both, x explicit]coordinates {(1.1e+17,2.50E-06) +- (9e+16,0)};
\addlegendentry{\reftext{Dann07}\cite{danno2007} $\taup$}
\addplot+[only marks, point meta=15.150515, mark size=(1-0.326879)*\mSizeMin+0.326879*\mSizeMax]coordinates {(5e12,8.60E-06)};
\addlegendentry{\reftext{Kimo08}\cite{kimoto2008} $\taup$}
\addplot+[only marks, point meta=15.349485, mark size=(1-0.362045)*\mSizeMin+0.362045*\mSizeMax, error bars/.cd, x dir=both, x explicit]coordinates {(1.1e+17,1.62E-06) +- (9e+16,0)};
\addlegendentry{\reftext{Hiyo09}\cite{hiyoshi2009} $\taup$}
\addplot+[only marks, point meta=14.602060, mark size=(1-0.229945)*\mSizeMin+0.229945*\mSizeMax, error bars/.cd, x dir=both, x explicit]coordinates {(5.05e+18,8.00E-07) +- (4.95e+18,0)};
\addlegendentry{\reftext{Jara10}\cite{jarasiunas2010} $\taup$}
\addplot+[only marks, point meta=14.977121, mark size=(1-0.296233)*\mSizeMin+0.296233*\mSizeMax, error bars/.cd, x dir=both, x explicit]coordinates {(2.75e+16,9.50E-06) +- (2.25e+16,0)};
\addlegendentry{\reftext{Kimo10}\cite{kimoto2010} $\taup$}
\addplot+[only marks, point meta=14.845098, mark size=(1-0.272899)*\mSizeMin+0.272899*\mSizeMax, error bars/.cd, x dir=both, x explicit]coordinates {(2.75e+16,1.31E-05) +- (2.25e+16,0)};
\addlegendentry{\reftext{Kimo10a}\cite{kimoto2010a} $\taup$}
\addplot+[only marks, point meta=13.845098, mark size=(1-0.096159)*\mSizeMin+0.096159*\mSizeMax]coordinates {(3e12,1.85E-05)};
\addlegendentry{\reftext{Miya10}\cite{miyazawa2010} $\taup$}
\addplot+[only marks, point meta=15.079181, mark size=(1-0.314271)*\mSizeMin+0.314271*\mSizeMax]coordinates {(1.5e14,4.60E-06)};
\addlegendentry{\reftext{Haya11a}\cite{hayashi2011a} $\taup$}
\addplot+[only marks, point meta=14.690106, mark size=(1-0.245506)*\mSizeMin+0.245506*\mSizeMax, error bars/.cd, x dir=both, x explicit]coordinates {(5.5e+15,3.32E-05) +- (4.5e+15,0)};
\addlegendentry{\reftext{Ichi12}\cite{ichikawa2012} $\taup$}
\addplot+[only marks, point meta=16.000000, mark size=(1-0.477017)*\mSizeMin+0.477017*\mSizeMax]coordinates {(1.00000000000000E+16,6.50E-06)};
\addlegendentry{\reftext{Kawa12}\cite{kawahara2012} $\taup$}
\addplot+[only marks, point meta=14.301030, mark size=(1-0.176741)*\mSizeMin+0.176741*\mSizeMax]coordinates {(100000000000000,2.16E-05)};
\addlegendentry{\reftext{Kaji15}\cite{kaji2015} $\taup$}
\addplot+[only marks, point meta=15.903090, mark size=(1-0.459890)*\mSizeMin+0.459890*\mSizeMax]coordinates {(6.00000000000000E+17,3.50E-07)};
\addlegendentry{\reftext{Suva15}\cite{suvanam2015} $\taup$}
\addplot+[only marks, point meta=14.000000, mark size=(1-0.123536)*\mSizeMin+0.123536*\mSizeMax]coordinates {(1.8e17,2.60E-05)};
\addlegendentry{\reftext{Sait16}\cite{saito2016} $\taup$}
\addplot+[only marks, point meta=14.000000, mark size=(1-0.123536)*\mSizeMin+0.123536*\mSizeMax, error bars/.cd, x dir=both, x explicit]coordinates {(5.5e+14,1.10E-04) +- (4.5e+14,0)};
\addlegendentry{\reftext{Kimo18}\cite{kimoto2018} $\taup$}
\addplot+[only marks, point meta=13.301030, mark size=(1-0.000000)*\mSizeMin+0.000000*\mSizeMax]coordinates {(4.00000000000000E+16,1.05E-06)};
\addlegendentry{\reftext{Cui19}\cite{cui2019} $\taup$}
\addplot+[only marks, point meta=18.000000, mark size=(1-0.830499)*\mSizeMin+0.830499*\mSizeMax]coordinates {(1.50000000000000E+18,1.00E-05)};
\addlegendentry{\reftext{Naga20}\cite{nagaya2020} $\taup$}
\addplot+[only marks, point meta=17.301030, mark size=(1-0.706962)*\mSizeMin+0.706962*\mSizeMax]coordinates {(7e14,1.40E-07)};
\addlegendentry{\reftext{Mura21}\cite{murata2021} $\taup$}
\addplot+[only marks,point meta=13.698970, mark size=(1-0.070332)*\mSizeMin+0.070332*\mSizeMax, error bars/.cd, x dir=both, x explicit,y dir=both, y explicit] table [x=x, y=y, x error=xerror,y error=yerror, col sep=comma] {data/regen_meli2022a.csv};
\addlegendentry{\reftext{Meli22a}\cite{meli2022a} $\taup$}
\addplot+[only marks, point meta=15.000000, mark size=(1-0.300277)*\mSizeMin+0.300277*\mSizeMax, error bars/.cd, x dir=both, x explicit]coordinates {(2.75e+16,4.50E-06) +- (2.25e+16,0)};
\addlegendentry{\reftext{Kato24}\cite{kato2024} $\taup$}
\addplot+[only marks, point meta=14.176091, mark size=(1-0.154659)*\mSizeMin+0.154659*\mSizeMax]coordinates {(4e17,6.09E-06)};
\addlegendentry{\reftext{Sozz24}\cite{sozzi2024} $\taup$}
\addlegendimage{empty legend}
\addlegendentry{}
\addlegendimage{empty legend}
\addlegendentry{}
\addlegendimage{empty legend}
\addlegendentry{}


==> data/regen_figure_lifetime_values.tex <==


\node[symbol] (lte) at (0,0) {$\taun$};
\coordinate (lte0) at (lte.north);
\node[ref, lwlte] (lte1) at (lte0.north west) {\tikz \node[paper] {\reftext{Ioff23}\cite{ioffe2023}}; \tikz \node[paper] {\reftext{Adit15}\cite{aditya2015}};};
\node[value, scale=1.200000] (ltevalue1) at (lte1.west) {\num{1}};
\node[ref, lwlte] (lte2) at (lte1.north west) {\tikz \node[paper] {\reftext{Das15}\cite{das2015}};};
\node[value, scale=1.100000] (ltevalue2) at (lte2.west) {\num{2.5}};
\node[ref, lwlte] (lte3) at (lte2.north west) {\tikz \node[paper] {\reftext{Cha08}\cite{cha2008}};};
\node[value, scale=1.100000] (ltevalue3) at (lte3.west) {\num{5}};
\node[ref, lwlte] (lte4) at (lte3.north west) {\tikz \node[paper] {\reftext{Bell11}\cite{bellone2011}};};
\node[value, scale=1.100000] (ltevalue4) at (lte4.west) {\num{8}};
\node[ref, lwlte] (lte5) at (lte4.north west) {\tikz \node[paper] {\reftext{Megh15}\cite{megherbi2015}};};
\node[value, scale=1.100000] (ltevalue5) at (lte5.west) {\num{10}};
\node[ref, lwlte] (lte6) at (lte5.north west) {\tikz \node[paper] {\reftext{Rao22}\cite{rao2022}}; \tikz \node[paper] {\reftext{Pezz13}\cite{pezzimenti2013}}; \tikz \node[paper] {\reftext{Bell09}\cite{bellone2009}}; \tikz \node[paper] {\reftext{Pezz08}\cite{pezzimenti2008}};};
\node[value, scale=1.400000] (ltevalue6) at (lte6.west) {\num{15}};
\node[ref, lwlte] (lte7) at (lte6.north west) {\tikz \node[paper] {\reftext{Zhao00}\cite{zhao2000}};};
\node[value, scale=1.100000] (ltevalue7) at (lte7.west) {\num{40}};
\node[ref, lwlte] (lte8) at (lte7.north west) {\tikz \node[paper] {\reftext{Usma12}\cite{usman2012}}; \tikz \node[paper] {\reftext{Nall99}\cite{nallet1999}};};
\node[value, scale=1.200000] (ltevalue8) at (lte8.west) {\num{50}};
\node[ref, lwlte] (lte9) at (lte8.north west) {\tikz \node[paper] {\reftext{Schr06}\cite{schroeder2006}}; \tikz \node[paper] {\reftext{Ayal04}\cite{ayalew2004}};};
\node[value, scale=1.200000] (ltevalue9) at (lte9.west) {\num{100}};
\node[ref, lwlte] (lte10) at (lte9.north west) {\tikz \node[paper] {\reftext{Nayd21}\cite{naydenov2021}};};
\node[value, scale=1.100000] (ltevalue10) at (lte10.west) {\num{150}};
\node[ref, lwlte] (lte11) at (lte10.north west) {\tikz \node[paper] {\reftext{Habi11}\cite{habib2011}};};
\node[value, scale=1.100000] (ltevalue11) at (lte11.west) {\num{260}};
\node[ref, lwlte] (lte12) at (lte11.north west) {\tikz \node[paper] {\reftext{Levi01b}\cite{levinshtein2001b}};};
\node[value, scale=1.100000] (ltevalue12) at (lte12.west) {\num{300}};
\node[ref, lwlte] (lte13) at (lte12.north west) {\tikz \node[paper] {\reftext{Zegh20}\cite{zeghdar2020}}; \tikz \node[paper] {\reftext{Zegh19}\cite{zeghdar2019}}; \tikz \node[paper] {\reftext{Megh18a}\cite{megherbi2018a}}; \tikz \node[paper] {\reftext{Choi05}\cite{choi2005}};};
\node[value, scale=1.400000] (ltevalue13) at (lte13.west) {\num{500}};
\node[ref, lwlte] (lte14) at (lte13.north west) {\tikz \node[paper] {\reftext{Lech21}\cite{lechner2021}};};
\node[value, scale=1.100000] (ltevalue14) at (lte14.west) {\num{600}};
\node[ref, lwlte] (lte15) at (lte14.north west) {\tikz \node[paper] {\reftext{Sole19}\cite{soler2019}}; \tikz \node[paper] {\reftext{Meno11}\cite{menon2011}};};
\node[value, scale=1.200000] (ltevalue15) at (lte15.west) {\num{1000}};
\node[ref, lwlte] (lte16) at (lte15.north west) {\tikz \node[paper] {\reftext{Nawa10}\cite{nawaz2010}}; \tikz \node[paper] {\reftext{Bala05}\cite{balachandran2005}};};
\node[value, scale=1.200000] (ltevalue16) at (lte16.west) {\num{1200}};
\node[ref, lwlte] (lte17) at (lte16.north west) {\tikz \node[paper] {\reftext{Liu21}\cite{liu2021}}; \tikz \node[paper] {\reftext{Joha19}\cite{johannesson2019}};};
\node[value, scale=1.200000] (ltevalue17) at (lte17.west) {\num{1500}};
\node[ref, lwlte] (lte18) at (lte17.north west) {\tikz \node[paper] {\reftext{Joha16}\cite{johannesson2016}};};
\node[value, scale=1.100000] (ltevalue18) at (lte18.west) {\num{2000}};
\node[ref, lwlte] (lte19) at (lte18.north west) {\tikz \node[paper] {\reftext{Tiwa19a}\cite{tiwari2019a}}; \tikz \node[paper] {\reftext{Zhan18}\cite{zhang2018}}; \tikz \node[paper] {\reftext{Loph18}\cite{lophitis2018}}; \tikz \node[paper] {\reftext{Arva17}\cite{arvanitopoulos2017}}; \tikz \node[paper] {\reftext{Zhao03}\cite{zhao2003}};};
\node[value, scale=1.500000] (ltevalue19) at (lte19.west) {\num{2500}};
\node[ref, lwlte] (lte20) at (lte19.north west) {\tikz \node[paper] {\reftext{Tama08a}\cite{tamaki2008a}};};
\node[value, scale=1.100000] (ltevalue20) at (lte20.west) {\num{39500}};


\node[symbol] (lth) at (0+ \dxlte,0) {$\taup$};
\coordinate (lth0) at (lth.north);
\node[ref, lwlth] (lth1) at (lth0.north west) {\tikz \node[paper] {\reftext{Bell11}\cite{bellone2011}};};
\node[value, scale=1.100000] (lthvalue1) at (lth1.west) {\num{0.015}};
\node[ref, lwlth] (lth2) at (lth1.north west) {\tikz \node[paper] {\reftext{Das15}\cite{das2015}};};
\node[value, scale=1.100000] (lthvalue2) at (lth2.west) {\num{0.05}};
\node[ref, lwlth] (lth3) at (lth2.north west) {\tikz \node[paper] {\reftext{Rao22}\cite{rao2022}}; \tikz \node[paper] {\reftext{Pezz13}\cite{pezzimenti2013}}; \tikz \node[paper] {\reftext{Bell09}\cite{bellone2009}}; \tikz \node[paper] {\reftext{Pezz08}\cite{pezzimenti2008}};};
\node[value, scale=1.400000] (lthvalue3) at (lth3.west) {\num{15}};
\node[ref, lwlth] (lth4) at (lth3.north west) {\tikz \node[paper] {\reftext{Schr06}\cite{schroeder2006}}; \tikz \node[paper] {\reftext{Ayal04}\cite{ayalew2004}};};
\node[value, scale=1.200000] (lthvalue4) at (lth4.west) {\num{20}};
\node[ref, lwlth] (lth5) at (lth4.north west) {\tikz \node[paper] {\reftext{Usma12}\cite{usman2012}}; \tikz \node[paper] {\reftext{Habi11}\cite{habib2011}}; \tikz \node[paper] {\reftext{Nall99}\cite{nallet1999}};};
\node[value, scale=1.300000] (lthvalue5) at (lth5.west) {\num{50}};
\node[ref, lwlth] (lth6) at (lth5.north west) {\tikz \node[paper] {\reftext{Zegh20}\cite{zeghdar2020}}; \tikz \node[paper] {\reftext{Zegh19}\cite{zeghdar2019}}; \tikz \node[paper] {\reftext{Megh18a}\cite{megherbi2018a}}; \tikz \node[paper] {\reftext{Choi05}\cite{choi2005}};};
\node[value, scale=1.400000] (lthvalue6) at (lth6.west) {\num{100}};
\node[ref, lwlth] (lth7) at (lth6.north west) {\tikz \node[paper] {\reftext{Lech21}\cite{lechner2021}};};
\node[value, scale=1.100000] (lthvalue7) at (lth7.west) {\num{120}};
\node[ref, lwlth] (lth8) at (lth7.north west) {\tikz \node[paper] {\reftext{Nayd21}\cite{naydenov2021}};};
\node[value, scale=1.100000] (lthvalue8) at (lth8.west) {\num{150}};
\node[ref, lwlth] (lth9) at (lth8.north west) {\tikz \node[paper] {\reftext{Cha08}\cite{cha2008}};};
\node[value, scale=1.100000] (lthvalue9) at (lth9.west) {\num{200}};
\node[ref, lwlth] (lth10) at (lth9.north west) {\tikz \node[paper] {\reftext{Levi01}\cite{levinshtein2001}};};
\node[value, scale=1.100000] (lthvalue10) at (lth10.west) {\num{260}};
\node[ref, lwlth] (lth11) at (lth10.north west) {\tikz \node[paper] {\reftext{Joha19}\cite{johannesson2019}}; \tikz \node[paper] {\reftext{Levi01b}\cite{levinshtein2001b}};};
\node[value, scale=1.200000] (lthvalue11) at (lth11.west) {\num{300}};
\node[ref, lwlth] (lth12) at (lth11.north west) {\tikz \node[paper] {\reftext{Joha16}\cite{johannesson2016}};};
\node[value, scale=1.100000] (lthvalue12) at (lth12.west) {\num{400}};
\node[ref, lwlth] (lth13) at (lth12.north west) {\tikz \node[paper] {\reftext{Tiwa19a}\cite{tiwari2019a}}; \tikz \node[paper] {\reftext{Zhan18}\cite{zhang2018}}; \tikz \node[paper] {\reftext{Loph18}\cite{lophitis2018}}; \tikz \node[paper] {\reftext{Arva17}\cite{arvanitopoulos2017}}; \tikz \node[paper] {\reftext{Zhao03}\cite{zhao2003}};};
\node[value, scale=1.500000] (lthvalue13) at (lth13.west) {\num{500}};
\node[ref, lwlth] (lth14) at (lth13.north west) {\tikz \node[paper] {\reftext{Ioff23}\cite{ioffe2023}}; \tikz \node[paper] {\reftext{Adit15}\cite{aditya2015}};};
\node[value, scale=1.200000] (lthvalue14) at (lth14.west) {\num{600}};
\node[ref, lwlth] (lth15) at (lth14.north west) {\tikz \node[paper] {\reftext{Nawa10}\cite{nawaz2010}};};
\node[value, scale=1.100000] (lthvalue15) at (lth15.west) {\num{1000}};
\node[ref, lwlth] (lth16) at (lth15.north west) {\tikz \node[paper] {\reftext{Lee02}\cite{lee2002}};};
\node[value, scale=1.100000] (lthvalue16) at (lth16.west) {\num{2000}};
\node[ref, lwlth] (lth17) at (lth16.north west) {\tikz \node[paper] {\reftext{Tama08a}\cite{tamaki2008a}};};
\node[value, scale=1.100000] (lthvalue17) at (lth17.west) {\num{39500}};


==> data/regen_figure_scharfetter.tex <==
\addplot+[domain=\pgfkeysvalueof{/pgfplots/xmin}:\pgfkeysvalueof{/pgfplots/xmax},no marks, samples=\samp] {scharfetter(3.00E+17,0.3)};
\addlegendentry{\reftext{Ruff94}\cite{ruff1994} (\num{3e+17} , \num[drop-zero-decimal]{0.3})}
\addplot+[domain=\pgfkeysvalueof{/pgfplots/xmin}:\pgfkeysvalueof{/pgfplots/xmax},no marks, samples=\samp] {scharfetter(1.00E+16,1)};
\addlegendentry{\reftext{Nall99}\cite{nallet1999} (\num{1e+16} , \num[drop-zero-decimal]{1})}
\addplot+[domain=\pgfkeysvalueof{/pgfplots/xmin}:\pgfkeysvalueof{/pgfplots/xmax},no marks, samples=\samp] {scharfetter(7.00E+17,1)};
\addlegendentry{\reftext{Levi01b}\cite{levinshtein2001b} (\num{7e+17} , \num[drop-zero-decimal]{1})}
\addplot+[domain=\pgfkeysvalueof{/pgfplots/xmin}:\pgfkeysvalueof{/pgfplots/xmax},no marks, samples=\samp] {scharfetter(5.00E+16,1)};
\addlegendentry{\reftext{Choi05}\cite{choi2005} (\num{5e+16} , \num[drop-zero-decimal]{1})}
\addplot+[domain=\pgfkeysvalueof{/pgfplots/xmin}:\pgfkeysvalueof{/pgfplots/xmax},no marks, samples=\samp] {scharfetter(2e18,1.9)};
\addlegendentry{\reftext{Donn12}\cite{donnarumma2012} (\num{2e+18} , \num[drop-zero-decimal]{1.9})}
\addplot+[domain=\pgfkeysvalueof{/pgfplots/xmin}:\pgfkeysvalueof{/pgfplots/xmax},no marks, samples=\samp] {scharfetter(4e18,1.4)};
\addlegendentry{\reftext{Donn12}\cite{donnarumma2012} (\num{4e+18} , \num[drop-zero-decimal]{1.4})}
\addplot+[domain=\pgfkeysvalueof{/pgfplots/xmin}:\pgfkeysvalueof{/pgfplots/xmax},no marks, samples=\samp] {scharfetter(5.00E+18,1.2)};
\addlegendentry{\reftext{Liau15}\cite{liaugaudas2015} $\taun$: (\num{5e+18} , \num[drop-zero-decimal]{1.2})}
\addplot+[domain=\pgfkeysvalueof{/pgfplots/xmin}:\pgfkeysvalueof{/pgfplots/xmax},no marks, samples=\samp] {scharfetter(7.00E+16,1)};
\addlegendentry{\reftext{Lech21}\cite{lechner2021} (\num{7e+16} , \num[drop-zero-decimal]{1})}
\addplot+[domain=\pgfkeysvalueof{/pgfplots/xmin}:\pgfkeysvalueof{/pgfplots/xmax},no marks, samples=\samp] {scharfetter(5.00E+15,0.55)};
\addlegendentry{\reftext{Maxi23}\cite{maximenko2023} $\taun$: (\num{5e+15} , \num[drop-zero-decimal]{0.55})}
\addplot+[domain=\pgfkeysvalueof{/pgfplots/xmin}:\pgfkeysvalueof{/pgfplots/xmax},no marks, samples=\samp] {scharfetter(5.00E+15,0.67)};
\addlegendentry{\reftext{Maxi23}\cite{maximenko2023} $\taup$: (\num{5e+15} , \num[drop-zero-decimal]{0.67})}
\addlegendimage{empty legend}
\addlegendentry{}
\addlegendimage{empty legend}
\addlegendentry{}


==> data/regen_figure_temperature.tex <==
\addplot+[domain=300:500] {powerT0(1.72,300)};
\addlegendentry{\reftext{Kord96}\cite{kordina1996} $\taup$: (\ref{eq:regen_powerT0})}
\addplot+[domain=300:500] {actEnergy(0.11)};
\addlegendentry{\reftext{Ivan99}\cite{ivanov1999} $\tau$: (\ref{eq:regen_actEnergy})}
\addplot+[domain=\pgfkeysvalueof{/pgfplots/xmin}:\pgfkeysvalueof{/pgfplots/xmax}] {expSimple(2.55,300)};
\addlegendentry{\reftext{Nall99}\cite{nallet1999} $\tau$: (\ref{eq:regen_expSimple})}
\addplot+[domain=200:450] {powerT0(2.2,300)};
\addlegendentry{\reftext{Udal00}\cite{udal2000} $\taup$: (\ref{eq:regen_powerT0})}
\addplot+[domain=300:500] {actEnergy(0.12)};
\addlegendentry{\reftext{Agar01}\cite{agarwal2001} $\taun$: (\ref{eq:regen_actEnergy})}
\addplot+[domain=\pgfkeysvalueof{/pgfplots/xmin}:\pgfkeysvalueof{/pgfplots/xmax}] {powerT0(5,300)};
\addlegendentry{\reftext{Bala05}\cite{balachandran2005} $\taun$: (\ref{eq:regen_powerT0})}
\addplot+[domain=300:550] {actEnergy(0.08)};
\addlegendentry{\reftext{Levi05}\cite{levinshtein2005} $\tau$: (\ref{eq:regen_actEnergy})}
\addplot+[domain=300:700] {powerT0(1.9,300)};
\addlegendentry{\reftext{Udal07}\cite{udal2007} $\taup$: (\ref{eq:regen_powerT0})}
\addplot+[domain=70:1000] {actEnergy51(0.125)};
\addlegendentry{\reftext{Scaj13}\cite{scajev2013} $\tau$: (\ref{eq:regen_actEnergy51})}
\addplot+[domain=300:525] {powerT0(1.2,300)};
\addlegendentry{\reftext{Chow15}\cite{chowdhury2015} $\tau$: (\ref{eq:regen_powerT0})}
\addplot+[domain=100:700] {power0(8,450)};
\addlegendentry{\reftext{Rakh20}\cite{rakheja2020} $\taup$: (\ref{eq:regen_power0}) $\alpha=8$}
\addplot+[domain=100:700] {power0(14,530)};
\addlegendentry{\reftext{Rakh20}\cite{rakheja2020} $\taup$: (\ref{eq:regen_power0}) $\alpha=14$}


==> data/regen_ref_chain.tex <==
\node[desc] at (0,0.000000*\dy) {Doping $\underbrace{( \nref , \gamma )}_{\text{electron}}$ $\underbrace{( \nref , \gamma )}_{\text{hole}}$};
\node[author] at (0,-1.500000*\dy) {\citeauthor{ruff1994}};
\node[no4H, ref] (ruff1994) at (0,-2.500000*\dy) {\reftext{Ruff94}\cite{ruff1994} (  \num{3.00E+17} , \num{0.3} ) ( \num{3.00E+17} , \num{0.3} )};
\coordinate (ruff1994C) at ($(ruff1994.west)+(\dxStart+\dy,0)$);
\node[guess, ref] (shah1998) at ($(ruff1994C |- 0,-3.500000*\dy)$) {\reftext{Shah98}\cite{shah1998} (  \num{3.00E+17} , \num{1} ) ( \num{3.00E+17} , \num{1} )};
\draw (shah1998.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (ladesmartin2000) at ($(shah1998.west |- 0,-4.500000*\dy)$) {\reftext{Lade00}\cite{ladesmartin2000} (  \num{3.00E+17} , \num{0.3} ) ( \num{3.00E+17} , \num{0.3} )};
\draw (ladesmartin2000.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (li2003) at ($(ladesmartin2000.west |- 0,-5.500000*\dy)$) {\reftext{Li03}\cite{li2003} (  \num{3.00E+17} , \num{0.3} ) ( -- , -- )};
\draw (li2003.west) -| ++(-\dy,\fy*\dy);
\coordinate (li2003C) at ($(li2003.west)+(\dxStart+\dy,0)$);
\node[ ref] (johannesson2016) at ($(li2003C |- 0,-6.500000*\dy)$) {\reftext{Joha16}\cite{johannesson2016} (  \num{3.00E+17} , \num{0.3} ) ( \num{3.00E+17} , \num{0.3} )};
\draw (johannesson2016.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (zhao2003) at ($(li2003.west |- 0,-7.500000*\dy)$) {\reftext{Zhao03}\cite{zhao2003} (  \num{3.00E+17} , \num{0.3} ) ( -- , -- )};
\draw (zhao2003.west) -| ++(-\dy,\fy*\dy);
\node[no4H, ref] (ayalew2004) at ($(zhao2003.west |- 0,-8.500000*\dy)$) {\reftext{Ayal04}\cite{ayalew2004} (  \num{6.00E+17} , \num{0.3} ) ( \num{3.00E+17} , \num{0.3} )};
\draw (ayalew2004.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (brosselard2004) at ($(ayalew2004.west |- 0,-9.500000*\dy)$) {\reftext{Bros04}\cite{brosselard2004} (  \num{3.00E+17} , \num{0.3} ) ( \num{3.00E+17} , \num{0.3} )};
\draw (brosselard2004.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (schroeder2006) at ($(brosselard2004.west |- 0,-10.500000*\dy)$) {\reftext{Schr06}\cite{schroeder2006} (  \num{3.00E+17} , \num{0.3} ) ( \num{3.00E+17} , \num{0.3} )};
\draw (schroeder2006.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (buono2010) at ($(schroeder2006.west |- 0,-11.500000*\dy)$) {\reftext{Buon10}\cite{buono2010} (  \num{3.00E+17} , \num{0.3} ) ( \num{3.00E+17} , \num{0.3} )};
\draw (buono2010.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (zhang2010) at ($(buono2010.west |- 0,-12.500000*\dy)$) {\reftext{Zhan10}\cite{zhang2010} (  \num{3.00E+17} , \num{0.3} ) ( -- , -- )};
\draw (zhang2010.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (buono2012) at ($(zhang2010.west |- 0,-13.500000*\dy)$) {\reftext{Buon12}\cite{buono2012} (  \num{3.00E+17} , \num{0.3} ) ( \num{3.00E+17} , \num{0.3} )};
\draw (buono2012.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (usman2012) at ($(buono2012.west |- 0,-14.500000*\dy)$) {\reftext{Usma12}\cite{usman2012} (  \num{3.00E+17} , \num{0.3} ) ( \num{3.00E+17} , \num{0.3} )};
\draw (usman2012.west) -| ++(-\dy,\fy*\dy);
\coordinate (usman2012C) at ($(usman2012.west)+(\dxStart+\dy,0)$);
\node[ ref] (usman2014) at ($(usman2012C |- 0,-15.500000*\dy)$) {\reftext{Usma14}\cite{usman2014} (  \num{3.00E+17} , \num{0.3} ) ( \num{3.00E+17} , \num{0.3} )};
\draw (usman2014.west) -| ++(-\dy,\fy*\dy);
\coordinate (usman2014C) at ($(usman2014.west)+(\dxStart+\dy,0)$);
\node[ ref] (liu2021) at ($(usman2014C |- 0,-16.500000*\dy)$) {\reftext{Liu21}\cite{liu2021} (  \num{3.00E+17} , \num{1} ) ( \num{3.00E+17} , \num{1} )};
\draw (liu2021.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (hatakeyama2013) at ($(usman2012.west |- 0,-17.500000*\dy)$) {\reftext{Hata13}\cite{hatakeyama2013} (  \num{3.00E+17} , \num{0.3} ) ( \num{3.00E+17} , \num{0.3} )};
\draw (hatakeyama2013.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (das2015) at ($(hatakeyama2013.west |- 0,-18.500000*\dy)$) {\reftext{Das15}\cite{das2015} (  \num{3.00E+17} , \num{0.3} ) ( \num{3.00E+17} , \num{0.3} )};
\draw (das2015.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (arvanitopoulos2017) at ($(das2015.west |- 0,-19.500000*\dy)$) {\reftext{Arva17}\cite{arvanitopoulos2017} (  \num{3.00E+17} , \num{0.3} ) ( \num{3.00E+17} , \num{0.3} )};
\draw (arvanitopoulos2017.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (hasegawa2017) at ($(arvanitopoulos2017.west |- 0,-20.500000*\dy)$) {\reftext{Hase17}\cite{hasegawa2017} (  \num{3.00E+17} , \num{0.3} ) ( \num{3.00E+17} , \num{0.3} )};
\draw (hasegawa2017.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (lophitis2018) at ($(hasegawa2017.west |- 0,-21.500000*\dy)$) {\reftext{Loph18}\cite{lophitis2018} (  \num{1.00E+17} , \num{0.3} ) ( \num{1.00E+17} , \num{0.3} )};
\draw (lophitis2018.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (zhang2018) at ($(lophitis2018.west |- 0,-22.500000*\dy)$) {\reftext{Zhan18}\cite{zhang2018} (  \num{3.00E+17} , \num{0.3} ) ( \num{3.00E+17} , \num{0.3} )};
\draw (zhang2018.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (kakarla2020) at ($(zhang2018.west |- 0,-23.500000*\dy)$) {\reftext{Kaka20}\cite{kakarla2020} (  \num{3.00E+17} , \num{0.3} ) ( \num{3.00E+17} , \num{0.3} )};
\draw (kakarla2020.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (koyama2020) at ($(kakarla2020.west |- 0,-24.500000*\dy)$) {\reftext{Koya20}\cite{koyama2020} (  \num{3.00E+17} , \num{0.3} ) ( \num{3.00E+17} , \num{0.3} )};
\draw (koyama2020.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-26.500000*\dy) {\citeauthor{bakowski1997}};
\node[ ref] (bakowski1997) at (0,-27.500000*\dy) {\reftext{Bako97}\cite{bakowski1997} (  -- , -- ) ( -- , -- )};
\coordinate (bakowski1997C) at ($(bakowski1997.west)+(\dxStart+\dy,0)$);
\node[ ref] (zeghdar2019) at ($(bakowski1997C |- 0,-28.500000*\dy)$) {\reftext{Zegh19}\cite{zeghdar2019} (  \num{5.00E+16} , \num{1} ) ( \num{5.00E+16} , \num{1} )};
\draw (zeghdar2019.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (zeghdar2020) at ($(zeghdar2019.west |- 0,-29.500000*\dy)$) {\reftext{Zegh20}\cite{zeghdar2020} (  \num{5.00E+16} , \num{1} ) ( \num{5.00E+16} , \num{1} )};
\draw (zeghdar2020.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,0.000000*\dy) {\citeauthor{nallet1999}};
\node[fund, ref] (nallet1999) at (\xSepOne,-1.000000*\dy) {\reftext{Nall99}\cite{nallet1999} (  \num{1.00E+16} , \num{1} ) ( \num{1.00E+16} , \num{1} )};
\coordinate (nallet1999C) at ($(nallet1999.west)+(\dxStart+\dy,0)$);
\node[guess, ref] (cha2008) at ($(nallet1999C |- 0,-2.000000*\dy)$) {\reftext{Cha08}\cite{cha2008} (  \num{1.00E+16} , \num{1} ) ( \num{1.00E+16} , \num{1} )};
\draw (cha2008.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-4.000000*\dy) {\citeauthor{donnarumma2012}};
\node[fund, ref] (donnarumma2012) at (\xSepOne,-5.000000*\dy) {\reftext{Donn12}\cite{donnarumma2012} (  M , M ) ( M , M )};
\coordinate (donnarumma2012C) at ($(donnarumma2012.west)+(\dxStart+\dy,0)$);
\node[ ref] (megherbi2015) at ($(donnarumma2012C |- 0,-6.000000*\dy)$) {\reftext{Megh15}\cite{megherbi2015} (  \num{2.00E+18} , \num{1.9} ) ( \num{2.00E+18} , \num{1.9} )};
\draw (megherbi2015.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-8.000000*\dy) {\citeauthor{lechner2021}};
\node[fund, ref] (lechner2021) at (\xSepOne,-9.000000*\dy) {\reftext{Lech21}\cite{lechner2021} (  \num{7.00E+16} , \num{1} ) ( \num{7.00E+16} , \num{1} )};
\coordinate (lechner2021C) at ($(lechner2021.west)+(\dxStart+\dy,0)$);
\node[guess, ref] (rao2022) at ($(lechner2021C |- 0,-10.000000*\dy)$) {\reftext{Rao22}\cite{rao2022} (  \num{7.00E+16} , \num{1} ) ( \num{7.00E+16} , \num{1} )};
\draw (rao2022.west) -| ++(-\dy,\fy*\dy);
\node[desc] at (\xSepOne,-13.000000*\dy) {Temperature ( $\alpha_\textrm{n}$ , $\alpha_\textrm{p}$ , $\alpha$ , $T_0$ ) ( $\eact$ , $C$ )};
\node[author] at (\xSepOne,-14.500000*\dy) {\citeauthor{schenk1992}};
\node[no4H, ref] (schenk1992) at (\xSepOne,-15.500000*\dy) {\reftext{Sche92}\cite{schenk1992} (  -- , -- , \num{-1.5} , \num{300} ) ( -- , -- )};
\coordinate (schenk1992C) at ($(schenk1992.west)+(\dxStart+\dy,0)$);
\node[ ref] (kakarla2020) at ($(schenk1992C |- 0,-16.500000*\dy)$) {\reftext{Kaka20}\cite{kakarla2020} (  \num{-1.5} , \num{-1.5} , -- , \num{300} ) ( -- , -- )};
\draw (kakarla2020.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-18.500000*\dy) {\citeauthor{kordina1996}};
\node[fund, ref] (kordina1996) at (\xSepOne,-19.500000*\dy) {\reftext{Kord96}\cite{kordina1996} (  -- , \num{1.72} , -- , \num{300} ) ( -- , -- )};
\coordinate (kordina1996C) at ($(kordina1996.west)+(\dxStart+\dy,0)$);
\node[ ref] (li2003) at ($(kordina1996C |- 0,-20.500000*\dy)$) {\reftext{Li03}\cite{li2003} (  \num{1.72} , -- , -- , -- ) ( -- , -- )};
\draw (li2003.west) -| ++(-\dy,\fy*\dy);
\coordinate (li2003C) at ($(li2003.west)+(\dxStart+\dy,0)$);
\node[ ref] (pezzimenti2013) at ($(li2003C |- 0,-21.500000*\dy)$) {\reftext{Pezz13}\cite{pezzimenti2013} (  \num{1.72} , \num{1.72} , -- , \num{300} ) ( -- , -- )};
\draw (pezzimenti2013.west) -| ++(-\dy,\fy*\dy);
\coordinate (pezzimenti2013C) at ($(pezzimenti2013.west)+(\dxStart+\dy,0)$);
\node[ ref] (zeghdar2020) at ($(pezzimenti2013C |- 0,-22.500000*\dy)$) {\reftext{Zegh20}\cite{zeghdar2020} (  -- , -- , -- , \num{300} ) ( -- , -- )};
\draw (zeghdar2020.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (johannesson2016) at ($(pezzimenti2013.west |- 0,-23.500000*\dy)$) {\reftext{Joha16}\cite{johannesson2016} (  \num{1.72} , \num{1.72} , -- , \num{300} ) ( -- , -- )};
\draw (johannesson2016.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (zeghdar2019) at ($(johannesson2016.west |- 0,-24.500000*\dy)$) {\reftext{Zegh19}\cite{zeghdar2019} (  -- , -- , -- , \num{300} ) ( -- , -- )};
\draw (zeghdar2019.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (zhao2003) at ($(li2003.west |- 0,-25.500000*\dy)$) {\reftext{Zhao03}\cite{zhao2003} (  \num{1.72} , -- , -- , \num{300} ) ( -- , -- )};
\draw (zhao2003.west) -| ++(-\dy,\fy*\dy);
\coordinate (zhao2003C) at ($(zhao2003.west)+(\dxStart+\dy,0)$);
\node[ ref] (das2015) at ($(zhao2003C |- 0,-26.500000*\dy)$) {\reftext{Das15}\cite{das2015} (  \num{1.72} , \num{1.72} , -- , \num{300} ) ( -- , -- )};
\draw (das2015.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (cha2008) at ($(zhao2003.west |- 0,-27.500000*\dy)$) {\reftext{Cha08}\cite{cha2008} (  \num{1.7} , \num{1.7} , -- , \num{300} ) ( -- , -- )};
\draw (cha2008.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (buono2010) at ($(cha2008.west |- 0,-28.500000*\dy)$) {\reftext{Buon10}\cite{buono2010} (  \num{1.72} , \num{1.72} , -- , -- ) ( -- , -- )};
\draw (buono2010.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (zhang2010) at ($(buono2010.west |- 0,-29.500000*\dy)$) {\reftext{Zhan10}\cite{zhang2010} (  \num{1.72} , -- , -- , \num{300} ) ( -- , -- )};
\draw (zhang2010.west) -| ++(-\dy,\fy*\dy);
\coordinate (zhang2010C) at ($(zhang2010.west)+(\dxStart+\dy,0)$);
\node[ ref] (johannesson2016) at ($(zhang2010C |- 0,-30.500000*\dy)$) {\reftext{Joha16}\cite{johannesson2016} (  \num{1.72} , \num{1.72} , -- , \num{300} ) ( -- , -- )};
\draw (johannesson2016.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (buono2012) at ($(zhang2010.west |- 0,-31.500000*\dy)$) {\reftext{Buon12}\cite{buono2012} (  \num{1.72} , \num{1.72} , -- , -- ) ( -- , -- )};
\draw (buono2012.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (usman2012) at ($(buono2012.west |- 0,-32.500000*\dy)$) {\reftext{Usma12}\cite{usman2012} (  \num{1.72} , \num{1.72} , -- , \num{300} ) ( -- , -- )};
\draw (usman2012.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (bellone2014) at ($(usman2012.west |- 0,-33.500000*\dy)$) {\reftext{Bell14}\cite{bellone2014} (  \num{1.72} , \num{1.72} , -- , \num{300} ) ( -- , -- )};
\draw (bellone2014.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (zhang2018) at ($(bellone2014.west |- 0,-34.500000*\dy)$) {\reftext{Zhan18}\cite{zhang2018} (  \num{1.72} , \num{1.72} , -- , \num{300} ) ( -- , \num{2.55} )};
\draw (zhang2018.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (liu2021) at ($(zhang2018.west |- 0,-35.500000*\dy)$) {\reftext{Liu21}\cite{liu2021} (  \num{1.72} , \num{1.72} , -- , \num{300} ) ( -- , -- )};
\draw (liu2021.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,0.000000*\dy) {\citeauthor{nallet1999}};
\node[fund, ref] (nallet1999) at (\xSepOne + \xSepTwo,-1.000000*\dy) {\reftext{Nall99}\cite{nallet1999} (  -- , -- , -- , \num{300} ) ( -- , \num{2.55} )};
\coordinate (nallet1999C) at ($(nallet1999.west)+(\dxStart+\dy,0)$);
\node[guess, ref] (zhang2018) at ($(nallet1999C |- 0,-2.000000*\dy)$) {\reftext{Zhan18}\cite{zhang2018} (  \num{1.72} , \num{1.72} , -- , \num{300} ) ( -- , \num{2.55} )};
\draw (zhang2018.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (lechner2021) at ($(zhang2018.west |- 0,-3.000000*\dy)$) {\reftext{Lech21}\cite{lechner2021} (  -- , -- , -- , \num{300} ) ( -- , \num{2.55} )};
\draw (lechner2021.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-5.000000*\dy) {\citeauthor{balachandran2005}};
\node[fund, ref] (balachandran2005) at (\xSepOne + \xSepTwo,-6.000000*\dy) {\reftext{Bala05}\cite{balachandran2005} (  \num{5} , -- , -- , \num{300} ) ( -- , -- )};
\coordinate (balachandran2005C) at ($(balachandran2005.west)+(\dxStart+\dy,0)$);
\node[ ref] (nawaz2010) at ($(balachandran2005C |- 0,-7.000000*\dy)$) {\reftext{Nawa10}\cite{nawaz2010} (  \num{5} , \num{5} , -- , \num{300} ) ( -- , -- )};
\draw (nawaz2010.west) -| ++(-\dy,\fy*\dy);
\coordinate (nawaz2010C) at ($(nawaz2010.west)+(\dxStart+\dy,0)$);
\node[ ref] (usman2014) at ($(nawaz2010C |- 0,-8.000000*\dy)$) {\reftext{Usma14}\cite{usman2014} (  \num{5} , \num{5} , -- , \num{300} ) ( -- , -- )};
\draw (usman2014.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-10.000000*\dy) {\citeauthor{ivanov2006a}};
\node[fund, ref] (ivanov2006a) at (\xSepOne + \xSepTwo,-11.000000*\dy) {\reftext{Ivan06a}\cite{ivanov2006a} (  -- , -- , -- , -- ) ( \num{0.105} , -- )};
\coordinate (ivanov2006aC) at ($(ivanov2006a.west)+(\dxStart+\dy,0)$);
\node[ ref] (tamaki2008) at ($(ivanov2006aC |- 0,-12.000000*\dy)$) {\reftext{Tama08}\cite{tamaki2008} (  -- , -- , -- , -- ) ( \num{0.105} , -- )};
\draw (tamaki2008.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (tamaki2008a) at ($(tamaki2008.west |- 0,-13.000000*\dy)$) {\reftext{Tama08a}\cite{tamaki2008a} (  -- , -- , -- , -- ) ( \num{0.105} , -- )};
\draw (tamaki2008a.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (kimoto2014a) at ($(tamaki2008a.west |- 0,-14.000000*\dy)$) {\reftext{Kimo14a}\cite{kimoto2014a} (  -- , -- , -- , -- ) ( \num{0.105} , -- )};
\draw (kimoto2014a.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-16.000000*\dy) {\citeauthor{donnarumma2012}};
\node[ ref] (donnarumma2012) at (\xSepOne + \xSepTwo,-17.000000*\dy) {\reftext{Donn12}\cite{donnarumma2012} (  -- , -- , -- , -- ) ( -- , -- )};
\coordinate (donnarumma2012C) at ($(donnarumma2012.west)+(\dxStart+\dy,0)$);
\node[ ref] (megherbi2015) at ($(donnarumma2012C |- 0,-18.000000*\dy)$) {\reftext{Megh15}\cite{megherbi2015} (  \num{1.72} , \num{1.72} , -- , \num{300} ) ( -- , -- )};
\draw (megherbi2015.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-20.000000*\dy) {\citeauthor{dibenedetto2014}};
\node[fund, ref] (dibenedetto2014) at (\xSepOne + \xSepTwo,-21.000000*\dy) {\reftext{Dibe14}\cite{dibenedetto2014} (  \num{2.15} , -- , -- , \num{300} ) ( -- , -- )};
\coordinate (dibenedetto2014C) at ($(dibenedetto2014.west)+(\dxStart+\dy,0)$);
\node[ ref] (dibenedetto2024) at ($(dibenedetto2014C |- 0,-22.000000*\dy)$) {\reftext{Dibe24}\cite{dibenedetto2024} (  \num{2.15} , -- , -- , \num{300} ) ( -- , -- )};
\draw (dibenedetto2024.west) -| ++(-\dy,\fy*\dy);


==> data/regen_ref_chain_II.tex <==
\node[desc] at (0,0.000000*\dy) {Bimolecular ( $B$ )};
\node[author] at (0,-1.500000*\dy) {\citeauthor{galeckas1997}};
\node[fund, ref] (galeckas1997) at (0,-2.500000*\dy) {\reftext{Gale97}\cite{galeckas1997} (  \num{1.50E-12} )};
\coordinate (galeckas1997C) at ($(galeckas1997.west)+(\dxStart+\dy,0)$);
\node[ ref] (galeckas1998) at ($(galeckas1997C |- 0,-3.500000*\dy)$) {\reftext{Gale98}\cite{galeckas1998} (  \num{1.50E-12} )};
\draw (galeckas1998.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (galeckas1999a) at ($(galeckas1998.west |- 0,-4.500000*\dy)$) {\reftext{Gale99a}\cite{galeckas1999a} (  \num{1.50E-12} )};
\draw (galeckas1999a.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (levinshtein2001) at ($(galeckas1999a.west |- 0,-5.500000*\dy)$) {\reftext{Levi01}\cite{levinshtein2001} (  \num{1.50E-12} )};
\draw (levinshtein2001.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (albanese2010) at ($(levinshtein2001.west |- 0,-6.500000*\dy)$) {\reftext{Alba10}\cite{albanese2010} (  \num{1.50E-12} )};
\draw (albanese2010.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (hayashi2011) at ($(albanese2010.west |- 0,-7.500000*\dy)$) {\reftext{Haya11}\cite{hayashi2011} (  \num{1.50E-12} )};
\draw (hayashi2011.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (kaji2015) at ($(hayashi2011.west |- 0,-8.500000*\dy)$) {\reftext{Kaji15}\cite{kaji2015} (  \num{1.50E-12} )};
\draw (kaji2015.west) -| ++(-\dy,\fy*\dy);
\coordinate (kaji2015C) at ($(kaji2015.west)+(\dxStart+\dy,0)$);
\node[ ref] (johannesson2019) at ($(kaji2015C |- 0,-9.500000*\dy)$) {\reftext{Joha19}\cite{johannesson2019} (  \num{1.50E-12} )};
\draw (johannesson2019.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (kimoto2016) at ($(kaji2015.west |- 0,-10.500000*\dy)$) {\reftext{Kimo16}\cite{kimoto2016} (  \num{1.50E-12} )};
\draw (kimoto2016.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (kimoto2018) at ($(kimoto2016.west |- 0,-11.500000*\dy)$) {\reftext{Kimo18}\cite{kimoto2018} (  \num{1.50E-12} )};
\draw (kimoto2018.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (asada2021) at ($(kimoto2018.west |- 0,-12.500000*\dy)$) {\reftext{Asad21}\cite{asada2021} (  \num{1.50E-12} )};
\draw (asada2021.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (ioffe2023) at ($(asada2021.west |- 0,-13.500000*\dy)$) {\reftext{Ioff23}\cite{ioffe2023} (  \num{1.50E-12} )};
\draw (ioffe2023.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-15.500000*\dy) {\citeauthor{galeckas1999}};
\node[ ref] (galeckas1999) at (0,-16.500000*\dy) {\reftext{Gale99}\cite{galeckas1999} (  -- )};
\coordinate (galeckas1999C) at ($(galeckas1999.west)+(\dxStart+\dy,0)$);
\node[ ref] (levinshtein2001a) at ($(galeckas1999C |- 0,-17.500000*\dy)$) {\reftext{Levi01a}\cite{levinshtein2001a} (  \num{1.00E-12} )};
\draw (levinshtein2001a.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (levinshtein2001b) at ($(levinshtein2001a.west |- 0,-18.500000*\dy)$) {\reftext{Levi01b}\cite{levinshtein2001b} (  \num{1.00E-12} )};
\draw (levinshtein2001b.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-20.500000*\dy) {\citeauthor{jarasiunas2010}};
\node[fund, ref] (jarasiunas2010) at (0,-21.500000*\dy) {\reftext{Jara10}\cite{jarasiunas2010} (  \num{1.2+-0.4e-12} )};
\coordinate (jarasiunas2010C) at ($(jarasiunas2010.west)+(\dxStart+\dy,0)$);
\node[ ref] (scajev2010) at ($(jarasiunas2010C |- 0,-22.500000*\dy)$) {\reftext{Scaj10}\cite{scajev2010} (  \num{1.2+-0.2e-12} )};
\draw (scajev2010.west) -| ++(-\dy,\fy*\dy);
\coordinate (scajev2010C) at ($(scajev2010.west)+(\dxStart+\dy,0)$);
\node[ ref] (liaugaudas2015) at ($(scajev2010C |- 0,-23.500000*\dy)$) {\reftext{Liau15}\cite{liaugaudas2015} (  \num{1.00E-12} )};
\draw (liaugaudas2015.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (gao2022a) at ($(liaugaudas2015.west |- 0,-24.500000*\dy)$) {\reftext{Gao22a}\cite{gao2022a} (  \num{1.00E-12} )};
\draw (gao2022a.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (tanaka2023) at ($(gao2022a.west |- 0,-25.500000*\dy)$) {\reftext{Tana23}\cite{tanaka2023} (  \num{1.00E-12} )};
\draw (tanaka2023.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-27.500000*\dy) {\citeauthor{scajev2013}};
\node[ ref] (scajev2013) at (0,-28.500000*\dy) {\reftext{Scaj13}\cite{scajev2013} (  \numrange{1e-14}{3e-14} )};
\coordinate (scajev2013C) at ($(scajev2013.west)+(\dxStart+\dy,0)$);
\node[ ref] (kato2020) at ($(scajev2013C |- 0,-29.500000*\dy)$) {\reftext{Kato20}\cite{kato2020} (  \num{2.00E-14} )};
\draw (kato2020.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (nagaya2020) at ($(kato2020.west |- 0,-30.500000*\dy)$) {\reftext{Naga20}\cite{nagaya2020} (  \num{2.00E-14} )};
\draw (nagaya2020.west) -| ++(-\dy,\fy*\dy);
\node[author] at (0,-32.500000*\dy) {\citeauthor{tanaka2023a}};
\node[fund, ref] (tanaka2023a) at (0,-33.500000*\dy) {\reftext{Tana23a}\cite{tanaka2023a} (  \num{<2e-12} )};
\coordinate (tanaka2023aC) at ($(tanaka2023a.west)+(\dxStart+\dy,0)$);
\node[ ref] (tanaka2024) at ($(tanaka2023aC |- 0,-34.500000*\dy)$) {\reftext{Tana24}\cite{tanaka2024} (  \num{2.00E-12} )};
\draw (tanaka2024.west) -| ++(-\dy,\fy*\dy);
\node[desc] at (\xSepOne,0.000000*\dy) {Auger ( $\cn$ , $\cp$ , $C$ , $T$ )};
\node[author] at (\xSepOne,-1.500000*\dy) {\citeauthor{ruff1994}};
\node[no4H, ref] (ruff1994) at (\xSepOne,-2.500000*\dy) {\reftext{Ruff94}\cite{ruff1994} (  \num{2.80E-31} , \num{9.90E-32} , -- , -- )};
\coordinate (ruff1994C) at ($(ruff1994.west)+(\dxStart+\dy,0)$);
\node[ ref] (das2015) at ($(ruff1994C |- 0,-3.500000*\dy)$) {\reftext{Das15}\cite{das2015} (  \num{5.00E-31} , \num{9.90E-32} , -- , -- )};
\draw (das2015.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne,-5.500000*\dy) {\citeauthor{galeckas1997}};
\node[fund, ref] (galeckas1997) at (\xSepOne,-6.500000*\dy) {\reftext{Gale97}\cite{galeckas1997} (  \num{5+-1e-31} , \num{2+-1e-31} , \num{7+-1E-31} , \num{300} )};
\coordinate (galeckas1997C) at ($(galeckas1997.west)+(\dxStart+\dy,0)$);
\node[ ref] (galeckas1998) at ($(galeckas1997C |- 0,-7.500000*\dy)$) {\reftext{Gale98}\cite{galeckas1998} (  \num{5+-1e-31} , -- , \num{7+-1e-31} , \num{300} )};
\draw (galeckas1998.west) -| ++(-\dy,\fy*\dy);
\coordinate (galeckas1998C) at ($(galeckas1998.west)+(\dxStart+\dy,0)$);
\node[ ref] (biondo2012) at ($(galeckas1998C |- 0,-8.500000*\dy)$) {\reftext{Bion12}\cite{biondo2012} (  \num{7.00E-31} , \num{7.00E-31} , -- , -- )};
\draw (biondo2012.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (das2015) at ($(biondo2012.west |- 0,-9.500000*\dy)$) {\reftext{Das15}\cite{das2015} (  \num{5.00E-31} , \num{9.90E-32} , -- , -- )};
\draw (das2015.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (galeckas1999a) at ($(galeckas1998.west |- 0,-10.500000*\dy)$) {\reftext{Gale99a}\cite{galeckas1999a} (  -- , -- , \num{7.00E-31} , -- )};
\draw (galeckas1999a.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (levinshtein2001) at ($(galeckas1999a.west |- 0,-11.500000*\dy)$) {\reftext{Levi01}\cite{levinshtein2001} (  \num{5.00E-31} , \num{2.00E-31} , \num{7.00E-31} , -- )};
\draw (levinshtein2001.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (lee2002) at ($(levinshtein2001.west |- 0,-12.500000*\dy)$) {\reftext{Lee02}\cite{lee2002} (  \num{5.00E-31} , \num{2.00E-31} , -- , -- )};
\draw (lee2002.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (neimontas2006) at ($(lee2002.west |- 0,-13.500000*\dy)$) {\reftext{Neim06}\cite{neimontas2006} (  \num{5.00E-31} , \num{2.00E-31} , \num{7.00E-31} , -- )};
\draw (neimontas2006.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (pezzimenti2008) at ($(neimontas2006.west |- 0,-14.500000*\dy)$) {\reftext{Pezz08}\cite{pezzimenti2008} (  \num{5.00E-31} , \num{2.00E-31} , -- , -- )};
\draw (pezzimenti2008.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (albanese2010) at ($(pezzimenti2008.west |- 0,-15.500000*\dy)$) {\reftext{Alba10}\cite{albanese2010} (  \num{5.00E-31} , \num{2.00E-31} , -- , -- )};
\draw (albanese2010.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (nawaz2010) at ($(albanese2010.west |- 0,-16.500000*\dy)$) {\reftext{Nawa10}\cite{nawaz2010} (  \num{5.00E-31} , \num{2.00E-31} , -- , -- )};
\draw (nawaz2010.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (habib2011) at ($(nawaz2010.west |- 0,-17.500000*\dy)$) {\reftext{Habi11}\cite{habib2011} (  \num{5.00E-31} , \num{2.00E-31} , -- , -- )};
\draw (habib2011.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (hayashi2011) at ($(habib2011.west |- 0,-18.500000*\dy)$) {\reftext{Haya11}\cite{hayashi2011} (  \num{5.00E-31} , \num{2.00E-31} , -- , -- )};
\draw (hayashi2011.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (buono2012) at ($(hayashi2011.west |- 0,-19.500000*\dy)$) {\reftext{Buon12}\cite{buono2012} (  \num{5.00E-31} , \num{2.00E-31} , -- , -- )};
\draw (buono2012.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (khalid2012) at ($(buono2012.west |- 0,-20.500000*\dy)$) {\reftext{Khal12}\cite{khalid2012} (  \num{7.00E-31} , \num{7.00E-31} , -- , -- )};
\draw (khalid2012.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (pezzimenti2013) at ($(khalid2012.west |- 0,-21.500000*\dy)$) {\reftext{Pezz13}\cite{pezzimenti2013} (  \num{5.00E-31} , \num{2.00E-31} , -- , -- )};
\draw (pezzimenti2013.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (bellone2014) at ($(pezzimenti2013.west |- 0,-22.500000*\dy)$) {\reftext{Bell14}\cite{bellone2014} (  \num{5.00E-31} , \num{2.00E-31} , -- , -- )};
\draw (bellone2014.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (usman2014) at ($(bellone2014.west |- 0,-23.500000*\dy)$) {\reftext{Usma14}\cite{usman2014} (  \num{5.00E-32} , \num{2.00E-32} , -- , -- )};
\draw (usman2014.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (kaji2015) at ($(usman2014.west |- 0,-24.500000*\dy)$) {\reftext{Kaji15}\cite{kaji2015} (  \num{5.00E-31} , \num{2.00E-31} , -- , -- )};
\draw (kaji2015.west) -| ++(-\dy,\fy*\dy);
\coordinate (kaji2015C) at ($(kaji2015.west)+(\dxStart+\dy,0)$);
\node[ ref] (johannesson2019) at ($(kaji2015C |- 0,-25.500000*\dy)$) {\reftext{Joha19}\cite{johannesson2019} (  \num{5.00E-31} , \num{2.00E-31} , -- , -- )};
\draw (johannesson2019.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (kimoto2016) at ($(kaji2015.west |- 0,-26.500000*\dy)$) {\reftext{Kimo16}\cite{kimoto2016} (  \num{5.00E-31} , \num{2.00E-31} , -- , -- )};
\draw (kimoto2016.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (arvanitopoulos2017) at ($(kimoto2016.west |- 0,-27.500000*\dy)$) {\reftext{Arva17}\cite{arvanitopoulos2017} (  \num{5.00E-31} , \num{2.00E-31} , -- , -- )};
\draw (arvanitopoulos2017.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (kimoto2018) at ($(arvanitopoulos2017.west |- 0,-28.500000*\dy)$) {\reftext{Kimo18}\cite{kimoto2018} (  \num{5.00E-31} , \num{2.00E-31} , -- , -- )};
\draw (kimoto2018.west) -| ++(-\dy,\fy*\dy);
\coordinate (kimoto2018C) at ($(kimoto2018.west)+(\dxStart+\dy,0)$);
\node[ ref] (choudhary2021) at ($(kimoto2018C |- 0,-29.500000*\dy)$) {\reftext{Chou21}\cite{choudhary2021} (  \num{5.00E-31} , \num{2.00E-31} , -- , -- )};
\draw (choudhary2021.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (megherbi2018a) at ($(kimoto2018.west |- 0,-30.500000*\dy)$) {\reftext{Megh18a}\cite{megherbi2018a} (  \num{5.00E-31} , \num{2.00E-31} , -- , -- )};
\draw (megherbi2018a.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (zeghdar2019) at ($(megherbi2018a.west |- 0,-31.500000*\dy)$) {\reftext{Zegh19}\cite{zeghdar2019} (  \num{5.00E-31} , \num{2.00E-31} , -- , -- )};
\draw (zeghdar2019.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (tian2020) at ($(zeghdar2019.west |- 0,-32.500000*\dy)$) {\reftext{Tian20}\cite{tian2020} (  \num{5.00E-31} , \num{2.00E-31} , -- , -- )};
\draw (tian2020.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (zeghdar2020) at ($(tian2020.west |- 0,-33.500000*\dy)$) {\reftext{Zegh20}\cite{zeghdar2020} (  \num{5.00E+31} , \num{2.00E-31} , -- , -- )};
\draw (zeghdar2020.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (asada2021) at ($(zeghdar2020.west |- 0,-34.500000*\dy)$) {\reftext{Asad21}\cite{asada2021} (  \num{5.00E-31} , \num{2.00E-31} , -- , -- )};
\draw (asada2021.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (murata2021) at ($(asada2021.west |- 0,-35.500000*\dy)$) {\reftext{Mura21}\cite{murata2021} (  \num{5.00E-31} , \num{2.00E-31} , -- , -- )};
\draw (murata2021.west) -| ++(-\dy,\fy*\dy);
\node[guess, ref] (gao2022a) at ($(murata2021.west |- 0,-36.500000*\dy)$) {\reftext{Gao22a}\cite{gao2022a} (  -- , -- , \num{7.00E-31} , -- )};
\draw (gao2022a.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (ioffe2023) at ($(gao2022a.west |- 0,-37.500000*\dy)$) {\reftext{Ioff23}\cite{ioffe2023} (  \num{5.00E-31} , \num{2.00E-31} , \num{7.00E-31} , -- )};
\draw (ioffe2023.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,0.000000*\dy) {\citeauthor{ramungul1998}};
\node[no4H, ref] (ramungul1998) at (\xSepOne + \xSepTwo,-1.000000*\dy) {\reftext{Ramu98}\cite{ramungul1998} (  -- , -- , \numrange{2.5e-29}{3.5e-29} , -- )};
\coordinate (ramungul1998C) at ($(ramungul1998.west)+(\dxStart+\dy,0)$);
\node[no4H, ref] (ayalew2004) at ($(ramungul1998C |- 0,-2.000000*\dy)$) {\reftext{Ayal04}\cite{ayalew2004} (  \num{3.00E-29} , \num{3.00E-29} , -- , -- )};
\draw (ayalew2004.west) -| ++(-\dy,\fy*\dy);
\coordinate (ayalew2004C) at ($(ayalew2004.west)+(\dxStart+\dy,0)$);
\node[ ref] (lechner2021) at ($(ayalew2004C |- 0,-3.000000*\dy)$) {\reftext{Lech21}\cite{lechner2021} (  \num{3.00E-29} , \num{3.00E-29} , -- , -- )};
\draw (lechner2021.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-5.000000*\dy) {\citeauthor{galeckas1999}};
\node[ ref] (galeckas1999) at (\xSepOne + \xSepTwo,-6.000000*\dy) {\reftext{Gale99}\cite{galeckas1999} (  -- , -- , -- , -- )};
\coordinate (galeckas1999C) at ($(galeckas1999.west)+(\dxStart+\dy,0)$);
\node[ ref] (levinshtein2001a) at ($(galeckas1999C |- 0,-7.000000*\dy)$) {\reftext{Levi01a}\cite{levinshtein2001a} (  -- , -- , \num{7.00E-31} , -- )};
\draw (levinshtein2001a.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (levinshtein2001b) at ($(levinshtein2001a.west |- 0,-8.000000*\dy)$) {\reftext{Levi01b}\cite{levinshtein2001b} (  -- , -- , \num{7.00E-31} , -- )};
\draw (levinshtein2001b.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (udal2007) at ($(levinshtein2001b.west |- 0,-9.000000*\dy)$) {\reftext{Udal07}\cite{udal2007} (  -- , -- , -- , -- )};
\draw (udal2007.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-11.000000*\dy) {\citeauthor{scajev2010}};
\node[fund, ref] (scajev2010) at (\xSepOne + \xSepTwo,-12.000000*\dy) {\reftext{Scaj10}\cite{scajev2010} (  -- , -- , M , \num{298} )};
\coordinate (scajev2010C) at ($(scajev2010.west)+(\dxStart+\dy,0)$);
\node[ ref] (liaugaudas2015) at ($(scajev2010C |- 0,-13.000000*\dy)$) {\reftext{Liau15}\cite{liaugaudas2015} (  -- , -- , \num{5.00E-31} , -- )};
\draw (liaugaudas2015.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (nipoti2016a) at ($(liaugaudas2015.west |- 0,-14.000000*\dy)$) {\reftext{Nipo16a}\cite{nipoti2016a} (  -- , -- , -- , -- )};
\draw (nipoti2016a.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-16.000000*\dy) {\citeauthor{scajev2013}};
\node[fund, ref] (scajev2013) at (\xSepOne + \xSepTwo,-17.000000*\dy) {\reftext{Scaj13}\cite{scajev2013} (  -- , -- , \num{5+-1e-31} , -- )};
\coordinate (scajev2013C) at ($(scajev2013.west)+(\dxStart+\dy,0)$);
\node[ ref] (kato2020) at ($(scajev2013C |- 0,-18.000000*\dy)$) {\reftext{Kato20}\cite{kato2020} (  -- , -- , \num{5.00E-31} , -- )};
\draw (kato2020.west) -| ++(-\dy,\fy*\dy);
\node[ ref] (nagaya2020) at ($(kato2020.west |- 0,-19.000000*\dy)$) {\reftext{Naga20}\cite{nagaya2020} (  -- , -- , \num{5.00E-31} , -- )};
\draw (nagaya2020.west) -| ++(-\dy,\fy*\dy);
\node[author] at (\xSepOne + \xSepTwo,-21.000000*\dy) {\citeauthor{tanaka2023a}};
\node[fund, ref] (tanaka2023a) at (\xSepOne + \xSepTwo,-22.000000*\dy) {\reftext{Tana23a}\cite{tanaka2023a} (  -- , -- , \num{<3e-31} , -- )};
\coordinate (tanaka2023aC) at ($(tanaka2023a.west)+(\dxStart+\dy,0)$);
\node[ ref] (tanaka2024) at ($(tanaka2023aC |- 0,-23.000000*\dy)$) {\reftext{Tana24}\cite{tanaka2024} (  -- , -- , \num{3.00E-31} , -- )};
\draw (tanaka2024.west) -| ++(-\dy,\fy*\dy);

